Learning Optimal Antenna Tilt Control Policies: A Contextual Linear Bandit Approach

Controlling antenna tilts in cellular networks is imperative to reach an efficient trade-off between network coverage and capacity. In this paper, we devise algorithms learning optimal tilt control policies from existing data (in the so-called passive learning setting) or from data actively generated by the algorithms (the active learning setting). We formalize the design of such algorithms as a Best Policy Identification (BPI) problem in Contextual Linear Multi-Arm Bandits (CL-MAB). An arm represents an antenna tilt update; the context captures current network conditions; the reward corresponds to an improvement of performance, mixing coverage and capacity; and the objective is to identify, with a given level of confidence, an approximately optimal policy (a function mapping the context to an arm with maximal reward). For CL-MAB in both active and passive learning settings, we derive information-theoretical lower bounds on the number of samples required by any algorithm returning an approximately optimal policy with a given level of certainty, and devise algorithms achieving these fundamental limits. We apply our algorithms to the Remote Electrical Tilt (RET) optimization problem in cellular networks, and show that they can produce optimal tilt update policy using much fewer data samples than naive or existing rule-based learning algorithms.

==> INFOCOM 2021 - FinalSubmission/Sections/AdditionalExperiments.tex <==
\newpage 
\section{Additional experimental results}
\label{app:experiments}

%\begin{figure}[h!]
%    \centering
%    \includegraphics[width = 8cm]{figures/example_cell.png}
%    \caption{Cell KPIs evolution example for up-tilt.}
%    \label{fig:ex_cell}
%\end{figure}

%Figure \ref{fig:two_action_exp_rew} shows the expectation actions' rewards over the context space fitted to the performance function.

%\begin{figure}[h!]
%    \centering
%    \includegraphics[width = 8 cm]{figures/planes.pdf}
%    \caption{Expected actions reward.}
%    \label{fig:two_action_exp_rew}
%\end{figure}
\begin{comment}

\section{Additional examples}
\subsection{$(U,\delta)$-PAC policy}
\textbf{Example 1:} We consider the following instance of LCB problem with $d = 3$, $K = 2$ and $C = 3$. We let $\theta = [1,1,1]$, and the feature vectors be specified as $\phi_{x_1,a_1} = [1,0,0]$, $\phi_{x_1,a_2} = [0,1-\Delta,0]$, $\phi_{x_2,a_1} = [0,1,0]$, $\phi_{x_2,a_2} = [1- \Delta,0,0]$, $\phi_{x_3,a_1} = [1,0,0]$, $\phi_{x_3,a_2} = [0,0,1-\Delta]$, 
for some $\Delta >0$. We assume to have uniform random probabilities across the context space, i.e., $p_\mathcal{X}(x) = 1/3$, for all $x\in\mathcal{X}$. It is easy to check that for a deterministic policy of the type $\bar{\alpha}_{x,a_1} = 1$, for all $x\in\mathcal{X}$, we have that $\textrm{det}(A(\bar{\alpha})) = 0$. In particular the second component of $\theta$ is not learnable, and we can hence focus on learning the best policy on $U = \mathbb{R}^2$. On the other hand, for any $\bar{\alpha}$ having non-zero probability, e.g. the uniform random policy $\bar{\alpha}_{x,a} = 1/2, \forall (x,a)$, we have $\textrm{det}(A(\bar{\alpha}))>0$ and $U = \mathbb{R}^3$. 

We report the results in terms of empirical sample complexity in Table \ref{tab:results_udelta}, when varying $\Delta$.

\begin{table}[ht!]
\fontsize{9.3}{9.3}\selectfont
\centering
\caption{Experimental results for the $(U,\delta)$-PAC example.}
\begin{tabular}{clrrr}\hline
Proportions  & Parameter & Lower bound & Sample complexity & BPI error \\ \hline \hline
\multirow{3}{*}{Deterministic} %& $\varepsilon = 0.20$ & $174.56$ & $323.48\pm71.10$ & $0.04 \pm 0.20$ \\ & $\varepsilon = 0.15$ & $319.82$ & $404.73 \pm 94.00$ & $0.05 \pm 0.23$ \\
& $\Delta= 1.5$  &  $ 13.81$ & $50.70 \pm 17.99$ & $0.000 \pm 0.000$ \\
& $\Delta= 0.9$  &  $ 34.28$ & $120.16 \pm 42.74$ & $0.010 \pm 0.099$ \\ & $\Delta = 0.5$ & $124.33$ & $491.40 \pm 138.22$ & $0.016 \pm 0.125$ \\ \hline \hline
\multirow{3}{*}{Random} 
& $\Delta= 1.5$  &  $35.47$ & $160.04 \pm 52.83$ & $0.000 \pm 0.000$ \\& $\Delta= 0.9$  & $102.16$ & $456.63\pm 138.41$ & $0.000 \pm 0.000$ \\ & $\Delta = 0.5$ & $319.29$ & $1654.73 \pm 469.77$ & $0.003 \pm 0.054$ \\ \hline 
\end{tabular} 
\label{tab:results_udelta}
\end{table}


\textbf{Example 2:} We consider the following instance of LCB problem with $d = 3$, $K = 2$ and $C = 2$. We let $\theta = [1,1,1]$, and the feature vectors be specified as $\phi_{x_1,a_1} = [1,0,0]$, $\phi_{x_1,a_2} = [0,1-\Delta,0]$, $\phi_{x_2,a_1} = [0,0,1]$, $\phi_{x_2,a_2} = [0,0,1- \Delta]$, %$\phi_{x_3,a_1} = [0,0,1]$, $\phi_{x_3,a_2} = [0,0,1-\Delta_3]$An Instance of the problem with $\Delta_i = 1/(i+1)$, for $i = 1,2$ is reported in Figure \ref{fig:u_delta_pac.pdf}.
for some $\Delta >0$. We assume to have uniform random probabilities across the context space, i.e., $p_\mathcal{X}(x) = 1/2$, for all $x\in\mathcal{X}$. It is easy to check that for a deterministic policy of the type $\bar{\alpha}_{x,a_1} = 1$, for all $x\in\mathcal{X}$, we have that $\textrm{det}(A(\bar{\alpha}))=0$. In particular the second component of $\theta$ is not learnable, and we can hence focus on learning the best policy on $U = \mathbb{R}^2$. On the other hand, for any $\bar{\alpha}$ having non-zero probability, e.g. the uniform random policy $\bar{\alpha}_{x,a} = 1/2, \forall (x,a)$, we have $\textrm{det}(A(\bar{\alpha}))>0$. 

The lower bound satisfies $\mathbb{E}[\tau] \geq \frac{4}{\Delta^2}\log(1/\delta)$. We fix $\delta = 0.01$, and we report the results in terms of empirical sample complexity in Table \ref{tab:results_udelta}, when varying $\Delta$.

\begin{table}[ht!]
\fontsize{9.3}{9.3}\selectfont
\centering
\caption{Experimental results for the $(U,\delta)$-PAC example.}
\begin{tabular}{clrrr}\hline
Proportions & Parameter & Lower bound & Sample complexity & BPI error \\ \hline \hline
\multirow{3}{*}{Deterministic} 
& $\Delta= 0.1$  & $417.54$ & $504.34 \pm 165.87$ & $0.005 \pm 0.070$ \\ & $\Delta = 0.05$ & $610.52$ & $583.33 \pm 111.06$ & $0.00 \pm 0.00$ \\ & $\Delta = 0.01$ & $610.52$ & $583.33 \pm 111.06$ & $0.00 \pm 0.00$ \\ \hline \hline
\multirow{3}{*}{Random} 
& $\Delta= 0.1$  & $417.54$ & $504.34 \pm 165.87$ & $0.005 \pm 0.070$ \\ & $\Delta = 0.05$ & $610.52$ & $583.33 \pm 111.06$ & $0.00 \pm 0.00$ \\ & $\Delta = 0.01$ & $610.52$ & $583.33 \pm 111.06$ & $0.00 \pm 0.00$ \\ \hline 
\end{tabular} 
\label{tab:results_udelta}
\end{table}

%$\hat{\theta} = [1,0,1]$.  $\gamma_{x_1,a_2} = \phi_{x_1,a_1} - \phi_{x_1,a_2} = [1,\Delta-1,0]$, $\gamma_{x_2,a_2} = \phi_{x_2,a_1} - \phi_{x_2,a_2} = [0,0,\Delta]$. $\hat{\theta}^\top \gamma_{x_1,a_2} = 1$, $\hat{\theta}^\top \gamma_{x_2,a_2} = \Delta$. $\gamma_{x_1,a_2}^\top A(\alpha)^\dagger\gamma_{x_1,a_2} = 2$, $\gamma_{x_2,a_2}^\top A(\alpha)^\dagger\gamma_{x_2,a_2} = 2\Delta^2$.
\end{comment}

==> INFOCOM 2021 - FinalSubmission/Sections/Algorithms.tex <==
\section{Algorithms}
In this section, we present our algorithm for the the active and passive learning settings. The first part of the section (see \ref{sec:LSE}, \ref{sec:stopping_rule}, and \ref{sec:sampling_rule}) describes the algorithm for active learning setting, while \ref{sec:passive_learning_algorithm} presents the algorithm in the passive learning setting. The algorithms apply the track-and-stop framework developed in \cite{Garivier16} and \cite{Jedra20} for regular and LB problems. In the active learning setting, the algorithm consists in $(i)$ estimating the unknown parameter $\theta$ using the Least-Squares Estimator (LSE), $(ii)$ using this estimator to compute the optimal sampling rule suggested by the lower bound optimization problem leading to $T_{\theta,\varepsilon}^\star$, and $(iii)$ tracking this sampling rule and stopping when enough information has been gathered. We detail these steps below. 
%In the passive learning setting, the algorithm modifies the stopping and decision rules from the active learning algorithm to accommodate the passive learning setting. 

\subsection{Least-Squares Estimator}
\label{sec:LSE}
The LSE for $\theta$ can be explicitly computed and is, after gathering $t\ge 1$ samples,
\begin{equation}
        \hat{\theta}_t = \left(\sum_{s = 1}^t \phi_{x_s,a_s}\phi^\top_{x_s,a_s}\right)^\dagger\left(\sum_{s = 1}^t\phi_{x_s,a_s}r_{s}\right).
        \label{eq:LS_estimator}
\end{equation}
As in absence of contexts, the quantity that will control the performance of the LSE is the smallest eigenvalue of the covariates matrix $A_t = \sum_{s = 1}^t \phi_{x_s,a_s}\phi^\top_{x_s,a_s}$. The following results are straightforward extensions of similar results derived for LB without context \cite{Jedra20}, and obtained applying concentration results for self-normalized processes \cite{Abbasi11}. 

\begin{lemma}
\label{lem:LS_concentration}
(i) If the sampling rule satisfies, for some $\alpha\in(0,1)$, $\lim\inf_{t \to \infty }\lambda_{1}\left( \frac{A_t}{t^\alpha} \right) > 0$ a.s., then $\lim_{t \to \infty} \hat{\theta}_t =  \theta$ a.s. In particular, for all $\beta \in (0,\alpha/2)$,
   $ \|\hat{\theta}_t - \theta\| = o\left(t^{-\beta}\right)$ a.s.. (ii)     Let $L = \max_{x,a}\|\phi_{x,a}\|$ and assume there exists $t_0 \geq 1$ such that for all $t\geq t_0$, $\lambda_{1}\left(A_t\right) \geq c t^\alpha$ a.s. for some $c>0$. Then for all $t\geq t_0$,
    $$
    \mathbb{P}_\theta(\|\hat{\theta}_t - \theta\| \geq \varepsilon) \leq \left(c^{-1 / 2} L\right)^{d} t^{\frac{(1-\alpha) d}{2}} \exp \left(-\frac{c \varepsilon^{2} t^{\alpha}}{4}\right).
    $$
\end{lemma}

\subsection{Stopping and decision rule}
\label{sec:stopping_rule}
Both rules leverage the Generalized Log-likelihood Ratio (GLR) $Z^x_{a, b, \varepsilon}(t)$ indicating whether arm $a$ is better than $b$ (up to a precision $\varepsilon$). For any pair of arms $(a,b)\in\mathcal{A}^2:a \neq b$, $x\in\mathcal{X}$, $t\geq1$, and $\varepsilon \geq 0$, it is defined as
{\begin{equation*}
Z^x_{a, b, \varepsilon}(t)=\log \left(\frac{\max_{\left\{\theta\in\mathbb{R}^d: \theta^{\top}\gamma_{a,b}^x \leq \varepsilon\right\}} \prod_{s=1}^t f_{x_s,a_s}^{\theta}(r_s)}{\max_{\left\{\theta \in\mathbb{R}^d:\theta^{\top}\gamma_{a,b}^x \geq \varepsilon \right\}} \prod_{s=1}^t f_{x_s,a_s}^{\theta}(r_s) }\right). 
\end{equation*}}
We can easily obtain an explicit expression of $Z^x_{a,b}$ as in \cite{Jedra20} for plain linear bandits. For $t\geq 1$ such that $A_t \succ 0$, for all $x \in\mathcal{X}$, and $(a,b) \in\mathcal{A}^2: a\neq b$, we have
\begin{equation*}
    Z^x_{a, b, \varepsilon}(t)=\operatorname{sgn}\left(\hat{\theta}_{t}^{\top}\gamma^x_{b,a}+\varepsilon\right) \frac{\left(\hat{\theta}_{t}^{\top}\gamma^x_{b,a}+\varepsilon\right)^{2}}{2\|\gamma^x_{b,a}\|_{A_t^{-1}}}.
\end{equation*}
\noindent
At the stopping time $\tau$, the decision rule is just defined as
\begin{equation}
\label{eq:recommendation_rule}
    \hat{a}_\tau(x) = \argmax_{a \in \mathcal{A}_\varepsilon(\hat{\theta}_\tau,x)} \min_{b \neq a} Z^x_{a, b, \varepsilon}(\tau), \quad \forall x\in\mathcal{X},
\end{equation}
and it can be computed using the above explicit expression of $Z^x_{a, b, \varepsilon}(t)$. The stopping rule is based on the GLR and the classical Chernoff stopping rule \cite{Garivier16}.

Define $Z_\varepsilon^x(t) = \max_{a \in \mathcal{A}_\varepsilon(\hat{\theta}_t,x)} \min_{b \neq a} Z^x_{a, b, \varepsilon}(t)$. The stopping time is 
\begin{align}
\begin{split}
    \tau =\inf \Big\{t:\forall x\in\mathcal{X}, Z_\varepsilon^x(t)>\beta(\delta, t) \text{ and } A_t \succeq c I_{d}\Big\},
\label{eq:stopping_rule_eps_delta_pac}
\end{split}
\end{align}
where $\beta(\delta,t)$ is an exploration threshold chosen to ensure that the algorithm is $(\varepsilon,\delta)$-PAC, and $c$ is a strictly positive constant. An exploration threshold leading to an $(\varepsilon,\delta)$-PAC algorithm is proposed in the following lemma. The proof sketches of all lemmas presented in this section are postponed to Section \ref{sec:lemmas}.
\begin{lemma}
\label{lem:stopping_rule_eps_delta_pac}
Let $u>0$, and define the exploration threshold
\begin{equation}
    \label{eq:expl_rate_eps_delta_pac}
        \beta(\delta, t) = (1+u) \log \left(\frac{\operatorname{det}\left((uc)^{-1}  A_t+I_{d}\right)^{\frac{1}{2}}}{\delta}\right).
\end{equation}
\noindent
Under the stopping rule defined by \eqref{eq:stopping_rule_eps_delta_pac}--\eqref{eq:expl_rate_eps_delta_pac} and under any sampling rule, we have
     $$\mathbb{P}_{\theta}\left(\exists x\in \mathcal{X}: \theta^\top (\phi_{x,a^\star_\theta(x)} - \phi_{x,\hat{a}_\tau(x)}) >\varepsilon, \tau <\infty\right)\leq\delta.$$
\end{lemma}
\noindent Note that the exploration threshold has the nice property of being independent on the number of contexts $|\mathcal{X}|$.

\subsection{Sampling rule} 
\label{sec:sampling_rule}
To obtain an algorithm with minimal sample complexity, we need to devise a sampling rule approaching an optimal proportion of arm draws $\alpha_\theta^\star\in C^\star_{\varepsilon}(\theta)$. To this aim, we propose a sampling rule based on two components: a forced exploration phase ensuring that $\theta$ is estimated accurately, and a tracking phase where, based on the estimated $\theta$, the allocation of arm draws is maintained close to the set $C^\star_{\varepsilon}(\theta)$.

\textit{a) Forced Exploration.} Lemma \ref{lem:LS_concentration} presents conditions under which the LSE of $\theta$ performs well. The forced exploration phase is designed so that these conditions hold. To design the forced exploration phase, we pick, for each context $x$, a set of arms $\mathcal{A}_x = \left\{{a}_x(1),\dots,{a}_x(d_x)\right\} \subseteq \mathcal{A}$ such that $\lambda_{d_x}\left(\sum_{{a}_x \in {\mathcal{A}}_x}\phi_{x,{a}_x}\phi_{x,{a}_x}^\top\right)>0$. The sets are chosen so that there exists $c>0$ such that $\sum_{x\in\mathcal{X}} \sum_{{a}_x \in {\mathcal{A}}_x}\phi_{x,{a}_x}\phi_{x,{a}_x}^\top \succeq c I_d$. Let $A_{t}(x) = \sum_{s = 1}^t\phi_{x_s,a_s}\phi_{x_s,a_s}^\top \mathbbm{1}_{\{x_s=x\}}$, $N_{x}(t) = \sum_{s = 1}^t \mathbbm{1}_{\{x_s=x\}}$, and $p_{\min} = \min\limits_{x\in\mathcal{X}}p_\mathcal{X}(x)$. The forced exploration phase is defined and analyzed in the following lemma. 
\begin{lemma}
\label{lem:forced_exploration}
      Let $(d_t(x))_{t\geq 1}$ be an arbitrary sequence of context-action mappings. for $t \geq 1$ and for all $x \in \mathcal{X}$. Define  $f_x(t) = \sqrt{\frac{N_x(t)}{d_x}} \sum_{{a}_x \in {\mathcal{A}}_x}\phi_{x,{a}_x}\phi_{x,{a}_x}^\top$, and the index $i_t(x)$ such that $i_0(x) = 1$, $i_{t+1}(x) = (i_t(x) \mod d_x) +\mathbbm{1}_{\{A_t(x) \prec f_x(t)\}}$. Define the sampling rule as
\begin{equation}
\label{eq:sampling_rule_force}
    a_{t+1}(x) =\left\{\begin{array}{ll}
    d_{t}(x) & \text {if } \quad A_t(x) \succeq f_x(t) \\
    a_x\left(i_{t}(x)\right)& \text {otherwise } \end{array}\right..
\end{equation}
Then $\forall \varepsilon \in(0,p_{\min})$, there exist $\kappa>0$, $t_1(\kappa)\geq1$ such that $\forall t\geq t_1(\kappa)$, we have
$\mathbb{P}_\theta\left(\frac{1}{\sqrt{t}} A_t \succeq \kappa I_d \right) \geq 1-2e^{\frac{t\varepsilon^2}{4}}$.
\end{lemma}

As described above, in the exploration phase, for the context $x$, we select an arm from $\mathcal{A}_x$ when necessary so that when covering all contexts, we increase the smallest eigenvalue of the covariates matrix. The result in Lemma \ref{lem:forced_exploration} specifying the rate at which this smallest eigenvalue increases is probabilistic and obtained using concentration results on the time taken to cover all contexts (contexts are \textit{i.i.d.} over time). This contrasts with the plain linear bandit scenario, where a similar forced exploration phase \cite{Jedra20} would actually lead to a deterministic growth of this eigenvalue. We show that the probabilistic guarantees of Lemma \ref{lem:forced_exploration} are sufficient to obtain, together with Lemma \ref{lem:LS_concentration} the appropriate convergence of the LSE $\hat{\theta}_t$ to $\theta$. 

\begin{comment}
The following remark provides a method to select $\{\mathcal{A}_x\}_{x\in\mathcal{X}}$ as the solution of an optimization problem. 
    \begin{remark}[Choice of ${\mathcal{A}}_x$]
    Define $\beta_{x,a}\in\{0,1\}$, $\forall (x,a) \in\mathcal{X}\times \mathcal{A}$. We may select $\mathcal{A}_x = \{a: \beta^\star_{x,a} \neq 0\}$ , $\forall x\in\mathcal{X}$, where $\beta^\star_{x,a}$ is the solution to 
    \begin{equation*}
    \begin{array}{ll}
    & \max\limits_{\beta} \lambda_{1}\left(\sum\limits_{(x,a)\mathcal{X}\times \mathcal{A}}\phi_{x,a}\phi_{x,a}^\top \beta_{x,a} p_\mathcal{X}(x) \right) \\
    &\text {subject to } \beta_{x,a} \in\{0,1\}, \quad \lambda_{1}\left(\sum\limits_{(x,a)\mathcal{X}\times \mathcal{A}} \phi_{x,a} \phi_{x,a}^\top\right) = d.
    \end{array}
    \end{equation*}
    \end{remark}
\end{comment}
\textit{b) Tracking rule.} To complete the design of the sampling rule, it remains to determine the sequence of context-action mappings $(d_t(x))_{t\geq 1}$. Recall that the optimal sampling rule must match an optimal proportion of arm draws in $C_\varepsilon^{\star}(\theta)$. Since $\theta$ is unknown, our sampling rule tracks, at time $t$, an estimated optimal allocation $\alpha(t) \in C_\varepsilon^{\star}(\hat{\theta}_t)$. The following lemma provides a way to devise such tracking rule. 
\begin{lemma}
\label{lem:tracking_lemma}
    Let $(\alpha(t))_{t \geq 1}$ be a sequence taking values in $\Lambda$, such that there exists a compact, convex and non-empty set $C \subset \Lambda$, there exist $\varepsilon>0$ and $t_0(\varepsilon)>0$, such that for all $t\geq t_0(\varepsilon)$, $d_\infty(\alpha(t),C)\leq \varepsilon$. Define 
\small{\begin{equation}
    \label{eq:sampling_rule_track}
    d_t(x) = \argmin_{a \in \supp \left(\sum_{s = 1}^t \alpha(s) \mathbbm{1}_{\{x_s = x\}}\right)} \left( N_{x,a}(t) - \sum_{s = 1}^t \alpha_{x,a}(s) \right), 
\end{equation}}\normalsize
\normalsize where $N_{x,a}(t) = \sum_{s = 1}^t \mathbbm{1}_{\{a_s = a,x_s = x\}}$. 
Then $\forall u \in (0,p_{\min})$, there exist $t_1(\varepsilon,u) \geq t_0(\varepsilon)$ such that $\forall t \geq t_1(\varepsilon,u)$, we have
\footnotesize{$$\mathbb{P}_\theta\left( d_\infty\left(\left(\frac{N_{x,a}(t)}{N_x(t)}\right)_{(x,a)\in\mathcal{X}\times\mathcal{A}},C \right) \le \varepsilon(z_t+d-1)\right)\geq 1-2e^{\frac{t u^2}{4}},$$
where $z_{t} = \max_{x\in \mathcal{X}} |\supp(\sum_{s = 1}^t \alpha(s)\mathbbm{1}_{\{x_s = x\}} ) \setminus \mathcal{A}_x|$.}\normalsize
\end{lemma}

To conclude the description of our sampling rule, we specify the sequence $(\alpha(t))_{t\geq 1}$ (whose asymptotic optimality will come from the previous lemma). We actually only require that 
this sequence satisfies the following condition: there exists $y >0$, and a non-decreasing sequence $(\ell(t))_{t\geq 1}$ such that $\ell(1) = 1$, $\ell(t) \leq t$ and $\lim\inf_{t\to \infty} \ell(t)/t^p $ for some $p>0$ and such that $\forall \kappa>0, \exists h(\kappa): \forall t \geq 1,$
\begin{equation}
    \label{eq:condition_convergence}
     \mathbb{P}\left(\min_{s \geq \ell(t)} d_{\infty}\left(\alpha(t), C_\varepsilon^{\star}\left(\hat{\theta}_{s}\right)\right)>\kappa\right) \leq \frac{h(\kappa)}{t^{2+y}}.
\end{equation}
The condition \eqref{eq:condition_convergence} is easy to ensure in practice (see \cite{Jedra20} for examples of updates of $\alpha(t)$ satisfying such condition).  

The following lemma summarizes the performance of our sampling rule.
\begin{lemma}
\label{lem:convergence_proportions}
Under any sampling rule defined by \eqref{eq:sampling_rule_force}-\eqref{eq:sampling_rule_track} and satisfying condition \eqref{eq:condition_convergence}, we have
$$\lim_{t\to \infty}d_\infty\left(\left(\frac{N_{x,a}(t)}{N_x(t)}\right)_{(x,a)\in\mathcal{X}\times\mathcal{A}},C^\star_\varepsilon(\theta) \right) = 0, \text { a.s.}.$$
\end{lemma}

\subsection{Passive learning algorithm}
\label{sec:passive_learning_algorithm}
We detail below the decision rule and the stopping rule defining our BPI algorithm in the passive learning setting.

\textit{a) Decision rule:} The decision rule is defined in terms of the GLR for parameters $\theta \in U$, expressed as
{\begin{equation*}
Z^x_{U,a,b,\varepsilon}(t) = \log \left(\frac{\max_{\left\{\theta \in U : \theta^{\top}\gamma_{a,b}^x \leq \varepsilon\right\}} \prod_{s=1}^t f_{x_s,a_s}^{\theta}(r_s)}{\max_{\left\{\theta \in U :\theta^{\top}\gamma_{a,b}^x \geq \varepsilon \right\}} \prod_{s=1}^t f_{x_s,a_s}^{\theta}(r_s)}\right).
\end{equation*}}
As for the active setting, we can express $Z^x_{U,a,b,\varepsilon}(t)$ explicitly for $t\geq 1$ such that $P A_t P^\top \succ0$, as 
$$Z^x_{U,a,b,\varepsilon} = \operatorname{sgn}\left(\hat{\theta}_{U,t}^{\top}(P\gamma^x_{b,a})+\varepsilon\right) \frac{\left(\hat{\theta}_{U,t}^{\top}(P\gamma^x_{b,a})+\varepsilon\right)^{2}}{2\|P \gamma^x_{b,a}\|_{(P A_t P^\top)^{-1}}},$$
where $\hat{\theta}_{U,t} = \left(P A_t P^\top\right)^{-1}P \left(\sum_{s = 1}^T \phi_{x_s,a_s}r_s \right)$. Note that $\hat{\theta}_{U,t} \in\mathbb{R}^r$. The \textit{decision rule} is then defined as
\begin{equation}
\label{eq:recommendation_rule_passive}
    \hat{a}_\tau(x) = \argmax_{a \in \mathcal{A}_\varepsilon(\hat{\theta}_{U,\tau},x)} \min_{b \neq a} Z^x_{U,a, b, \varepsilon}(\tau), \quad \forall x\in\mathcal{X}.
\end{equation}

\textit{b) Stopping rule:} Denote by $Z_{U,\varepsilon}^x(t) = \max_{a \in \mathcal{A}_\varepsilon(\hat{\theta}_{U,\tau},x)} \min_{b \neq a} Z^x_{U, a, b, \varepsilon}(t)$. Then, the \textit{stopping rule} is defined as
\small{\begin{align}
    \begin{split}
    \label{eq:stopping_rule_eps_delta_pac_passive}
        \tau =\inf \Big\{t: \forall x, Z_{U,\varepsilon}^x(t)>\beta_U(\delta, t) \text{ and } P A_t P^\top \succeq c I_{r}\Big\}.
    \end{split}
\end{align}}\normalsize
The exploration threshold $\beta_U(\delta,t)$ is selected to ensure that the algorithm is $(U,\varepsilon,\delta)$-PAC, and is defined in the following lemma.
\begin{lemma}
\label{lem:stopping_rule_eps_delta_pac_passive}
Let $u>0$, and define the exploration threshold
\small{\begin{equation}
    \label{eq:expl_rate_eps_delta_pac_passive}
        \beta_U(\delta, t) = (1+u) \log \left(\frac{\operatorname{det}\left((uc)^{-1} P A_t P^\top + I_{r}\right)^{\frac{1}{2}}}{\delta}\right).
\end{equation}}\normalsize
\noindent Under the stopping rule defined by
\eqref{eq:stopping_rule_eps_delta_pac_passive}--\eqref{eq:expl_rate_eps_delta_pac_passive} and under any sampling rule, we have
     $$\mathbb{P}_{\theta}\left(\exists x\in \mathcal{X}: \theta^\top (\phi_{x,a^\star_\theta(x)} - \phi_{x,\hat{a}_\tau(x)}) >\varepsilon, \tau <\infty\right)\leq\delta.$$
\end{lemma}

\subsection{Sample complexity guarantees} 
Next, we establish performance guarantees for the algorithms presented above. Our algorithms achieve a sample complexity, matching (up to a universal multiplicative constant) the approximated lower bound $T^\star_{\theta,\varepsilon}\mathrm{kl}(\delta,1-\delta)$ (or $T_{\theta,\varepsilon}(\alpha)\mathrm{kl}(\delta,1-\delta)$ in the passive learning setting). 

\begin{theorem}
\label{th:optimality}
In the active learning setting, the algorithm defined by \eqref{eq:recommendation_rule}-\eqref{eq:stopping_rule_eps_delta_pac}-\eqref{eq:sampling_rule_force}-\eqref{eq:sampling_rule_track}
is $(\varepsilon,\delta)-$PAC, and its sample complexity satisfies, $\forall \theta\in \mathbb{R}^d$, $\mathbb{P}_\theta\Big(\limsup_{\delta \to 0} \frac{\tau}{\log \left(\frac{1}{\delta}\right)} \lesssim T_{\theta, \varepsilon}^{\star}\Big) = 1$, and $\limsup_{\delta \to 0} \frac{\mathbb{E}_\theta[\tau]}{\log \left(\frac{1}{\delta}\right)} \lesssim T_{\theta,\varepsilon}^{\star}$.
\end{theorem}

\begin{theorem}
\label{th:optimality_passive}
Let $U$ be a linear subspace of $\mathrm{Span}(\Phi_\alpha)$. The algorithm defined by \eqref{eq:recommendation_rule_passive}-\eqref{eq:stopping_rule_eps_delta_pac_passive}
is $(U,\varepsilon,\delta)-$PAC, and its sample complexity satisfies, $\forall \theta\in U$,
$\mathbb{P}_\theta\Big(\limsup_{\delta \to 0} \frac{\tau}{\log \left(\frac{1}{\delta}\right)} \lesssim T_{\theta,\varepsilon}(\alpha)\Big) = 1$, and $\limsup_{\delta \to 0} \frac{\mathbb{E}_\theta[\tau]}{\log \left(\frac{1}{\delta}\right)} \lesssim T_{\theta,\varepsilon}(\alpha)$.
\end{theorem}

==> INFOCOM 2021 - FinalSubmission/Sections/Conclusions.tex <==
\section{Conclusions} 
\label{sec:conclusions}
In this paper, we solved the BPI problem in linear contextual bandits: we derived sample complexity lower bounds and devised algorithms achieving these limits in both the active and passive learning settings. We applied the CL-MAB framework to the RET optimization problem, and demonstrated that our algorithms can identify the best tilt update policy using much fewer samples than rule-based or naive algorithms. Our results are promising and could be extended to various other optimization problems, such as the design of BPI algorithms that accounts for coordination across different sectors. We also plan to investigate, using our framework, the problem of beam management in multiple antenna systems such as Multiple Input Multiple Output (MIMO) systems in 5G networks. 

\section*{Acknowledgements}
This work was partially supported by the Wallenberg AI, Autonomous Systems and Software Program (WASP) funded
by the Knut and Alice Wallenberg Foundation.

%In the active learning setting, the algorithm tracks the optimal allocations suggested by the characteristic time $T^\star_{\theta,\varepsilon}$. In the passive learning setting, given a fixed allocation $\alpha$, based on the GLR, the algorithm stops and outputs the best policy with a sample complexity matching the characteristic time $T_{\theta,\varepsilon}(\alpha)$ suggested by the lower bound. We apply the CL-MAB framework to the RET optimization problem, showing that our algorithms can identify the best tilt update policy using much fewer samples rule-based or naive algorithms. Possible future research directions include the design of BPI algorithms for continuous contexts and applications to Multiple-Input Multiple-Output (MIMO) systems in 5G networks.   

==> INFOCOM 2021 - FinalSubmission/Sections/Experiments.tex <==
\section{Experiments}\label{sec:experiments}
\subsection{Network settings and experimental set-up}
\label{sec:antenna_tilt_experiments}

\noindent
{\it Network simulator.} We run the RET optimization experiments in a 4G simulation environment. The simulation is executed on an urban network consisting of $\mathcal{B}$ BSs, $\mathcal{S}$ sector antennas, and $\mathcal{U}$ users randomly positioned in the environment. The network environment is shown in Fig. \ref{fig:network_env}, and the simulation parameters reported in Table \ref{tab:simulator_setup}. Once the user positions and network parameters are provided, the simulator computes the path loss in the urban environment using the Okomura-Hata propagation model \cite{Rappaport01}, and returns a set of KPIs by conducting user association and resource allocation in a full-buffer traffic demand scenario.

\medskip
\noindent
{\it Learning process.} At each round $t\geq 1$ the network environment generates a new set of random antenna tilts $v_{s,t}$, and user positions, for all $s\in\mathcal{S}$. This yields new values for $N_{\text{OS}}(s,t)$ and $R_{\text{OS}}(s,t)$, that represents the current context (see Sec. \ref{sec:LCB_RET_formulation}). Subsequently, the agent proposes a tilt change $a_{s,t}$, observes $N_{\text{OS}}(s,t+1)$ and $R_{\text{OS}}(s,t+1)$, and computes $p_{s,t}$. The goal is to identify the best tilt change $a_{s,t}$ that, given the current context $x_{s,t}$, produces improved network coverage and capacity as described by the performance function $p_{s,t}$. 

\medskip
\noindent
{\it Optimal update policy.} The best tilt update policy depends on the KPIs importance weight vector $w$. We show the impact of $w$ on $p_{s,t}$ in Fig. \ref{fig:DecisionBoundaries2D}. There, we present the policy decision regions when varying $N_{\text{OS}} \left(s,t\right)$ and $R_{\text{BC}}\left(s,t\right)$, for different values of $w$. Note that when both values of $N_{\textsc{OS}}\left(s,t\right)$ and $R_{\text{BC}}\left(s,t\right)$ are low (i.e., there is an acceptable level of coverage and capacity in the sector), the no-change action is optimal. For high values of $N_{\text{OS}}\left(s,t\right)$ (i.e., when there is a problem in the capacity of the sector), the \textit{down-tilt} action is predicted to be the best. On the contrary, for high values of $R_{\textsc{BC}}\left(s, t\right)$, occurring when there is a problem in the capacity of the sector, the \textit{up-tilt} action becomes optimal. It can be observed that, based on the values of $w$, greater importance is given to $R_{\text{BC}}$ or $N_{\text{OS}}$ in determining of the decision regions. 

\begin{figure}
\centering
  \includegraphics[width = 0.8\columnwidth]{Figures/axcel-map_simple_new.png}
  \caption{Network environment.}
  \label{fig:network_env}
  \vskip -0.1in
\end{figure}
\begin{table}
\centering
\caption{Simulator parameters.}
\begin{tabular}{lcl}
\toprule
\textsc{Simulator parameter} & \textsc{Symbol} & \textsc{Value} \\ \midrule \midrule 
Number of BSs & $\mathcal{B}$ & $7$ \\
Number of sectors & $\mathcal{S}$& $21$ \\
Number of UEs & $\mathcal{U}$ &$2000$ \\
Carrier frequency & $f$ & $1800$ MHz \\
Antenna height&$h$ & $32$ m \\
Minimum tilt angle & $v_{\text{min}}$ & $1^{\circ}$\\
Maximum tilt angle & $v_{\text{max}}$& $16^{\circ}$ \\ \bottomrule 
\label{tab:simulator_setup}
\end{tabular}
\vskip -0.2in
\end{table}

\medskip
\noindent
{\it Algorithms.} In the passive learning setting, in which the sampling rule is fixed, we implement two types of sampling rules: $(i)$ a \textit{random sampling rule}, i.e., $a_t(x)$ is selected with probability $\alpha_{x,a} = 1/K$, for all $(x,a)\in\mathcal{X}\times\mathcal{A}$, and $(ii)$ a \textit{rule-based sampling rule}, selecting actions according to the fuzzy logic algorithm proposed by Buenostado et al. \cite{Buenostado17}. Note that, as opposed to the random sampling, the rule-based one is deterministic, i.e., $\forall x\in\mathcal{X}$, there exists $a(x) \in\mathcal{A}$ such that $\alpha_{x,a(x)} = 1$, and for all $a\in\mathcal{A}\setminus \{a(x)\}$, $\alpha_{x,a(x)} = 0$. For the passive learning setting, we use the decision rule in \eqref{eq:LS_estimator} and the stopping rule in \eqref{lem:stopping_rule_eps_delta_pac}. For the active learning setting, we use the tracking rule as specified in \eqref{eq:sampling_rule_force}-\eqref{eq:sampling_rule_track}.

The algorithm parameters are fixed as $u = 1$ and $c = 0.1$, and we execute our experiments for $\delta = 0.1$ and $\varepsilon \in \{0.1,0.05,0.025\}$. We use $w = [0.6,0.4]$ in our experiments. Since $\mathcal{X}$ is continuous, we use a discrete uniform mesh having $\mathcal{C} = 20^d$ bins to discretize it. We report the lower bound on the sample complexity in terms of $T^\star_{\theta,\varepsilon}\mathrm{kl}(\delta,1-\delta)$ and the empirical sample complexity in terms of mean and standard deviation over $N_{\text{sim}} = 10^3$ runs. Note that to compute $T^\star_{\theta,\varepsilon}$, we use the parameter $\theta$ obtained fitting observations to a linear model as explained below.
\begin{figure}[ht!]
    \centering
    \includegraphics[width = \columnwidth]{Figures/merged-legend-final.png}
    \caption{Policy decision regions for different values of $w$.}
    \label{fig:DecisionBoundaries2D}
\end{figure}
\subsection{Linear model validation}
\label{sec:validation}
We present here results validating the linear model used in the paper. To validate the model, we use the dataset $D$, with $N = 1,125,537$ samples, collected while running the BPI algorithms. First, we split $D$ in a training-set $D_{\text{train}}$ ($80\%)$ and a testing-set $D_{\text{test}}$ ($20\%$), containing $N_{\text{train}} = 900,430 $ and $N_{\text{test}} = 225,107$ samples, respectively. Then, we fit a linear model $\theta$ by computing the LSE solution on the samples contained in $D_{\text{train}}$. We measure the Normalized Root Mean-Squared Error (NRMSE) on $D_{\text{test}}$ between the performance function $p_{s,t}$ (see Section \ref{sec:LCB_RET_formulation}) and the fitted reward model $r^\theta_{s,t} = \theta^\top\phi_{x_{s,t},a_{s,t}}$. The NRMSE is defined as $\mathrm{NRMSE}(\theta) = \frac{1}{\bar{p}}\sqrt{\frac{1}{\mathcal{S}N_\text{test}}\sum_{s = 1}^\mathcal{S}\sum_{t = 1}^{N_{\text{test}}} (p_{s,t} - r^{\theta}_{s,t})^2}$, where $\Bar{p} = \max_{s,t} p_{s,t} - \min_{s,t} p_{s,t}$ is the range of $p_{s,t}$. We attain an NRMSE equal to $\mathrm{NRMSE}(\theta) = 0.15$. Fig. \ref{fig:MSE} reports a sample of the fit between $p_{s,t}$ and $r^{\theta}_{s,t}$ from $100$ randomly sampled data points from $D_{\text{test}}$. The fit is extremely accurate. 

\begin{figure}[ht!]
    \centering
    \includegraphics[width = 0.75\columnwidth]{Figures/fit.png}
    \caption{Comparison of $p_{s,t}$ and $r^\theta_{s,t}$ on $D_{\text{test}}$.}
    \label{fig:MSE}
\end{figure}

\subsection{Results}
The experimental results are shown in Table \ref{tab:results}. Before commenting these results, we note that both sampling rules (random and rule-based) in the passive learning setting allow us to determine $\theta$ accurately, i.e., $U=\mathbb{R}^d$.  

A first observation is that as expected, an active learning approach yields lower sample complexity than the passive learning approach. This can be seen for both the lower bounds and the actual sample complexity achieved under our algorithms. Indeed, being active allows us to explore unexplored dimensions of $\theta$ and in turn to learn faster.

Further, we observe that collecting data using a random policy yields better results than using the rule-based policy. This can be easily explained by noting that the random policy explores more than the rule-based policy and hence speeds up the learning process.

Finally, we note that the proposed algorithms exhibit a sample complexity close to the corresponding information-theoretical limit (they differ from a small multiplicative factor depending on the setting). 

\begin{table}[ht!]
%   \fontsize{8.7}{8.7}\selectfont
\centering
\caption{BPI results for RET optimization.}
\begin{tabular}{clll}\toprule
Sampling rule & $\varepsilon$ & $T^\star_{\theta,\varepsilon}$ & Sample complexity \\ \midrule \midrule
\multirow{3}{*}{Rule-Based} 
& $0.10$  & $123.58$ & $246.16\pm 64.23$  \\ & $0.05$ & $425.63$ & $719.01\pm142.93$  \\ & $0.025$ & $1531.47$ & $2384.03 \pm 313.01$  \\
\midrule 
\multirow{3}{*}{Random} 
& $0.10$  & $69.40$ & $240.58\pm92.75$  \\ & $0.05$  & $231.69$ & $494.55 \pm 89.89$ \\ & $0.025$ & $1487.28$ & $1857.50\pm332.48$  \\ \midrule
\multirow{3}{*}{Adaptive} 
& $0.10$  & $53.23$ & $226.32 \pm52.73$  \\ & $0.05$  & $214.83$ & $444.51 \pm 49.94$ \\ & $0.025$ & $1286.38$ & 
$1545.24\pm212.93$ \\ \bottomrule
\end{tabular} 
\label{tab:results}
\vskip -0.15in
\end{table}

\begin{comment}
\subsection{Passive learning: a synthetic example}
\label{sec:synthtetic_experiments}

To conclude this section, we present experiments for passive learning in Linear Contextual Bandits where the maximal learnable set $U$ is strictly included in $\mathbb{R}^d$. We consider a simplistic example with $d = 3$, $K = 2$ and ${\cal C} = 3$. Let $\theta = [1,1,1]$, and the feature vectors be specified as $\phi_{x_1,a_1} = e_1= [1,0,0]$, $\phi_{x_1,a_2} = [0,1-\Delta,0]$, $\phi_{x_2,a_1} =e_2= [0,1,0]$, $\phi_{x_2,a_2} = [1- \Delta,0,0]$, $\phi_{x_3,a_1} = [1,0,0]$, $\phi_{x_3,a_2} = [0,0,1-\Delta]$, 
for some $\Delta >0$. Contexts have equal probabilities, i.e., $p_\mathcal{X}(x) = 1/3$ for all $x\in\mathcal{X}$. It is easy to see that for a deterministic sampling rule that selects actions $a_t(x) = a_1$, for all $t\geq 1$ and $x\in\mathcal{X}$, we have that $\text{Span}(\Phi_{\alpha})=\text{Span}(e_1,e_2)$. In particular, the third component of $\theta$ is not learnable. In this case, we focus on learning the best policy on the set $U = \text{Span}(e_1,e_2)$. Now, for any sampling rule that selects arms with non-zero probability, e.g. a uniform random policy, we have $\text{Span}(\Phi_{\alpha}) = \mathbb{R}^3$. We conduct experiments to show the performance of our $(U,\delta)-$PAC algorithm, with $U=\text{Span}(e_1,e_2)$ for the deterministic sampling rule and with $U=\mathbb{R}^3$ for a uniform sampling rule. Results are shown in Table \ref{tab:results_udelta} for $N_{\text{sim}} =1000$ independent runs and for $\Delta\in \{0.5,0.9,1.5\}$. Observe that under the deterministic policy, we have a lower information theoretical limit for the sample complexity than under the uniform sampling rule. This is explained by the fact that under the deterministic sampling rule, we just need to identify two components of $\theta$.
\begin{table}[ht!]
\fontsize{9.7}{9.7}\selectfont
\centering
\caption{BPI results for the $(U,\delta)$-PAC example.}
\begin{tabular}{ccrr}\toprule
Sampling Rule  & $\Delta$ & Lower bound & Sample complexity \\ \midrule\midrule    
\multirow{3}{*}{\shortstack{Deterministic\\$(U=\mathbb{R}^2)$}}
& $1.5$  &  $ 13.81$ & $50.70 \pm 17.99$ \\
& $0.9$  &  $ 34.28$ & $120.16 \pm 42.74$ \\ & $0.5$ & $124.33$ & $491.40 \pm 138.22$ \\ \midrule %\hdashline
\multirow{3}{*}{\shortstack{Random\\$(U=\mathbb{R}^3)$}} 
& $1.5$  &  $35.47$ & $160.04 \pm 52.83$ \\& $0.9$  & $102.16$ & $456.63\pm 138.41$ \\ & $0.5$ & $319.29$ & $1654.73 \pm 469.77$ \\ \bottomrule 
\end{tabular} 
\label{tab:results_udelta}
\vskip -0.15in
\end{table}
\end{comment}

==> INFOCOM 2021 - FinalSubmission/Sections/Introduction.tex <==
\section{Introduction}
\label{sec:introduction}
In modern wireless communication systems, algorithms for self-optimization of network parameters constitute an essential tool to increase the network efficiency and reduce its operational cost. Important examples of such algorithms are those controlling the Remote Electrical Tilt (RET) of the antennas at Base Stations (BSs). Coverage Capacity Optimization (CCO) is actually one of the key use-cases specified by Self-Organizing Networks (SONs), the network automation technology introduced by the $3^{rd}$ Generation Partnership Project (3GPP) \cite{Waldhauser11}. The goal in CCO is to maximize the network capacity while ensuring that a targeted service area remains covered. There is a clear trade-off between these two performance indicators: tilting down the antenna decreases the coverage at the sector edge and increases the capacity in the sector center. On the other hand, tilting up the antenna may result in excessive sector overlapping; This increases the interference level in surrounding sectors and leads to a high number of unnecessary handovers and ping-pong effects.

In this paper, we investigate the design of algorithms learning tilt control policies achieving an optimal coverage/capacity trade-off. A tilt control policy takes as input the observed network indicators and outputs a tilt update. We consider two scenarios depending on how the data used in the learning process is generated: $(i)$ in the passive learning scenario, this data corresponds to records of previous events in the network; $(ii)$ in the active learning scenario, the policy used to generate data is actively controlled by the learning algorithm (e.g., putting some emphasis on tilt updates for which we are missing information). The passive learning scenario is particularly relevant in real-world applications where there exists a legacy policy deployed into production and there is no possibility to execute unconstrained exploration due to risk or cost reasons. Active learning algorithms can be applied in test-bed network scenarios in which the operator managing the network allows for unconstrained exploration of tilt configurations to determine the best tilt for each sector. 

The objective of the learning algorithms in both the passive and active learning settings is to come up with an approximately optimal tilt update policy using as few data samples as possible. We formalize the design of these algorithms as a Best Policy Identification (BPI) problem in Contextual Linear Multi-Armed Bandit (CL-MAB) \cite{Langford08}. In such a problem, in each round, the learner observes a {\it context}, selects an {\it arm} depending on this context, and receives in return a random {\it reward} whose mean depends on the (context, arm) pair and is initially unknown. Her goal is, using as few samples (or rounds) as possible, to identify a policy that has maximal expected reward with some level of confidence. 

In our case, contexts correspond to current network indicators, arms to the possible tilt updates, and the reward to the resulting improvement in performance, mixing coverage and capacity. We additionally assume that the expected reward can be modeled as an (unknown) linear function of a feature vector encoding a context-action pair \cite{Li11}. This assumption, that we will justify in the case of tilt policy learning, is often made when the number of contexts or arms become large to make the learning problem tractable.

\begin{samepage}
For CL-MAB, in both active and passive learning settings, we derive for the first time information-theoretic lower bounds on the number of samples required by any algorithm returning an approximately optimal policy with a given level of certainty. We devise algorithms in both learning settings achieving these fundamental limits. We then apply our algorithms to the RET optimization problem in cellular networks. Using extensive experiments in a proprietary simulator, we show that our algorithms can produce optimal tilt update policies using much fewer data samples than naive or rule-based algorithms.
\end{samepage}

==> INFOCOM 2021 - FinalSubmission/Sections/LowerBounds.tex <==
\section{Sample Complexity Lower Bounds}
We present lower bounds on the expected sample complexity satisfied by any $(\varepsilon,\delta)$-PAC (or $(U,\varepsilon,\delta)$-PAC in the passive learning setting) algorithm in CL-MAB. These bounds extend those derived for the plain linear bandit problems \cite{Soare15} to the case of contextual bandits and to that of identification of $\varepsilon$-optimal policies. Our lower bounds are obtained using classical change-of-measure arguments introduced in \cite{lai1985}, and due to space constraints, we just present a sketch of their proofs. The fact that we wish to identify  an $\varepsilon$-optimal policy (rather than the best policy)  significantly complicates the derivation of the lower bounds; these complications are discussed in details in \cite{garivier2019nonasymptotic}. To state our lower bounds, we introduce the following notations. For $x\in\mathcal{X}$ and $(a,b)\in\mathcal{A}^2: a\neq b$, define $\gamma^x_{a,b} = \phi_{x,b}-\phi_{x,a}$. For any given context $x$, we define the set of $\varepsilon$-optimal arms as $\mathcal{A}_\varepsilon(\theta,x) = \{a\in\mathcal{A}: \theta^\top(\phi_{x,a^\star_\theta(x)}-\phi_{x,a})<\varepsilon\}$, and for $a\notin \mathcal{A}_\varepsilon(\theta,x)$, the set $\mathcal{A}_\varepsilon(\theta,x,a) = \{b\in \mathcal{A}_\varepsilon(\theta,x): \theta^\top \gamma_{a,b}^x \geq \varepsilon\}$. For any $\alpha\in \Lambda$, let  $A(\alpha) = \sum_{(x,a) \in\mathcal{X}\times \mathcal{A}} \phi_{x,a} \phi_{x,a}^\top \alpha_{x,a} p_{\mathcal{X}}(x)$. Finally, we introduce the set $B_\varepsilon(\theta)$ of confusing parameters as $B_\varepsilon(\theta) = {\left\lbrace \mu\in\mathbb{R}^d: \exists x \in \mathcal{X}, \forall a \in \mathcal{A}_\varepsilon(\theta,x), \; \mu^{\top}(\phi_{x,a_{\mu}^\star(x)}- \phi_{x,a})>\varepsilon \right\rbrace}$ (when $\mu\in B_\varepsilon(\theta)$, the best policy for $\mu$ is not $\varepsilon$-optimal for $\theta$). 

\subsection{Active learning}
\begin{theorem}
\label{theorem:lb_eps_delta_discrete}
The sample complexity of any $(\varepsilon,\delta)$-PAC algorithm satisfies, $\forall \theta \in \mathbb{R}^d$, $\mathbb{E}_\theta[\tau] \ge (\psi^\star_{\theta,\varepsilon})^{-1}\mathrm{kl}(\delta,1-\delta)$, where 
\begin{equation}
\label{eq:eps_delta_equivalent_lb}
\psi^\star_{\theta,\varepsilon} = \sup_{\alpha\in \Lambda}\inf_{\mu \in B_\varepsilon(\theta)} \frac{1}{2}\|\mu - \theta\|^2_{A(\alpha)}.
\end{equation}%and where $\mathrm{kl}(a,b)$ denotes the KL divergence between two Bernoulli distributions of means $a$ and $b$. 
\end{theorem}

\noindent
{\it Sketch of the proof.} The proof of Theorem \ref{theorem:lb_eps_delta_discrete} proceeds as follows. Consider an $(\varepsilon,\delta)$-PAC algorithm. Let $\mu\in B_\varepsilon(\theta)$. One can show that the expected log-likelihood ratio of the observations under the true parameter $\theta$ and $\mu$ can be written as $\sum_{x,a}\mathbb{E}_\theta \left[N_{x,a}(\tau)\right] \KL(\nu^\theta_{x,a},\nu^{\mu}_{x,a})$ where $N_{x,a}(\tau)$ is the number of times the (context, action) pair $(x,a)$ has been observed before the stopping time $\tau$. Defining $\alpha_{x,a}=\mathbb{E}_\theta \left[N_{x,a}(\tau)\right]/(p_{\cal X}(x)\mathbb{E}_\theta[\tau])$ as the proportion of time arm $a$ is selected when context $x$ appears, we can rewrite the expected log-likelihood ratio as $\frac{\mathbb{E}_\theta[\tau]}{2}\| \theta-\mu\|^2_{A(\alpha)}$. Now define the event $\mathcal{E} = \lbrace \forall x \in \mathcal{X}\; a^\star_\theta(x) = \hat{a}_\tau(x) \rbrace \in \mathcal{F}_\tau$. Since the algorithm is $(\varepsilon,\delta)$-PAC, we have $\mathbb{P}_\theta({\mathcal{E}}) \ge 1- \delta$ and $\mathbb{P}_\mu({\mathcal{E}}) \le\delta$. We conclude, using the data-processing inequality \cite{Garivier19}, that implies $\frac{\mathbb{E}_\theta[\tau]}{2}\| \theta-\mu\|^2_{A(\alpha)}\ge \mathrm{kl}(\mathbb{P}_\theta({\mathcal{E} }),\mathbb{P}_\mu({\mathcal{E} }))\ge \mathrm{kl}(1-\delta,\delta)$. The lower bound is obtained optimizing $\mu$ over the confusing parameters, and selecting the best allocation $\alpha\in \Lambda$.~\ep

\medskip \noindent
{\it Interpretation and tight approximation.} As suggested in the above proof, the allocation $\alpha\in \Lambda$ solving the optimization problem \eqref{eq:eps_delta_equivalent_lb} is optimal: an algorithm relying on a sampling strategy realizing $\alpha$ would yield the lowest possible sample complexity. This allocation however depends on the unknown parameter $\theta$, and to approach it, we need to estimate $\theta$ and repeatedly solve \eqref{eq:eps_delta_equivalent_lb} using these estimators. This is how the so-called track-and-stop algorithms work \cite{Garivier16}. Eq. \eqref{eq:eps_delta_equivalent_lb} is however hard to solve, mainly due to the complexity of the set of confusing parameters $B_\varepsilon(\theta)$.% We can express $\psi^\star_{\theta,\varepsilon}$ as
%$$
%    \psi^\star_{\theta,\varepsilon} = \sup_{\alpha\in \Lambda}\min\limits_{x\in \mathcal{X}} \min \limits_{a\notin \mathcal{A}_\varepsilon(\theta,x)}  \frac{1}{2}\|\Gamma_{x,a} \theta+ e\varepsilon\|^2_{(\Gamma_{x,a}A(\alpha)^{\dagger}\Gamma_{x,a}^\top)^{\dagger}},
%$$
%where $\Gamma_{x,a} = [(\gamma^x_{a,b})^\top]_{b\in I}$, $I \subseteq \mathcal{A}_\varepsilon(\theta,x,a)$ corresponds to the set of active constraints when solving the optimization problem $\inf_{\mu \in B_\varepsilon(\theta, x)} \frac{1}{2} \Vert \mu - \theta\Vert^2_{A(\alpha)}$, and where $e$ is a $|I|$-dimensional vector of ones. Unfortunately, determining $I$ is not easy since it requires a combinatorial search over the set of constraints.

% We can characterize $I$ theoretically 
% \begin{align*}
%     \mathcal{I}_{\theta,x,a} & = \lbrace J \subseteq \mathcal{A}_\varepsilon (\theta, x): \forall b \not\in J, \mu(J)^\top \gamma^x_{a,b} + \varepsilon < 0 \rbrace \\
%     \mu(J) & = \theta + A(\alpha)^{\dagger} \Gamma_{a,x,J}^\top (\Gamma_{a,x,J}A(\alpha)^{\dagger} \Gamma_{a,x,J}^\top)^{\dagger}(\varepsilon e_J - \Gamma_{a,x,J} \theta) \\
%     I &= \argmin_{J \in \mathcal{I}}  \frac{1}{2}\|\Gamma_{x,a,J} \theta+ e_J\varepsilon\|^2_{(\Gamma_{x,a,J}A(\alpha)^{\dagger}\Gamma_{x,a,J}^\top)^{\dagger}}
% \end{align*}
 
% $$
% \psi^\star_{\theta,\varepsilon} = \sup_{\alpha\in \Lambda}\min\limits_{x\in \mathcal{X}} \min \limits_{a\notin \mathcal{A}_\varepsilon(\theta,x)} \frac{1}{2}\|\Gamma_{x,a} \theta+ e\varepsilon\|^2_{(\Gamma_{x,a}A(\alpha)\Gamma_{x,a})^{\dagger}},
% $$
% where $\Gamma_{x,a} = [(\gamma^x_{a,b})^\top]_{b\in I}$, $I = \{b \in \mathcal{A}_\varepsilon(\theta,x): \rho_{b} \neq 0\}$ the set of active constraints, $\rho_b$ is the Lagrange multiplier associated to the $b$-th constraint of the optimization problem, and where $e$ is a $|I|$-dimensional vectors of ones. Unfortunately, determining $I$ is not easy since it requires a combinatorial search over the set of constraints.    

To circumvent this issue, we propose below a simple and tight approximation of the lower bound, easy to compute and hence easy to leverage in the design of a sampling rule. Specifically, we can show that $T^\star_{\theta,\varepsilon}\mathrm{kl}(\delta,1-\delta)$ with
\begin{equation*}
\label{eq:lb_eps_delta_discrete}
       T^\star_{\theta,\varepsilon} = \inf \limits_{\alpha\in\Lambda} \max\limits_{x\in \mathcal{X}} \max  \limits_{a\notin \mathcal{A}_\varepsilon(\theta,x)}\max\limits_{b\in \mathcal{A}_\varepsilon(\theta,x,a)} \frac{2 \|\gamma^x_{a,b}\|^2_{ A(\alpha)^{-1}}}{ (\theta^\top\gamma^x_{a,b}+\varepsilon)^2},
\end{equation*}
is a tight approximation (actually an upper bound) of the lower bound. It is worth noting that the approximation is exact when the objective is to identify the best policy, i.e., when $\varepsilon=0$. Indeed, adapting the proof of the sample complexity lower bound presented in \cite[Theorem 3.1]{Soare15} to the case of CL-MAB, one can readily show that, for any $(0,\delta)$-PAC (or simply $\delta$-PAC) algorithm, the sample complexity lower bound is $T^\star_\theta \mathrm{kl}(\delta,1-\delta)$, with\\ 
$$ 
    T^\star_\theta = \inf\limits_{\alpha \in \Lambda}\max\limits_{x \in \mathcal{X}, a \in \mathcal{A}\setminus\{a^\star_\theta(x)\}} \frac{\|\phi_{x,a_\theta^\star(x)} - \phi_{x,a}\|^2_{ A(\alpha)^{-1}}}{(\theta^\top
    (\phi_{x,a_\theta^\star(x)} - \phi_{x,a}))^2}.$$
This bound coincides with our approximation for $\varepsilon=0$. 

We note that an equivalent way to define $(T^\star_{\theta,\varepsilon})^{-1}$ is through a convex program: $\bar{\psi}^\star_{\theta,\varepsilon} = \sup_{\alpha\in\Lambda}\bar{\psi}_{\theta,\varepsilon}(\alpha)$, where 
$\bar{\psi}_{\theta,\varepsilon}(\alpha) = \inf_{\mu \in \bar{B}_{\varepsilon}(\theta)} \frac{1}{2}\|\theta - \mu\|^2_{A(\alpha)},$
and $\bar{B}_\varepsilon(\theta) = {\left\lbrace \mu\in\mathbb{R}^d: \exists x \in \mathcal{X}, \exists a \in \mathcal{A}_\varepsilon(\theta,x), \; \mu^{\top}(\phi_{x,a_{\mu}^\star(x)}- \phi_{x,a})>\varepsilon \right\rbrace}$.
The following lemma provides a set of properties $\bar{\psi}_{\theta,\varepsilon}$ satisfies.
\begin{lemma}
\label{lem:properties_eps_delta} Let $C_\varepsilon^\star(\theta) = \argsup_{\alpha \in \Lambda} \bar{\psi}_{\theta,\varepsilon}(\alpha)$. For any $\varepsilon\geq 0$, we have
\begin{enumerate}
    \item $\bar{\psi}_{\theta,\varepsilon}(\alpha)$ is continuous in $\theta$ and $\alpha$,
    \item $\exists \; \alpha^\star \in C^\star_{\varepsilon}(\theta)$ such that $A(\alpha^\star) \succ 0$,
    \item $\bar{\psi}_{\theta,\varepsilon}^\star$ is continuous in $\theta$,
    \item $C_{\varepsilon}^\star(\theta)$ is convex, compact and upper hemi-continuous. 
\end{enumerate}
\end{lemma}
\noindent The proof of the above lemma is similar to the one presented in \cite[Lem. 1 \& 2]{Jedra20}. We finish the active learning section by presenting a lemma that gives an upper bound of $T^\star_{\theta,\varepsilon}$. 
\begin{lemma}
\label{lem:T_star_scaling_eps_delta_pac}
$\forall \theta \in \mathbb{R}^d$, $T^\star_{\theta,\varepsilon} \le \frac{d}{\varepsilon^2} \mathbbm{1}_{ \{ \varepsilon>0\} } +\frac{4d}{\Delta_{\min}^2}\mathbbm{1}_{ \{ \varepsilon = 0\} }$, where $\Delta_{\min}=\min_{x, a\neq a_\theta^\star(x)} \theta^\top (\phi_{x,a_\theta^\star(x)}-\phi_{x,a})$ is the minimal gap between the optimal arm and a sub-optimal arm. 
\end{lemma}

\noindent This lemma is proved using similar techniques as those used in \cite[Lem. 2]{Soare15} for plain linear bandits. It provides a worst-case scaling of our lower bound. Note that the lower bound does not scale with the number of contexts (this is expected as $\theta$ is a unique parameter driving the reward in {\it all} contexts). Importantly, the number of samples required to identify the best policy grows as $1/\Delta_{\min}^2$, and typically the minimal gap $\Delta_{\min}$ goes to 0 as the number of contexts grows large. When applying the CL-MAB framework to the RET optimization problem, we may face a very large number of contexts, and this is why we wish to identify $\varepsilon$-optimal policies. Looking for the best policy instead would require too many samples. 

\subsection{Passive learning}
In the passive learning setting, the way arms are selected is fixed and defined through $\alpha\in \Lambda$. Denote by $\Phi_\alpha=\{\phi_{x,a}: \alpha_{x,a}>0\}$. The following theorem states that if $U$ is included in $\mathrm{Span}(\Phi_\alpha)$, then $U$ is PAC-learnable, in which case it also provides a sample complexity lower bound satisfied by any $(U,\varepsilon,\delta)$-PAC algorithm. When $U$ is not included in $\mathrm{Span}(\Phi_\alpha)$, we can easily build an example where $U$ is not PAC-learnable. Indeed, using the data, we can only learn the projection of $\theta$ on $\mathrm{Span}(\Phi_\alpha)$; now, select two vector $\theta$ and $\mu$ whose projections on $\mathrm{Span}(\Phi_\alpha)$ coincide but with different optimal policy (this happens only if for some context $x$, $\alpha_{x,a_\mu^\star(x)}$ or $\alpha_{x,a_\theta^\star(x)}$ is $0$). Obviously, in this case, we cannot learn the optimal policy from the data.  

\begin{theorem}
\label{theorem:off_policy_lb}
Let $U$ be a linear subspace of $\mathrm{Span}(\Phi_\alpha)$. $U$ is PAC-learnable and the sample complexity of any $(U,\varepsilon,\delta)$-PAC algorithm satisfies, $\forall \theta \in U$, $\mathbb{E}_{{\theta}}[\tau]\ge (\psi_{{\theta,\varepsilon}}(\alpha))^{-1}\mathrm{kl}(\delta,1-\delta)$, where $
\psi_{\theta,\varepsilon}(\alpha)=\inf_{\mu \in B_\varepsilon(\theta)\cap U} \frac{1}{2}\|\mu - \theta\|^2_{A(\alpha)}.$
\end{theorem}
    Note that the maximal PAC-learnable set $U$ is $\mathrm{Span}(\Phi_\alpha)$. As for the active learning setting, we can approximate the above lower bound by $T_{\theta,\varepsilon}(\alpha) \mathrm{kl}(\delta,1-\delta)$, with
\begin{equation*}
        T_{{\theta},\varepsilon}(\alpha) = \max\limits_{x\in \mathcal{X}} \max  \limits_{a\notin \mathcal{A}_\varepsilon({\theta},x)}\max\limits_{b\in \mathcal{A}_\varepsilon({\theta},x,a)} \frac{2 \|P\gamma_{a,b}^x\|^2_{ (PA(\alpha)P^\top)^{\dagger}}}{ ({\theta}^\top\gamma_{a,b}^x+\varepsilon)^2},
\end{equation*}
and where we define $P$ be the $r\times d$  orthogonal matrix such that  $\textrm{rows}(P) = \{u_1^\top,\dots,u_r^\top\}$, and $(u_1,\dots,u_r)$ is an orthonormal basis of the subspace $U$.

==> INFOCOM 2021 - FinalSubmission/Sections/ProblemSetting.tex <==
\section{Problem setting}
\label{sec:problemsetting}
In this section, we introduce various BPI problems in CL-MAB. We then explain how to formalize the RET optimization probem using our contextual bandit framework. 
\subsection{Linear Contextual Bandit - Best Policy Identification}
\label{sec:problem_setting}
In CL-MAB, the decision maker or learner observes a context, selects an action based on this context, and receives a noisy sample of the reward associated to the (context, action) pair. Her objective is to learn as fast as possible the best policy, i.e., the policy selecting an action yielding the maximal expected reward when the context $x$ is observed. We denote by $x_t$ the context observed in round $t$, and assume that it is drawn in an \textit{i.i.d.} (over rounds) manner from $p_\mathcal{X}$, a probability distribution over the context space $\mathcal{X} = \{1,\dots,\mathcal{C}\}\subset \mathbb{R}^d$. The learner sequentially interacts with the environment as follows. Given the observed context $x_t$ and observations made in previous rounds, the learner selects an action from a discrete action set $\mathcal{A}=~\{1,\dots,K\}$. 
In CL-MAB, when the learner selects the action $a_t$, she observes and receives a noisy linear reward $r_t = \theta^\top 
\phi_{x_t,a_t} + \xi_t$, where $\xi_t \sim \mathcal{N}(0,1)$ is the noise, and where the feature map $\phi:\mathcal{X}\times \mathcal{A} \mapsto \mathbb{R}^d$ is known, whereas the vector $\theta \in \mathbb{R}^d$ is unknown. In such CL-MAB, the best policy selects for context $x$ an action $a_\theta^\star(x)\in \arg \max_{a\in \mathcal{A}}\theta^\top\phi_{x,a}$. For any given context-action pair $(x,a)$, we denote by $\nu^\theta_{x,a}~=~\mathcal{N}(\theta^\top \phi_{x,a},1)$ the distribution of the corresponding reward, and by $f_{x,a}^\theta$ its density (w.r.t. the Lebesgue measure). We also define, for any context $x$, $\Phi_x \triangleq \{\phi_{x,a}\}_{a \in \mathcal{A}}$, and $\Phi \triangleq \bigcup_{x\in\mathcal{X}}\Phi_x$. We assume that the dimension of the span of $\Phi_x$ (denoted by $\Span(\Phi_x)$) is $d_x\le d$, and that $\Span(\Phi)=\mathbb{R}^d$. Finally, we denote by $\mathbb{P}_\theta$ the probability measure of the observations generated under the parameter $\theta$, and by $\mathbb{E}_\theta$ the respective expectation.  

In this paper, we investigate the problem of BPI in CL-MAB and in the fixed confidence setting. There, the objective is to devise an algorithm that returns, using as few trials as possible, the best policy (or a nearly optimal policy) with some fixed confidence level. Such an algorithm is defined through a sampling rule, a stopping rule, and a recommendation rule.  
\begin{enumerate}
    \item \textit{Sampling rule:} it specifies the action selected in each round. The sampling rule is a sequence of mappings $(a_t)_{t \ge 1}$, where $a_t: \mathcal{X} \to \mathcal{A}$ may depend on past observations ($a_t(x)$ is the selected action in round $t$ when $x_t=x$). Formally, if $\mathcal{D}_{t-1} = \{(x_s,a_s,r_s)\}_{s = 1}^{t-1}$ represents the history of observations up to round $t$, then $a_t$ is $\mathcal{F}_{t-1}$-measurable, where $\mathcal{F}_{t}$ is the $\sigma$-algebra generated by $\mathcal{D}_{t}$ and the context $x_{t+1}$. 
    \item \textit{Stopping rule:} it controls the end of the data acquisition phase and is defined as a stopping time $\tau$ with respect to the filtration $(\mathcal{F}_t)_{t\ge 1}$ such that $\mathbb{P}_\theta(\tau < \infty) = 1$.
    \item \textit{Recommendation rule:} in round $\tau$, after the data acquisition phase ends, the algorithm returns an estimated best policy $\hat{a}_\tau(x)$, $\forall x \in \mathcal{X}$.
\end{enumerate}

We further distinguish two learning scenarios: $(i)$ in the \textit{active learning} setting, the sampling rule has to be designed, and $(ii)$ in the {\it passive learning} setting, it is fixed and imposed. 

\medskip
\noindent
{\it $(i)$ Active learning.} In this setting, we define an $(\varepsilon,\delta)-$PAC algorithm as follows:
\begin{definition}[\textit{$(\varepsilon,\delta)$-PAC algorithm}] Let $\varepsilon \geq 0$ and $\delta\in(0,1)$. An algorithm is $(\varepsilon,\delta)$-PAC if $\forall \theta \in \mathbb{R}^d$, 
$\mathbb{P}_\theta(\exists x \in \mathcal{X}, \; \theta^\top(\phi_{x,a_{{\theta}}^\star(x)}-\phi_{x,\hat{a}_\tau(x)}) > \varepsilon ) \leq \delta$ and $\mathbb{P}_\theta\left(\tau<\infty\right) = 1$.
\label{def:eps_delta_PAC}
\end{definition}
\noindent The objective for active learning is to devise an $(\varepsilon,\delta)-$PAC algorithm with minimal expected sample complexity $\mathbb{E}_\theta[\tau]$.

\medskip
\noindent
\textit{$(ii)$ Passive learning.} In this setting, the sampling rule is fixed. Specifically, we assume that $a_t(x)$ is selected with probability $\alpha_{x,a}$, independently of the actions selected in previous rounds. Here, an algorithm is defined through its stopping and decision rules only. Note that, since the sampling rule is fixed and imposed, the learner may never have enough information to identify $\theta$ completely, and hence to deduce the best policy. This happens when the set of vectors $\phi_{x,a}$ such that $\alpha_{x,a}>0$ does not span $\mathbb{R}^d$.

\noindent To formalize these cases, we introduce, for any linear subspace $U$ of $\mathbb{R}^d$, the notion of $(U,\varepsilon,\delta)-$PAC algorithm as follows:

\begin{definition}[\textit{$(U,\varepsilon,\delta)$-PAC algorithm}] 
    Let $U$ be a non-empty linear subspace of $\mathbb{R}^d$ with dimension $r\leq d$, $\varepsilon \geq 0$, and $\delta \in (0,1)$. We say that an algorithm is ($U,\varepsilon,\delta$)-PAC if $\forall \theta \in U$, 
    $\mathbb{P}_{{\theta}}\left(\exists x \in \mathcal{X}, \; {\theta}^\top(\phi_{x,a_{{{\theta}}}^\star(x)}-\phi_{x,\hat{a}_\tau(x)}) >\varepsilon\right) \leq \delta$ and $\mathbb{P}_{{\theta}}\left(\tau < \infty\right) = 1$.
    \label{def:u_delta_pac}
\end{definition}

In addition, we say that the linear subspace $U \subset \mathbb{R}^d$ is PAC-learnable if there exists a $(U,\varepsilon,\delta)$-PAC algorithm for some $\varepsilon$ and $\delta$. The objective in the passive learning setting is to devise an $(U,\varepsilon,\delta)-$PAC algorithm with minimal expected sample complexity $\mathbb{E}_\theta[\tau]$ whenever $U$ is PAC-learnable.

\medskip
\noindent
\textbf{Notations.} For a Positive Semi Definite (PSD) matrix $G$ (written $G \succcurlyeq 0$) and a vector $v \in \mathbb{R}^d$, define $\|v\|_G = \sqrt{v^\top Gv}$. Denote by $I_d$ the $d$-dimensional identity matrix. For a matrix $M$, denote by $M^\dagger$ its pseudo-inverse, by $\lambda_i(M)$ its $i$-th smallest eigenvalue, and by $\text{vec}(M)$ its vectorization. Define the Kullback-Leibler (KL) divergence for distributions $\nu$ and $\nu^\prime$ as $\KL(\nu, \nu^\prime)$ and the KL divergence between two Bernoulli distributions of mean $a$ and $b$ as $\mathrm{kl}(a,b)$.  Given two vectors $v$ and $u$, their outer product is denoted by $v\otimes u$. Let $\Lambda = \left\{\alpha \in [0,1]^{\vert \mathcal{X}\vert \times \vert \mathcal{A}\vert}: \forall x\in\mathcal{X} \; \sum_{a\in \mathcal{A}} \alpha_{x,a} = 1 \right\}$ denote the set of vectors representing, for each context, a distribution over arms or actions. For any $\alpha, \alpha' \in\Lambda$, we define $d_\infty(\alpha,\alpha') = \max_{(x,a)\in\mathcal{X}\times \mathcal{A}} |\alpha_{x,a}-\alpha'_{x,a}|$. For $\alpha \in \Lambda$, and a set $C \subseteq \mathbb{R}^{|\mathcal{X}|\times |\mathcal{A}|}$, define $d_\infty(\alpha,C) = \inf_{\alpha' \in C} d_\infty(\alpha,\alpha')$.
 We write $\lesssim$ to denote $\leq$ up to a multiplicative constant. 
\subsection{Remote Electrical Tilt Optimization}
\label{sec:ret_setting}

Consider a mobile network consisting of $\mathcal{S}$ sectors, indexed by $s = 1,\dots,\mathcal{S}$. Each sector $s$ is equipped with an antenna, whose tilt angle at time $t$ is denoted by $v_{s,t}$. We assume there are $\mathcal{U}$ User Equipments (UEs) randomly distributed in the network. Our objective is to control the antenna tilts to maximize the network performance, defined as a function of Key Performance Indicators (KPIs). We are after the best RET policy such that when applied to sectors individually, the network performance is optimized. Devising such a unique best RET policy has the advantage of simplicity and is easier to learn as we can exploit the data from all sectors to learn it. 

\subsubsection{Network performance} We use the framework introduced by Buenostado et al. \cite{Buenostado17} to quantify the network performance. There, the network \textit{coverage} and \textit{capacity} are represented through a set of driver KPIs. These KPIs are sector-specific but include the impact of neighboring sectors. They are functions of the Reference Signal Received Power (RSRP), the received power level from the UEs in the sector, and the Timing Advance (TA) that measures the round-trip time from the serving BS to UEs in a sector. We use the two most significant KPIs, $(i)$ the \textit{sector overshooting factor} and $(ii)$ the \textit{bad coverage} indicators.

The \textit{overshooting factor} $N_{\text{OS}}(s,t)$ for sector $s$ at time $t$ quantifies the interference generated by the antenna of sector $s$ in neighbouring sectors. The set of neighboring sectors is denoted as ${\cal N}(s)$. To construct $N_{\text{OS}}(s,t)$, we look, for a given sector $s'\in {\cal N}(s)$, at the proportion of RSRP samples measured in $s'$ that do not differ significantly (using a fixed threshold for the difference) from the RSRP samples corresponding to the signal coming from the antenna of $s$. This proportion indicates the interference generated by $s$ in $s'$. $N_{\text{OS}}(s,t)$ aggregates these interference indicators for sectors in ${\cal N}(s)$. Refer to \cite{Buenostado17} for a detailed expression of the overshooting factor. 
The \textit{bad coverage} $R_{\text{BC}}(s,t)$ for sector $s$ at time $t$ quantifies the lack of coverage at the sector edge, which can be solved by up-tilting the antenna. An RSRP sample is defined as belonging to the edge of sector $s$ if its TA measurement is beyond the \nth{95} percentile of the TA distribution of sector $s$. $R_{\text{BC}}(s,t)$ is defined as the proportion of edge RSRP samples that are below a given threshold. 

\subsubsection{CL-MAB formulation for RET optimization} \label{sec:LCB_RET_formulation} In CL-MAB, the selected action is a function of the context. Naturally, here, the bad coverage and overshooting indicators provide the context. For a given sector $s$, this context is, at time $t$, $x_{s,t}~=~[1, R_{\text{BC}}(s,t),N_{\text{OS}}(s,t)]~\subseteq~[0,1]^3$. In sector $s$, the action $a_{s,t}$ at time $t$ is chosen from the set $\mathcal{A} = \{[1,0,0],[0,1,0],[0,0,1]\}$, representing tilting the antenna up (\textit{up-tilt}), tilting the antenna down (\textit{down-tilt}) or keeping the same tilt (\textit{no-change}), respectively. The reward obtained for given context and action corresponds to the variations in the two KPIs, weighted by some fixed vector $w=[w_{\text{BC}},w_{\text{OS}}]$ with positive components. At time $t$ in sector $s$, the reward is $p_{s,t} = w_\text{BC}(R_\text{BC}(s,t) -R_\text{BC}(s,t+1)) + w_\text{OS}(N_\text{OS}(s,t) -N_\text{OS}(s,t+1))$. The reward function is the same in all sectors, and we approximate it using a unique linear model $(x,a)\mapsto \phi_{x,a}^\top\theta +\xi$. The feature vector for the (context, action) pair $(x,a)$ is defined as $\phi_{x,a} = \text{vec}\left(x \otimes a \right) \in \mathbb{R}^{9}$ (the vector representation of the outer product of $x$ and $a$). In Section \ref{sec:antenna_tilt_experiments}, we justify the choice of this linear model, and illustrate its accuracy (the model is fitted using the least squares estimator on data from different experiments). 

It is worth emphasizing that the reward model is the same across sectors. Hence, we can use the data gathered in any sector to learn the model $\theta$ and identify the best policy. When applying a BPI algorithm, the successive data samples come from various sectors, and the corresponding contexts can be considered as generated in an \textit{i.i.d.} manner, complying to the CL-MAB framework (refer to Section \ref{sec:experiments} for details).


==> INFOCOM 2021 - FinalSubmission/Sections/Proofs.tex <==
\section{Proofs}\label{sec:lemmas}
Due to space constraints, we focus on the active learning setting. The results for passive learning can be established in a similar way. The proofs of many intermediate results are similar to those of the corresponding results for plain linear bandits presented in \cite{Jedra20}. The main difference lies in the fact that, since the sequence of contexts is random (not under our control), we can obtain results with probabilistic guarantees only. This is for example the case for the growth rate of the smallest eigenvalue of the covariates matrix (we could have deterministic guarantees in absence of contexts \cite{Jedra20}). To deal with this randomness, we present the following lemma that provides a concentration result on the number of times a context is observed, and that will be extensively applied in the proofs of the remaining results. 
\begin{lemma}
\label{lem:Nx_concentration_tight}
For any $t\geq 1$, and $\varepsilon>0$, we have
$$\mathbb{P}_\theta\left(\max_{x\in\mathcal{X}} \left|\frac{N_x(t)}{t}-p_{\mathcal{X}}(x)\right|\geq \varepsilon\right) \leq 2e^{-\frac{t \varepsilon^2}{4}}.$$
\end{lemma}
\subsection{Sketch of the proof of Lemma \ref{lem:Nx_concentration_tight}}
The proof follows by applying the concentration result on vector-valued martingales in \cite[Th. 3.5]{iosif_concentration}. Define $N_t-tp_\mathcal{X}=\sum_{s = 1}^t Y_s,$
where $N_t$ is the random vector in $\mathbb{N}^{|\mathcal{X}|}$ with coordinates $N_x(t)$ for $x\in\mathcal{X}$, $p_\mathcal{X}$ is the vector with coordinates $p_\mathcal{X}(x)$ that lies in $\Lambda_\mathcal{X} = \{p_{\mathcal{X}}(x) \in[0,1]^{|\mathcal{X}|}: \sum_{x\in\mathcal{X}} p_\mathcal{X}(x) = 1\}$, and 
$Y_s$ is an i.i.d. zero-mean random vector in $\mathbb R^{|\mathcal{X}|}$ with coordinates $Y_s(x)=\mathbbm{1}_{\{x_s=x\}} - p_\mathcal{X}(x)$ for $x\in \mathcal{X}$. We have 
\begin{align*}
   \|Y_s\|_2^2 & =\sum_{x\in\mathcal{X}}(\mathbbm{1}_{\{x_s=x\}}-p_\mathcal{X}(x))^2 \\&\le \sum_{x\in\mathcal{X
}}(\mathbbm{1}_{\{x_s=x\}}+p_\mathcal{X}(x)^2)  = 1+\sum_{x\in\mathcal{X}}p_\mathcal{X}(x)^2\le2. 
\end{align*}
Hence the assumptions of \cite[Th. 3.5]{iosif_concentration} are satisfied with $r=t\varepsilon$, $D=1$, and $b_*^2=2t$, and we get
{\small\begin{align*}
& \mathbb{P}\Bigg( \max_{x\in\mathcal{X}}\left|\frac{N_x(t)}{t}-p_\mathcal{X}(x)\right|\ge\varepsilon\Bigg) = \mathbb{P}\bigg(\max_{x\in\mathcal{X}}\left|N_x(t)-tp_{\mathcal{X}}(x)\right|\ge t\varepsilon\bigg) \\
& = \mathbb{P}\left(\|N_t-t p_\mathcal{X}\|_\infty \geq t\varepsilon\right) 
\leq \mathbb{P}\left(\|N_t-t p_\mathcal{X}\|_2 \geq t\varepsilon\right) \leq 2 e^{-t\varepsilon^2/4}. \end{align*}}\normalsize 

\subsection{Sketch of the proof of Lemma \ref{lem:stopping_rule_eps_delta_pac}}
The main step of the proof is to show that the probability of the error event, in which the stopping condition is satisfied and there is a context for which the algorithm outputs an $\varepsilon$-suboptimal arm, is smaller than $\delta$.
This follows by $(i)$ upper bounding $Z^x_\varepsilon(t)$ in terms of $\hat{\theta}_t$ and $(ii)$ applying the concentration results for self-normalized processes by \cite{Abbasi11}. More precisely, one can show that for all $x\in\mathcal{X}$,
$Z^x_\varepsilon(t) \leq Z^x_{\hat{a}_t(x), a^\star_\theta(x), \varepsilon}(t) \leq \frac{1}{2}\|\theta - \hat{\theta}_t\|_{A_t}^2.$ Also, it is easy to verify that, under the error event $\mathcal{E} = \Big\{\exists t, \exists x: Z_\varepsilon^x(t)>\beta(\delta, t)\text{ and }  \theta^\top(\phi_{x,a^\star_\theta(x)} - \phi_{x,\hat{a}_t(x)})>\varepsilon  \text{ and } A_t \succeq c I_{d} \Big\}$, and for $u>0$, we have
$$
\|\theta-\hat{\theta}_{t}\|_{A_t}^{2} \leq(1+u)\left\|\sum_{s=1}^{t} \phi_{x_s,a_s} \xi_{s}\right\|_{\left(A_t+u c I_{d}\right)^{-1}}^{2}.
$$
Hence, the error event satisfies 
{\small\begin{align*}
    \mathcal{E} \subseteq \left\{\exists t ,\exists x:  \frac{1+u}{2}\left\|\sum_{s=1}^{t} \phi_{x_s,a_s} \xi_{s}\right\|_{\left(A_t^{\top}+u c I_{d}\right)^{-1}}^{2} \geq \beta(\delta, t)\right\},
\end{align*}}\normalsize
The result follows immediately by selecting $\beta(\delta,t)$ as in  \eqref{eq:expl_rate_eps_delta_pac} and applying the concentration results in \cite[Theorem 1]{Abbasi11}.

\subsection{Sketch of the proof of Lemma \ref{lem:forced_exploration}}
The proof proceeds as follows. First, we show that if for some context $x\in\mathcal{X}$, the condition $A_t(x) \succ f_x(t)$ is violated, then the number of contexts to be observed in order to satisfy the condition again cannot exceed $d_x$ rounds. In fact, one can actually show using similar arguments to \cite[Lem. 5]{Jedra20} applied to each context, to show that exists $t_0 \geq 1$, such that for all $t\geq t_0$, and for all $x\in\mathcal{X}$, $A_t(x) \succeq C_x\sqrt{N_x(t)-d_x-1}$, where $C_x = \frac{1}{\sqrt{d_x}}\sum_{a_x \in \mathcal{A}_x} \phi_{x,a_x} \phi_{x,a_x}^{\top}$. 
Then, applying the concentration results of Lemma \ref{lem:Nx_concentration_tight}, we have $\forall \varepsilon \in\left(0,p_{\min}\right)$, $\forall t\geq t_0$, and w.p. at least $1-2 e^{-\frac{t\varepsilon^2}{4}}$, $A_t(x) \succeq  C_x\sqrt{(p_\mathcal{X}(x)-\varepsilon)t - d_x - 1}.$ By summing over $x$, one can show that
$$
A_t = \sum_{x \in \mathcal{X}}A_t(x) \succeq \min_{x\in\mathcal{X}}\sqrt{\frac{(p_\mathcal{X}(x)-\varepsilon)t-(d_x+1)}{d_x}}  cI_d,
$$
and the result follows by determining, from the above expression, a $t_1(\kappa) \geq t_0$ such that $A_t \succeq \kappa \sqrt{t} I_d.$

\subsection{Sketch of the proof of Lemma \ref{lem:tracking_lemma}}
The proof follows similar steps to \cite[Lem. 6]{Jedra20}. Such steps are applied to each of the contexts, and one can finish by applying the concentration results in Lemma \ref{lem:Nx_concentration_tight}. A key difference is that we actually require convexity on each of the sets $C_x \subset C$, that is guaranteed by the convexity of $C$. To see this, define for $x\in\mathcal{X}$, the projection operator $\text{proj}_x(\cdot)$ that takes $\alpha \in C$ as input, and outputs $\alpha_x$, the $K$-dimensional vector containing the component of $\alpha$ relative to the context $x$. Let $C_x = \{\alpha_x: \alpha_x = \text{proj}_x(\alpha), \forall \alpha \in C\}$.
Note that, since $C \subset \Lambda$ is convex, we have that each of the sets $C_x$ is also convex, and we have $   \forall t\geq t_0, \forall x\in\mathcal{X}, d_\infty(\alpha_x, C_x) \leq \varepsilon.
$
Now, define for all $t\geq 1$, $\varepsilon_{x,a,t} = N_{x,a}(t) - N_x(t)\hat{\alpha}_{x,a}(t)$. One can prove using similar arguments to \cite[Lem. 6]{Jedra20} that (i) there exists $t_0^{\prime}\geq t_0$, $c>0$ such that for all $t \geq t_0'$ we have $\varepsilon_{x,a,t}\leq\left(z_{t}+d- 1\right) \max \left\{t_{0}^{\prime}, c+1\right\},$ and (ii)
for $t\geq t_0'$, $
d_{\infty}\left(\left(N_{x,a}(t)/N_{x}(t)\right)_{(x,a) \in \mathcal{X}\times \mathcal{A}}, C\right) 
\leq \max _{(x,a) \in \mathcal{X}\times \mathcal{A}}\left|\frac{\varepsilon_{x,a,t}}{N_x(t)}\right|. $
Finally, applying Lemma \ref{lem:Nx_concentration_tight}, and determining $t_1(\varepsilon,u)$ such that such that for all $t \ge t_1$ we have $\max_{(x,a) \in \mathcal{X}\times \mathcal{A}}\left|\frac{\varepsilon_{x,a,t}}{(p_\mathcal{X}(x) -u)t}\right| \leq (z_t + d -1)\varepsilon$,  the result follows.

\subsection{Sketch of the proof of Theorem \ref{th:optimality}}
%We divide the proof for the guarantee in probability (a.s.) and in expectation. 
%\\ \noindent \textit{1) Guarantee in probability.}
By Lemma \ref{lem:LS_concentration}, we have $\lim_{t\to \infty} \theta_t = \theta$, a.s. and by Lemma \ref{lem:convergence_proportions} we have $\lim_{t\to \infty}d_\infty\left(\left(N_{x,a}(t)/N_x(t)\right)_{(x,a)\in\mathcal{X}\times\mathcal{A}},C^\star_\varepsilon(\theta) \right) = 0$ a.s. Let $q>0$. By continuity of $\bar{\psi}_\varepsilon$ (Lemma \ref{lem:properties_eps_delta}), one can actually show that there exists $t_0 \geq 1$ such that for all $t\geq t_0$, $ \bar{\psi}_\varepsilon\left(\hat{\theta}_t,\left(N_{x,a}(t)/N_x(t)\right)_{(x,a)\in\mathcal{X} \times \mathcal{A}}\right) \geq (1-q)\bar{\psi}_\varepsilon\left(\theta,\alpha^\star \right),$ for some $\alpha^\star \in C^\star_\varepsilon(\theta)$.
By the definitions of $Z^x_{\varepsilon}$ and $\bar{\psi}_\varepsilon$, for all $t\geq t_0$ we have\\
$
\min_{x\in\mathcal{X}} Z^x_\varepsilon(t) \geq  t \bar{\psi}_\varepsilon\left(\hat{\theta}_{t},\left(N_{x,a}(t)/N_x(t)\right)_{(x,a)\in\mathcal{X} \times \mathcal{A}}\right).
$
By Lemma \ref{lem:forced_exploration}, and by applying the first Borel-Cantelli Lemma, there exists a $t_1 \geq 1$ such that $A_t \succeq c I_d$, for some $c > 0$. This implies that for all $t \geq \max \{t_0,t_1\}$ we have 
\small{\begin{align*}
& \tau  =\inf \Big\{t: \min_{x\in\mathcal{X}} Z_\varepsilon^x(t)>\beta(\delta, t) \text{ and } A_t \succeq c I_{d}\Big\} \\&  \leq \max \{t_0,t_1\} \lor \inf \Big\{t: t(1-q) \bar{\psi}_\varepsilon\left(\theta,\alpha^\star \right)>\beta(\delta, t),\ A_t \succeq c I_{d}\Big\} \\ & \lesssim \max\left\{t_0,t_1, \frac{1}{1-q}T^\star_{\varepsilon,\theta}\log\left(\frac{1}{\delta}\right)\right\},
\end{align*}}\normalsize
where we used \cite[Lem. 18]{Garivier16} for $\delta$ sufficiently small in the last inequality. When $q\to 0$, we get 
$
\mathbb{P}_\theta(\limsup_{\delta \to 0} \frac{\tau}{\log (\frac{1}{\delta})} \lesssim T_{\varepsilon,
\theta}^{\star}) = 1.
$
The proof of the guarantee in expectation is more complex. It proceeds using similar arguments as \cite[Th. 3]{Jedra20}. First, we construct an event $\mathcal{E}_T$ under which, for all $t\geq T$, the stopping time is well-behaved. The event includes the probabilistic results for the tracking and forced exploration rules in Lemma \ref{lem:forced_exploration} and \ref{lem:tracking_lemma}. One can then show that the probabilities of the events under which the sample complexity is not well-behaved are negligible. The proof is concluded by giving an upper bound on the expected sample complexity. 
    


==> INFOCOM 2021 - FinalSubmission/Sections/ProofsApp.tex <==

\begin{comment}
\subsection{Proof of Theorem \ref{theorem:lb_delta}}
\label{app:proof_th_lb_delta}
In order to derive the asymptotic lower bound on the sample complexity, we follow a similar approach to Lemma 1 in \cite{Kauffman16}.
\begin{proof}
We divide the proof in $5$ steps:
\paragraph{The log-likelihood ratio} Let $\nu^\theta$ and $\nu^{\mu}$ be two LCB bandit problems such that for all $(x,a) \in \mathcal{X}\times\mathcal{A}$ the distributions $\nu^\theta_{x,a}$ and $\nu^{\mu}_{x,a}$ are mutually absolutely continuous. We define the log-likelihood ratio of the observation under policy $\pi$ for all $T \ge 1$ 
\begin{equation}
\begin{aligned}
    L_T^{\theta,\mu}(X_1,A_1,R_1,\dots,X_T,A_T,R_T) & =  \log\left(\frac{f^\theta(X_1,A_1,R_1,\dots,X_T,A_T,R_T)}{f^{\mu}(X_1,A_1,R_1,\dots,X_T,A_T,R_T)}\right)\\
    & = \sum_{t=1}^T \log\left(\frac{f^\theta(R_t\vert X_t, A_t)}{f^{\mu}(R_t \vert X_t,A_t)}\right) \\ 
    & =\sum_{t=1}^{T} \sum\limits_{(x,a) \in\mathcal{X}\times \mathcal{A}}\mathbbm{1}\left\{ X_{t}=x,A_{t}=a\right\} \log \left(\frac{f_{x,a}^\theta\left(R_{t}\right)}{f_{x,a}^{\mu}\left(R_{t}\right)}\right). \\
    \end{aligned}
\end{equation}

\paragraph{The change of measure argument} Lemma 19 in \cite{Kauffman16} ensures that for all parameters $\theta,\mu \in \mathbb{R}^d$ and any stopping time $\tau$ w.r.t. $\mathcal{F}_t$. 
$$
\mathbb{E}\left[ L_\tau^{\theta,\mu} \right] \ge \sup_{\mathcal{E} \in \mathcal{F}_\tau}\mathrm{kl}\left(\mathbb{P}_\theta(\mathcal{E}), \mathbb{P}_{\mu}( \mathcal{E} ) \right) 
$$
Define the set of confusing parameters 
\begin{align*}
B(\theta) & \triangleq \left\lbrace \mu \in \mathbb{R}^d: \; \exists x \in \mathcal{X},\; a_{\mu}^\star(x) \neq a^\star_{\theta}(x) \right\rbrace \\
& = \left\lbrace \mu \in \mathbb{R}^d: \; \exists x \in \mathcal{X},\; \mu^\top (\phi_{x,a_{\mu}^\star(x)} - \phi_{x,a^\star_{\theta}(x)}) > 0 \right\rbrace \\ 
& = \bigcup_{x\in\mathcal{X}, a \in \mathcal{A} \backslash\lbrace a_\theta^\star(x) \rbrace}  \left\lbrace \mu \in \mathbb{R}^d: \; \mu^\top (\phi_{x,a} - \phi_{x,a^\star_{\theta}(x)}) > 0 \right\rbrace
\end{align*}
Define the event $\mathcal{E} = \lbrace \forall x \in \mathcal{X}\; a^\star_\theta(x) = \hat{a}_\tau(x) \rbrace \in \mathcal{F}_\tau$, and note that since $\pi$ is $\delta$-PAC it holds that 
$$
\mathbb{P}_\theta(\mathcal{E}) \ge 1- \delta,
$$
and for all $\mu \in B(\theta)$ that 
$$
\mathbb{P}_{\mu}(\mathcal{E}) \le \delta.
$$
Therefore 
$$
\forall \mu \in B(\theta) \qquad \mathbb{E}\left[ L_\tau^{\theta,\mu} \right] \ge \mathrm{kl}\left(1- \delta, \delta \right).
$$

\paragraph{The expected log-likelihood ratio} Taking expectation we have 
\begin{align*}
    \mathbb{E}_\theta\left[L_\tau^{\theta,\mu} \right] 
    & = \mathbb{E}_\theta \left[ \sum_{t=1}^\infty \mathbbm{1}\left\{ \tau > t-1 \right\} \sum\limits_{(x,a) \in\mathcal{X}\times \mathcal{A}} \mathbbm{1}\left\{X_{t}=x, A_{t}=a\right\} \log \left(\frac{f_{x,a}^\theta\left(R_{t}\right)}{f_{x,a}^{\mu}\left(R_{t}\right)}\right) \right]  
    \\ & =  \mathbb{E}_\theta \left[\sum_{t=1}^\infty \mathbb{E}_\theta \left[  \sum\limits_{(x,a) \in\mathcal{X}\times \mathcal{A}}\mathbbm{1}\left\{ \tau > t-1 \right\} \mathbbm{1}\left\{X_{t}=x, A_{t}=a\right\} \log \left(\frac{f_{x,a}^\theta\left(R_{t}\right)}{f_{x,a}^{\mu}\left(R_{t}\right)}\right)  \bigg\vert \mathcal{F}_{t-1}\right] \right] 
    \\ & = \mathbb{E}_\theta \left[\sum_{t=1}^\infty \sum\limits_{(x,a) \in\mathcal{X}\times \mathcal{A}}\mathbbm{1}\left\{ \tau > t-1 \right\} \mathbbm{1}\left\{X_{t}=x, A_{t}=a\right\} \mathbb{E}_\theta \left[ \log \left(\frac{f_{x,a}^\theta\left(R_{t}\right)}{f_{x,a}^{\mu}\left(R_{t}\right)}\right)  \bigg\vert \mathcal{F}_{t-1}\right] \right] 
    \\ & = \sum\limits_{(x,a) \in\mathcal{X}\times \mathcal{A}} \mathbb{E}_\theta \left[\sum_{t=1}^\infty \mathbbm{1}\left\{ \tau > t-1 \right\} \mathbbm{1}\left\{X_{t}=x, A_{t}=a\right\} \KL(\nu^\theta_{x,a},\nu^{\mu}_{x,a}) \right] \\
    & = \sum\limits_{(x,a) \in\mathcal{X}\times \mathcal{A}} \mathbb{E}_\theta \left[N_{x,a}(\tau)\right] \KL(\nu^\theta_{x,a},\nu^{\mu}_{x,a}) 
\end{align*}
where we used $\lbrace X_t = x, A_t = a\rbrace, \lbrace \tau > t-1\rbrace \in \mathcal{F}_{t-1}$, noted that $\mathbb{E}_{\theta}\left[\log \left(\frac{f_{x,a}^\theta\left(Y_{x,a,t}\right)}{f_{   x,a}^{\mu}\left(Y_{x,a,t}\right)}\right)\right] = \KL(\nu^\theta_{x,a},\nu^{\mu}_{x,a})$, and introduced $N_{x,a}(\tau) = \sum_{t = 1}^\tau \mathbbm{1}\left\{X_{t}=x, A_{t}=a\right\}$. Some integrability assumptions are needed for the exchange of integrals but these are mild and we will assume that they hold. Under Gaussian noise model we obtain 
\begin{equation}
    \mathbb{E}_\theta\left[ L_\tau^{\theta,\mu} \right] = \frac{1}{2} (\theta - \mu)^\top \left(\sum\limits_{(x,a) \in\mathcal{X}\times \mathcal{A}} \mathbb{E}_\theta\left[N_{x,a}(\tau)\right] \phi_{x,a} \phi_{x,a}^\top\right) (\theta - \mu)
\end{equation}

\paragraph{Optimizing the lower bound} From the above we have 
\begin{align}
    \inf_{\mu \in B(\theta)} \frac{1}{2} (\theta - \mu)^\top \left(\sum\limits_{(x,a) \in\mathcal{X}\times \mathcal{A}} \mathbb{E}_\theta\left[N_{x,a}(\tau)\right] \phi_{x,a} \phi_{x,a}^\top\right) (\theta - \mu) \ge \mathrm{kl}(1- \delta, \delta).
\label{eq:optimization_lb}
\end{align}
We may further note that 
\begin{equation}
\begin{aligned}
     \inf_{\mu \in B(\theta)} \frac{1}{2} (\theta - \mu)^\top &  \left(\sum\limits_{(x,a) \in\mathcal{X}\times \mathcal{A}} \mathbb{E}_\theta\left[N_{x,a}(\tau)\right] \phi_{x,a} \phi_{x,a}^\top\right) (\theta - \mu)\\ 
     & = \mathbb{E}[\tau] \inf_{\mu \in B(\theta)} \frac{1}{2} (\theta - \mu)^\top \left(\sum\limits_{(x,a) \in\mathcal{X}\times \mathcal{A}} \frac{\mathbb{E}_\theta\left[N_{x,a}(\tau)\right]}{\mathbb{E}_\theta\left[N_x(\tau)\right]}\frac{\mathbb{E}_\theta\left[N_{x}(\tau)\right]}{\mathbb{E}_\theta\left[\tau\right]} \phi_{x,a} \phi_{x,a}^\top\right) (\theta - \mu) \\
     & = \mathbb{E}_\theta[\tau] \inf_{\mu \in B(\theta)} \frac{1}{2} (\theta - \mu)^\top \left(\sum\limits_{(x,a) \in\mathcal{X}\times \mathcal{A}} \alpha_{x,a}p_{\mathcal{X}}(x)\phi_{x,a} \phi_{x,a}^\top \right) (\theta - \mu) \\
     & \le \mathbb{E}[\tau] \sup_{\alpha \in \Lambda}\inf_{\mu \in B(\theta)} \frac{1}{2} (\theta - \mu)^\top \left(\sum\limits_{(x,a) \in\mathcal{X}\times \mathcal{A}} \alpha_{x,a} p_{\mathcal{X}}(x) \phi_{x,a} \phi_{x,a}^\top\right) (\theta - \mu) \\
     & = \mathbb{E}[\tau] \sup_{\alpha \in \Lambda}\inf_{\mu \in B(\theta)} \frac{1}{2} \|\theta - \mu\|^2_{A(\alpha)},
\end{aligned}
     \label{eq:optim_lb_discrete}
\end{equation}
where we introduced the context count $N_x(\tau) = \sum_{t =1}^\tau \mathbbm{1}\{X_t = x\}$, the conditional context-arm proportions $\alpha_{x,a} = \frac{\mathbb{E}_{\theta}\left[N_{x,a}(\tau)\right]}{\mathbb{E}_{\theta}\left[N_x(\tau)\right]}$, the matrix $A(\alpha) = \left(\sum\limits_{(x,a) \in\mathcal{X}\times \mathcal{A}} \alpha_{x,a} p_{\mathcal{X}(x)}\phi_{x,a} \phi_{x,a}^\top\right)$, the joint probability simplex by $\Lambda =\lbrace \alpha \in [0,1]^{\vert \mathcal{A} \vert\times\vert \mathcal{X} \vert}: \forall x\in\mathcal{X} \; \sum_{a\in \mathcal{A}} \alpha_{x,a} = 1 \rbrace$ and noted that $ p_{\mathcal{X}}(x) = \frac{\mathbb{E}_\theta\left[N_x(\tau)\right]}{\mathbb{E}_\theta\left[\tau\right]}$. Here, $\alpha \in \Lambda$ may be interpreted as the asymptotic arm proportions conditioned on context $x$, i.e., the fraction of times that arm $a$ is selected given that context $x$ is observed.

We define the characteristic time $T^\star_\theta$ as follows 
$$
(T^\star_\theta)^{-1} = \sup_{\alpha \in \Lambda} \inf_{\mu \in B(\theta)}  \frac{1}{2} \|\theta - \mu\|^2_{A(\alpha)},
$$ 
and write the lower bound as 
\begin{equation*}
    \mathbb{E}[\tau] \ge T^\star_\theta  \mathrm{kl}(1- \delta, \delta) \gtrsim T^\star_\theta\log\left(\frac{1}{\delta}\right).
\end{equation*}

\paragraph{Solution of the optimization problem} Introduce the following function 
$$
\psi(\theta, \alpha) =  \inf_{\mu \in B(\theta)}  \frac{1}{2} \|\theta - \mu\|^2_{A(\alpha)} 
$$
and note that $(T^\star_\theta)^{-1} 
= \sup_{\alpha \in \Lambda} \psi(\theta, \alpha)$. Further note that the set of confusing parameters may be partitioned as follows   
$$
B(\theta) = \bigcup_{x\in\mathcal{X}} \bigcup _{a \in \mathcal{A}\backslash\lbrace a^\star_\theta(x)\rbrace} B(\theta, x, a),
$$
where $B(\theta, x, a) \triangleq \left\lbrace \mu \in \mathbb{R}^d: \; \mu^\top (\phi_{x,a} - \phi_{x,a^\star_{\theta}(x)}) > 0 \right\rbrace$. So we may carry the following split 
\begin{equation*}
    \psi(\theta, \alpha) = \min_{x \in \mathcal{X}, a \in \mathcal{A}\backslash\lbrace a_\theta^\star(x) \rbrace} \inf_{\mu \in B(\theta, x, a)} \|\theta - \mu\|^2_{A(\alpha)}.
\end{equation*}
The resulting sub-optimization problems are convex optimization problems that may be solved explicitly. The solution closely follows the approach in \cite{Soare15}. Consider $\Gamma^\star_\theta(x) = \{\phi_{x,a^\star_\theta(x)} - \phi_{x,a}, \forall a \in\mathcal{A}\}$ and $\omega = \theta-\mu$. 
The event that two arms differ in two environments $\theta$, $\mu$ implies that there exists at least one $\gamma \in \Gamma^\star_\theta(x)$ such that
$$ \gamma^{\top} \mu<0 \Leftrightarrow \gamma^{\top} \theta-\gamma^{\top} \mu>\gamma^{\top} \theta  \Leftrightarrow \gamma^{\top} \omega>\gamma^{\top} \theta .$$ 

Thus, we can rewrite the optimization problem as 
\begin{equation*}
    \begin{aligned} 
    &\inf \frac{1}{2}\omega^\top A(\alpha) \omega 
    \\&\text{subject to } \exists \gamma \in \Gamma^\star_\theta(x), \gamma^{\top} \omega \geq \gamma^{\top} \theta.
    \end{aligned}
\end{equation*}

The Lagrangian for this optimization problem is
$$L(\omega, \rho) = \frac{1}{2}\omega^{\top} A(\alpha) \omega+\rho\left(-\gamma^{\top} \omega+\gamma^\top\theta\right),$$
with Lagrange multipliers $\rho \in \mathbb{R}$. Imposing the optimality conditions leads to the system
\begin{equation}
\begin{cases}
    \frac{\partial L}{\partial \omega} = A(\alpha)\omega-\rho \gamma=0 \Leftrightarrow A(\alpha) \omega= \rho\gamma \\ 
    \rho\frac{\partial L}{\partial \rho}=\rho(-\gamma^{\top} \omega+\gamma^{\top} \theta)=0 
    \\ \gamma^\top\omega \geq \gamma^\top \theta
    \\ \rho \geq 0
\end{cases}.
\label{eq:KKT_approx_delta_pac}
\end{equation}

Let $\rho\neq 0 \Rightarrow (-\gamma^{\top} \omega+\gamma^{\top} \theta)=0 $. For $A(\alpha) \succ 0$, solving for $\omega$ from the first equation of Eq. \eqref{eq:KKT_approx_delta_pac} and substituting in the second equation of Eq. \eqref{eq:KKT_approx_delta_pac}, we get
$$\rho = \frac{\gamma^\top\theta }{\|\gamma\|^2_{A(\alpha)^{-1}}}. $$
Note that $\rho > 0$, thus we have a feasible solution to the optimization problem.
We have $$\frac{1}{2}\omega^\top A(\alpha)\omega = \frac{(\gamma^\top \theta)^\top\gamma^\top A(\alpha)^{-1}A(\alpha)A(\alpha)^{-1}\gamma(\gamma^\top \theta )}{2\|\gamma\|_{A(\alpha)^{-1}}^4}= \frac{(\gamma^\top \theta)^\top\gamma^\top A(\alpha)^{-1}\gamma(\gamma^\top \theta )}{\|\gamma\|_{A(\alpha)^{-1}}^4} = \frac{(\gamma^\top \theta )^2 }{2\|\gamma\|^2_{A(\alpha)^{-1}}}.$$

In case $\lambda_{1}(A(\alpha)) = 0$ we have $\frac{\omega^\top A(\alpha)\omega}{2} = 0$. 
By substitution into the lower bound we get
\begin{align*}
    \inf_{\mu \in B(\theta, x, a)} \frac{1}{2}  \|\theta - \mu\|^2_{A(\alpha)} =
     \begin{cases}
    \frac{ (\theta^\top\gamma_{x,a})^2}{2\gamma_{x,a}^\top A(\alpha)^{-1} \gamma_{x,a}} & \text{ if } A(\alpha) \succ 0 \\
    0 &\text{ otherwise}
    \end{cases},
\end{align*}
where $\gamma_{x,a} = (\phi_{x,a^\star_\theta(x)} - \phi_{x,a})$.
Thus we may conclude that $\mathbb{E}_\theta[\tau] \gtrsim T^\star_{\theta}\log\left(\frac{1}{\delta}\right)$ with
\begin{equation*}
    T^\star_\theta = \begin{cases} \inf\limits_{\alpha\in\Lambda}\max\limits_{x \in \mathcal{X}, a \in \mathcal{A}\backslash\lbrace a_\theta^\star(x) \rbrace} \frac{ (\theta^\top\gamma_{x,a})^2}{2\gamma_{x,a}^\top A(\alpha)^{-1} \gamma_{x,a}} & \text{ if } A(\alpha) \succ 0 \\
    0 & \text{ otherwise}
    \end{cases}.
\end{equation*}
\end{proof}
\end{comment}
\section{Proofs}
\subsection{Proof of Theorem \ref{theorem:lb_eps_delta_discrete}}
\label{app:proof_th_eps_delta_lb}
\begin{proof}
%The proof follows the proof of Theorem \ref{theorem:lb_delta}. The main differences are at step $2$ (change of measure argument) and at step $5$ (solution of the optimization problem). %Indeed the main change is in the PAC policy definition that in turn modifies the set of confusing parameters and the optimization problem.
We divide the proof in $5$ steps:

\textit{1) The log-likelihood ratio:} Let $\nu^\theta$ and $\nu^{\mu}$ be two LCB bandit problems such that for all $(x,a) \in \mathcal{X}\times\mathcal{A}$ the distributions $\nu^\theta_{x,a}$ and $\nu^{\mu}_{x,a}$ are mutually absolutely continuous. We define the log-likelihood ratio of the observation under algorithm $(a_t,\tau,\hat{a}_\tau)$, for all $T \geq 1$ as
\begin{equation}
\label{label:log_like}
\begin{aligned}
    L_T^{\theta,\mu}(x_1,a_1,r_1,\dots,x_T,a_T,r_T) & =  \log\left(\frac{f^\theta(x_1,a_1,r_1,\dots,x_T,a_T,r_T)}{f^{\mu}(x_1,a_1,r_1,\dots,x_T,a_T,r_T)}\right)\\
    & = \sum_{t=1}^T \log\left(\frac{f^\theta(r_t\vert x_t, a_t)}{f^{\mu}(r_t \vert x_t,a_t)}\right) \\ 
    & =\sum_{t=1}^{T} \sum\limits_{(x,a) \in\mathcal{X}\times \mathcal{A}}\mathbbm{1}\left\{ x_{t}=x,a_{t}=a\right\} \log \left(\frac{f_{x,a}^\theta\left(r_{t}\right)}{f_{x,a}^{\mu}\left(r_{t}\right)}\right). \\
    \end{aligned}
\end{equation}

\textit{2) The change of measure argument:} Recall the definition of set of $\varepsilon$-optimal arms $\mathcal{A}_\varepsilon(\theta, x) = \{ b\in\mathcal{A}: \theta^\top (\phi_{x,a^\star_\theta(x)} - \phi_{x,b}) \le \varepsilon \}$. Define the set of confusing parameters as
$$ B_{\varepsilon}(\theta) \triangleq \left \lbrace \mu \in \mathbb{R}^d: \; \exists x \in \mathcal{X}, \forall b \in \mathcal{A}_\varepsilon(\theta,x), \; \mu^{\top}(\phi_{x,a_{\mu}^\star(x)}- \phi_{x,b})>\varepsilon \right\rbrace. $$
Define the event:

$$ \mathcal{E}_{\theta} = \{\forall x \in \mathcal{X}, \theta^{\top}(\phi_{x,a_{\theta}^\star(x)} - \phi_{x,\hat{a}_{\tau}(x)})< \varepsilon \} = \{ \forall x \in \mathcal{X}, \hat{a}_{\tau}(x) \in \mathcal{A}_\varepsilon(\theta,x) \}, $$ 
and note that, since the algorithm is $(\varepsilon,\delta)$-PAC, it holds that
$$
\mathbb{P}_{\theta}(\mathcal{E}_{\theta}) \ge 1-\delta,
$$
and $\forall \mu \in B_{\varepsilon}(\theta)$ 
$$
\mathbb{P}_{\mu}(\mathcal{E}_{\theta}) \leq \delta.
$$
The last inequality follows from the fact that $\forall \mu\in B_\varepsilon(\theta)$ we have $\mathcal{A}_\varepsilon(\theta, x) \cap \mathcal{A}_\varepsilon(\mu, x) = \emptyset$, and hence $\mathcal{A}_\varepsilon(\theta,x) \subseteq \mathcal{A}^c_\varepsilon(\mu,x)$. This in turn implies 
$$
\mathbb{P}_{\mu}(\mathcal{E}_{\theta}) = \mathbb{P}_{\mu}(\forall x \in \mathcal{X}, \hat{a}_{\tau}(x) \in \mathcal{A}_\varepsilon(\theta,x)) \leq \mathbb{P}_{\mu}(\forall x \in \mathcal{X}, \hat{a}_{\tau}(x) \in \mathcal{A}^{c}_{\varepsilon}(\mu,x)) \leq \delta.
$$
Therefore we get by Lemma 19 in \cite{Kauffman16} that
$$
\forall \mu \in B_{\varepsilon}(\theta) \qquad \mathbb{E}\left[ L_\tau^{\theta,\mu} \right] \ge \mathrm{kl}\left(1-\delta, \delta \right) \gtrsim \log(1/\delta).
$$

\textit{3) The expected log-likelihood ratio:} Taking the expectation of \eqref{label:log_like}, we get 
\begin{align*}
    \mathbb{E}_\theta\left[L_\tau^{\theta,\mu} \right] 
    & = \mathbb{E}_\theta \left[ \sum_{t=1}^\infty \mathbbm{1}\left\{ \tau > t-1 \right\} \sum\limits_{(x,a) \in\mathcal{X}\times \mathcal{A}} \mathbbm{1}\left\{X_{t}=x, A_{t}=a\right\} \log \left(\frac{f_{x,a}^\theta\left(R_{t}\right)}{f_{x,a}^{\mu}\left(R_{t}\right)}\right) \right]  
    \\ & =  \mathbb{E}_\theta \left[\sum_{t=1}^\infty \mathbb{E}_\theta \left[  \sum\limits_{(x,a) \in\mathcal{X}\times \mathcal{A}}\mathbbm{1}\left\{ \tau > t-1 \right\} \mathbbm{1}\left\{X_{t}=x, A_{t}=a\right\} \log \left(\frac{f_{x,a}^\theta\left(R_{t}\right)}{f_{x,a}^{\mu}\left(R_{t}\right)}\right)  \bigg\vert \mathcal{F}_{t-1}\right] \right] 
    \\ & = \mathbb{E}_\theta \left[\sum_{t=1}^\infty \sum\limits_{(x,a) \in\mathcal{X}\times \mathcal{A}}\mathbbm{1}\left\{ \tau > t-1 \right\} \mathbbm{1}\left\{X_{t}=x, A_{t}=a\right\} \mathbb{E}_\theta \left[ \log \left(\frac{f_{x,a}^\theta\left(R_{t}\right)}{f_{x,a}^{\mu}\left(R_{t}\right)}\right)  \bigg\vert \mathcal{F}_{t-1}\right] \right] 
    \\ & = \sum\limits_{(x,a) \in\mathcal{X}\times \mathcal{A}} \mathbb{E}_\theta \left[\sum_{t=1}^\infty \mathbbm{1}\left\{ \tau > t-1 \right\} \mathbbm{1}\left\{X_{t}=x, A_{t}=a\right\} \KL(\nu^\theta_{x,a},\nu^{\mu}_{x,a}) \right] \\
    & = \sum\limits_{(x,a) \in\mathcal{X}\times \mathcal{A}} \mathbb{E}_\theta \left[N_{x,a}(\tau)\right] \KL(\nu^\theta_{x,a},\nu^{\mu}_{x,a}),
\end{align*}
where we used $\lbrace x_t = x, a_t = a\rbrace, \lbrace \tau > t-1\rbrace \in \mathcal{F}_{t-1}$, noted that $\mathbb{E}_{\theta}\left[\log \left(\frac{f_{x,a}^\theta\left(Y_{x,a,t}\right)}{f_{   x,a}^{\mu}\left(Y_{x,a,t}\right)}\right)\right] = \KL(\nu^\theta_{x,a},\nu^{\mu}_{x,a})$, and introduced $N_{x,a}(\tau) = \sum_{t = 1}^\tau \mathbbm{1}\left\{x_{t}=x, a_{t}=a\right\}$. Some integrability assumptions are needed for the exchange of integrals but these are mild and we will assume that they hold. Under Gaussian noise we obtain 
\begin{equation}
    \mathbb{E}_\theta\left[ L_\tau^{\theta,\mu} \right] = \frac{1}{2} (\theta - \mu)^\top \left(\sum\limits_{(x,a) \in\mathcal{X}\times \mathcal{A}} \mathbb{E}_\theta\left[N_{x,a}(\tau)\right] \phi_{x,a} \phi_{x,a}^\top\right) (\theta - \mu)
\end{equation}


\textit{4) Optimizing the lower bound.} From the above we have 
\begin{align}
    \inf_{\mu \in B_\varepsilon(\theta)} \frac{1}{2} (\theta - \mu)^\top \left(\sum\limits_{(x,a) \in\mathcal{X}\times \mathcal{A}} \mathbb{E}_\theta\left[N_{x,a}(\tau)\right] \phi_{x,a} \phi_{x,a}^\top\right) (\theta - \mu) \ge \mathrm{kl}(1- \delta, \delta).
\label{eq:optimization_lb}
\end{align}
We may further note that 
\begin{equation}
\begin{aligned}
     \inf_{\mu \in B_\varepsilon(\theta)} \frac{1}{2} (\theta - \mu)^\top &  \left(\sum\limits_{(x,a) \in\mathcal{X}\times \mathcal{A}} \mathbb{E}_\theta\left[N_{x,a}(\tau)\right] \phi_{x,a} \phi_{x,a}^\top\right) (\theta - \mu)\\ 
     & = \mathbb{E}[\tau] \inf_{\mu \in B_\varepsilon(\theta)} \frac{1}{2} (\theta - \mu)^\top \left(\sum\limits_{(x,a) \in\mathcal{X}\times \mathcal{A}} \frac{\mathbb{E}_\theta\left[N_{x,a}(\tau)\right]}{\mathbb{E}_\theta\left[N_x(\tau)\right]}\frac{\mathbb{E}_\theta\left[N_{x}(\tau)\right]}{\mathbb{E}_\theta\left[\tau\right]} \phi_{x,a} \phi_{x,a}^\top\right) (\theta - \mu) \\
     & = \mathbb{E}_\theta[\tau] \inf_{\mu \in B_\varepsilon(\theta)} \frac{1}{2} (\theta - \mu)^\top \left(\sum\limits_{(x,a) \in\mathcal{X}\times \mathcal{A}} \alpha_{x,a}p_{\mathcal{X}}(x)\phi_{x,a} \phi_{x,a}^\top \right) (\theta - \mu) \\
     & \le \mathbb{E}[\tau] \sup_{\alpha \in \Lambda}\inf_{\mu \in B_\varepsilon(\theta)} \frac{1}{2} (\theta - \mu)^\top \left(\sum\limits_{(x,a) \in\mathcal{X}\times \mathcal{A}} \alpha_{x,a} p_{\mathcal{X}}(x) \phi_{x,a} \phi_{x,a}^\top\right) (\theta - \mu) \\
     & = \mathbb{E}[\tau] \sup_{\alpha \in \Lambda}\inf_{\mu \in B_\varepsilon(\theta)} \frac{1}{2} \|\theta - \mu\|^2_{A(\alpha)},
\end{aligned}
     \label{eq:optim_lb_discrete}
\end{equation}
where we introduced the context count $N_x(\tau) = \sum_{t =1}^\tau \mathbbm{1}\{x_t = x\}$, the conditional context-arm proportions $\alpha_{x,a} = \frac{\mathbb{E}_{\theta}\left[N_{x,a}(\tau)\right]}{\mathbb{E}_{\theta}\left[N_x(\tau)\right]}$, the matrix $A(\alpha) = \left(\sum\limits_{(x,a) \in\mathcal{X}\times \mathcal{A}} \alpha_{x,a} p_{\mathcal{X}(x)}\phi_{x,a} \phi_{x,a}^\top\right)$, $\Lambda =\lbrace \alpha \in [0,1]^{\vert \mathcal{X} \vert\times\vert \mathcal{A} \vert}: \forall x\in\mathcal{X} \; \sum_{a\in \mathcal{A}} \alpha_{x,a} = 1 \rbrace$ and noted that $ p_{\mathcal{X}}(x) = \frac{\mathbb{E}_\theta\left[N_x(\tau)\right]}{\mathbb{E}_\theta\left[\tau\right]}$. Here, $\alpha \in \Lambda$ may be interpreted as the asymptotic arm proportions conditioned on context $x$, i.e., the fraction of times that arm $a$ is selected given that context $x$ is observed. Define $\psi_{\varepsilon}^\star(\theta) = \sup_{\alpha \in \Lambda}\inf_{\mu \in B_\varepsilon(\theta)} \frac{1}{2} \|\theta - \mu\|^2_{A(\alpha)}$. We may write the lower bound as 
\begin{equation*}
    \mathbb{E}[\tau] \psi_{\varepsilon}^\star(\theta) \ge  \mathrm{kl}(1- \delta, \delta) %\gtrsim T^\star_{\theta,\varepsilon}\log\left(\frac{1}{\delta}\right).
\end{equation*}

\textit{4) The optimization problem:}
Now we aim at finding a closed-form solution to $\psi_{\varepsilon}(\theta,\alpha)$. What follows extends the approach in \cite[Sec. 3.1]{Soare15} for LB to LCB. Let $\Gamma^\star_\theta(x) = \{\phi_{x,a^\star_\theta(x)} - \phi_{x,a}, \forall a \in\mathcal{A}\}$ and $\omega = \theta-\mu$. 
The event that two arms differ under $\theta$ and $\mu$ implies that there exists at least one $\gamma \in \Gamma^\star_\theta(x)$ such that
$$ \gamma^{\top} \mu<0 \Leftrightarrow \gamma^{\top} \theta-\gamma^{\top} \mu>\gamma^{\top} \theta  \Leftrightarrow \gamma^{\top} \omega>\gamma^{\top} \theta .$$
Thus, we can rewrite the optimization problem as 
\begin{equation*}
    \begin{aligned} 
    &\inf_{\omega} \frac{1}{2}\omega^\top A(\alpha) \omega 
    \\&\text{subject to } \exists \gamma \in \Gamma^\star_\theta(x), \gamma^{\top} \omega \geq \gamma^{\top} \theta.
    \end{aligned}
\end{equation*}
Now, introduce the following function 
$$
\psi_\varepsilon(\theta, \alpha) =  \inf_{\mu \in B_{\varepsilon}(\theta)}  \frac{1}{2} \|\theta - \mu\|^2_{A(\alpha)},
$$
and note that set of confusing parameters may decomposed as
\begin{align*}
B_{\varepsilon}(\theta) & = \left\lbrace \mu \in \mathbb{R}^d: \; \exists x \in \mathcal{X}, \forall b \in \mathcal{A}_\varepsilon(\theta,x), \; \mu^{\top}(\phi_{x,a_{\mu}^\star(x)}- \phi_{x,b})>\varepsilon \right\rbrace
\\& = \bigcup_{x\in \mathcal{X}} \left\lbrace \mu \in \mathbb{R}^d: \; \forall b \in \mathcal{A}_\varepsilon(\theta,x), \; \mu^{\top}(\phi_{x,a_{\mu}^\star(x)}- \phi_{x,b})>\varepsilon \right\rbrace
\\& = \bigcup_{x\in \mathcal{X}} \bigcup_{a\in  \mathcal{A}^c_\varepsilon(\theta,x)} \left\lbrace \mu \in \mathbb{R}^d: \; \forall b \in \mathcal{A}_\varepsilon(\theta,x), \; \mu^{\top}(\phi_{x,a}- \phi_{x,b})>\varepsilon \right\rbrace \\& = \bigcup_{x\in \mathcal{X}} \bigcup_{a\in \mathcal{A}^c_\varepsilon(\theta,x)} B_{\varepsilon}(\theta,x,a),
\end{align*}
where $B_\varepsilon(\theta,x,a) = \left\lbrace \mu \in \mathbb{R}^d: \; \forall b \in \mathcal{A}_\varepsilon(\theta,x), \; \mu^{\top}\gamma^x_{a,b}\leq-\varepsilon \right\rbrace$ and $\gamma^x_{a,b} = \phi_{x,b}- \phi_{x,a}$. Hence, we can write
\begin{equation*}
    \psi_\varepsilon(\theta, \alpha) = \min_{x\in\mathcal{X}}\min_{a\in \mathcal{A}^c_\varepsilon(\theta,x)} \inf_{\mu \in B_{\varepsilon}(\theta, x, a)} \|\theta - \mu\|^2_{A(\alpha)}.
\end{equation*}
Define $\omega = \theta-\mu$, and rewrite the constraint as 
$$ \mu^{\top}\gamma^x_{a,b} \leq -\varepsilon  \iff \omega^{\top}\gamma^x_{a,b} > (\theta^{\top}\gamma^x_{a,b}  + \varepsilon) .$$ 
Formulate the optimization problem
\begin{equation}
\label{eq:linear_prog}
    \begin{aligned} 
    & \inf \frac{1}{2} \omega^\top A(\alpha) \omega \\  &\text{s.t. } \forall b \in \mathcal{A}_\varepsilon(\theta,x),\; \omega^{\top}
    \gamma^x_{a,b} \geq \theta^{\top} \gamma^x_{a,b} + \varepsilon.
    \end{aligned}
\end{equation}
Note that the problem in \eqref{eq:linear_prog} is a Quadratic Program with $|\mathcal{A}_\varepsilon(\theta,x)|$ linear constraints. Although the problem can be solved numerically in an efficient way (e.g. by active set methods, interior point methods, etc.), the solution cannot be easily expressed in closed form. To find a closed-form solution we define for $a\in \mathcal{A}_\varepsilon^c(\theta,x)$ the set  $\mathcal{A}_\varepsilon(\theta,x,a) = \{b\in \mathcal{A}_\varepsilon(\theta,x): \theta^\top (\phi_{x,b}-\phi_{x,a}) > \varepsilon\}$. In order to get a closed form solution we instead focus on solving a relaxed problem. Take a different decomposition of the set of confusing parameters as
\begin{align*}
B_{\varepsilon}(\theta) & = \bigcup_{x\in \mathcal{X}} \bigcup_{a\in \mathcal{A}^c_\varepsilon(\theta,x)} \left\lbrace \mu \in \mathbb{R}^d: \; \forall b \in \mathcal{A}_\varepsilon(\theta,x), \; \mu^{\top}(\phi_{x,a}- \phi_{x,b})>\varepsilon \right\rbrace \\ & \subseteq  \bigcup_{x\in \mathcal{X}} \bigcup_{a\in \mathcal{A}^c_\varepsilon(\theta,x)} \left\lbrace \mu \in \mathbb{R}^d: \; \exists b \in \mathcal{A}_\varepsilon(\theta,x,a), \; \mu^{\top}(\phi_{x,a}- \phi_{x,b})>\varepsilon \right\rbrace \\ & =  \bigcup_{x\in \mathcal{X}} \bigcup_{a\in \mathcal{A}^c_\varepsilon(\theta,x)} \bigcup_{b\in \mathcal{A}_\varepsilon(\theta,x,a)} \left\lbrace \mu \in \mathbb{R}^d: \mu^{\top}(\phi_{x,a}- \phi_{x,b})>\varepsilon \right\rbrace.
\end{align*}
Hence we have for $\bar{B}_\varepsilon(\theta,x,a) = \left\lbrace \mu \in \mathbb{R}^d: \; \exists b \in \mathcal{A}_\varepsilon(\theta,x), \; \mu^{\top}\gamma^x_{a,b}\leq-\varepsilon \right\rbrace$, 
$$  \bar{\psi}^\star_\varepsilon(\theta) = \sup_{\alpha\in\Lambda}\min_{x\in\mathcal{X}}\min_{a\in \mathcal{A}^c_\varepsilon(\theta,x)} \inf_{\mu \in \bar{B}_{\varepsilon}(\theta, x, a)} \|\theta - \mu\|^2_{A(\alpha)} \leq \psi^\star_\varepsilon(\theta),$$
%so that the lower bound can be written as 
%$$
%\mathbb{E}_\theta[\tau] \bar{\psi}^\star_\varepsilon(\theta)\geq \mathrm{kl}(1- \delta, \delta).
%$$
%The optimization problem becomes for $a\in\mathcal{A}^c_\varepsilon(\theta,x)$

\begin{equation*}
    \begin{aligned} 
    & \inf \frac{1}{2} \omega^\top A(\alpha) \omega \\  &\text{s.t. } \exists b \in \mathcal{A}_\varepsilon(\theta,x),\; \omega^{\top}
    \gamma^x_{a,b} \geq \theta^{\top} \gamma^x_{a,b} + \varepsilon.
    \end{aligned}
\end{equation*}
Let $\gamma = \gamma_{a,b}^x$, and define the Lagrangian of this optimization problem is
$$L(\omega, \rho) = \frac{1}{2}\omega^{\top} A(\alpha) \omega+\rho\left(-\gamma^{\top} \omega+\gamma^\top\theta + \varepsilon\right),$$
with Lagrange multipliers $\rho \in \mathbb{R}$. Imposing the optimality conditions leads to the system
\begin{equation}
\begin{cases}
    \frac{\partial L}{\partial \omega} = A(\alpha)\omega-\rho \gamma=0 \Leftrightarrow A(\alpha) \omega= \rho\gamma \\ 
    \rho\frac{\partial L}{\partial \rho}=\rho(-\gamma^{\top} \omega+\gamma^{\top} \theta + \varepsilon)=0 
    \\ \gamma^\top\omega \geq \gamma^\top \theta
    \\ \rho \geq 0
\end{cases}.
\label{eq:KKT_approx_delta_pac}
\end{equation}
Let $\rho\neq 0 \Rightarrow (-\gamma^{\top} \omega+\gamma^{\top} \theta + \varepsilon)=0 $. For $A(\alpha) \succ 0$, solving for $\omega$ in the first  of the Eq. in \eqref{eq:KKT_approx_delta_pac} and substituting in the second of the Eq. in \eqref{eq:KKT_approx_delta_pac}, we get
$$\rho = \frac{\gamma^\top\theta + \varepsilon}{\|\gamma\|^2_{A(\alpha)^{-1}}}. $$
Note that $\rho > 0$, thus we have a feasible solution to the optimization problem.
We have $$\frac{1}{2}\omega^\top A(\alpha)\omega = \frac{(\gamma^\top \theta + \varepsilon)^\top\gamma^\top A(\alpha)^{-1}A(\alpha)A(\alpha)^{-1}\gamma(\gamma^\top \theta + \varepsilon)}{2\|\gamma\|_{A(\alpha)^{-1}}^4}= \frac{(\gamma^\top \theta + \varepsilon)^\top\gamma^\top A(\alpha)^{-1}\gamma(\gamma^\top \theta + \varepsilon )}{\|\gamma\|_{A(\alpha)^{-1}}^4} = \frac{(\gamma^\top \theta +\varepsilon)^2 }{2\|\gamma\|^2_{A(\alpha)^{-1}}}.$$
Hence we get
\begin{align*}
    \bar{\psi}_\varepsilon(\theta,\alpha) = \inf_{\mu \in \hat{B}_\varepsilon(\theta, x, a)} \frac{1}{2} \|\theta - \mu\|^2_{A(\alpha)} =
     \begin{cases}
    \frac{ (\theta^\top\gamma^x_{a,b}+\varepsilon)^2}{2{\gamma_{a,b}^x}\top A(\alpha)^{-1} \gamma^x_{a,b}} & \text{ if } A(\alpha) \succ 0 \\
    0 &\text{ otherwise}
    \end{cases},
\end{align*}
Thus we may conclude that $\mathbb{E}_\theta[\tau] \gtrsim T^\star_{\theta,\varepsilon}\log\left(\frac{1}{\delta}\right)$ with

$$
    (T^\star_{\theta,\varepsilon})^{-1} = \begin{cases} \sup\limits_{\alpha\in\Lambda}\min\limits_{x\in \mathcal{X}} \min\limits_{a\in \mathcal{A}_\varepsilon^{c}(\theta,x)}\min\limits_{b\in \mathcal{A}_\varepsilon(\theta,x,a)} \frac{ (\theta^\top(\phi_{x,b}- \phi_{x,a})+\varepsilon)^2}{2(\phi_{x,b}- \phi_{x,a})^\top A(\alpha)^{-1} (\phi_{x,b}- \phi_{x,a})} & \text{ if } A(\alpha) \succ 0 \\
    0 & \text{ otherwise}
    \end{cases}.
$$
\end{proof}

\subsection{Proof of Theorem \ref{theorem:off_policy_lb}}
\begin{proof}
The proof follow closely the proof of Theorem \ref{theorem:lb_eps_delta_discrete}. 
The main differences are the following:
\begin{enumerate}
    \item At step $1$ (the log-likelihood ratio), we consider the log-likelihood ratio $ L_T^{\theta,\mu}$ between $\theta, \mu \in U$.
    \item At step $2$ (the change of measure argument),
    the set of confusing parameters is 
\begin{align*}
B_{\varepsilon}(\theta) & = \left\lbrace \mu \in U: \exists x \in \mathcal{X}, \forall b \in \mathcal{A}_\varepsilon({\theta},x), \; \mu^{\top}(\phi_{x,a_{\mu}^\star(x)}- \phi_{x,b})>\varepsilon \right\rbrace,
\end{align*}
and similarly, it holds
$$
\forall {\mu} \in B_\varepsilon({{\theta}}) \qquad \mathbb{E}\left[ L_\tau^{{\theta},{\mu}} \right] \ge \mathrm{kl}\left(1- \delta, \delta \right). 
$$
\item At step $5$ (solution to the optimization problem), when the invertibility of $A(\alpha)$ is required, we consider the pseudo-inverse $A(\alpha)^\dagger$. The condition $\text{dim}(U) > 0$ is required in order to avoid singularities. The solution to the optimization problem is similar to the one in the proof of Theorem \ref{theorem:lb_eps_delta_discrete}, with the exception that the condition for the invertibility in the solution to the optimization problem is ${\omega} =({\mu} - {\theta}) \in\Span(\Phi_\alpha)$.
\end{enumerate}
\end{proof}
\begin{comment}
\subsection{Proof of Lemma \ref{lem:T_star_scaling_delta_pac}}
The lemma follows naturally from the application of the Kiefer-Wolfowitz equivalence Theorem in \cite{Kiefer60}. 
We have 
\begin{align*}
T^\star_\theta & = \inf_{\alpha\in\Lambda}\max_{x\in\mathcal{X}}\max_{a\in\mathcal{A}\setminus 
\{a^\star_\theta(x)\}}\frac{\|\gamma_{x,a}\|^2_{A(\alpha)^{-1}}}{\Delta_{x,a}^2} \\&\leq \inf_{\alpha\in\Lambda}\max_{x\in\mathcal{X}}\max_{a\in\mathcal{A}\setminus\{a^\star_\theta(x)\}}\frac{\|\gamma_{x,a}\|^2_{A(\alpha)^{-1}}}{\Delta_{\min}^2} \\&\leq \inf_{\alpha\in\Lambda}\max_{x\in\mathcal{X}}\max_{a\in\mathcal{A}\setminus\{a^\star_\theta(x)\}}\frac{4\|\phi_{x,a}\|^2_{A(\alpha)^{-1}}}{\Delta_{\min}^2}  \leq \frac{4d}{\Delta_{\min}^2}.
\end{align*}
\end{comment}

\subsection{Proof of Lemma \ref{lem:T_star_scaling_eps_delta_pac}}
\begin{proof}
The lemma follows naturally from the application of the Kiefer-Wolfowitz equivalence Theorem in \cite{Kiefer60} and generalize Proposition $3$ from Soare et al. \cite{Soare15} in the LB case. For $\varepsilon>0$, we have
\begin{align*}
T^\star_{\theta,\varepsilon}& = \inf_{\alpha\in\Lambda} \max_{x\in\mathcal{X}}\max_{a\not \in \mathcal{A}_\varepsilon(\theta,x)}\max_{b\in \mathcal{A}_\varepsilon(\theta,x,a)}\frac{\|\gamma^x_{a,b}\|^2_{A(\alpha)^{-1}}}{(\theta^\top\gamma^x_{a,b}+\varepsilon)^2} \\&\leq \inf_{\alpha\in\Lambda}\max_{x\in\mathcal{X}}\max_{a\not \in \mathcal{A}_\varepsilon(\theta,x)}\max_{b\in \mathcal{A}_\varepsilon(\theta,x,a)}\frac{\|\gamma^x_{a,b}\|^2_{A(\alpha)^{-1}}}{4\varepsilon^2} \\&\leq \inf_{\alpha\in\Lambda}\max_{x\in\mathcal{X}}\max_{a\not \in \mathcal{A}_\varepsilon(\theta,x)}\frac{4\|\phi_{x,a}\|^2_{A(\alpha)^{-1}}}{4\varepsilon^2} \leq \frac{d}{\varepsilon^2}.
\end{align*}
For $\varepsilon = 0$, we have 
\begin{align*}
T^\star_{0,\theta} & = \inf_{\alpha\in\Lambda} \max_{x\in\mathcal{X}}\max_{a\neq a^\star_\theta(x)}\frac{\|\gamma^x_{a,a^\star_\theta(x)}\|^2_{A(\alpha)^{-1}}}{(\theta^\top\gamma^x_{a,a^\star_\theta(x)})^2} \\&\leq \inf_{\alpha\in\Lambda}\max_{x\in\mathcal{X}}\max_{a\neq a^\star_\theta(x)}\frac{\|\gamma^x_{a,a^\star_\theta(x)}\|^2_{A(\alpha)^{-1}}}{\Delta_{\min}^2} \\&\leq \inf_{\alpha\in\Lambda}\max_{x\in\mathcal{X}}\frac{4\|\phi_{x,a}\|^2_{A(\alpha)^{-1}}}{\Delta_{\min}^2} \leq \frac{4d}{\Delta_{\min}^2}.
\end{align*}
\end{proof}

\subsection{Proof of Lemma \ref{lem:properties_eps_delta}}
\begin{proof}

\textit{1) Continuity of $\psi_\varepsilon$:} 
Let $(\theta_t,\alpha_t)_{t\geq 1}$ be a sequence taking values in $\mathbb{R}^d\times \Lambda$, and converging to $(\theta,\alpha)$. Recall the definition of set of confusing parameters 
$$
 B_\varepsilon(\theta) = {\left\lbrace \mu\in\mathbb{R}^d: \exists x \in \mathcal{X}, \forall b \in \mathcal{A}_\varepsilon(\theta,x), \; \mu^{\top}(\phi_{x,a_{\mu}^\star(x)}- \phi_{x,b})>\varepsilon \right\rbrace}
$$
Since $(\theta_t,\alpha_t)$ converges to  $(\theta,\alpha)$, there exists $\upsilon < \varepsilon$, such that for some $t_1 \geq 1: \forall t\geq t_1$, $\|(\theta,\alpha) - (\theta_t,\alpha_t) \| <\upsilon$. Also, since $\mathcal{A}_\varepsilon(\theta,x)$ is defined as an open set $\forall x\in\mathcal{X}$, we have $B_\varepsilon(\theta) = B_\varepsilon(\theta_t)$. 
Now, define $g_\mu(\theta,\alpha) \triangleq \|\mu - \theta\|^2_{A(\alpha)}$, and note that $g_\mu(\theta,\alpha)$ is a polynomial in $(\theta,\alpha)$, and hence is continuous. As a consequence, there exist $
t_2\geq 1: \forall t \geq t_2$, 
$ |g_\mu(\theta,\alpha)- g_\mu(\theta_t,\alpha_t)| \leq \upsilon g_\mu(\theta,\alpha)$.  With our choice of $\upsilon$ and for $t\geq \max\{t_1,t_2\}$, we get
\begin{align*}
\left|\psi_\varepsilon(\theta,\alpha)-\psi\left(\mu_{t}, \alpha_{t}\right)\right| &=\left|\min_{\mu \in B_\varepsilon(\theta)} g_\mu(\theta, \alpha)-\min_{\mu \in B_\varepsilon(\theta)} g_\mu\left(\theta_t, \alpha_t\right)\right| 
\\ & \leq \upsilon\left|\min_{\mu \in B_\varepsilon(\theta)} g_\mu(\theta, \alpha)\right| 
\\ & \leq \upsilon|\psi_\varepsilon(\theta,\alpha)|.
\end{align*}

\textit{2) Invertibility of $A(\alpha_\theta^\star)$:}
By continuity of $\psi_\varepsilon$ in $\alpha$ and compactness of $\Lambda$, there exists $\alpha_\theta^\star \in \argsup_{\alpha \in\Lambda} \psi_\varepsilon(\theta,\alpha)$.
To verify that $A(\alpha_\theta^\star) \succ 0$, note that $\forall \mu \in B_\varepsilon(\theta)$. Since by assumption we have $\Span(\Phi) = \mathbb{R}^d$ and $\forall x \in\mathcal{X}$ $p_\mathcal{X}(x) >0$, we may construct an allocation $\tilde{\alpha} \in \Lambda$ such that $A(\tilde{\alpha}) \succ 0$.

\textit{3) Convexity, Compactness and Upper Hemicontinuity of $C^\star_\varepsilon(\theta)$ \& 4) Continuity of $\psi_\varepsilon^\star$ in $\theta$:} The result follows from an application of Berge's Theorem \cite{Berge63}. Since $\psi_\varepsilon$ is continuous in $(\theta,\alpha)$, $\Lambda$ is compact, convex, and non-empty, and $\psi_\varepsilon$ is concave in $\alpha$ for any $\theta'\in\mathbb{R}^d$ in an open neighborhood of $\theta'$. Hence the hypothesis of Berge's Theorem are satisfied and the result follows.
\end{proof}

\subsection{Proof of Lemma
\ref{lem:Nx_concentration_tight}}
\begin{proof}
The proof of this concentration results follows directly by the application of Theorem 3.5 in \cite{iosif_concentration}. Define $N_t-tp_\mathcal{X}=\sum_{s = 1}^t J_s,$
where $N_t$ is the random vector in $\mathbb{N}^{|\mathcal{X}|}$ with coordinates $N_t(x)$ for $x\in\mathcal{X}$, $p_\mathcal{X}$ is the vector with coordinates $p_\mathcal{X}(x)$ that lies in $\Lambda_\mathcal{X} = \{p_{\mathcal{X}}(x) \in[0,1]^{|\mathcal{X}|}: \sum_{x\in\mathcal{X}} p_\mathcal{X}(x) = 1\}$, and 
the $J_i$'s are i.i.d. zero-mean random vectors in $\mathbb R^{|\mathcal{X}|}$ with coordinates $J_s(x)=\mathbbm{1}\{x_s = x\} - p_\mathcal{X}(x)$ for $x\in \mathcal{X}$. We have 
$$\|J_s\|_2^2=\sum_{x\in\mathcal{X}}(\mathbbm{1}\{x_s=x\}-p_\mathcal{X}(x))^2
\le \sum_{x\in\mathcal{X
}}(\mathbbm{1}\{x_s=x\}+p_\mathcal{X}(x)^2) = 1+\sum_{x\in\mathcal{X}}p_\mathcal{X}(x)^2\le2.$$
Hence the assumption of Theorem 3.5 in  \cite{iosif_concentration} are satisfied with $r=t\varepsilon$, $D=1$, and $b_*^2=2t$, and we get
\begin{align*}
\mathbb{P}\left(\max_{x\in\mathcal{X}}\left|\frac{1}{t}\, N_t(x)-p_\mathcal{X}(x)\right|\ge\varepsilon\right) & = \mathbb{P}\left(\max_{x\in\mathcal{X}}\left|N_t(x)-tp_\mathcal{X}(x)\right|\ge t\varepsilon\right) \\& = \mathbb{P}\left(\|N_t-t p_\mathcal{X}\|_\infty \geq t\varepsilon\right) 
\\& \leq \mathbb{P}\left(\|N_t-t p_\mathcal{X}\|_2 \geq t\varepsilon\right) \\& \leq e^{-t\varepsilon^2/4}. 
\end{align*}
\end{proof}

\subsection{Proof of Lemma \ref{lem:stopping_rule_eps_delta_pac}}
\begin{proof}
Under the Gaussian noise assumption $f^{\theta}\left(r_{t}, a_{t}, x_{t} \ldots, r_{1}, a_{1}, x_{1}\right) \propto \exp \left(-\frac{1}{2} \sum_{s=1}^{t}\left(r_{s}-\theta^{\top} \phi_{x_s,a_s}\right)^{2}\right).$ By \cite[Lemma 7]{Jedra20}, we may write $Z^x_{a, b,\varepsilon}(t)$ in closed form as:
\begin{equation*}
Z^x_{a, b,\varepsilon}(t)=\operatorname{sign}\left(\hat{\theta}_{t}^{\top}(\phi_{x,a}-\phi_{x,b})+\varepsilon\right) \frac{\left(\hat{\theta}_{t}^{\top}(\phi_{x,a}-\phi_{x,b})+\varepsilon\right)^{2}}{2(\phi_{x,a}-\phi_{x,b})^{\top}\left(\sum_{s=1}^{t} \phi_{x_s,a_s}\phi_{x_s,a_s}^{\top}\right)^{-1}(\phi_{x,a}-\phi_{x,b})}, 
        \end{equation*}
where $\hat{\theta}_t$ is the LS estimator defined in \eqref{eq:LS_estimator}. Recall that, since $Z_\varepsilon^x(t) = \max_{a \in \mathcal{A}_\varepsilon(\hat{\theta}_t,x)} \min_{b \neq a} Z^x_{a, b, \varepsilon}(t)$ and $\hat{a}_t(x) \in \argmax_{a \in \mathcal{A}_\varepsilon(\hat{\theta}_t,x)} \min_{b \neq a} Z^x_{a, b, \varepsilon}(t) $, we have $\forall x \in\mathcal{X}$,
$$\min_{b \neq \hat{a}_t(x)}Z^x_{\hat{a}_t(x), b, \varepsilon}(t) \geq \max_{a \in \mathcal{A}_\varepsilon(\hat{\theta}_t,x)} \min_{b \neq a} Z^x_{a,b,\varepsilon}(t).$$
Define the event
\begin{align*}\mathcal{E}& = \left\{\exists t, \exists x: Z_\varepsilon^x(t)>\beta(\delta, t)\text{ and }  \theta^\top(\phi_{x,a^\star_\theta(x)} - \phi_{x,\hat{a}_t(x)})>\varepsilon  \text{ and } \sum_{s=1}^{t} \phi_{x_s,a_{s}}\phi_{x_s,a_{s}}^{\top} \succeq c I_{d} \right\} 
\\ & = \left\{\exists t,\exists x: \max_{a \in \mathcal{A}_\varepsilon(\hat{\theta}_t,x)} \min_{b \neq a} Z^x_{a, b, \varepsilon}(t) >\beta(\delta,t) \text{ and } \theta^\top(\phi_{x,a^\star_\theta(x)} - \phi_{x,\hat{a}_t(x)})>\varepsilon \text{ and } \sum_{s=1}^t\phi_{x_s,a_s}\phi_{x_s,a_s}^{\top} \succeq c I_{d}\right\}\\ & \subseteq  \left\{\exists t, \exists x: Z_{\hat{a}_t(x),  a^\star_\theta(x),\varepsilon}^x >\beta(\delta,t) \text{ and } \theta^\top(\phi_{x,a^\star_\theta(x)} -\phi_{x,\hat{a}_t(x)})>\varepsilon \text{ and } \sum_{s=1}^t\phi_{x_s,a_s}\phi_{x_s,a_s}^{\top} \succeq c I_{d}\right\}.
\end{align*}
On the event $\mathcal{E}$, it holds $\exists x\in\mathcal{X} : \hat{\theta}_t^\top(\phi_{x,\hat{a}_t(x)}-\phi_{x,a^\star_\theta(x)})\geq -\varepsilon$ and $\theta^\top(\phi_{x,\hat{a}_t(x)}-\phi_{x,a^\star_\theta(x)} )<
-\varepsilon$. Thus
\begin{align*}
    &\max\limits_{\left\{\mu: \mu^{\top}(\phi_{x,\hat{a}_t(x)}-\phi_{x,a^\star_\theta(x)}) \geq -\varepsilon\right\}} f^{\mu}\left(r_{t}, a_{t}, x_{t} \ldots, r_{1}, a_{1},x_{1}\right)= f^{\hat{\theta}}\left(r_{t}, a_{t}, x_{t} \ldots, r_{1}, a_{1},x_{1}\right),\\ 
    &\max\limits_{\left\{\mu: \mu^{\top}(\phi_{x,\hat{a}_t(x)}-\phi_{x,a^\star_\theta(x)}) \leq -\varepsilon \right\}} f^{\mu}\left(r_{t}, a_{t}, x_{t} \ldots, r_{1}, a_{1},x_{1}\right) \geq f^{\theta}\left(r_{t}, a_{t}, x_{t} \ldots, r_{1}, a_{1},x_{1}\right).
\end{align*}

\begin{align*}
 Z^x_{\hat{a}_t(x),a^\star_\theta(x),\varepsilon} &= \log \left(\frac{\max\limits_{\left\{\mu: \mu^{\top}(\phi_{x,\hat{a}_t(x)}-\phi_{x,a^\star_\theta(x)}) \geq -\varepsilon\right\}} f^{\mu}\left(r_{t}, a_{t}, x_{t} \ldots, r_{1}, a_{1},x_{1}\right)}{\max\limits_{\left\{\mu:\mu^{\top}(\phi_{x,\hat{a}_t(x)}-\phi_{x,a^\star_\theta(x)}) \leq -\varepsilon\right\}} f^{\mu}\left(r_{t}, a_{t}, x_{t} \ldots, r_{1}, a_{1}, x_{1}\right)}\right) \\& \leq \log \left(\frac{f^{\hat{\theta}_t}(r_{t}, a_{t}, x_{t} \ldots, r_{1}, a_{1})}{f^{\theta}(r_{t}, a_{t}, x_{t} \ldots, r_{1}, a_{1})}\right) \\&= \frac{1}{2} \| \theta - \hat{\theta}_t\|^2_{\sum_{s=1}^t \phi_{x_s,a_s}\phi_{x_s,a_s}^\top}. 
\end{align*}
Hence $ \mathcal{E} \subseteq \left\{\exists t\in\mathbb{N}^*,\exists x \in\mathcal{X}: \frac{1}{2} \| \theta - \hat{\theta}_t\|^2_{\sum_{s=1}^t \phi_{x_s,a_s}\phi_{x_s,a_s}^\top} >\beta(\delta,t) \text{ and } \sum_{s=1}^t\phi_{x_s,a_s}\phi_{x_s,a_s}^{\top} \succeq c I_{d}\right\}.$ The rest of the proof would go along the same line as \cite[Prop. 2]{Jedra20}. We note that for any $u>0$, $(1+u)(\sum_{s=1}^t\phi_{x_s,a_s}\phi_{x_s,a_s}^{\top} + cu I_d)^{-1} \succeq (\sum_{s=1}^t\phi_{x_s,a_s}\phi_{x_s,a_s}^{\top})^{-1}$. Hence
$$
\|\hat{\theta}_{t}-\theta\|_{\sum_{s=1}^t\phi_{x_s,a_s}\phi_{x_s,a_s}^{\top}}^{2}=\left\|\sum_{s=1}^{t} \phi_{x_s,a_{s}} \xi_{s}\right\|^{2}_{\left( \sum_{s=1}^t\phi_{x_s,a_s}\phi_{x_s,a_s}^{\top}\right)^{-1}} \leq(1+u)\left\|\sum_{s=1}^{t} \phi_{x_s,a_s} \xi_{s}\right\|_{\left(\sum_{s=1}^{t} \phi_{x_s,a_{s}} \phi_{x_s,a_{s}}^{\top}+u c I_{d}\right)^{-1}}^{2}.
$$
This implies 
$\mathcal{E}\subseteq\left\{\exists t \in \mathbb{N}^{*},\exists x \in\mathcal{X}:  \frac{1}{2}(1+u)\left\|\sum_{s=1}^{t} \phi_{x_s,a_s} \xi_{s}\right\|_{\left(\sum_{s=1}^{t} \phi_{x_s,a_{s}} \phi_{x_s,a_{s}}^{\top}+u c I_{d}\right)^{-1}}^{2} \geq \beta(\delta, t)\right\},$
and with the choice 
$$
\beta(\delta, t)=(1+u) \sigma^{2} \log \left(\frac{\operatorname{det}\left((u c)^{-1} \sum_{s=1}^{t} \phi_{x_s,a_{s}} \phi_{x_s,a_{s}}^{\top}+I_{d}\right)^{1 / 2}}{\delta}\right),
$$
it follows directly from \cite[Lemma 9]{Abbasi11} that $\mathbb{P}[\mathcal{E}] \leq \delta.$

\end{proof}


\subsection{Proof of Lemma \ref{lem:forced_exploration}}
\label{app:proof_forced_expl_delta}
The proof of this lemma is similar to that of the forced exploration for LB presented in \cite[Lemma 5]{Jedra20}, but there are crucial differences. As opposed to the deterministic result proved in \cite{Jedra20}, due to the random nature of the context arrivals and the fact that the feature vectors for context $x$ spans a different subspace of dimension $d_x \leq d$, the forced exploration may not be guaranteed at each time step. Hence, we prove a probabilistic (and stronger) result on the growth of the minimum eigenvalue by leveraging Lemma \ref{lem:Nx_concentration_tight}.

\begin{proof}
Let $t>0$, and for all $x\in\mathcal{X}$ define $\mathcal{I}_{x}(t) = \{i_k\in [1,t]:x_{i_k} = x\}$, the indices at which context $x$ is observed, with $k\in\{1,\dots,N_x(t)\}$. Note that, for all $x\in\mathcal{X}$, we have $d_x = \inf \{k>0: \sum_{j=1}^{k} \phi_{x,a_{i_j}} \phi_{x,a_{i_j}}^\top \succeq f_x(t)\}$. Fix an $x$, and assume there exists $k_0(x) > d_x$ such that 
$$\sum_{j=1}^{k_0(x)}\phi_{x,a_{i_j}}\phi_{x,a_{i_j}}^\top \succeq f_x(k_0(x)) \text{ and } \sum_{j=1}^{k_0(x)+1}\phi_{x,a_{i_j}}\phi_{x,a_{i_j}}^\top \prec f_x(k_0(x)+1).$$
Define $k_1(x) = \inf \left\{k>k_0(x): \sum_{j=1}^{k} \phi_{x,a_{i_j}} \phi_{x,a_{i_j}}^\top \succeq f_x(k)\right\}$, and note that for all $k$ such that $k_0(x) \leq k \leq k_1(x)$, we have
$$\sum_{j=1}^k\phi_{x,a_{i_j}}\phi_{x,a_{i_j}}^\top \succeq \sum_{j=1}^{k_0(x)}\phi_{x,a_{i_j}}\phi_{x,a_{i_j}}^\top \succeq f(k_0(x)).$$
Let $C_x = \frac{1}{\sqrt{d_x}}\sum_{a_x \in \mathcal{A}_x} \phi_{x,a_x} \phi_{x,a_x}^{\top}$. For $k_1(x)\geq k_0(x)+d_x+1$, we have
\begin{equation*}
\begin{aligned}
\sum_{j=1}^{k_{1}(x)} \phi_{x,a_{i_j}} \phi_{x,a_{i_j}}^{\top} & \succeq \sum_{j=1}^{k_{0}(x)+d_x+1} \phi_{x,a_{i_j}} \phi_{x,a_{i_j}}^{\top} \\
& \succeq \sum_{j=1}^{k_{0}(x)+1} \phi_{x,a_{i_j}} \phi_{x,a_{i_j}}^{\top}+\sum_{a_x \in \mathcal{A}_x} \phi_{x,a_x} \phi_{x,a_x}^{\top} \\
&=\sum_{j=1}^{k_{0}(x)+1} \phi_{x,a_{i_j}} \phi_{x,a_{i_j}}^{\top}+C_x\sqrt{d_x} \\
& \succeq \sum_{j=1}^{k_{0}(x)} \phi_{x,a_{i_j}} \phi_{x,a_{i_j}}^{\top}+C_x \sqrt{d_x} \\
& \succeq f_x\left(k_{0}(x)\right)+C_x \sqrt{d_x}.
\end{aligned}
\end{equation*}
However, we have
$$
k_{0}(x) \geq \frac{1}{4}\left(d_x+\frac{1}{d_x}+2\right) \Longrightarrow \sqrt{k_{0}(x)+d_x+1}+\sqrt{k_{0}(x)} \geq \sqrt{d_x}+\frac{1}{\sqrt{d_x}} \Longrightarrow f_x\left(k_{0}(x)\right)+C_x \sqrt{d_x} \succeq f_x\left(k_{0}(x)+d_x+1\right) .
$$
Therefore, if $k_{0}(x) \geq \frac{1}{4}\left(d_x+\frac{1}{d_x}+2\right),$ then it holds that $k_{1}(x) \leq k_{0}(x)+d_x+1$. In other words, we have shown that for all $N_x(t) \geq \frac{1}{4}\left(d_x+\frac{1}{d_x}+2\right)+d_x+1,$ we have
$$\sum_{k=1}^{N_x(t)} \phi_{x,a_{i_k}}\phi_{x,a_{i_k}}^{\top} \succeq C_x\sqrt{N_x(t)-d_x-1}
$$
Let $t_0 = \inf\left\{t\geq 0: \forall x\in\mathcal{X}, N_x(t) \geq \frac{1}{4}\left(d_x+\frac{1}{d_x}+2\right)+d_x+1\right\}$ and denote $p_{\min} = \min\limits_{x\in\mathcal{X}}p_\mathcal{X}(x)$. By Lemma \ref{lem:Nx_concentration_tight}, $\forall \varepsilon \in\left(0,p_{\min}\right)$ and $\forall t\geq t_0$, we get
$$
\mathbb{P}_\theta\left( \sum_{k=1}^{N_x(t)} \phi_{x,a_{i_k}}\phi_{x,a_{i_k}}^{\top} \succeq  C_x\sqrt{(p_\mathcal{X}(x)-\varepsilon)t - d_x - 1}\right) \geq 1-2 e^{-\frac{t\varepsilon^2}{4}}.
$$
Hence, w.p. at least $1-2 e^{-\frac{t\varepsilon^2}{4}}$, we get
\begin{align*}
\sum_{s = 1}^t\phi_{x_s,a_s}\phi_{x_s,a_s}^\top & = \sum_{x \in \mathcal{X}}\sum_{i_k \in\mathcal{I}_x }\phi_{x,a_{i_k}}\phi_{x,a_{i_k}}^\top 
\\ & \succeq \sum_{x \in \mathcal{X}} \left(C_x\sqrt{(p_\mathcal{X}(x)-\varepsilon)t-d_x-1} \right)
\\ & = \sum_{x\in\mathcal{X}}\sqrt{\frac{(p_\mathcal{X}(x)-\varepsilon)t-(d_x+1)}{d_x}}   \sum_{a_x \in \mathcal{A}_x} \phi_{x,a_x}\phi_{x,a_x}^{\top}
\\ & \succeq \sum_{x\in\mathcal{X}}\sqrt{\frac{(p_\mathcal{X}(x)-\varepsilon)t-(d_x+1)}{d_x}}  cI_d. 
\\ & \succeq \min_{x\in\mathcal{X}}\sqrt{\frac{(p_\mathcal{X}(x)-\varepsilon)t-(d_x+1)}{d_x}}  cI_d. 
\end{align*}
Now, let $x^\star = \arg\min_{x\in\mathcal{X}} \sqrt{\frac{(p_\mathcal{X}(x)-\varepsilon)t-(d_x+1)}{d_x}}$,  $0<\kappa< c\sqrt{\frac{p_\mathcal{X}(x^\star)-\varepsilon}{d_{x^\star}}}$, and $t_0' = \left\{\inf t: t \geq \left(\frac{\sqrt{\frac{d_{x^\star}+1}{d_x}}}{\sqrt{\frac{p_\mathcal{X}(x^\star)-\varepsilon}{d_{x^\star}}}-\kappa}\right)^2 \right\}$.
We have that for any 
$t\geq t_1 = \max\{t_0,t_0'(\kappa)\}$ we have  $\sqrt{\frac{(p_\mathcal{X}({x^\star})-\varepsilon)t-(d_{x^\star}+1)}{d_{x^\star}}} \geq \frac{\kappa}{c}\sqrt{t}$.
Hence, we have proved that $\exists t_1,\kappa: \forall t \geq t_1$ we have that     
$$
\mathbb{P}_\theta\left( \frac{1}{\sqrt{t}}\sum_{s = 1}^t\phi_{x_s,a_s}\phi_{x_s,a_s}^\top\succeq \kappa I_d\right) \geq 1-2 e^{-\frac{t\varepsilon^2}{4}}.
$$
\end{proof}

%\subsection{Proof of Corollary \ref{cor:Z}}
%Recall the expression of $\hat{O}_\varepsilon(\theta,x) = \{b\in\mathcal{A}: \max_{a\in\mathcal{A}}\hat{\theta}_t^\top (a-b) < \varepsilon\}$


\begin{comment}
\subsection{Proof of Lemma \ref{lem:stopping_rule_delta_pac}}
\begin{proof}
\label{app:proof_stopping_rule_delta_pac}
Under the Gaussian noise assumption $f^{\theta}\left(r_{t}, a_{t}, x_{t} \ldots, r_{1}, a_{1}, x_{1}\right) \propto \exp \left(-\frac{1}{2} \sum_{s=1}^{t}\left(r_{s}-\theta^{\top} \phi_{x_s,a_s}\right)^{2}\right).$ By Lemma \ref{lem:closed_form_Z}, we may write $Z^x_{a, b,\varepsilon}(t)$ in closed form as:
\begin{equation*}
Z^x_{a, b}(t)=\operatorname{sign}\left(\hat{\theta}_{t}^{\top}(\phi_{x,a}-\phi_{x,b})\right) \frac{\left(\hat{\theta}_{t}^{\top}(\phi_{x,a}-\phi_{x,b})\right)^{2}}{2(\phi_{x,a}-\phi_{x,b})^{\top}\left(\sum_{s=1}^{t} \phi_{x_s,a_s}\phi_{x_s,a_s}^{\top}\right)^{-1}(\phi_{x,a}-\phi_{x,b})},
\end{equation*}
where $\hat{\theta}_t$ is the LS estimator defined in \eqref{eq:LS_estimator}. Also, by Corollary 1 in \cite{Jedra20} it holds that $\forall x \in\mathcal{X}$ $$Z^x(t) = \max_{a\in\mathcal{A}}\min_{b\in\mathcal{A}\setminus\{a\}} = \min_{b\in\mathcal{A}\setminus\{\hat{a}_t(x)\}}Z_{\hat{a}(x),b}^x(t).$$

Define 
$\mathcal{E} \triangleq \left\{\exists t \in\mathbb{N}^*, \exists x\in\mathcal{X}: Z^x(t)>\beta(\delta, t) \text{ and }  a^\star_\theta(x) \neq \hat{a}_t(x)\text{ and } \sum_{s=1}^{t} \phi_{x_s,a_{s}}\phi_{x_s,a_{s}}^{\top} \succeq c I_{d}\right \},$ and note that %We need to show that $\mathbb{P}_{\theta}[\mathcal{E}] \leq \delta.$ 
\begin{align*}
\mathcal{E} & =\left\{ \exists t, \exists x:  Z^x(t) >\beta(\delta,t) \text{ and }  a^\star_\theta(x) \neq \hat{a}_t(x) \text{ and } \sum_{s=1}^t\phi_{x_s,a_s}\phi_{x_s,a_s}^{\top} \succeq c I_{d}\right\} \\ & = \left\{\exists t,\exists x: \min_{b\in\mathcal{A}\setminus\{\hat{a}_t(x)\}} Z_{\hat{a}_t(x),b}^x >\beta(\delta,t) \text{ and } a^\star_\theta(x) \neq \hat{a}_t(x) \text{ and } \sum_{s=1}^t\phi_{x_s,a_s}\phi_{x_s,a_s}^{\top} \succeq c I_{d}\right\}\\ & \subseteq  \left\{\exists t, \exists x: Z_{\hat{a}_t(x),  a^\star_\theta(x)}^x >\beta(\delta,t) \text{ and } \theta^\top(\phi_{x,a^\star_\theta(x)} -\phi_{x,\hat{a}_t(x)})>0 \text{ and } \sum_{s=1}^t\phi_{x_s,a_s}\phi_{x_s,a_s}^{\top} \succeq c I_{d}\right\}  
\end{align*}

%Define $\bar{\mathcal{X}}_t = \{x\in\mathcal{X}: \hat{a}_t(x) \neq a^\star_\theta(x)\}$, and note that on the event $\mathcal{E}$ the set $\bar{\mathcal{X}}_t$ is non-empty.

Note that on the event $\mathcal{E}$, it holds $\exists x\in\mathcal{X} : \hat{\theta}_t^\top(\phi_{x,\hat{a}_t(x)}-\phi_{x,a^\star_\theta(x)})\geq 0$ and $\theta^\top(\phi_{x,a^\star_\theta(x)} -\phi_{x,\hat{a}_t(x)})>0$. 
\begin{align*}
    &\max\limits_{\left\{\mu: \mu^{\top}(\phi_{x,\hat{a}_t(x)}-\phi_{x,a^\star_\theta(x)}) \geq 0\right\}} f^{\mu}\left(r_{t}, a_{t}, x_{t} \ldots, r_{1}, a_{1},x_{1}\right)= f^{\hat{\theta}}\left(r_{t}, a_{t}, x_{t} \ldots, r_{1}, a_{1},x_{1}\right),\\ 
    &\max\limits_{\left\{\mu: \mu^{\top}(\phi_{x,\hat{a}_t(x)}-\phi_{x,a^\star_\theta(x)}) \leq 0\right\}} f^{\mu}\left(r_{t}, a_{t}, x_{t} \ldots, r_{1}, a_{1},x_{1}\right) \geq f^{\theta}\left(r_{t}, a_{t}, x_{t} \ldots, r_{1}, a_{1},x_{1}\right).
\end{align*}
Hence, it follows that $\exists x \in\mathcal{X}$:
\begin{align*}
Z^x_{\hat{a}_t(x),a^\star_\theta(x)} &= \log \left(\frac{\max\limits_{\left\{\mu: \mu^{\top}(\phi_{x,\hat{a}_t(x)}-\phi_{x,a^\star_\theta(x)}) \geq 0\right\}} f^{\mu}\left(r_{t}, a_{t}, x_{t} \ldots, r_{1}, a_{1},x_{1}\right)}{\max\limits_{\left\{\mu:\mu^{\top}(\phi_{x,\hat{a}_t(x)}-\phi_{x,a^\star_\theta(x)}) \leq 0\right\}} f^{\mu}\left(r_{t}, a_{t}, x_{t} \ldots, r_{1}, a_{1}, x_{1}\right)}\right) \\& \leq \log \left(\frac{f^{\hat{\theta}_t}(r_{t}, a_{t}, x_{t} \ldots, r_{1}, a_{1})}{f^{\theta}(r_{t}, a_{t}, x_{t} \ldots, r_{1}, a_{1})    }\right) \\&= \frac{1}{2} \| \theta - \hat{\theta}_t\|^2_{\sum_{s=1}^t \phi_{x_s,a_s}\phi_{x_s,a_s}^\top}.
\end{align*}
Hence $ \mathcal{E} \subseteq \left\{\exists t\in\mathbb{N}^*,\exists x \in\mathcal{X}: \frac{1}{2} \| \theta - \hat{\theta}_t\|^2_{\sum_{s=1}^t \phi_{x_s,a_s}\phi_{x_s,a_s}^\top} >\beta(\delta,t) \text{ and } \sum_{s=1}^t\phi_{x_s,a_s}\phi_{x_s,a_s}^{\top} \succeq c I_{d}\right\}.$ The rest of the proof would go along the same line of \cite[Prop. 2]{Jedra20}. We note that for any $u>0$, $(1+u)(\sum_{s=1}^t\phi_{x_s,a_s}\phi_{x_s,a_s}^{\top} + cu I_d)^{-1} \succeq (\sum_{s=1}^t\phi_{x_s,a_s}\phi_{x_s,a_s}^{\top})^{-1}$. Hence
$$
\left\|\hat{\mu}_{t}-\mu\right\|^{2}=\left\|\sum_{s=1}^{t} \phi_{x_s,a_{s}} \xi_{s}\right\|^{2}_{\left( \sum_{s=1}^t\phi_{x_s,a_s}\phi_{x_s,a_s}^{\top}\right)^{-1}} \leq(1+u)\left\|\sum_{s=1}^{t} \phi_{x_s,a_s} \xi_{s}\right\|_{\left(\sum_{s=1}^{t} \phi_{x_s,a_{s}} \phi_{x_s,a_{s}}^{\top}+u c I_{d}\right)^{-1}}^{2}.
$$
This implies $\mathcal{E} \subseteq \left\{\exists t \in \mathbb{N}^{*},\exists x \in\mathcal{X}: \frac{1}{2}(1+u) \left\|\sum_{s=1}^{t} \phi_{x_s,a_s} \xi_{s}\right\|_{\left(\sum_{s=1}^{t} \phi_{x_s,a_{s}} \phi_{x_s,a_{s}}^{\top}+u c I_{d}\right)^{-1}}^{2} \geq \beta(\delta, t)\right\},$

and with the choice 
$$
\beta(\delta, t)=(1+u) \sigma^{2} \log \left(\frac{\operatorname{det}\left((u c)^{-1} \sum_{s=1}^{t} a_{s} a_{s}^{\top}+I_{d}\right)^{1 / 2}}{\delta}\right),
$$
it follows directly from \cite{Abbasi11} that  $\mathbb{P}[\exists x \in\mathcal{X}: a^\star_\theta(x) \neq \hat{a}_t(x), \tau < \infty] = \mathbb{P}[\mathcal{E}] \leq \delta.$

\end{proof}
\end{comment}
\subsection{Proof of Lemma
\ref{lem:tracking_lemma}}
\begin{proof}
Define for $x\in\mathcal{X}$, the projection operator $\text{proj}_x(\cdot)$ that takes $\alpha \in C$ as input, and outputs $\alpha_x$, the $K$-dimensional vector that contains the component of $\alpha$ relative to the context $x$. Let $C_x = \{\alpha_x: \alpha_x = \text{proj}_x(\alpha), \forall \alpha \in C\}$.
Note that, since $C \subset \Lambda$ is convex and non-empty, 
we have that each of the sets $C_x$, for $x\in\mathcal{X}$, is also convex. Also, note that 
$$
\exists t_0: \forall t\geq t_0, d_\infty(\alpha,C) \leq \varepsilon \Rightarrow \forall t\geq t_0, \forall x\in\mathcal{X}, d_\infty(\alpha_x, C_x) \leq \varepsilon.
$$
Now, define for all $x\in\mathcal{X}$, and $t \in \mathbb{N}^*$ such that $N_x(t) \geq 1$
$$
\bar{\alpha}_x(t) = \frac{1}{N_x(t)}\sum_{s = 1}^t \alpha_x(s)\mathbbm{1}\{x_s = x\}, \quad \hat{\alpha}_x(t)= \argmin_{\alpha' \in C_x} d_{\infty}(\bar{\alpha}_x(t), \alpha'), \quad v_x(t) = \argmin_{\alpha' \in C_x} d_{\infty}(\alpha_x(t), \alpha').$$  %Note that, by convexity of $C$, there exists $t_0'\geq t_0$ such that for all $t\geq t_0'$ we have 
%$$
%d_{\infty}\left(\left(N_{x,a}(t)/N_{x}(t)\right)_{(x,a) \in \mathcal{X}\times \mathcal{A}}, C\right) \leq d_{\infty}\left(\left(N_{x,a}(t)/N_{x}(t)\right)_{(x,a) \in \mathcal{X}\times \mathcal{A}}, \hat{\alpha}(t)\right).
%$$
Observe that for all $(x,a)\in\mathcal{X}\times \mathcal{A}$, we have 
\begin{align*}
& \left|\frac{1}{N_x(t)} \left(\sum_{s=1}^{t} \alpha_{x,a}(s)- \sum_{s=1}^{t} v_{x,a}(s)\right) \mathbbm{1}\{x_s = x\} \right| \\ &  \leq \frac{1}{N_x(t)} \sum_{s=1}^{t_{0}}\left|\alpha_{x,a}(s)-v_{x,a}(s)\right|\mathbbm{1}\{x_s = x\}+\frac{1}{N_x(t)} \sum_{s=t_{0}+1}^{t}\left|\alpha_{x,a}(s)-v_{x,a}(s)\right| \mathbbm{1}\{x_s = x\}\\
& \leq \frac{N_x(t_{0})}{N_x(t)}+\frac{N_x(t)-N_x(t_0)}{N_x(t)} \varepsilon.
\end{align*}
By Lemma \ref{lem:Nx_concentration_tight}, $\forall \kappa \in\left(0,p_{\min}\right)$ we get that w.p. at least $1-2e^{-\frac{t \kappa^2}{4}}$
$$ c_1(\kappa)t\leq N_x(t) \leq c_2(\kappa)t,$$
with $c_1(\kappa) =  (p_\mathcal{X}(x) -\kappa)$ and $c_2(\kappa) = (p_\mathcal{X}(x) +\kappa)$. Hence we get, w.p. at least $1-2e^{-\frac{t \kappa^2}{4}}$, that
$$
\left|\frac{1}{N_x(t)} \left(\sum_{s=1}^{t} \alpha_{x,a}(s)- \sum_{s=1}^{t} v_{x,a}(s)\right) \mathbbm{1}\{x_s = x\} \right| \leq \frac{t_{0}}{t c_1}+\frac{(t - t_0)}{tc_1}\varepsilon = \frac{t_0}{c_1t} + \frac{t-t_0}{c_1t}\varepsilon,
$$
with $c = \frac{1}{c_1}$. Hence for all $t \geq t_0' = \frac{t_0}{\varepsilon}$, we also have $d_{\infty}\left(\bar{\alpha}_x(t),\frac{1}{N_x(t)} \sum_{s = 1}^t v_x(s)\mathbbm{1}\{x_s = x\}\right)\leq 2c\varepsilon$, for all $x\in \mathcal{X}$. By convexity of $C_x$ we have $\frac{1}{N_x(t)}\sum_{s = 1}^tv_x(s)\mathbbm{1}\{x_s = x\} \in C_x$. Hence, we may conclude that
$$
\forall x\in\mathcal{X}, \forall t \geq t_{0}^{\prime} \quad d_{\infty}(\bar{\alpha}_x(t), \hat{\alpha}_x(t)) \leq d_{\infty}\left(\bar{\alpha}_x(t), \frac{1}{N_x(t)} \sum_{s=1}^{t} v_x(s)\mathbbm{1}\{x_s = x\}\right) \leq 2c\varepsilon.  
$$
Further define for all $t\geq 1$, $\varepsilon_{x,a,t} = N_{x,a}(t) - N_x(t)\hat{\alpha}_{x,a}(t)$, and the events
\begin{align*}
\mathcal{E}_{1}(t,x) &=\left\{a=\underset{a \in \supp(\bar{\alpha}_x(t))}{\argmin}\{N_{x,a}(t)- N_x(t) \bar{\alpha}_{x,a}(t)\}\right\}, \\
\mathcal{E}_{2}(t,x)&=\left\{A_x(t) \prec f_x(t) \quad \text { and } \quad a=a_x(i_t(x))\right\}.
\end{align*}
The rest of the proof will show that $\exists c'(\kappa)>0$, $\exists t_0'' \geq t_0'$ such that for all $t\geq t_0''$, for all $(x,a) \in\mathcal{X}\times \mathcal{A}$, and w.p. at least $1-2e^{-\frac{t \kappa^2}{4}}$, we have 
$$
\{a_{t+1}(x) = a\}\subseteq \mathcal{E}_{1}(t,x) \cup \mathcal{E}_{2}(t,x) \subseteq \{\varepsilon_{x,a,t} \leq c't\varepsilon\}.
$$
We differentiate two cases: 
\begin{enumerate}
    \item \textit{Case 1:} Let $x\in\mathcal{X}$. If $\{a_{t+1}(x) = a\}\subseteq \mathcal{E}_{1}(t,x)$, we have 
\begin{align*}
\varepsilon_{x,a,t} &= N_{x,a}(t)- N_x(t)\hat{\alpha}_{x,a}(t) \\
&= N_{x,a}(t) - N_x(t)\bar{\alpha}_{x,a}(t) + t\bar{\alpha}_{x,a}(t) - N_x(t)\hat{\alpha}_{x,a}(t) \\
& \leq N_{x,a}(t)- N_x(t)\bar{\alpha}_{x,a}(t)+ c\varepsilon t\\
& \leq \min_{a \in \operatorname{supp}(\bar{\alpha}_x(t))} {N_{x,a}(t)}- t\bar{\alpha}_{x,a}(t)+ 2c\varepsilon t\\
& \leq 2tc\varepsilon ,
\end{align*}
where the last inequality holds because 
$
\sum_{a \in \operatorname{supp}(\bar{\alpha}_x(t))} N_{x,a}(t)- N_x(t)\bar{\alpha}_{x,a}(t) \leq 0.
$
Hence $\mathcal{E}_1(t,x) \subseteq \{\varepsilon_{x,a,t}\leq 2ct\varepsilon\}$  $\forall x \in\mathcal{X}$. \newline
\item \textit{Case 2:} Let $x\in\mathcal{X}$. If $\{a_{t+1}(x) = a\}\subseteq \mathcal{E}_{2}(t,x)$, we have $a\in\mathcal{A}_x$. Define 

\begin{align*}
N_{x,a,1}(k)& = \sum_{s=1}^{k} \mathbbm{1}{\left\{x_{k} = x \text { and } a_{k}(x) = a \text { and } A_x(k-1) \prec f_x(k-1)\right\}}, \\
N_{x,a,2}(k)& = \sum_{s=1}^{k} \mathbbm{1}{\left\{ x_{k} = x \text { and }  a_{k}(x) = a \text { and } A_x(k-1) \succeq f_x(k-1)\right\}}.
\end{align*}

Note that $N_{x,a}(k)= N_{x,a,1}(k) + N_{x,a,2}(k)$, and by definition of the forced exploration sampling rule it follows that for all $x\in\mathcal{X}$ it holds $N_{x,a,1}(k)-1 \leq \min_{a_x \in \mathcal{A}_{x}} N_{x,a_x,1}(k) \leq N_{x,a, 1}(k)$. Since the event $\mathcal{E}_{2}(t,x)$ holds, we observe that
\begin{align*}
\left(N_{x,a,1}(t)-1\right)\lambda_{d_x}\left(\sum_{a_x \in \mathcal{A}_x} \phi_{x,a_x}\phi_{x,a_x}^\top \right) & \leq \min_{a_x \in \mathcal{A}_{x}} N_{x,a_x, 1}(t) \lambda_{d_x}\left(\sum_{a_x \in \mathcal{A}_x} \phi_{x,a_x}\phi_{x,a_x}^\top \right) \\& \leq \lambda_{d_x }\left(\sum_{s =1}^t \phi_{x_s,a_s}\phi_{x_s,a_s}^\top \mathbbm{1}\{x_s = x\} \right) \\& < f_x(t) = \sqrt{\frac{N_x(t)}{d_x}}\lambda_{d_x}\left(\sum_{a_x \in \mathcal{A}_x} \phi_{x,a_x}\phi_{x,a_x}^\top \right)
\end{align*}
Hence we obtain $ N_{x,a,1}(t) \leq \sqrt{N_x(t)/d_x} + 1. $
Let $k \leq t$ be the largest integer such that $N_{x,a,2}(k) = N_{x,a,2}(k-1) + 1$. Note that at
such $k$ the event $\mathcal{E}_1(k-1,x)$ must hold by definition of $N_{x,a,2}(k - 1)$, and we have 
$$
N_{x,a,2}(t)=N_{x,a,2}(k)=N_{x,a,2}(k-1)+1 \quad \text { and } \quad a_{k}(x)=\underset{a \in \operatorname{supp}(\bar{\alpha}_x(k-1))}{\argmin} N_{x,a}(k-1)-k \bar{\alpha}_{x,a}(k-1).
$$
We also have 
\begin{align*}
\varepsilon_{x,a,t} & = N_{x,a,t} - N_{x}(t)\hat{\alpha}_{x,a}(t)\\
&=N_{x,a, 1}(t)+N_{x,a,2}(t) - N_{x}(t) \hat{\alpha}_{x,a}(t) \\
& \leq \sqrt{N_x(t)/d_x} + 1 + N_{x,a,2}(t)-N_{x}(t) \hat{\alpha}_{x,a}(t)
\\& \leq \sqrt{c_2 t/d_x} + 1 + N_{x,a,2}(t)-N_{x}(t) \hat{\alpha}_{x,a}(t).
\end{align*}

If $k-1\leq t_0'$, then we have $N_{x,a,2}(k) \leq t_0'$, otherwise $\mathcal{E}_1(x,k-1)$ holds,and we have
\begin{align*}
N_{x,a,2}(t) &=1+N_{x,a,2}(k-1)-(k-1) \hat{\alpha}_{x,a}(k-1)+(k-1) \hat{\alpha}_{x,a}(k-1) \\
& \leq 1+2(k-1)c\varepsilon+(k-1) \hat{\alpha}_{x,a}(k-1).
\end{align*}

Hence we get
$$
\varepsilon_{x,a,t} \leq \sqrt{c_2 t/d_x} + 1 + \max\{t_0', 1+2(k-1)c\varepsilon + (k-1) \hat{\alpha}_{x,a}(k-1)-N_x(t) \hat{\alpha}_{x,a}(t)\},
$$
and since
\begin{align*}
(k-1) \hat{\alpha}_{x,a}(k-1)-N_x(t) \hat{\alpha}_{x,a}(t)= &(k-1) \hat{\alpha}_{x,a}(k-1)-(k-1) \bar{\alpha}_{x,a}(k-1) +(k-1) \bar{\alpha}_{x,a}(k-1)-N_x(t)\hat{\alpha}_{x,a}(t) \\
\leq &(k-1) \hat{\alpha}_{x,a}(k-1)-(k-1) \bar{\alpha}_{x,a}(k-1)+N_x(t) \bar{\alpha}_{x,a}(t)-N_x(t) \hat{\alpha}_{x,a}(t) \\
\leq & 2(k-1) c\varepsilon+2 N_x(t) \varepsilon\\
\leq & 2 ct\varepsilon+2 c_2 t \varepsilon \\
\leq & 2(c+c_2)t \varepsilon
\end{align*}
we can conclude that 
$$
\varepsilon_{x,a,t} \leq \sqrt{c_2 t/d_x} + 1 + \max\{t_0', 1+ 2t(c_2+2c)\varepsilon\} \leq \sqrt{t/d_x} + 1 + \max\{t_0', 1+ 2(1+2c)t\varepsilon\}.
$$
%Hence for $t\geq t_0'' =\max\left\{\frac{1}{c'\varepsilon},\frac{1+t_0'}{c'\varepsilon - \sqrt{\frac{c_2}{d}}},\frac{1}{\varepsilon(c'-2(c_2+2c))}- \frac{1}{\sqrt{d}}\right\}$ 
Hence for $t\geq t_0'' = \max\left\{\frac{9}{c'^2\varepsilon^2 d},\frac{3t_0'}{c'\varepsilon},\frac{6}{c'\varepsilon}\right\}$
it holds that $\varepsilon_{x,a,t} \leq c' t\varepsilon$ and thus
$\mathcal{E}_2(x,t) \subseteq \{\varepsilon_{x,a,t}\leq c' t\varepsilon\},$ for some $c'\geq 2(1+2c)$.
Thus we have proved that for our choice of $t_0'',c'$ and for all $t\geq t_0''$, for all $(x,a) \in\mathcal{X}\times \mathcal{A}$, we have 
$$
\{a_{t+1} = a\}\subseteq \mathcal{E}_{1}(t,x) \cup \mathcal{E}_{2}(t,x) \subseteq \{\varepsilon_{x,a,t} \leq c' t\varepsilon\},
$$
\end{enumerate}
Note that, since $c \geq 1$, we may pick $c' = 6$. This results in $ t_0'' = \max\left\{\frac{1}{4\varepsilon^2 d},\frac{t_0'}{2\varepsilon},\frac{1}{\varepsilon}\right\}$. Now, by Lemma 17 in \cite{Garivier16}, for all $(x,a)\in\mathcal{X}\times \mathcal{A}$, it holds that for all $t\geq t_0''$
$$
\varepsilon_{x,a,t} \leq \max\{\varepsilon_{x,a,t_0''},2t(c_2+2c)\varepsilon +1\} \leq\max\{t_0'',6 t\varepsilon +1\}.
$$
We note that for all $t\geq0$, we have $\bar{\alpha}_x(t-1) \subseteq \bar{\alpha}_x(t)$. Hence we have 
$$
\sum_{a \in \operatorname{supp}(\bar{\alpha}_x(t)) \cup \mathcal{A}_{x}} \varepsilon_{x,a, t}=\sum_{a \in \mathcal{A} \backslash \operatorname{supp}(\bar{\alpha}_x(t)) \cup \mathcal{A}_{x}} t \hat{\alpha}_{x,a}(t) \geq 0.
$$
Let $z_{t,x} = |\supp(\bar{\alpha}_x(t))\setminus \mathcal{A}_x|$, and $z_{t} = \max_{x\in \mathcal{X}} |\supp(\bar{\alpha}_x(t))\setminus \mathcal{A}_x|$ and note that
$$
\begin{array}{l}
\forall x\in\mathcal{X}, \forall a \in \operatorname{supp}(\bar{\alpha}_x(t)) \cup \mathcal{A}_{x}, \quad \max \left(t_{0}^{\prime \prime}, c' t \varepsilon+1\right) \geq \varepsilon_{x,a,t} \geq-\left(z_{t,x}+d-1\right) \max \left(t_{0}^{\prime \prime}, c' t \varepsilon+1\right), \\
\forall x\in\mathcal{X}, \forall a \in \mathcal{A} \backslash \operatorname{supp}(\bar{\alpha}_x(t)) \cup \mathcal{A}_{x}, \quad 0 \geq \varepsilon_{x,a, t} \geq - c_2 t \varepsilon,
\end{array}
$$
which implies for all $t\geq t_0''$    
$$
\max_{(x,a)\in\mathcal{X}\times \mathcal{A}}\left|\varepsilon_{x,a, t}\right| \leq\left(z_{t}+d- 1\right) \max \left\{t_{0}^{\prime \prime}, 6t \varepsilon+1\right\} \leq\left(z_{t}+d- 1\right) \max \left\{t_{0}^{\prime \prime}, 7\right\}  .
$$
This finally implies that for $t_1(\varepsilon,\kappa) = \frac{1}{c_1(\kappa)\varepsilon}\max\{t_0'',7\}$, we have for all $t \ge t_1$,
\begin{align*}
d_{\infty}\left(\left(N_{x,a}(t)/N_{x}(t)\right)_{(x,a) \in \mathcal{X}\times \mathcal{A}}, C\right) & \leq d_{\infty}\left(\left(N_{x,a}(t)/N_{x}(t)\right)_{(x,a) \in \mathcal{X}\times \mathcal{A}}, \hat{\alpha}(t)\right) \\& =\max_{(x,a) \in \mathcal{X}\times \mathcal{A}}\left|N_{x,a}(t) / N_x(t) -\hat{\alpha}_{x,a}(t)\right|\\& = \max _{(x,a) \in \mathcal{X}\times \mathcal{A}}\left|\frac{\varepsilon_{x,a, t}}{N_x(t)}\right| \leq\max _{(x,a) \in \mathcal{X}\times \mathcal{A}}\left|\frac{\varepsilon_{x,a, t}}{c_1(\kappa)t}\right| \leq\left(z_{t}+d-1\right) \varepsilon.
\end{align*}
More precisely, we have
\begin{equation}
\label{eq:t1}
t_1(\varepsilon,\kappa) =\max\left\{\frac{1}{4c_1(\kappa) d\varepsilon^3},\frac{t_0(\varepsilon)}{2c_1(\kappa)\varepsilon^3}\frac{1}{c_1(\kappa)\varepsilon^2}, \frac{7}{c_1(\kappa) \varepsilon}\right\}. %\max\left\{\frac{1}{c_1\varepsilon^2},\frac{1+t_0}{(c'\varepsilon - \sqrt{\frac{c_1}{d}})c_1\varepsilon},\frac{1}{\varepsilon^2 c_1(c'-2(c_1+2c))}- \frac{1}{\sqrt{d}c_1\varepsilon},\frac{c' +1}{c_1\varepsilon}\right\}.
\end{equation}

\end{proof}
\begin{comment}
    \subsection{Proof of Lemma
\ref{lem:tracking_lemma}}
\begin{proof}
Let $t>0$, and for all $x\in\mathcal{X}$ define $\mathcal{I}_{x}(t) = \{i_k\in [1,t]:x_{i_k} = x\}$, the indices at which context $x$ is observed, with $k\in\{1,\dots,N_x(t)\}$. Note that with probability at least $1-2^{-t\kappa^2/4}$, for all 
$$
|\mathcal{I}_x(t)| = N_x(t) \geq (p_\mathcal{X}(x)-\kappa)t
$$
Note that $C$ is non-empty, and for all $k>0$ define
$$
\bar{\alpha}_x(k) = \frac{1}{k}\sum_{j = 1}^k \alpha_x(i_j), \quad \hat{\alpha}(t)= \argmin_{\alpha \in C} d_{\infty}(\bar{\alpha}(t), \alpha), \quad v(t) = \argmin_{\alpha \in C} d_{\infty}(\alpha(t), \alpha).$$ 
Observe that $\exists k_0(x)$ such that $\forall k \geq k_0$, we have 
$$
    d_\infty(\alpha_x(k),C_x)\leq \varepsilon,
$$
where $C_x = \{\alpha_x \in[0,1]^K: \sum_{a = 1}^K \alpha_{x,a} = 1\}$ such that $C_x\cap C_y = \emptyset$, $\bigcup_{x\in\mathcal{X}} C_x = C$, and $\alpha_x = \text{proj}_{C_x}(\alpha)$. Now, observe that for all $a\in \mathcal{A}$, we have 
\begin{align*}
\left|\frac{1}{k} \sum_{j=1}^{k} \alpha_{x,a}(i_j)-\frac{1}{k} \sum_{j=1}^{k} v_{x,a}(i_j)\right| & \leq \frac{1}{k} \sum_{j=1}^{k_{0}}\left|\alpha_{x,a}(i_j)-v_{x,a}(i_j)\right|+\frac{1}{k} \sum_{j=k_{0}+1}^{k}\left|\alpha_{x,a}(i_j)-v_{x,a}(i_j)\right| \\
& \leq \frac{k_{0}}{k}+\frac{k-k_{0}}{k} \varepsilon.
\end{align*}
Hence for all $k_0$h
$N_x(t) \geq \frac{t(p_\mathcal{X}(x) -\kappa) }{\varepsilon}$, we  have $d_{\infty}\left(\bar{\alpha}_x(k),\frac{1}{k} \sum_{j =1}^k v_x(k)\right)\leq 2\varepsilon$. Since by convexity of $C_x$ we have $\frac{1}{k}\sum_{j = 1}^k v(i_j) \in C_x$, we may conclude that
$$
\forall k \geq k_{0}^{\prime} \quad d_{\infty}(\bar{\alpha}_x(k), \hat{\alpha}_x(k)) \leq d_{\infty}\left(\bar{\alpha}_x(k), \frac{1}{k} \sum_{j=1}^{k} v(i_j)\right) \leq 2 \varepsilon.  
$$
Further define for all $t\geq 1$, $\varepsilon_{x,a,t} = N_{x,a}(t) - N_x(t)\hat{\alpha}_{x,a}(t)$, and the events
\begin{align*}
\mathcal{E}_{1}(t,x) &=\left\{a=\underset{a \in \supp(\bar{\alpha}_x(t))}{\argmin}\{N_{x,a}(t)- N_x(t) \bar{\alpha}_{x,a}(t)\}\right\}, \\
\mathcal{E}_{2}(t,x)&=\left\{A_x(t) \prec f_x(t) \quad \text { and } \quad a=a_x(i_t(x))\right\}.
\end{align*}
The rest of the proof will be aimed at showing that exists $t_0'' \geq t_0'$ such that for all $t\geq t_0''$, for all $(x,a) \in\mathcal{X}\times \mathcal{A}$, we have 
$$
\{a_{t+1} = a\}\subseteq \mathcal{E}_{1}(t,x) \cup \mathcal{E}_{2}(t,x) \subseteq \{\varepsilon_{x,a,t} \leq 9N_x(t)\varepsilon\}.
$$
We differentiate two cases: 
\begin{enumerate}
    \item \textit{Case 1:} If $\{a_{t+1} = a\}\subseteq \mathcal{E}_{1}(t,x)$, we have 
\begin{align*}
\varepsilon_{x,a,t} &= N_{x,a(t)}- N_x(t)\hat{\alpha}_{x,a}(t) \\
&= {N_{x,a}(t)} - N_x(t)\bar{\alpha}_{x,a}(t) + N_x(t)\bar{\alpha}_{x,a}(t) - N_x(t)\hat{\alpha}_{x,a}(t) \\
& \leq N_{x,a}(t)- N_x(t)\bar{\alpha}_{x,a}(t)+ \varepsilon N_x(t) \\
& \leq \min_{a \in \operatorname{supp}(\bar{\alpha}_x(t))} {N_{x,a}(t)}- N_x(t)\bar{\alpha}_{x,a}(t)+ \varepsilon N_x(t) \\
& \leq 2 N_x(t) \varepsilon,
\end{align*}
where the last inequality holds because 
$
\sum_{a \in \operatorname{supp}(\bar{\alpha}_x(t))} N_{x,a}(t)- N_x(t)\bar{\alpha}_{x,a}(t) \leq 0.
$
Hence $\forall x \in\mathcal{X}, \mathcal{E}_1(t,x) \subseteq \{\varepsilon_{x,a,t}\leq 2t\varepsilon\}$. \newline
\item \textit{Case 2:} If $\{a_{t+1} = a\}\subseteq \mathcal{E}_{2}(t,x)$, we have $a\in\mathcal{A}_x$. Define 

\begin{align*}
N_{x,a,1}(k)& = \sum_{s=1}^{k} \mathbbm{1}{\left\{x_{k} = x \text { and } a_{k} = a \text { and } A_x(k-1) \prec f_x(k-1)\right\}}, \\
N_{x,a,2}(k)& = \sum_{s=1}^{k} \mathbbm{1}{\left\{ x_{k} = x \text { and }  a_{k} = a \text { and } A_x(k-1) \succeq f_x(k-1)\right\}}.
\end{align*}

Note that $N_{x,a}(k)= N_{x,a,1}(k) + N_{x,a,1}(k)$, and by definition of the forced exploration sampling rule it follows that for all $x\in\mathcal{X}$ it holds $N_{x,a,1}(k)-1 \leq \min_{a_x \in \mathcal{A}_{x}} N_{x,a_x,1}(k) \leq N_{a, 1}(k)$. Since the event $\mathcal{E}_{2}(t,x)$ holds, we observe that
\begin{align*}
\left(N_{x,a,1}(t)-1\right)\lambda_{d_x}\left(\sum_{a_x \in \mathcal{A}_x} \phi_{x,a_x}\phi_{x,a_x}^\top \right) & \leq \min_{a_x \in \mathcal{A}_{x}} N_{x,a, 1}(t) \lambda_{d_x}\left(\sum_{a_x \in \mathcal{A}_x} \phi_{x,a_x}\phi_{x,a_x}^\top \right) \\& \leq \lambda_{d_x }\left(\sum_{a_x \in \mathcal{A}_x} \phi_{x,a_x}\phi_{x,a_x}^\top \right) \\& \leq \sqrt{\frac{N_x(t)}{d_x}}\lambda_{d_x}\left(\sum_{a_x \in \mathcal{A}_x} \phi_{x,a_x}\phi_{x,a_x}^\top \right)
\end{align*}
Hence we obtain $ N_{x,a,1}(t) \leq \sqrt{N_x(t)/d_x} + 1. $
Let $k \leq t$ be the largest integer such that $N_{x,a,2}(k) = N_{x,a,2}(k-1) + 1$. Note that at
such $k$ the event $\mathcal{E}_1(k-1,x)$ must hold by definition of $N_{x,a,2}(k - 1)$, and we have 
$$
N_{x,a,2}(t)=N_{x,a,2}(k)=N_{x,a,2}(k-1)+1 \quad \text { and } \quad a_{k}=\underset{a \in \operatorname{supp}(\bar{\alpha}_x(k-1))}{\argmin} N_{x,a}(k-1)-k \bar{\alpha}_{x,a}(k-1).
$$
We also have 
\begin{align*}
\varepsilon_{x,a,t} & = N_{x,a,t} - N_{x}(t)\hat{\alpha}_{x,a}(t)\\
&=N_{x,a, 1}(t)+N_{x,a,2}(t) - N_{x}(t) \hat{\alpha}_{x,a}(t) \\
& \leq \sqrt{N_x(t)/d_x} + 1 + N_{x,a,2}(t)-N_{x}(t) \hat{\alpha}_{x,a}(t).
\end{align*}

If $k-1\leq t_0'$, then we have $N_{x,a,2}(k) \leq t_0'$, otherwise $\mathcal{E}_1(k-1)$ holds, we have
\begin{align*}
N_{x,a,2}(t) &=1+N_{x,a,2}(k-1)-(k-1) \hat{\alpha}_{x,a}(k-1)+(k-1) \hat{\alpha}_{x,a}(k-1) \\
& \leq 1+2(k-1) \varepsilon+(k-1) \hat{\alpha}_{x,a}(k-1).
\end{align*}

Hence
$$
\varepsilon_{x,a,t} \leq \sqrt{N_x(t)/d_x} + 1 + \max\{t_0', 1+2(k-1)\varepsilon\},
$$
and since
\begin{align*}
(k-1) \hat{\alpha}_{x,a}(k-1)-N_x(t) \hat{\alpha}_{x,a}(t)= &(k-1) \hat{\alpha}_{x,a}(k-1)-(k-1) \bar{\alpha}_{x,a}(k-1) +(k-1) \bar{\alpha}_{x,a}(k-1)-N_x(t)\hat{\alpha}_{x,a}(t) \\
\leq &(k-1) \hat{\alpha}_{x,a}(k-1)-(k-1) \bar{\alpha}_{x,a}(k-1)+N_x(t) \bar{\alpha}_{x,a}(t)-N_x(t) \hat{\alpha}_{x,a}(t) \\
\leq & 2(k-1) \varepsilon+2 N_x(t) \varepsilon \\
\leq & 4 N_x(t) \varepsilon
\end{align*}
we can conclude that 
$$
\varepsilon_{x,a,t} \leq \sqrt{N_x(t)/d_x} + 1 + \max\{t_0', 1+6N_x(t)\varepsilon\}. 
$$
Hence for $t\geq t_0'' =\max\left\{\frac{1}{\varepsilon},\frac{1}{\varepsilon^2 d_x},\frac{t_0'}{\varepsilon}\right\}$ it holds that $\varepsilon_{x,a,t} \leq 2t(c_2+2c)\varepsilon$ and thus
$
\mathcal{E}_2(x,t) \subseteq \{\varepsilon_{x,a,t}\leq 9N_x(t)\varepsilon\}.
$
Thus we have proved that for our choice of $t_0''$ and for all $t\geq t_0''$, for all $(x,a) \in\mathcal{X}\times \mathcal{A}$, we have 
$$
\{a_{t+1} = a\}\subseteq \mathcal{E}_{1}(t,x) \cup \mathcal{E}_{2}(t,x) \subseteq \{\varepsilon_{x,a,t} \leq 9N_x(t)\varepsilon\}.
$$
\end{enumerate}
By Lemma 17 in \cite{Garivier16} it holds that for all $x\in\mathcal{X}$
$$
\varepsilon_{x,a,t} \leq \max\{\varepsilon_{x,a,t_0''},c't\varepsilon +1\} \leq\max\{  t_0'',9c't\varepsilon +1\}.
$$
We note that for all $t\geq0$,$x\in\mathcal{X}$ we have $\bar{\alpha}_x(t-1) \subseteq \bar{\alpha}_x
(t)$. Hence we have 
$$
\sum_{a \in \operatorname{supp}(\bar{\alpha}_x(t)) \cup \mathcal{A}_{x}} \varepsilon_{x,a, t}=\sum_{a \in \mathcal{A} \backslash \operatorname{supp}(\bar{\alpha}_x(t)) \cup \mathcal{A}_{x}} t \hat{\alpha}_{x,a}(t) \geq 0.
$$
Let $z_{t,x} = |\supp(\bar{\alpha}_x(t))\setminus \mathcal{A}_x|$, $z_{t,x} = \max_{x} |\supp(\bar{\alpha}_x(t))\setminus \mathcal{A}_x|$, and note that
$$
\begin{array}{l}
\forall x\in\mathcal{X}, \forall a \in \operatorname{supp}(\bar{\alpha}_x(t)) \cup \mathcal{A}_{x}, \quad \max \left(t_{0}^{\prime \prime}, 9 N_x(t) \varepsilon+1\right) \geq \varepsilon_{x,a,t} \geq-\left(z_{t,x}+d-1\right) \max \left(t_{0}^{\prime \prime}, 9 N_x(t) \varepsilon+1\right), \\
\forall x\in\mathcal{X}, \forall a \in \mathcal{A} \backslash \operatorname{supp}(\bar{\alpha}_x(t)) \cup \mathcal{A}_{x}, \quad 0 \geq \varepsilon_{x,a, t} \geq-N_x(t) \varepsilon,
\end{array}
$$
which implies for all $t\geq t_0''$ and $x\in\mathcal{X}$ that    
$$
\max_{a \in \mathcal{A}}\left|\varepsilon_{x,a, t}\right| \leq\left(z_{t,x}+d-1\right) \max \left(t_{0}^{\prime \prime}, 9 N_x(t) \varepsilon+1\right).
$$
This finally implies that for $t_1 = \frac{1}{\varepsilon}$, we have for all $t \ge t_1$,
\begin{align*}
d_{\infty}\left(\left(N_{x,a}(t)/N_{x}(t)\right)_{(x,a) \in \mathcal{X}\times \mathcal{A}}, C\right) & \leq d_{\infty}\left(\left(N_{x,a}(t)/N_{x}(t)\right)_{(x,a) \in \mathcal{X}\times \mathcal{A}}, \hat{\alpha}(t)\right) \\& =\max_{(x,a) \in \mathcal{X}\times \mathcal{A}}\left|N_{x,a}(t) / N_x(t) -\hat{\alpha}_{x,a}(t)\right|\\& =\max _{(x,a) \in \mathcal{X}\times \mathcal{A}}\left|\frac{\varepsilon_{x,a, t}}{N_x(t)}\right| \leq\left(z_{t,x}+d-1\right) \varepsilon.
\end{align*}

By Lemma \ref{lem:Nx_concentration_tight}, $\forall \kappa \in\left(0,p_{\min}\right)$ we get that with probability at least $1-2e^{-\frac{t \kappa^2}{4}}$

$$ (p_\mathcal{X}(x) -\kappa)t\leq N_x(t) \leq (p_\mathcal{X}(x)+\kappa)t.$$

\end{proof}
\end{comment}

\subsection{Proof of Lemma \ref{lem:convergence_proportions}}
\begin{proof}
Fix $\varepsilon>0$. By Lemma \ref{lem:properties_eps_delta} there exists $g(q) >0$ such that for all $\theta'$ that satisfies $\|\theta' - \theta\| \leq g(q)$, we have $\sup_{\alpha \in C_\varepsilon(\theta')} d_\infty(\alpha, C^\star_\varepsilon(\theta)) \leq \varepsilon/2$. By Lemma \ref{lem:LS_concentration}, we have that $\hat{\theta}_t$ converges to $\theta$ a.s. Hence there exists $t_0 \geq 1$ such that for all $t\geq t_0$ we have 
$$
\|\hat{\theta}_t - \theta\| \leq g(q).
$$
The condition \eqref{eq:condition_convergence} implies that there exists $t_1\geq 1$, and there exists a sequence of integers $(h(t))_{t\geq 1}$ such that for all $t\geq t_1$ we have $h(t) \geq \ell(t) \geq t$, and $d_\infty(\alpha(t), C^\star_\varepsilon(\hat{\theta}_{h(t)})) < \varepsilon/2$. Hence for all $t\geq \max\{t_0,t_1\}$, we get

$$
d_{\infty}\left(\alpha(t), C_\varepsilon^{\star}(\theta)\right) \leq d_{\infty}\left(\alpha(t), C_\varepsilon^{\star}\left(\hat{\theta}_{h(t)}\right)\right)+\max _{\alpha \in C_\varepsilon^{\star}\left(\hat{\theta}_{h(t)}\right)} d_{\infty}\left(\alpha, C_\varepsilon^{\star}(\theta)\right)<\varepsilon.
$$
Hence we have that $\lim_{t\to \infty}d_{\infty}\left(\alpha(t), C_\varepsilon^{\star}(\theta)\right) = 0$ a.s., and by Lemma \ref{lem:tracking_lemma}, we can conclude that 
$$\lim_{t\to \infty}d_\infty\left(\left(\frac{N_{x,a}(t)}{N_x(t)}\right)_{(x,a)\in\mathcal{X}\times\mathcal{A}},C^\star_\varepsilon(\theta) \right) = 0, \text { a.s.}$$
\end{proof}

\subsection{Proof of Theorem \ref{th:optimality}}
\begin{proof}

\textit{1) Almost sure guarantee: } Define the event:
$$\mathcal{E}=\left\{d_{\infty}\left(\left(N_{x,a}(t)/N_x(t)\right)_{(x,a)\in\mathcal{X} \times \mathcal{A}}, C_\varepsilon^{\star}(\alpha)\right) \underset{t \rightarrow \infty}{\longrightarrow} 0 \text { and } \hat{\theta}_{t} \underset{t \rightarrow \infty}{\longrightarrow} \theta\right\},
$$
and, by Lemma \ref{lem:LS_concentration} and Lemma \ref{lem:convergence_proportions}, the event $\mathcal{E}$ holds with w.p. $1$. Note that an equivalent way to define $(T^\star_{\theta,\varepsilon})^{-1}$ is through a convex program: $\bar{\psi}_\varepsilon(\theta) = \sup_{\alpha\in\Lambda}\bar{\psi}_\varepsilon(\theta,\alpha)$, where 
$$
\bar{\psi}_\varepsilon(\theta,\alpha) = \min_{x\in\mathcal{X}}\min_{a\in \mathcal{A}^c_\varepsilon(\theta,x)} \inf_{\mu \in \hat{B}_{\varepsilon}(\theta, x, a)} \|\theta - \mu\|^2_{A(\alpha)}, %\inf_{{\left\lbrace \mu\in\mathbb{R}^d: \exists x \in \mathcal{X}, \forall a \in \mathcal{A}_\varepsilon(\theta,x), \; \mu^{\top}(\phi_{x,a_{\mu}^\star(x)}- \phi_{x,a})>\varepsilon \right\rbrace}}
$$
and $\hat{B}_\varepsilon(\theta,x,a) = \left\lbrace \mu \in \mathbb{R}^d: \; \exists b \in \mathcal{A}_\varepsilon(\theta,x), \; \mu^{\top}\gamma^x_{a,b}\leq-\varepsilon \right\rbrace$. Let $q>0$. By continuity of $\bar{\psi}_\varepsilon$ (Lemma \ref{lem:properties_eps_delta}), there exist an open neighborhood, $\mathcal{N}(q)$ of $\{\theta\}\times C_\varepsilon^\star(\theta)$, such that for all $(\theta',\alpha')\in \mathcal{N}(q)$, we have 
$$
    \bar{\psi}_\varepsilon(\theta',\alpha') \geq (1-q)\bar{\psi}_\varepsilon(\theta,\alpha^\star),
$$
for some $\alpha^\star \in C_\varepsilon^\star(\theta)$. Since $\mathcal{E}$ holds, there exists $t_0\geq1$ such that for all $t\geq t_0$ we have that $\left(\hat{\theta}_t,\left(N_{x,a}(t)/N_x(t)\right)_{(x,a)\in\mathcal{X} \times \mathcal{A}}\right) \in\mathcal{N}(q)$. Hence, for $t\geq t_0$ we have 
$$
    \bar{\psi}_\varepsilon\left(\hat{\theta}_t,\left(N_{x,a}(t)/N_x(t)\right)_{(x,a)\in\mathcal{X} \times \mathcal{A}}\right) \geq (1-q)\bar{\psi}_\varepsilon\left(\theta,\alpha^\star\right).
$$
%Since $\hat{\theta}_t \to \theta$, there exists $t_1 \geq 0$
Hence, $\forall x\in\mathcal{X}$ and $t\geq t_0$, we get:
\begin{align*}
    Z^x_\varepsilon(t) & = \max_{a\in\mathcal{A}_\varepsilon(\hat{\theta}_t,x)} \min_{b \neq a} \frac{(\hat{\theta}_{t}^{\top}\left(\phi_{x,a}-\phi_{x,b})+\varepsilon\right)^{2}}{2\left(\phi_{x,a}-\phi_{x,b}\right)^{\top}\left(\sum_{s=1}^{t} \phi_{x_s,a_s} \phi_{x_s,a_s}^{\top}\right)^{-1}\left(\phi_{x,a}-\phi_{x,b}\right)} \\& \geq 
    \min_{a\in\mathcal{A}_\varepsilon(\hat{\theta}_t,x)} \min_{b \in \mathcal{A}^c_\varepsilon(\hat{\theta}_t,x.a)} \frac{(\hat{\theta}_{t}^{\top}\left(\phi_{x,a}-\phi_{x,b})+\varepsilon\right)^{2}}{2\left(\phi_{x,a}-\phi_{x,b}\right)^{\top}\left(\sum_{s=1}^{t} \phi_{x_s,a_s} \phi_{x_s,a_s}^{\top}\right)^{-1}\left(\phi_{x,a}-\phi_{x,b}\right)}
    \\& \geq \min_{a\in\mathcal{A}_\varepsilon(\hat{\theta}_t,x)} \min_{b \in \mathcal{A}^c_\varepsilon(\hat{\theta}_t,x,a)} \frac{(\hat{\theta}_{t}^{\top}\left(\phi_{x,a}-\phi_{x,b})+\varepsilon\right)^{2}}{2\left(\phi_{x,a}-\phi_{x,b}\right)^{\top}\left(\sum_{s=1}^{t} \phi_{x_s,a_s} \phi_{x_s,a_s}^{\top}\right)^{-1}\left(\phi_{x,a}-\phi_{x,b}\right)}.% \\& =t \bar{\psi}_\varepsilon\left(\hat{\theta}_{t},\left(N_{x,a}(t)/N_x(t)\right)_{(x,a)\in\mathcal{X} \times \mathcal{A}}\right).
\end{align*}
Hence we get $$\min_{x\in\mathcal{X}} Z^x_\varepsilon(t) \geq \min_{x\in\mathcal{X}}\min_{a\in\mathcal{A}_\varepsilon(\hat{\theta}_t,x)} \min_{b \in \mathcal{A}^c_\varepsilon(\hat{\theta}_t,x,a)} \frac{(\hat{\theta}_{t}^{\top}\left(\phi_{x,a}-\phi_{x,b})+\varepsilon\right)^{2}}{2\left(\phi_{x,a}-\phi_{x,b}\right)^{\top}\left(\sum_{s=1}^{t} \phi_{x_s,a_s} \phi_{x_s,a_s}^{\top}\right)^{-1}\left(\phi_{x,a}-\phi_{x,b}\right)} = \bar{\psi}_\varepsilon(\theta,\alpha^\star). $$

By Lemma \ref{lem:forced_exploration}, for all $\varepsilon \in (0,p_{\min})$, there exists $\kappa$, $t_1(\kappa,\varepsilon) \geq 1$ such that for all $t \geq t_1$, we have $ \sum_{s = 1}^t \phi_{x_s,a_s}\phi_{x_s,a_s}^\top \succeq \sqrt{t}\kappa I_d$ with probability at least $1-2e^{-\varepsilon^2t/4}$ for some $\kappa>0$. By an immediate application of the first Borel-Cantelli Lemma, we obtain that the event $\left\{ \sum_{s = 1}^t\phi_{x_s,a_s}\phi_{x_s,a_s}^\top \not \succeq \sqrt{t}\kappa I_d \text{ i.o.}\right\}$ holds with probability $0$. Therefore, with probability $1$, there exists $t_2 \ge 0$ such that for all $t \ge t_2$, $ \sum_{s = 1}^t \phi_{x_s,a_s}\phi_{x_s,a_s}^\top \succeq \sqrt{t}\kappa I_d \succeq c I_d$. Let $t \ge \max\lbrace t_0, t_2\rbrace$, we have 

\begin{align*}
 \tau & =\inf \Big\{t \in \mathbb{N}^{*}: \forall x\in\mathcal{X}, Z_\varepsilon^x(t)>\beta(\delta, t) \text{ and } \sum_{s=1}^{t} \phi_{x_s,a_{s}}\phi_{x_s,a_{s}}^{\top} \succeq c I_{d}\Big\} \\&  \leq \max \{t_0,t_2\} \lor \inf \Big\{t \in \mathbb{N}^{*}: t(1-q) \bar{\psi}_\varepsilon\left(\theta,\alpha^\star \right)>\beta(\delta, t) \text{ and } \sum_{s=1}^{t} \phi_{x_s,a_{s}}\phi_{x_s,a_{s}}^{\top} \succeq c I_{d}\Big\}\\&  \leq \max \{t_0,t_2\} \lor \inf \Big\{t\in\mathbb{N}^*: t \bar{\psi}_\varepsilon\left(\theta,\alpha^\star \right)>\frac{1+u}{1-q} \log \left(\frac{\operatorname{det}\left((uc)^{-1} \sum_{s=1}^{t} \phi_{x_s,a_{s}}\phi_{x_s,a_{s}}^{\top}+I_{d}\right)^{\frac{1}{2}}}{\delta}\right) \text{ and } \sum_{s=1}^{t} \phi_{x_s,a_{s}}\phi_{x_s,a_{s}}^{\top} \succeq c I_{d}\Big\} \\ & \lesssim \max\left\{t_0,t_2, \frac{1}{1-q}T^\star_{\theta,\varepsilon}\log\left(\frac{1}{\delta}\right)\right\},
\end{align*}
where we used \cite[Lemma 18]{Garivier16} for $\delta$ sufficiently small in the last inequality. By letting $q\to 0$, we get 
$$
\mathbb{P}_\theta\Bigg(\limsup_{\delta \to 0} \frac{\tau}{\log \left(\frac{1}{\delta}\right)} \lesssim T_{\varepsilon,
\theta}^{\star}\Bigg) = 1.
$$
\textit{2) Guarantee in expectation.}

\textit{Step 1:} By continuity of $\bar{\psi}_\varepsilon$ (Lemma \ref{lem:properties_eps_delta}), there exist $g_1(q)>0$ such that for all $\theta' \in\mathbb{R}^d$ and $\alpha' \in \Lambda$
\begin{equation}
\label{eq:fact1}
    \left\{\begin{array}{ll}
    \left\|\theta^{\prime}-\theta\right\| & \leq g_1(q) \\
    d_{\infty}\left(\alpha^{\prime}, C_\varepsilon^{\star}(\theta)\right) & \leq g_1(q)
    \end{array} \Longrightarrow\left|\bar{\psi}_{\varepsilon}\left(\theta, \alpha^{\star}\right)-\bar{\psi}_\varepsilon\left(\theta^{\prime}, \alpha^{\prime}\right)\right| \leq q \bar{\psi}_\varepsilon\left(\theta, \alpha^{\star}\right) = q(T^\star_{\theta,\varepsilon})^{-1}\right .,
\end{equation}
for any $\alpha^\star \in\argmin_{\alpha \in C_\varepsilon^\star(\theta)}d_\infty(\alpha',\alpha)$. By the continuity properties of  $C^\star_\varepsilon(\theta)$, there exists a $g_2(q)>0$ such that for all $\theta'\in\mathbb{R}^d$ we have
$$
\|\theta - \theta'\| \leq g_2(q) \Rightarrow
\max_{\alpha'' \in C^\star_\varepsilon(\theta')}d_\infty(\alpha'',C^\star_\varepsilon(\theta)) \leq \frac{g_2(q)}{(K-1)}.
$$
Let $g(q) = \min\{g_1(q),g_2(q)\}$. Now we construct $T_0$ and an event $\mathcal{E}_T$ with $T\geq T_0$ under which for all $t\geq T$ we have 
$$
\|\hat{\theta}_t - \theta\|\leq g(q) \Rightarrow d_{\infty}\left(\left(N_{x,a}(t)/N_x(t)\right)_{(x,a)\in\mathcal{X} \times \mathcal{A}}, C_\varepsilon^{\star}(\alpha)\right) \leq  g_1(q).
$$
Define for $T\geq 1$ the events
\begin{align*}
\mathcal{E}_{1,T} & = \bigcap_{t = \ell(T)}^\infty   \{\|\theta- \hat{\theta}_t\|\leq g(q)\} 
\\ \mathcal{E}_{2, T} &=\bigcap_{t=T}^{\infty}\left\{\inf _{s \geq \ell(t)} d_{\infty}\left(\alpha(t), C_\varepsilon^{\star}\left(\hat{\theta}_{s}\right)\right) \leq \frac{g_{1}(q)}{4(K-1)}\right\} \\
& \subseteq \bigcap_{t=T}^{\infty}\left\{\exists s \geq \ell(t): d_{\infty}\left(\alpha(t), C_\varepsilon^{\star}\left(\hat{\theta}_{s}\right)\right) \leq \frac{g_{1}(q)}{2(K-1)}\right\}
\\  \mathcal{E}_{3,T} & = \bigcap_{t=T}^{\infty}\left\{ d_{\infty}\left(\left(N_{x,a}(t)/N_x(t)\right)_{(x,a)\in\mathcal{X} \times \mathcal{A}}, C_\varepsilon^{\star}(\theta)\right) \leq\left(z_{t}+d-1\right) \frac{g_{1}(q)}{K-1} \right\} \\ & \subseteq \bigcap_{t=T}^{\infty}\left\{ d_{\infty}\left(\left(N_{x,a}(t)/N_x(t)\right)_{(x,a)\in\mathcal{X} \times \mathcal{A}}, C_\varepsilon^{\star}(\theta)\right) \leq g_{1}(q) \right\} 
\\ \mathcal{E}_{4,T} & = \bigcap_{t=T}^{\infty}\left\{\sum_{s = 1}^t \phi_{x_s,a_s}\phi_{x_s,a_s}^\top \succeq c\sqrt{t} I_d \right\}
\end{align*}
Under the  $ \mathcal{E}_{1,T} \cap \mathcal{E}_{2,T}$, we have for all $t \geq T$, there exists $s\geq \ell(t)$ such that 
\begin{align*}
d_{\infty}\left(\alpha(t), C_\varepsilon^{\star}(\theta)\right) & \leq d_{\infty}\left(\alpha(t), C_\varepsilon^{\star}\left(\hat{\theta}_{s}\right)\right)+\max_{\alpha^{\prime} \in C_\varepsilon^{\star}\left(\hat{\theta}_{s}\right)} d_{\infty}\left(\alpha^{\prime}, C_\varepsilon^{\star}\left(\theta\right)\right) \\ &<\frac{g_{1}(q)}{2(K-1)}+\frac{g_{1}(q)}{2(K-1)}=\frac{g_{1}(q)}{K-1}.
\end{align*}
By lemma $3$, there exists a $t_1$ such that for $T\geq t_1$, the event 
$$
\left\{d_{\infty}\left(\left(N_{x,a}(t)/N_x(t)\right)_{(x,a)\in\mathcal{X} \times \mathcal{A}}, C_\varepsilon^{\star}(\theta)\right) \leq g_{1}(q)\right\},
$$
holds with probability at least $1-2 e^{-\frac{T\varepsilon^2}{4}}$. In particular we have
$q_1 = g_1(q)/(K-1)$ and $ t_1(q_1,\kappa) =\max\left\{\frac{1}{4c_1(\kappa) dq_1^3},\frac{T}{2c_1(\kappa)q_1^3},\frac{1}{c_1(\kappa)q_1^2}, \frac{7}{c_1(\kappa) q_1}\right\}.$ Hence for $T\geq \max\left\{  2q_1,14q_1^2,1/2d \right\}$ we have $t_1(q_1,\kappa) = \frac{T}{2 c_1 q_1^3}$. Hence, defining for $T\geq \lceil 1/(2c_1q_1^3)\rceil$, the event 
$$
\mathcal{E}_{1,\lceil 2c_1q_1^3T \rceil} \cap \mathcal{E}_{2,\lceil 2c_1q_1^3T \rceil} \cap \mathcal{E}_{3,\lceil 2c_1q_1^3T \rceil}
$$
we have shown that exists a $T_0$ such that for $T \geq T_0$% = \max\left\{a,v,\right\}$
, it holds that 
\begin{equation}
\label{eq:fact2}
    \forall t \geq T, \quad\left\|\theta-\hat{\theta}_{t}\right\| \leq g(q) \Longrightarrow d_{\infty}\left(\left(N_{x,a}(t)/N_x(t)\right)_{(x,a)\in\mathcal{X} \times \mathcal{A}}, C_\varepsilon^{\star}(\theta)\right)  \leq g_{1}(q) .
\end{equation}

Finally, combining the implication \eqref{eq:fact2} with the fact that \eqref{eq:fact1} holds under $\mathcal{E}_T$, we conclude that for $T \geq T_0$ we have 
\begin{equation}
\label{eq:inequality1_th3}
\bar{\psi}_\varepsilon\left(\hat{\theta}_t,\left(N_{x,a}(t)/N_x(t)\right)_{(x,a)\in\mathcal{X} \times \mathcal{A}}\right)\geq (1-q) \bar{\psi}_\varepsilon^\star(\theta).
\end{equation}


\textit{Step 2:} Now, by Lemma \ref{lem:forced_exploration}, we have that, for all $T\geq T_1(c)$, the event $\left\{\sum_{s = 1}^t \phi_{x_s,a_s}\phi_{x_s,a_s}^\top \succeq c\sqrt{t} I_d \right\}$ holds with probability at least $1-2 e^{-\frac{Tc^2}{4}}$, where $c$ is a constant independent of $\delta$. Now we note that for all $t\geq T_1$ we have  $Z_\varepsilon^x(t) \leq t \bar{\psi}_\varepsilon\left(\hat{\theta}_{t},\left(N_{x,a}(t)/N_x(t)\right)_{(x,a)\in\mathcal{X} \times \mathcal{A}}\right).$ Under the event $\mathcal{E}_T$ we have that \eqref{eq:inequality1_th3}, holds and we get
$$
Z_\varepsilon^x(t) \geq t(1-q)(T^\star_{\theta,\varepsilon})^{-1}.
$$
Hence, under $\mathcal{E}_T$, and for $T\geq \max\{T_0,T_1\}$, we get 
\begin{align*}
 \tau & =\inf \Big\{t \in \mathbb{N}^{*}: \forall x\in\mathcal{X}, Z_\varepsilon^x(t)>\beta(\delta, t) \text{ and } \sum_{s=1}^{t} \phi_{x_s,a_{s}}\phi_{x_s,a_{s}}^{\top} \succeq c I_{d}\Big\} \\& \leq \Big\{t: \forall x\in\mathcal{X}, Z_\varepsilon^x(t)>\beta(\delta, t) \Big\} \\& \leq T \lor \inf \Big\{t: \forall x\in\mathcal{X}, t(1-q)T^\star_{\theta,\varepsilon}>\beta(\delta, t) \Big\} \\& \leq T \lor \inf \Big\{t: \forall x\in\mathcal{X}, t(1-q) T^\star_{\theta,\varepsilon}>c_1\log(c_2t^\gamma/\delta)\Big\},
\end{align*}
where $k_1, k_2, \gamma$ appears in the definition of $\beta(\delta,t)$. Applying  \cite[Lemma 18]{Garivier16} leads to 
$$
\inf\Big\{t: \forall x\in\mathcal{X}, t(1-q)T^\star_{\theta,\varepsilon}>k_1\log(k_2t^\gamma/\delta)\Big\} \leq T_2(\delta),
$$
where $T_{2}^{\star}(\delta)=\frac{k_{1}}{1-q} T_{\theta,\varepsilon}^{\star} \log (1 / \delta)+o(\log (1 / \delta))$.
Hence, for $T\geq \max\{T_0,T_1,T_2^\star(\delta)\}$ we get $\mathcal{E}_T \subseteq \{\tau \leq T\}.$ Let $T_3^\star(\delta) = \max\{T_0,T_1,T_2^\star(\delta)\}$. Then for $T\geq T_3^\star(\delta)$ 
$$
\tau_{\delta} \leq \tau_{\delta} \wedge T_{3}^{\star}(\delta)+\tau_{\delta} \vee T_{3}^{\star}(\delta) \leq T_{3}^{\star}(\delta)+\tau_{\delta} \vee T_{3}^{\star}(\delta),
$$
and taking the expectation of the above inequality 
$$
\mathbb{E}[\tau_\delta] \leq T_{3}^{\star}(\delta)+\mathbb{E}[\tau_{\delta} \vee T_{3}^{\star}(\delta)]
$$
Now, note that
\begin{align*}
\mathbb{E}\left[\tau \vee T_{3}^{\star}(\delta)\right] &=\sum_{T=0}^{\infty} \mathbb{P}\left(\tau \vee T_{3}^{\star}(\delta)>T\right) \\
&=\sum_{T=T_{3}^{\star}(\delta)+1}^{\infty} \mathbb{P}\left(\tau \vee T_{3}^{\star}(\delta)>T\right) \\
&=\sum_{T=T_{3}^{\star}(\delta)+1}^{\infty} \mathbb{P}(\tau>T) \\
& \leq \sum_{T=T_{3}^{\star}(\delta)+1}^{\infty} \mathbb{P}\left(\mathcal{E}_{T}^{c}\right) \\
& \leq \sum_{T=T_{0} \vee T_{1}}^{\infty} \mathbb{P}\left(\mathcal{E}_{T}^{c}\right).
\end{align*}
Hence, we can conclude that 
$$\mathbb{E}[\tau] \leq \frac{k_{1}}{1-q} T_{\theta,\varepsilon}^{\star} \log (1 / \delta)+o(\log (1 / \delta))+T_{0} \vee T_{1}+\sum_{T=T_{0} \vee T_{1}}^{\infty} \mathbb{P}\left(\mathcal{E}_{T}^{c}\right).$$
\textit{Step 3:} The next step is to show that $\sum_{T=T_{0} \vee T_{1}}^{\infty} \mathbb{P}\left(\mathcal{E}_{T}^{c}\right) < \infty$ and it can be upper-bounded by a universal constant independent of $\delta$. We observe that there exists a $h(g_1(q))/4(K-1)>0$, $y>0$ such that for $T_0 \vee T_{1}$, 
\begin{align*}
\mathbb{P}\left(\mathcal{E}_{1,\left\lceil 2 c_1  q_{1}^{3} T \right\rceil}^{c}\right) & \leq \sum_{t=\left\lceil 2 c_1  q_{1}^{3} T \right\rceil}^{\infty} \mathbb{P}\left(\inf _{s \geq \ell(t)} d_{\infty}\left(\alpha(t), C^{\star}\left(\hat{\theta}_{s}\right)\right)>\frac{g_{1}(q)}{4(K-1)}\right) \\
& \leq h\left(\frac{g_{1}(q)}{4(K-1)}\right) \sum_{t=\left\lceil 2 c_1  q_{1}^{3} T \right\rceil}^{\infty} \frac{1}{t^{2+y}} \\
& \leq h\left(\frac{g_{1}(q)}{4(K-1)}\right) \int_{\left\lceil 2 c_1  q_{1}^{3} T \right\rceil-1}^{\infty} \frac{1}{t^{2+y}} d t \\
& \leq h\left(\frac{g_{1}(q)}{4(K-1)}\right) \frac{1}{(1+y)\left(\left\lceil 2 c_1  q_{1}^{3} T \right\rceil-1\right)^{1+y}}.
\end{align*}
Hence 
$$
\mathbb{P}\left(\mathcal{E}_{T}^{c}\right) \leq \mathbb{P}\left(\mathcal{E}_{1,\left\lceil 2 c_1  q_{1}^{3} T \right\rceil}^{c}\right) + \mathbb{P}\left(\mathcal{E}_{1,\left\lceil 2 c_1  q_{1}^{3} T \right\rceil}^{c}\right) \leq 2  h\left(\frac{g_{1}(q)}{4(K-1)}\right) \frac{1}{(1+y)\left(\left\lceil 2 c_1  q_{1}^{3} T \right\rceil-1\right)^{1+y}} \Rightarrow \sum_{T=T_{0} \vee T_{1}}^{\infty} \mathbb{P}\left(\mathcal{E}_{1,\left\lceil 2 c_1  q_{1}^{3} T \right\rceil}^{c}\right)<\infty.
$$
Second, we observe, using a union bound, and Lemma \ref{lem:LS_concentration}, that there exists strictly positive constants $c_3, c_4$ independent of $q$ and $T$, and such that
\begin{align*}
\mathbb{P}\left(\mathcal{E}_{2,\left\lceil 2 c_1  q_{1}^{3} T \right\rceil}^{c}\right) & \leq \sum_{t=\ell\left(\left\lceil 2 c_1  q_{1}^{3} T \right\rceil\right)}^{\infty} \mathbb{P}\left(\left\|\theta-\hat{\theta}_{t}\right\|>g(q)\right)\\
& \leq c_{3} \sum_{t=\ell\left(\left\lceil 2 c_1  q_{1}^{3} T \right\rceil\right)}^{\infty} t^{d/4} \exp \left(-c_{4} g(q)^{2} \sqrt{t}\right).
\end{align*}
For $t$ large enough, we have that the function $t \mapsto t^{d/4} \exp \left(-c_{4} g(q)^{2} \sqrt{t}\right)$ is decreasing. Also, since $(\ell(t))_{t\geq1}$ is non-decrasing, and $\lim_{t\to\infty}\ell(t) = \infty$, we may find $T_2\geq T_0 \lor T_1$ such that for all $t\geq T_2$ we have that $t \mapsto t^{d/4} \exp \left(-c_{4} g(q)^{2} \sqrt{t}\right)$ is decreasing on $[\ell(\varepsilon_1 T)-1,\infty)$. Thus for $T\geq T_2$, we get
$$
\mathbb{P}\left(\mathcal{E}_{2,\left\lceil 2 c_1  q_{1}^{3} T \right\rceil}^{c}\right) \leq c_{3} \int_{\ell\left(\left\lceil 2 c_1  q_{1}^{3} T \right\rceil\right)-1}^{\infty} t^{d / 4} \exp \left(-c_{4} g(q)^{2} \sqrt{t}\right) d t.
$$
Furthermore, for some $T_3 \geq T_2$ large enough, we may bound the integral for all $T \geq T_3$ as follows
$$
\int_{\ell\left(\left\lceil 2 c_1  q_{1}^{3} T \right\rceil\right)-1}^{\infty} t^{d / 4} \exp \left(-c_{4} g(q)^{2} \sqrt{t}\right) d t \lesssim \frac{\ell\left(\left(\left\lceil 2 c_1  q_{1}^{3} T \right\rceil\right)-1\right)^{d / 2+1}}{g(q)^{4} \exp \left(c_{4} g(q)^{2} \sqrt{\ell\left(\left\lceil 2 c_1  q_{1}^{3} T \right\rceil\right)-1}\right)}.
$$
Now the condition 
$$
\mathbb{P}\left(\mathcal{E}_{2,\left\lceil 2 c_1  q_{1}^{3} T \right\rceil}^{c}\right) \lesssim \frac{\ell\left(\left(\left\lceil 2 c_1  q_{1}^{3} T \right\rceil\right)-1\right)^{d / 2+1}}{g(q)^{4} \exp \left(c_{4} g(q)^{2} \sqrt{\ell\left(\left\lceil 2 c_1  q_{1}^{3} T \right\rceil\right)-1}\right)} \lesssim \frac{T^{d / 2+1}}{\exp \left(c_{5}(\varepsilon) T^{\gamma / 2}\right)}
$$
This show that 
\begin{align*}
\sum_{T=T_{0} \vee T_{1}}^{\infty} \mathbb{P}\left(\mathcal{E}_{2,\left\lceil 2 c_1  q_{1}^{3} T \right\rceil}^{c}\right) &=\sum_{T=T_{0} \vee T_{1}}^{T_{4}} \mathbb{P}\left(\mathcal{E}_{2,\left\lceil 2 c_1  q_{1}^{3} T \right\rceil}^{c}\right)+\sum_{T=T_{4}+1}^{\infty} \mathbb{P}\left(\mathcal{E}_{2,\left\lceil 2 c_1  q_{1}^{3} T \right\rceil}^{c}\right) \\
& \lesssim \sum_{T=T_{0} \vee T_{1}}^{T_{4}} \mathbb{P}\left(\mathcal{E}_{2,\left\lceil 2 c_1  q_{1}^{3} T \right\rceil}^{c}\right)+\sum_{T=T_{4}+1}^{\infty} \frac{T^{d / 2+1}}{\exp \left(c_{5}(\varepsilon) T \gamma / 2\right)} \\
&<\infty
\end{align*}
where the last inequality follows from the fact that we can upper bound the infinite sum by a Gamma function, which is convergent as long as 
$\gamma > 0$.
Hence we can conclude that 
$$
\sum_{T=T_{0} \vee T_{1}}^{\infty}\mathbb{P}\left(\mathcal{E}_{T}^{c}\right) \leq \sum_{T=T_{0} \vee T_{1}}^{\infty} \mathbb{P}\left(\mathcal{E}_{1,\left\lceil 2 c_1  q_{1}^{3} T \right\rceil}^{c}\right)+\mathbb{P}\left(\mathcal{E}_{1,\left\lceil 2 c_1  q_{1}^{3} T \right\rceil}^{c}\right) \leq \infty.
$$

We have shown that 
$$
\mathbb{E}[\tau] \leq \frac{k_{1}}{1-\varepsilon} T_{\theta,\varepsilon}^{\star} \log (1 / \delta)+o(\log (1 / \delta))+T_{0} \vee T_{1}+\sum_{T=T_{0} \vee T_{1}}^{\infty} \mathbb{P}\left(\mathcal{E}_{T}^{c}\right),
$$
where $\sum_{T=T_{0} \vee T_{1}}^{\infty}\mathbb{P}\left(\mathcal{E}_{T}^{c}\right)$ is independent of $\delta$.
Hence, 
$$
\limsup _{\delta \rightarrow 0} \frac{\mathbb{E}\left[\tau_{\delta}\right]}{\log (1 / \delta)} \leq \frac{k_{1}}{1-q} T_{\theta,\varepsilon}^{\star}.
$$
By Letting $q\to 0$, we get the result.
\end{proof}


==> INFOCOM 2021 - FinalSubmission/Sections/RelatedWork.tex <==
\section{Previous Work}
\label{sec:previous_work}
\subsection{Contextual Linear Bandits}
Recently, CL-MAB have received considerable attention in the active learning setting for regret minimization \cite{Chu11, Li10, Hao20}. There, the learner aims at minimizing her cumulative regret over a given time horizon. To the best of our knowledge, this paper is the first to analyze and solve the BPI problem in CL-MAB. Closely related work include Best Arm Identification (BAI) in the Linear Bandit (LB) setting without contexts \cite{Soare15, Jedra20, Fiez19}. The BAI problem in the LB setting was initially studied by Soare et al. \cite{Soare15}, that proposes an instance-specific lower bound on the sample complexity as the solution of a max-min optimization problem, and algorithms based on approximations of this optimization problem. Jedra and Proutiere \cite{Jedra20} propose an algorithm whose sampling complexity matches the lower bounds, asymptotically almost surely and in expectation. However, the LB framework is not flexible enough to model more complex applications that require contextual side information. 

\subsection{Antenna Tilt Optimization}
There has been a considerable amount of work in the area of antenna tilt optimization. Recent methods are mainly based on the use of Reinforcement Learning (RL) \cite{Guo13, Balevi19, Vannella21, Dreifuerst21, EricssonMobility}, Contextual Bandits (CBs), \cite{Vannella20} or MABs \cite{Cai10, Gulati14, Dhahri17, Shen18}. Remarkably, RL methods have been actually implemented in real networks and performance gains have been observed \cite{EricssonMobility}. However, the aforementioned papers focus on regret minimization or on identifying an efficient tilt update policy without any consideration for the number of samples used to do so. We should also mention that most existing studies (see e.g, \cite{Vannella20}) investigate off-policy learning problems which correspond to our passive learning setting. Since the proposed methods there do not include any stopping rule, the algorithms may actually stop much before they have collected enough data to learn an optimal policy with reasonable confidence. The way we formulate our BPI problem circumvents this difficulty.  

==> INFOCOM 2021 - FinalSubmission/Sections/deleted_text.tex <==
\begin{comment}
\begin{lemma}[Properties of the optimization problem]
Assume $a^\star_\theta(x)$ is unique $\forall x\in\mathcal{X}$, and
define $\psi(\theta,\alpha) = \sup_{\alpha \in \Lambda}\min_{x \in \mathcal{X}, a \in \mathcal{A}\backslash\lbrace a_\theta^\star(x) \rbrace} \frac{ (\theta^\top \gamma_{x, a})^2}{2\gamma_{x,a}^\top A(\alpha)^{-1} \gamma_{x,a}}$. Then $\psi$ is continuous in $\theta$ and $\alpha$, and $\alpha \mapsto \psi(\theta,\alpha)$ is concave and attains its maximum at a point $\alpha^\star\in\Lambda$ such that $A(\alpha^\star) \succ 0$.
\end{lemma}

Previous works \cite{Fiez19,Jedra20} use Frank-Wolfe type of algorithms to solve the problem of the optimal allocations in \eqref{eq:lb_delta}. We note that the problem of deriving the optimal allocation is a convex optimization problem since $h(\alpha) = \max\limits_{x \in \mathcal{X}}\max\limits_{a \in \mathcal{A}\setminus\{a^\star_\theta(x)\}} \frac{2\gamma_{x,a}^\top A(\alpha)^{-1} \gamma_{x,a}}{(\theta^\top
\gamma_{x,a})^2}$ is a maximum of convex functions, and hence is convex.
Thus, the optimal allocation problem corresponds to solve $\inf \limits_{\alpha \in \Lambda} h(\alpha)$, or equivalently: 
\begin{equation*}
    \begin{aligned} 
    \inf_{z,\alpha} \;& z
    \\\text{ s.t. } & z \geq \frac{2\gamma_{y,b}^\top A(\alpha)^{-1} \gamma_{y,b}}{(\theta^\top
    \gamma_{y,b})^2}, \;\; \forall y\in\mathcal{X}, \forall b \in\mathcal{A}\setminus\{a^\star_\theta(y)\} \\ &
    \mathbf{1}^{\top}\alpha = 1,
    \\& 0\preceq \alpha \preceq  1.
    \end{aligned}
\end{equation*}
\end{comment}

%for some $\alpha \in \Lambda$ and for all $t\geq 1$. Hence, an algorithm in the passive learning setting only accounts for devising $(\tau, \hat{a}_\tau)$. Note that since we do not control the sampling rule, it may not be possible to learn the best policy exactly. In this case, we focus on identifying the best learnable policy on a subset of $\mathbb{R}^d$. Let $U \subseteq \mathbb{R}^d$ and denote by $U^\perp = \left\{v \in \mathbb{R}^d : v \cdot u = 0,\; \forall u \in U\right\}$, the orthogonal complement of $U$. By the orthogonal decomposition Theorem we have that $\mathbb{R}^d = U \oplus U^\perp$, and each $\theta\in \mathbb{R}^d$ can be uniquely written as a sum $\theta = \tilde{\theta} + \theta_\perp$, where $\tilde{\theta} \in U$ and $\theta_\perp \in U^\perp$. We define the orthogonal projection operator $\text{proj}_U(\cdot):\mathbb{R}^d \to U$ such that for all $\theta \in \mathbb{R}^d$, $\text{proj}_U(\theta) = \tilde{\theta}$. We may define the \textit{projected reward} $\tilde{R}_t = \tilde{\theta}^{\top}\phi_{X_t,A_t} + \xi_t$ and the \textit{projected best arm} for context $x$ as $a^\star_{\tilde{\theta}}(x) = \argmax_{a\in\mathcal{A}} \tilde{\theta}^{\top}\phi_{x,a}$. Intuitively, $U$ may be thought as a subspace of $\mathbb{R}^d$ on which it is possible to learn a PAC algorithm. 

%In the passive learning case, we focus on identifying the best learnable policy on a subset of $\mathbb{R}^d$. Let $U \subseteq \mathbb{R}^d$ and denote by $U^\perp = \left\{v \in \mathbb{R}^d : v \cdot u = 0,\; \forall u \in U\right\}$, the orthogonal complement of $U$. By the orthogonal decomposition Theorem we have that $\mathbb{R}^d = U \oplus U^\perp$, and each $\theta\in \mathbb{R}^d$ can be uniquely written as a sum $\theta = \tilde{\theta} + \theta_\perp$, where $\tilde{\theta} \in U$ and $\theta_\perp \in U^\perp$. We define the orthogonal projection operator $\text{proj}_U(\cdot):\mathbb{R}^d \to U$ such that for all $\theta \in \mathbb{R}^d$, $\text{proj}_U(\theta) = \tilde{\theta}$. We may define the \textit{projected reward} $\tilde{R}_t = \tilde{\theta}^{\top}\phi_{X_t,A_t} + \xi_t$ and the \textit{projected best arm} for context $x$ as $a^\star_{\tilde{\theta}}(x) = \argmax_{a\in\mathcal{A}} \tilde{\theta}^{\top}\phi_{x,a}$. Intuitively, $U$ may be thought as a subspace of $\mathbb{R}^d$ on which it is possible to learn a PAC algorithm. 

%Theorem \ref{theorem:off_policy_lb} ensures that if $U \subseteq \mathcal{R}(A(\alpha))$ then $U$ is PAC-learnable. In particular, it implies that the maximal PAC-learnable set is achieved for $U = \mathcal{R}(A(\alpha))$, i.e., $\forall B\subseteq \mathbb{R}^d$ if $U = B$ is PAC-learnable and $\mathcal{R}(A(\alpha)) \subseteq B$, then $B = \mathcal{R}(A(\alpha))$. Similarly to Remark \ref{rem:delta_pac}, we can derive a lower bound for $(U,0,\delta)-$PAC policies. %Thus we conclude that the best choice is $U = \mathcal{R}(A(\alpha))$. 
\begin{lemma}[Convergence of $\alpha(t)$ to $C_\varepsilon^\star(\alpha)$]
\label{lem:convergence_C_star}
    Let $(l(t))_{t\geq 1}$ a non-decreasing sequence of integers such that $l(1) = 1$, $l(t-1) \leq t-1$ for $t > 1$, $\lim_{t\to \infty} l(t) = \infty$, and $\lim_{t\to\infty}\min_{s\geq l(t)} d_\infty(\alpha(t),C_\varepsilon^\star(\hat{\theta}_s)) = 0$ a.s. 
    Then under sampling rule \eqref{eq:sampling_rule_force}, \eqref{eq:sampling_rule_track} we have
    $$
    \lim_{t\to\infty} d_\infty(\alpha(t),C_\varepsilon^\star(\theta)) = 0 \quad \text{a.s.}
    $$
\end{lemma}

The following Lemma show that the optimization problem in \eqref{eq:eps_delta_equivalent_lb} satisfies a set of convenient properties.
\begin{lemma}[Properties of the optimization problem]
\label{lem:properties_eps_delta}Let $\psi_{\varepsilon}(\theta,\alpha) =  \inf_{\mu \in B_\varepsilon(\theta)}\frac{1}{2}\|\mu-\theta\|^2_{A(\alpha)}$, and $C_\varepsilon^\star(\theta) = \argsup_{\alpha \in \Lambda} \psi_\varepsilon(\theta,\alpha)$.  For any $\varepsilon\geq 0$, we have
\begin{enumerate}
    \item $\psi_\varepsilon$ is continuous in $\theta$ and $\alpha$,
    \item $\exists \; \alpha^\star \in C^\star_\varepsilon(\theta)$ such that $A(\alpha^\star) \succ 0$,
    \item $\psi_{\varepsilon}^\star$ is continuous in $\theta$,
    \item $C_\varepsilon^\star(\theta)$ is convex, compact and upper hemicontinuous. 
\end{enumerate}
\end{lemma}

\begin{comment}
\begin{lemma}[Closed-form solution of $Z^x_{a,b,\varepsilon}$ \cite{Jedra20}]
\label{lem:closed_form_Z}
Let $t\geq 1$ and $\sum_{s = 1}^t \phi_{x_s,a_s}\phi_{x_s,a_s}^\top \succ 0$. Then for for all $x \in\mathcal{X}$, $(a,b) \in\mathcal{A}^2: a\neq b$, we have
\begin{equation*}
    Z^x_{a, b, \varepsilon}(t)=\operatorname{sgn}\left(\hat{\theta}_{t}^{\top}\gamma^x_{a,b}+\varepsilon\right) \frac{\left(\hat{\theta}_{t}^{\top}\gamma^x_{a,b}+\varepsilon\right)^{2}}{2\|\gamma^x_{a,b}\|_{(\sum_{s=1}^{t} \phi_{x_s,a_s} \phi_{x_s,a_s}^{\top})^{-1}}}.
\end{equation*}
\end{lemma}
\end{comment}

\begin{comment}
Define $Z_\varepsilon^x(t) = \min_{\{b \in \mathcal{A}:|\hat{\theta}_t^\top(\phi_{x,\hat{a}_t(x)} - \phi_{x,b})| \geq \varepsilon\}} Z^x_{\hat{a}_t(x), b,\varepsilon}(t)$. The stopping time is 
\begin{align}
\begin{split}
    \tau =\inf \Bigg\{t \in \mathbb{N}^{*}: \forall x\in\mathcal{X}, Z_{\varepsilon}^x(t)>\beta(\delta, t) \text{ and } A_t \succeq \max \Bigg\{c, \frac{\rho(\delta, t)}{\|\hat{\theta}_{t}\|^{2}}\Bigg\}\Bigg\},
\end{split}
\label{eq:stopping_rule_eps_delta_pac}
\end{align}
where $\beta(\delta,t)$, and $\rho(\delta,t)$ are exploration thresholds defined in \eqref{eq:expl_rate_eps_delta_pac} and $c>0$. %With respect to the $\delta$-PAC case, we impose the additional condition $\min_{b\in O^c_\varepsilon(\theta,x)} \tilde{\theta}_t(\phi_{x,\hat{a}_t} - \phi_{x,b})$. 
The following Lemma provides a sufficient condition on the stopping rule of any $(\varepsilon,\delta)$-PAC algorithm. 
\begin{lemma}[Stopping rule $(\varepsilon,\delta)$-PAC]
\label{lem:stopping_rule_eps_delta_pac}
Let $\left(\delta_{t}\right)_{t \geq 1},\left(\varepsilon_{t}\right)_{t \geq 1}$ be two sequences with values in $(0,1)$ and $(0, \varepsilon)$, respectively, and such that $\sum_{t=1}^{\infty} \delta_{t}\leq \delta$, and $\lim _{t \rightarrow \infty} \varepsilon_{t}=\varepsilon .$ Let $\zeta_{t}=\log \left(2 \operatorname{det}\left(c^{-1} \sum_{s=1}^{t}\phi_{x_s,a_{s}} \phi_{x_s,a_{s}} ^{\top}+I_{d}\right)^{\frac{1}{2}}\right)-\log \left(\delta_{t}\right)$, and define:
\begin{equation}
\beta(\delta, t)=2 \zeta_{t} \quad \text { and } \quad \rho(\delta, t)=\frac{4  \varepsilon_{t}^{2} \zeta_{t}}{\left(\varepsilon-\varepsilon_{t}\right)^{2}}
\label{eq:expl_rate_eps_delta_pac}
\end{equation}
Under any sampling rule, and stopping rule \eqref{eq:stopping_rule_eps_delta_pac} with exploration threshold \eqref{eq:expl_rate_eps_delta_pac}, we have:
     $$\mathbb{P}_{\theta}\left(\exists x\in \mathcal{X}: \theta^\top (\phi_{x,a^\star_\theta(x)} - \phi_{x,\hat{a}_\tau(x)}) >\varepsilon, \tau <\infty\right)\leq\delta.$$
\end{lemma}
\end{comment}

\begin{comment}
\subsubsection{Discretized continuous contexts}
We consider a synthetic example of LCB-BPI problem with continuous context. We consider a uniform distribution $p_\mathcal{X} = \mathcal{U}(\mathcal{X})$ over $\mathcal{X} = [-1,1]$, with two actions $\mathcal{A} = \{a_1,a_2\}$. The feature vectors are specified as
$\phi_{x,a_1} = [1,x]$, $\phi_{x,a_2} = [1,-x]$,
$\theta = [1,1/2]$. Figure \ref{fig:continuous} shows the expected rewards and the gap $\Delta(x,\varepsilon) = |\theta^\top(\phi_{x,a_1} - \phi_{x,a_2})|$. In the $(\varepsilon,\delta)$-PAC setting, the goal is to learn the best policy on  $X_\varepsilon =  \mathbbm{1}\{|\theta^\top(\phi_{x,a_1}-\phi_{x,a_2})| > \varepsilon\}$, as shown in Figure \ref{fig:continuous}. 
\begin{figure}
    \centering
    \includegraphics[width = 7.5cm]{Figures/continuous.png}
    \caption{LCB instance in the continuous-context setting.}
    \label{fig:continuous}
\end{figure}
For each experiment, we report the theoretical lower bound on the sample complexity and the empirical sample complexity. The empirical quantities are reported in terms of mean and standard deviation, taken over $N_{\text{sim}} = 200$ Monte-Carlo runs with $\mathcal{X}$ discretized in $C = 10^{3}$ bins. For the passive learning setting we report results for the \textit{deterministic sampling rule}, selecting action $a_t(x) = a_1$, for all $x\in\mathcal{X}$, and the \textit{random sampling rule} selecting action $a_i$ with probability $\alpha_{x,a_1} = 1/2$, $\forall x \in \mathcal{X}$. For the active learning setting we report the results with the adaptive sampling rule.

\begin{table}[ht!]
\fontsize{9.3}{9.3}\selectfont
\centering
\caption{BPI results for the continuous-context example.}
\begin{tabular}{clrr}\toprule
Sampling rule & Parameter & Lower bound & Sample complexity  \\ \hline \hline
\multirow{3}{*}{Deterministic} 
& $\varepsilon= 0.10$  & $417.54$ & $504.34 \pm 165.87$ \\ & $\varepsilon = 0.05$ & $610.52$ & $583.33 \pm 111.06$\\ & $\varepsilon = 0.01$ & $610.52$ & $583.33 \pm 111.06$ \\ \hline 
\multirow{3}{*}{Random} 
& $\varepsilon= 0.10$  & $65.63$ & $234.05 \pm 48.04$\\ & $\varepsilon = 0.05$ & $193.30$ & $316.89\pm85.42$ \\ & $\varepsilon = 0.01$ & $610.52$ & $583.33 \pm 111.06$\\\hline  
\multirow{3}{*}{Adaptive} 
& $\varepsilon= 0.10$ & $65.63$ & $234.05 \pm 48.04$ \\ 
& $\varepsilon = 0.05$ & $193.30$ & $316.89\pm85.42$\\ & $\varepsilon = 0.01$ & $610.52$ & $583.33 \pm 111.06$\\ \bottomrule
\end{tabular} 
\label{tab:results_continuous}
\end{table}
\subsubsection{$(U,\delta)$-PAC synthetic example} 
\end{comment}

\begin{comment}
\begin{table}[ht!]
\fontsize{9.3}{9.3}\selectfont
\centering
\caption{Experimental results for the $3$-KPIs experiments.}
\begin{tabular}{clll}\hline 
Sampling Rule & Parameter & Lower bound & Sample complexity  \\ \hline 
\multirow{3}{*}{Rule-Based} 
& $\varepsilon= 0.10$  & $64.91$ & $456.55\pm 149.61$  \\ & $\varepsilon = 0.05$ & $259.11$ & $1887.22\pm 
472.71\pm142.93$  \\ & $\varepsilon = 0.025$ & $1531.47$ & $2384.03 \pm 313.01$  \\
\hline 
\multirow{3}{*}{Random} 
& $\varepsilon= 0.10$  & $69.40$ & $240.58\pm92.75$  \\ & $\varepsilon= 0.05$  & $231.69$ & $494.55 \pm 89.89$ \\ & $\varepsilon = 0.025$ & $1487.28$ & $1557.50\pm332.48$  \\ \hline
\end{tabular} 
\label{tab:results}
\end{table}
    \begin{table}[ht!]
\fontsize{9.3}{9.3}\selectfont
\centering
\caption{Experimental results for the $2$-KPIs experiments}
\begin{tabular}{llllll}\hline
Parameter & Lower bound & Sample complexity & BPI error & DM error & IPS error \\ \hline 
$\varepsilon = 0.20$ & $515.70$ & $744\pm228.43$ & $0.04 \pm 0.20$ & $0.10\pm 0.05$ & $0.17\pm 0.32$ \\
$\varepsilon = 0.15$ & $855.26$ & $1291.79\pm 289.09$ & $0.05 \pm 0.23$ & $0.12 \pm 0.05$ &  $0.16\pm 0.28$  \\
$\varepsilon= 0.10$ & $1276.13$ & $2766.48 \pm 416.02$  & $0.09 \pm 0.03$ &  $0.19\pm 0.25$ \\ \hline 
\end{tabular} 
\label{tab:results}
\end{table}
\end{comment}

%\textit{The lower bounds and the sample complexity for the active learning setting are lower than the ones for the passive setting}. This is to be expected since (i) the algorithm in the active setting adapts its proportions to $\hat{\alpha}_t$, and hence is supposed to achieve a sample complexity matching $T^\star_{\varepsilon,\theta}\log(1/\delta)$, and (ii) in our experiments $U = \mathbb{R}^d$ for both the random and the rule-based sampling rules. In fact, with our formulation, and when the context space is large, it is easy to ensure that $U = \mathbb{R}^d$. In particular, it is sufficient to have $\exists a \in \mathcal{A}$ and $\exists x_1,x_2,x_3 \in\mathcal{X}$ such that $p_\mathcal{X}(x_i)\alpha_{x_i,a} >0$, for $i = 1,2,3$. In our case, both the random and rule-based sampling rules satisfy this condition.

%\textit{The lower bounds and sample complexity for the random policy is lower than the one for the rule-based policy}. This may be imputed to the increased exploration ability of the random sampling rule compared to the rule-based one, resulting in faster identification of the best policy. We may also observe that, for the purpose of identifying the best antenna tilt update policy, the sample complexity achieved by the random policy is close to the one. 

%\textit{The sample complexity for all sampling rules match the lower bounds on the sample complexity up to a constant}. This show that the proposed algorithms matches the lower bounds and achieve good performance for the task of best policy identification. 

% By Lemma \ref{lem:forced_exploration}, there exists $t_1 \geq 0$ such that for all $t\geq t_1$, we have $ \sum_{s = 1}^t \phi_{x_s,a_s}\phi_{x_s,a_s}^\top \succeq c I_d$ with probability at least $1-2e^{-c^2t/4}$. This implies that for all $t \geq \max \{t_0,t_1\}$ we have 

%\begin{remark}[Alternative sampling rule]
%An alternative sampling strategy would be
%$$
%    a_{t+1}(x) =\left\{\begin{array}{ll}
%    d_{t}(x) & \text { if } \quad \sum_{s = 1}^t\phi_{x_s,a_s}\phi_{x_s,a_s}^\top \mathbbm{1}_{\{x_s = x\}}\succeq f_x(t) \\
%    \argmax\limits_{\tilde{a}_x \in\tilde{\mathcal{A}}_x}\lambda_{d_x}\left( \sum_{s = 1}^t \phi_{x_s,a_s}\phi_{x_s,a_s} + \phi_{x,\tilde{a}_x}\phi_{x,\tilde{a}_x}^\top \right) & \text { otherwise }
 %   \end{array} \right.
%$$
%This way, the forced exploration step would ensure that the feature vector leading to the maximum growth of the minimum eigenvalue is selected and would not require to keep track of indices for each context.  
%\end{remark}

%The result in Lemma \ref{lem:forced_exploration} implies that $\lim\inf_{t \to \infty }\lambda_{1}\left( \frac{1}{\sqrt{t}} \sum_{s = 1}^t (\phi_{x_s,a_s}\phi^\top_{x_s,a_s})\right) > 0$ a.s., and hence the sufficient condition on the convergence of the LS estimator is satisfied under the sampling rule \eqref{eq:sampling_rule_force}. 

%\begin{figure}
%    \centering
%     \includegraphics[width=\columnwidth]{figures/antenasv2.eps}
%     \caption{Abstract representation of the mobile network environment.}
%     \label{fig:env}
%\end{figure}

%\inf_{{\left\lbrace \mu\in\mathbb{R}^d: \exists x \in \mathcal{X}, \forall a \in \mathcal{A}_\varepsilon(\theta,x), \; \mu^{\top}(\phi_{x,a_{\mu}^\star(x)}- \phi_{x,a})>\varepsilon \right\rbrace}}

$$
    r^\theta_{s,t} = \theta^\top \phi_{x_{s,t},a_{s,t}}. 
$$
$$
    \phi_{s,t} = x_{s,t} \otimes a_{s,t}
$$
$$
    \theta = \left(\sum_{s = 1}^S \sum_{k = 1}^t \phi_{x_{s,k},a_{s,k}}\phi_{x_{s,k},a_{s,k}}\right)^\dagger \sum_{s = 1}^S \sum_{k = 1}^t\phi_{x_{s,k},a_{s,k}}p_{s,k}.
$$
$$
    p_{s,t} = w_\text{BC}(R_\text{BC}(s,t) -R_\text{BC}(s,t+1)) + w_\text{OS}(N_\text{OS}(s,t) -N_\text{OS}(s,t+1))
$$


% In fact, the LCB problem may be seen as a LB with time varying action space. %of the optimization problem involved, their algorithm is not easy to generalize to the contextual case when the number of context is large. 

  % T_{{\theta},\varepsilon}(\alpha) = \max\limits_{x\in \mathcal{X}} \max  \limits_{a\notin \mathcal{A}_\varepsilon({\theta},x)}\max\limits_{b\in \mathcal{A}_\varepsilon({\theta},x,a)} \frac{2 \|\gamma_{a,b}^x\|^2_{ (A(\alpha))^{\dagger}}}{ ({\theta}^\top\gamma_{a,b}^x+\varepsilon)^2}.
  
  %Z^x_{a, b, \varepsilon}(t)=\log \left(\frac{\max_{\left\{\mu: \mu^{\top}(\phi_{x,a}-\phi_{x,b}) \geq -\varepsilon\right\}} \prod_{s=1}^t f_{x_s,a_s}^{\mu}(r_s)}{\max _{\left\{\mu:\mu^{\top}(\phi_{x,a}-\phi_{x,b}) \leq -\varepsilon \right\}} \prod_{s=1}^t f_{x_s,a_s}^{\mu}(r_s) }\right). 
  
  
\subsection{Passive setting algorithm}
Define 
{\begin{equation*}
Z^x_{U,a, b, \varepsilon}(t)=\log \left(\frac{\max_{\left\{\mu \in U : \mu^{\top}\gamma_{a,b}^x \leq \varepsilon\right\}} \prod_{s=1}^t f_{x_s,a_s}^{\mu}(r_s)}{\max_{\left\{\mu \in U :\mu^{\top}\gamma_{a,b}^x \geq \varepsilon \right\}} \prod_{s=1}^t f_{x_s,a_s}^{\mu}(r_s)}\right).
\end{equation*}}
We can express $Z^x_{U,a, b, \varepsilon}(t)$, for $t$ such that $\lambda_1\left(P A_t P^\top\right) >0$, as 
$$Z^x_{U,a,b,\varepsilon} = \operatorname{sgn}\left(\hat{\theta}_{U,t}^{\top}(P\gamma^x_{b,a})+\varepsilon\right) \frac{\left(\hat{\theta}_{U,t}^{\top}(P\gamma^x_{b,a})+\varepsilon\right)^{2}}{2\|P \gamma^x_{b,a}\|_{(P^T A_tP)^{-1}}},$$
where $\hat{\theta}_{U,t} = \left(P A_t P^\top\right)^{-1} \left(P \sum_{s = 1}^T \phi_{x_s,a_s}r_s \right)$. The decision rule for the passive learning setting is defined as 
\begin{equation}
\label{eq:recommendation_rule}
    \hat{a}_\tau(x) = \argmax_{a \in \mathcal{A}_\varepsilon(\hat{\theta}_{U,\tau},x)} \min_{b \neq a} Z^x_{U,a, b, \varepsilon}(\tau), \quad \forall x\in\mathcal{X}.
\end{equation}
Define $Z_{U,\varepsilon}^x(t) = \max_{a \in \mathcal{A}_\varepsilon(\hat{\theta}_{U,\tau},x)} \min_{b \neq a} Z^x_{U, a, b, \varepsilon}(t)$. The stopping time is 
\begin{align}
\begin{split}
    \tau =\inf \Big\{t: \forall x\in\mathcal{X}, Z_{U,\varepsilon}^x(t)>\beta_U(\delta, t) \text{ and } P A_t P^\top \succeq c I_{r}\Big\},
\label{eq:stopping_rule_eps_delta_pac}
\end{split}
\end{align}

\begin{lemma}
\label{lem:stopping_rule_eps_delta_pac_passive}
Let $u>0$, and define the exploration threshold
\begin{equation}
    \label{eq:expl_rate_eps_delta_pac}
        \beta_U(\delta, t) = (1+u) \log \left(\frac{\operatorname{det}\left((uc)^{-1}  P A_t P^\top+I_{r}\right)^{\frac{1}{2}}}{\delta}\right).
\end{equation}
\noindent Under the stopping rule defined by
\eqref{eq:stopping_rule_eps_delta_pac}--\eqref{eq:expl_rate_eps_delta_pac} and under any sampling rule satisfying the hypotheses of Corollary \ref{cor:LS_concentration_passive}, we have
     $$\mathbb{P}_{\theta}\left(\exists x\in \mathcal{X}: \theta^\top (\phi_{x,a^\star_\theta(x)} - \phi_{x,\hat{a}_\tau(x)}) >\varepsilon, \tau <\infty\right)\leq\delta.$$
\end{lemma}


\begin{corollary}
    \label{cor:LS_concentration_passive}
    Let $\theta \in U$, and assume the sampling rule satisfies $\lim\inf_{t \to \infty }\lambda_{1}\left(\frac{1}{t^\alpha}(P A_t P^\top)\right) > 0$ a.s. for some, $\alpha\in(0,1)$. Then $\lim_{t \to \infty} \hat{\theta}_t = \theta $. In particular, for all $\beta \in (0,\alpha/2)$, 
   $ \|\hat{\theta}_t - \theta\| = o\left(t^{-\beta}\right)$ a.s.
\end{corollary}

\begin{comment}
\subsection{Algorithm}
The optimal allocation problem is a convex program since $h(\alpha) = \max\limits_{x \in \mathcal{X}, a \in \mathcal{A}\setminus\{a^\star_\theta(x)\}} \frac{2\gamma_{x,a}^\top A(\alpha)^{-1} \gamma_{x,a}}{(\theta^\top
\gamma_{x,a})^2}$ is the maximum of convex functions. Thus, the optimal allocation problem corresponds to solving $\inf \limits_{\alpha \in \Lambda} h(\alpha)$. Previous works use Frank-Wolfe type of algorithms to solve the optimal allocation problem exactly for all $t \in \mathbb{N}^+$ \cite{Fiez19} or for a subset $t \in \mathcal{T} \subseteq \mathbb{N}^+$ \cite{Jedra20}. The major drawback of this strategy is that solving a new convex optimization problem is computationally expensive, especially when $|\mathcal{X} \times \mathcal{A}|$ pair is large. We take a different approach based on the computation of an approximate solution to \eqref{eq:lb_delta} at each time step: we take $n$ gradient steps for all $t\in\mathbb{N^+}$. This will allow to decrease the sample complexity while retaining the asymptotic optimality of the algorithm. Denote by $(x_\star,a_\star) = \argmax\limits_{x \in \mathcal{X}, a \in \mathcal{A}\setminus\{a^\star_\theta(x)\}} \frac{2\gamma_{x,a}^\top A(\alpha)^{-1} \gamma_{x,a}}{(\theta^\top
\gamma_{x,a})^2}$, then we can express the gradients coordinates as 
$$\left(\nabla h(\alpha)\right)_{x,a} = \left( \frac{\gamma_\star^\top A(\alpha)^{-1} \phi_{x,a}}{\theta^\top \gamma_\star}\right)^2.$$

\begin{algorithm}[H]
\SetAlgoLined
\textbf{Input:} $\delta$, $\Tilde{\mathcal{A}}_x = \left\{\Tilde{a}_x(1),\dots,\Tilde{a}_x(d_x)\right\}$ for all $x\in\mathcal{X}$
\\ \textbf{Initialization:} $t=0, (i(x))_{x\in\mathcal{X}} = 0, (N_x(0))_{x\in\mathcal{X}} = 0, (N_{x,a}(0))_{(x,a)\in\mathcal{X}\times \mathcal{A}} = 0$, $(\alpha_{x,a}(0))_{(x,a)\in\mathcal{X}\times \mathcal{A}} = \frac{1}{K}$
\\ \While{Stopping rule not satisfied}{
\\  $x_t \sim p_\mathcal{X}$
\\ \eIf{$\sum_{s = 1}^t\phi_{x_s,a_s}\phi_{x_s,a_s}^\top \mathbbm{1}_{\{x_s = x\}}\succeq f_x(t)$}{
   $a_t(x_t) \leftarrow  \argmin_{a\in \text{supp}\left(\sum_{s =1}^t \alpha_{x,a}(s)\right)} \left( \frac{N_{x,a}(t)}{N_x(t)} - \sum_{s = 1}^t \alpha_{x,a}(s) \right)$ 
   }{$a_t(x_t)\leftarrow \tilde{a}_{x_t}(i_{t}(x_t)), i_{t+1}(x) = (i_t(x) \mod d_x)$}
  $t \leftarrow t+1$, update $N_x(t)$, $N_{x,a}(t)$ $\hat{\theta}_t$, $Z_\varepsilon(t)$,  
  \\ $s^\star(t) \leftarrow \arg\min_{s\in \Lambda} s^T \left( \frac{\hat{\gamma}_\star^\top A(\alpha_t)^{-1} \phi_{x,a}}{\hat{\theta}^\top \hat{\gamma}_\star}\right)^2$
  \\$\alpha(t) \leftarrow \alpha(t-1) + \frac{2}{t+2}(\alpha(t-1)- s^\star(t))$
 }
 \textbf{return} $\hat{a}_\tau(x) = \argmax_{a \in\mathcal{A}} \hat{\theta}_\tau \phi_{x,a}$, for all $x\in\mathcal{X}$
\caption{Online Gradient Track and Stop}
\end{algorithm} 

%Unlike the Lazy-TS algorithm here we execute a single gradient update step at each time step. This drastically reduces the computational complexity. 
Formulate the Lagrangian of the problem:
$$
L(z,\alpha,\rho) = z + \sum_{(y,b)\in\mathcal{X}\times\mathcal{A}\setminus\{a^\star_\theta(y)\}}\lambda_{y,b}\left(\frac{2\gamma_{y,b}^\top A(\alpha)^{-1} \gamma_{y,b}}{(\theta^\top
    \gamma_{y,b})^2}-z \right) +  \rho(\mathbf{1}^{\top}\alpha - 1).
$$
The first-order optimality condition impose:
\begin{equation*}
\begin{cases}
(i) \;\frac{dL}{dz} = 1 - \sum_{(y,b)}\lambda_{y,b} = 0
\\ 
(ii) \;\frac{dL}{d\alpha_{x,a}} = -\sum_{(y,b)}\frac{2{\gamma_{y,b}}^\top A(\alpha)^{-1}\phi_{x,a}\phi_{x,a}^\top A(\alpha)^{-1}{\gamma_{y,b}}}{(\theta^\top\gamma_{y,b})^2}\lambda_{y,b} + \rho = 0, \;\forall (x,a)\in\mathcal{X}\times\mathcal{A}
\\ (iii) \; \frac{dL}{d\rho} = \mathbf{1}^{\top}\alpha - 1 = 0
\\ (vi) \; \frac{dL}{d\lambda_{y,b}} = \frac{2\gamma_{x,a}^\top A(\alpha)^{-1} \gamma_{x,a}}{(\theta^\top\gamma_{x,a})^2}-z =0
\\ (v) \; \rho(\mathbf{1}^{\top}\alpha - 1) = 0
\\ (vi) \;\rho \geq 0,\lambda_{y,b} \geq 0.
\end{cases}
\end{equation*}
The size of the constraint set scales in linearly with $\mathcal{X}$ and $\mathcal{A}$.
%From $(ii)$ we get 
%$$
%\sum_{(y,b)}\frac{2\lambda_{y,b}}{(\theta^\top\gamma_{y,b})^2}\gamma_{y,b}^\top(A(\alpha)^{-1}(\phi_{x,a}\phi_{x,a}^{\top}-\phi_{x,c}\phi_{x,c}^{\top})A(\alpha)^{-1})\gamma_{y,b} = 0, \; \forall (a,c)\in\mathcal{A}^2
%$$
%We can conclude that the optimal allocation satisfy the following set of equations:
%\begin{equation*}
%\begin{cases}
%\frac{\|\gamma^\star\|^2}{|\mathcal{X}||\mathcal{A}|}\sum_{x,a}\frac{1}{\|\phi_{x,a}\|^2\alpha_{x,a}^2}={\gamma_\star}^\top A(\alpha)^{-1}\phi_{x,a}\phi_{x,a}^\top A(\alpha)^{-1}{\gamma_\star}, \;\forall (x,a)\in\mathcal{X}\times\mathcal{A}
%\\ \sum_{x,a}\alpha_{x,a} = 1.
%\end{cases}
%\end{equation*}
\end{comment}
%For $\varepsilon\geq0$, $x\in\mathcal{X}$, and $\theta\in\mathbb{R}^d$, define the set of $\varepsilon$-optimal arms as $\mathcal{A}_\varepsilon(\theta,x) = \{a\in\mathcal{A}: \theta^\top(\phi_{x,a^\star_\theta(x)}-\phi_{x,a})<\varepsilon\}$, and for $a\in \mathcal{A}_\varepsilon^c(\theta,x)$ the set $\mathcal{A}_\varepsilon(\theta,x,a) = \{b\in \mathcal{A}_\varepsilon(\theta,x): \theta^\top (\phi_{x,b}-\phi_{x,a}) \geq \varepsilon\}$.  Denote by $\mathbb{P}_\theta(\cdot)$ the probability measure of observations under the LCB problem defined by $\theta$ and by $\mathbb{E}_\theta[\cdot]$ its expectation. Define the simplex $\Lambda = \left\{\alpha \in [0,1]^{\vert \mathcal{X}\vert \times \vert \mathcal{A}\vert}: \forall x\in\mathcal{X} \; \sum_{a\in \mathcal{A}} \alpha_{x,a} = 1 \right\}.


%The \textit{coverage} indicator measures to what extent the area of interest is covered with a minimum signal power and is computed using measurements of the Reference Signal Received Power (RSRP). The \textit{capacity} indicator measures the amount of UE that the cell can handle simultaneously (e.g., in terms of number of calls) with a reference bit rate. The antenna tilt is a key parameters that determines a trade-off between coverage and capacity. On the one hand, low tilt values result in a larger covered area and smaller capacity due to an increased number of served UE; excessively low tilt values  may increase cell overshooting, causing the scope of antenna coverage to exceed the one intended and increasing the interference in neighbouring cells. On the other hand, high tilt values result in a smaller covered area with a lower number of UE served with increased capacity, but it risks to create \textit{coverage holes} in the cells. The joint optimization of coverage and capacity ensures that the targeted area remains covered while maximizing the capacity.

%In Contextual Bandits (CBs), an agent observes an input context, selects an action, and in turn receives a random reward sample. Given its versatility, several CB algorithms have been effectively employed in a broad range of real-world applications such as recommendation systems and network parameters optimization \cite{Langford08,Saxena19}. The Contextual Linear Multi-Armed Bandits (CL-MAB) problem \cite{Li11} is a particular instance of CBs in which the expected reward is modeled linearly in the feature vector encoding a context-action pair.

%The Best Policy Identification (BPI) problem with fixed confidence consists of devising a Probably Approximately Correct (PAC) algorithm using the least possible number of samples. The BPI problem can be studied in (i) \textit{active learning}, in which the agent adaptively selects its sampling rule based on the accumulated experience,  or (ii) \textit{passive learning}, in which the sampling rule is fixed and imposed. 

%In this paper we provide lower bound on the sample complexity of different types of PAC algorithms in both the active and passive learning settings. We then devise optimal algorithms matching such lower bounds. We apply our method to the RET optimization problem in 4G cellular networks. The experimental results show that our method is able to produce an optimal tilt update policy with intuitive interpretations of the results. To the best of our knowledge, this is the first paper considering BPI in the CL-MAB setting applied to RET optimization, and the first to consider the passive learning setting in CL-MAB-BPI.

%value maximization. The authors of \cite{Vannella20} apply off-policy estimators to the RET optimization problem. However such estimators are often unreliable, especially when data are biased or contain high amount of noise and do not provide a stopping rule. 

%Another related line of work is the one of off-policy evaluation and learning. Previous works in the off-policy setting, mostly focused on the general CB problem without reward structure \cite{Strehl10, Dudik14}. These work focused on learning a policy maximizing the value of a policy using data from an offline policy and off-policy value estimators. 

%These results reflects the trade-off between network coverage and capacity discussed in Section \ref{sec:introduction}. 

% there exists a sequence $(\ell(t))_{t\geq 1}$ of integers with $\ell(1) = 1$ and $\ell(t-1) \leq t-1$ for $t>1$, such that 
%\begin{equation}
%\label{eq:condition_convergence}
%\lim _{t \rightarrow \infty} \min _{s \geq \ell(t)} d_{\infty}\left(\alpha(t), C_\varepsilon^{\star}\left(\hat{\theta}_{s}\right)\right)=0 . \quad \text {a.s.}
%\end{equation}

==> Sections/AdditionalExperiments.tex <==
\newpage 
\section{Additional experimental results}
\label{app:experiments}

%\begin{figure}[h!]
%    \centering
%    \includegraphics[width = 8cm]{figures/example_cell.png}
%    \caption{Cell KPIs evolution example for up-tilt.}
%    \label{fig:ex_cell}
%\end{figure}

%Figure \ref{fig:two_action_exp_rew} shows the expectation actions' rewards over the context space fitted to the performance function.

%\begin{figure}[h!]
%    \centering
%    \includegraphics[width = 8 cm]{figures/planes.pdf}
%    \caption{Expected actions reward.}
%    \label{fig:two_action_exp_rew}
%\end{figure}
\begin{comment}

\section{Additional examples}
\subsection{$(U,\delta)$-PAC policy}
\textbf{Example 1:} We consider the following instance of LCB problem with $d = 3$, $K = 2$ and $C = 3$. We let $\theta = [1,1,1]$, and the feature vectors be specified as $\phi_{x_1,a_1} = [1,0,0]$, $\phi_{x_1,a_2} = [0,1-\Delta,0]$, $\phi_{x_2,a_1} = [0,1,0]$, $\phi_{x_2,a_2} = [1- \Delta,0,0]$, $\phi_{x_3,a_1} = [1,0,0]$, $\phi_{x_3,a_2} = [0,0,1-\Delta]$, 
for some $\Delta >0$. We assume to have uniform random probabilities across the context space, i.e., $p_\mathcal{X}(x) = 1/3$, for all $x\in\mathcal{X}$. It is easy to check that for a deterministic policy of the type $\bar{\alpha}_{x,a_1} = 1$, for all $x\in\mathcal{X}$, we have that $\textrm{det}(A(\bar{\alpha})) = 0$. In particular the second component of $\theta$ is not learnable, and we can hence focus on learning the best policy on $U = \mathbb{R}^2$. On the other hand, for any $\bar{\alpha}$ having non-zero probability, e.g. the uniform random policy $\bar{\alpha}_{x,a} = 1/2, \forall (x,a)$, we have $\textrm{det}(A(\bar{\alpha}))>0$ and $U = \mathbb{R}^3$. 

We report the results in terms of empirical sample complexity in Table \ref{tab:results_udelta}, when varying $\Delta$.

\begin{table}[ht!]
\fontsize{9.3}{9.3}\selectfont
\centering
\caption{Experimental results for the $(U,\delta)$-PAC example.}
\begin{tabular}{clrrr}\hline
Proportions  & Parameter & Lower bound & Sample complexity & BPI error \\ \hline \hline
\multirow{3}{*}{Deterministic} %& $\varepsilon = 0.20$ & $174.56$ & $323.48\pm71.10$ & $0.04 \pm 0.20$ \\ & $\varepsilon = 0.15$ & $319.82$ & $404.73 \pm 94.00$ & $0.05 \pm 0.23$ \\
& $\Delta= 1.5$  &  $ 13.81$ & $50.70 \pm 17.99$ & $0.000 \pm 0.000$ \\
& $\Delta= 0.9$  &  $ 34.28$ & $120.16 \pm 42.74$ & $0.010 \pm 0.099$ \\ & $\Delta = 0.5$ & $124.33$ & $491.40 \pm 138.22$ & $0.016 \pm 0.125$ \\ \hline \hline
\multirow{3}{*}{Random} 
& $\Delta= 1.5$  &  $35.47$ & $160.04 \pm 52.83$ & $0.000 \pm 0.000$ \\& $\Delta= 0.9$  & $102.16$ & $456.63\pm 138.41$ & $0.000 \pm 0.000$ \\ & $\Delta = 0.5$ & $319.29$ & $1654.73 \pm 469.77$ & $0.003 \pm 0.054$ \\ \hline 
\end{tabular} 
\label{tab:results_udelta}
\end{table}


\textbf{Example 2:} We consider the following instance of LCB problem with $d = 3$, $K = 2$ and $C = 2$. We let $\theta = [1,1,1]$, and the feature vectors be specified as $\phi_{x_1,a_1} = [1,0,0]$, $\phi_{x_1,a_2} = [0,1-\Delta,0]$, $\phi_{x_2,a_1} = [0,0,1]$, $\phi_{x_2,a_2} = [0,0,1- \Delta]$, %$\phi_{x_3,a_1} = [0,0,1]$, $\phi_{x_3,a_2} = [0,0,1-\Delta_3]$An Instance of the problem with $\Delta_i = 1/(i+1)$, for $i = 1,2$ is reported in Figure \ref{fig:u_delta_pac.pdf}.
for some $\Delta >0$. We assume to have uniform random probabilities across the context space, i.e., $p_\mathcal{X}(x) = 1/2$, for all $x\in\mathcal{X}$. It is easy to check that for a deterministic policy of the type $\bar{\alpha}_{x,a_1} = 1$, for all $x\in\mathcal{X}$, we have that $\textrm{det}(A(\bar{\alpha}))=0$. In particular the second component of $\theta$ is not learnable, and we can hence focus on learning the best policy on $U = \mathbb{R}^2$. On the other hand, for any $\bar{\alpha}$ having non-zero probability, e.g. the uniform random policy $\bar{\alpha}_{x,a} = 1/2, \forall (x,a)$, we have $\textrm{det}(A(\bar{\alpha}))>0$. 

The lower bound satisfies $\mathbb{E}[\tau] \geq \frac{4}{\Delta^2}\log(1/\delta)$. We fix $\delta = 0.01$, and we report the results in terms of empirical sample complexity in Table \ref{tab:results_udelta}, when varying $\Delta$.

\begin{table}[ht!]
\fontsize{9.3}{9.3}\selectfont
\centering
\caption{Experimental results for the $(U,\delta)$-PAC example.}
\begin{tabular}{clrrr}\hline
Proportions & Parameter & Lower bound & Sample complexity & BPI error \\ \hline \hline
\multirow{3}{*}{Deterministic} 
& $\Delta= 0.1$  & $417.54$ & $504.34 \pm 165.87$ & $0.005 \pm 0.070$ \\ & $\Delta = 0.05$ & $610.52$ & $583.33 \pm 111.06$ & $0.00 \pm 0.00$ \\ & $\Delta = 0.01$ & $610.52$ & $583.33 \pm 111.06$ & $0.00 \pm 0.00$ \\ \hline \hline
\multirow{3}{*}{Random} 
& $\Delta= 0.1$  & $417.54$ & $504.34 \pm 165.87$ & $0.005 \pm 0.070$ \\ & $\Delta = 0.05$ & $610.52$ & $583.33 \pm 111.06$ & $0.00 \pm 0.00$ \\ & $\Delta = 0.01$ & $610.52$ & $583.33 \pm 111.06$ & $0.00 \pm 0.00$ \\ \hline 
\end{tabular} 
\label{tab:results_udelta}
\end{table}

%$\hat{\theta} = [1,0,1]$.  $\gamma_{x_1,a_2} = \phi_{x_1,a_1} - \phi_{x_1,a_2} = [1,\Delta-1,0]$, $\gamma_{x_2,a_2} = \phi_{x_2,a_1} - \phi_{x_2,a_2} = [0,0,\Delta]$. $\hat{\theta}^\top \gamma_{x_1,a_2} = 1$, $\hat{\theta}^\top \gamma_{x_2,a_2} = \Delta$. $\gamma_{x_1,a_2}^\top A(\alpha)^\dagger\gamma_{x_1,a_2} = 2$, $\gamma_{x_2,a_2}^\top A(\alpha)^\dagger\gamma_{x_2,a_2} = 2\Delta^2$.
\end{comment}

==> Sections/ProofsApp.tex <==

\begin{comment}
\subsection{Proof of Theorem \ref{theorem:lb_delta}}
\label{app:proof_th_lb_delta}
In order to derive the asymptotic lower bound on the sample complexity, we follow a similar approach to Lemma 1 in \cite{Kauffman16}.
\begin{proof}
We divide the proof in $5$ steps:
\paragraph{The log-likelihood ratio} Let $\nu^\theta$ and $\nu^{\mu}$ be two LCB bandit problems such that for all $(x,a) \in \mathcal{X}\times\mathcal{A}$ the distributions $\nu^\theta_{x,a}$ and $\nu^{\mu}_{x,a}$ are mutually absolutely continuous. We define the log-likelihood ratio of the observation under policy $\pi$ for all $T \ge 1$ 
\begin{equation}
\begin{aligned}
    L_T^{\theta,\mu}(X_1,A_1,R_1,\dots,X_T,A_T,R_T) & =  \log\left(\frac{f^\theta(X_1,A_1,R_1,\dots,X_T,A_T,R_T)}{f^{\mu}(X_1,A_1,R_1,\dots,X_T,A_T,R_T)}\right)\\
    & = \sum_{t=1}^T \log\left(\frac{f^\theta(R_t\vert X_t, A_t)}{f^{\mu}(R_t \vert X_t,A_t)}\right) \\ 
    & =\sum_{t=1}^{T} \sum\limits_{(x,a) \in\mathcal{X}\times \mathcal{A}}\mathbbm{1}\left\{ X_{t}=x,A_{t}=a\right\} \log \left(\frac{f_{x,a}^\theta\left(R_{t}\right)}{f_{x,a}^{\mu}\left(R_{t}\right)}\right). \\
    \end{aligned}
\end{equation}

\paragraph{The change of measure argument} Lemma 19 in \cite{Kauffman16} ensures that for all parameters $\theta,\mu \in \mathbb{R}^d$ and any stopping time $\tau$ w.r.t. $\mathcal{F}_t$. 
$$
\mathbb{E}\left[ L_\tau^{\theta,\mu} \right] \ge \sup_{\mathcal{E} \in \mathcal{F}_\tau}\mathrm{kl}\left(\mathbb{P}_\theta(\mathcal{E}), \mathbb{P}_{\mu}( \mathcal{E} ) \right) 
$$
Define the set of confusing parameters 
\begin{align*}
B(\theta) & \triangleq \left\lbrace \mu \in \mathbb{R}^d: \; \exists x \in \mathcal{X},\; a_{\mu}^\star(x) \neq a^\star_{\theta}(x) \right\rbrace \\
& = \left\lbrace \mu \in \mathbb{R}^d: \; \exists x \in \mathcal{X},\; \mu^\top (\phi_{x,a_{\mu}^\star(x)} - \phi_{x,a^\star_{\theta}(x)}) > 0 \right\rbrace \\ 
& = \bigcup_{x\in\mathcal{X}, a \in \mathcal{A} \backslash\lbrace a_\theta^\star(x) \rbrace}  \left\lbrace \mu \in \mathbb{R}^d: \; \mu^\top (\phi_{x,a} - \phi_{x,a^\star_{\theta}(x)}) > 0 \right\rbrace
\end{align*}
Define the event $\mathcal{E} = \lbrace \forall x \in \mathcal{X}\; a^\star_\theta(x) = \hat{a}_\tau(x) \rbrace \in \mathcal{F}_\tau$, and note that since $\pi$ is $\delta$-PAC it holds that 
$$
\mathbb{P}_\theta(\mathcal{E}) \ge 1- \delta,
$$
and for all $\mu \in B(\theta)$ that 
$$
\mathbb{P}_{\mu}(\mathcal{E}) \le \delta.
$$
Therefore 
$$
\forall \mu \in B(\theta) \qquad \mathbb{E}\left[ L_\tau^{\theta,\mu} \right] \ge \mathrm{kl}\left(1- \delta, \delta \right).
$$

\paragraph{The expected log-likelihood ratio} Taking expectation we have 
\begin{align*}
    \mathbb{E}_\theta\left[L_\tau^{\theta,\mu} \right] 
    & = \mathbb{E}_\theta \left[ \sum_{t=1}^\infty \mathbbm{1}\left\{ \tau > t-1 \right\} \sum\limits_{(x,a) \in\mathcal{X}\times \mathcal{A}} \mathbbm{1}\left\{X_{t}=x, A_{t}=a\right\} \log \left(\frac{f_{x,a}^\theta\left(R_{t}\right)}{f_{x,a}^{\mu}\left(R_{t}\right)}\right) \right]  
    \\ & =  \mathbb{E}_\theta \left[\sum_{t=1}^\infty \mathbb{E}_\theta \left[  \sum\limits_{(x,a) \in\mathcal{X}\times \mathcal{A}}\mathbbm{1}\left\{ \tau > t-1 \right\} \mathbbm{1}\left\{X_{t}=x, A_{t}=a\right\} \log \left(\frac{f_{x,a}^\theta\left(R_{t}\right)}{f_{x,a}^{\mu}\left(R_{t}\right)}\right)  \bigg\vert \mathcal{F}_{t-1}\right] \right] 
    \\ & = \mathbb{E}_\theta \left[\sum_{t=1}^\infty \sum\limits_{(x,a) \in\mathcal{X}\times \mathcal{A}}\mathbbm{1}\left\{ \tau > t-1 \right\} \mathbbm{1}\left\{X_{t}=x, A_{t}=a\right\} \mathbb{E}_\theta \left[ \log \left(\frac{f_{x,a}^\theta\left(R_{t}\right)}{f_{x,a}^{\mu}\left(R_{t}\right)}\right)  \bigg\vert \mathcal{F}_{t-1}\right] \right] 
    \\ & = \sum\limits_{(x,a) \in\mathcal{X}\times \mathcal{A}} \mathbb{E}_\theta \left[\sum_{t=1}^\infty \mathbbm{1}\left\{ \tau > t-1 \right\} \mathbbm{1}\left\{X_{t}=x, A_{t}=a\right\} \KL(\nu^\theta_{x,a},\nu^{\mu}_{x,a}) \right] \\
    & = \sum\limits_{(x,a) \in\mathcal{X}\times \mathcal{A}} \mathbb{E}_\theta \left[N_{x,a}(\tau)\right] \KL(\nu^\theta_{x,a},\nu^{\mu}_{x,a}) 
\end{align*}
where we used $\lbrace X_t = x, A_t = a\rbrace, \lbrace \tau > t-1\rbrace \in \mathcal{F}_{t-1}$, noted that $\mathbb{E}_{\theta}\left[\log \left(\frac{f_{x,a}^\theta\left(Y_{x,a,t}\right)}{f_{   x,a}^{\mu}\left(Y_{x,a,t}\right)}\right)\right] = \KL(\nu^\theta_{x,a},\nu^{\mu}_{x,a})$, and introduced $N_{x,a}(\tau) = \sum_{t = 1}^\tau \mathbbm{1}\left\{X_{t}=x, A_{t}=a\right\}$. Some integrability assumptions are needed for the exchange of integrals but these are mild and we will assume that they hold. Under Gaussian noise model we obtain 
\begin{equation}
    \mathbb{E}_\theta\left[ L_\tau^{\theta,\mu} \right] = \frac{1}{2} (\theta - \mu)^\top \left(\sum\limits_{(x,a) \in\mathcal{X}\times \mathcal{A}} \mathbb{E}_\theta\left[N_{x,a}(\tau)\right] \phi_{x,a} \phi_{x,a}^\top\right) (\theta - \mu)
\end{equation}

\paragraph{Optimizing the lower bound} From the above we have 
\begin{align}
    \inf_{\mu \in B(\theta)} \frac{1}{2} (\theta - \mu)^\top \left(\sum\limits_{(x,a) \in\mathcal{X}\times \mathcal{A}} \mathbb{E}_\theta\left[N_{x,a}(\tau)\right] \phi_{x,a} \phi_{x,a}^\top\right) (\theta - \mu) \ge \mathrm{kl}(1- \delta, \delta).
\label{eq:optimization_lb}
\end{align}
We may further note that 
\begin{equation}
\begin{aligned}
     \inf_{\mu \in B(\theta)} \frac{1}{2} (\theta - \mu)^\top &  \left(\sum\limits_{(x,a) \in\mathcal{X}\times \mathcal{A}} \mathbb{E}_\theta\left[N_{x,a}(\tau)\right] \phi_{x,a} \phi_{x,a}^\top\right) (\theta - \mu)\\ 
     & = \mathbb{E}[\tau] \inf_{\mu \in B(\theta)} \frac{1}{2} (\theta - \mu)^\top \left(\sum\limits_{(x,a) \in\mathcal{X}\times \mathcal{A}} \frac{\mathbb{E}_\theta\left[N_{x,a}(\tau)\right]}{\mathbb{E}_\theta\left[N_x(\tau)\right]}\frac{\mathbb{E}_\theta\left[N_{x}(\tau)\right]}{\mathbb{E}_\theta\left[\tau\right]} \phi_{x,a} \phi_{x,a}^\top\right) (\theta - \mu) \\
     & = \mathbb{E}_\theta[\tau] \inf_{\mu \in B(\theta)} \frac{1}{2} (\theta - \mu)^\top \left(\sum\limits_{(x,a) \in\mathcal{X}\times \mathcal{A}} \alpha_{x,a}p_{\mathcal{X}}(x)\phi_{x,a} \phi_{x,a}^\top \right) (\theta - \mu) \\
     & \le \mathbb{E}[\tau] \sup_{\alpha \in \Lambda}\inf_{\mu \in B(\theta)} \frac{1}{2} (\theta - \mu)^\top \left(\sum\limits_{(x,a) \in\mathcal{X}\times \mathcal{A}} \alpha_{x,a} p_{\mathcal{X}}(x) \phi_{x,a} \phi_{x,a}^\top\right) (\theta - \mu) \\
     & = \mathbb{E}[\tau] \sup_{\alpha \in \Lambda}\inf_{\mu \in B(\theta)} \frac{1}{2} \|\theta - \mu\|^2_{A(\alpha)},
\end{aligned}
     \label{eq:optim_lb_discrete}
\end{equation}
where we introduced the context count $N_x(\tau) = \sum_{t =1}^\tau \mathbbm{1}\{X_t = x\}$, the conditional context-arm proportions $\alpha_{x,a} = \frac{\mathbb{E}_{\theta}\left[N_{x,a}(\tau)\right]}{\mathbb{E}_{\theta}\left[N_x(\tau)\right]}$, the matrix $A(\alpha) = \left(\sum\limits_{(x,a) \in\mathcal{X}\times \mathcal{A}} \alpha_{x,a} p_{\mathcal{X}(x)}\phi_{x,a} \phi_{x,a}^\top\right)$, the joint probability simplex by $\Lambda =\lbrace \alpha \in [0,1]^{\vert \mathcal{A} \vert\times\vert \mathcal{X} \vert}: \forall x\in\mathcal{X} \; \sum_{a\in \mathcal{A}} \alpha_{x,a} = 1 \rbrace$ and noted that $ p_{\mathcal{X}}(x) = \frac{\mathbb{E}_\theta\left[N_x(\tau)\right]}{\mathbb{E}_\theta\left[\tau\right]}$. Here, $\alpha \in \Lambda$ may be interpreted as the asymptotic arm proportions conditioned on context $x$, i.e., the fraction of times that arm $a$ is selected given that context $x$ is observed.

We define the characteristic time $T^\star_\theta$ as follows 
$$
(T^\star_\theta)^{-1} = \sup_{\alpha \in \Lambda} \inf_{\mu \in B(\theta)}  \frac{1}{2} \|\theta - \mu\|^2_{A(\alpha)},
$$ 
and write the lower bound as 
\begin{equation*}
    \mathbb{E}[\tau] \ge T^\star_\theta  \mathrm{kl}(1- \delta, \delta) \gtrsim T^\star_\theta\log\left(\frac{1}{\delta}\right).
\end{equation*}

\paragraph{Solution of the optimization problem} Introduce the following function 
$$
\psi(\theta, \alpha) =  \inf_{\mu \in B(\theta)}  \frac{1}{2} \|\theta - \mu\|^2_{A(\alpha)} 
$$
and note that $(T^\star_\theta)^{-1} 
= \sup_{\alpha \in \Lambda} \psi(\theta, \alpha)$. Further note that the set of confusing parameters may be partitioned as follows   
$$
B(\theta) = \bigcup_{x\in\mathcal{X}} \bigcup _{a \in \mathcal{A}\backslash\lbrace a^\star_\theta(x)\rbrace} B(\theta, x, a),
$$
where $B(\theta, x, a) \triangleq \left\lbrace \mu \in \mathbb{R}^d: \; \mu^\top (\phi_{x,a} - \phi_{x,a^\star_{\theta}(x)}) > 0 \right\rbrace$. So we may carry the following split 
\begin{equation*}
    \psi(\theta, \alpha) = \min_{x \in \mathcal{X}, a \in \mathcal{A}\backslash\lbrace a_\theta^\star(x) \rbrace} \inf_{\mu \in B(\theta, x, a)} \|\theta - \mu\|^2_{A(\alpha)}.
\end{equation*}
The resulting sub-optimization problems are convex optimization problems that may be solved explicitly. The solution closely follows the approach in \cite{Soare15}. Consider $\Gamma^\star_\theta(x) = \{\phi_{x,a^\star_\theta(x)} - \phi_{x,a}, \forall a \in\mathcal{A}\}$ and $\omega = \theta-\mu$. 
The event that two arms differ in two environments $\theta$, $\mu$ implies that there exists at least one $\gamma \in \Gamma^\star_\theta(x)$ such that
$$ \gamma^{\top} \mu<0 \Leftrightarrow \gamma^{\top} \theta-\gamma^{\top} \mu>\gamma^{\top} \theta  \Leftrightarrow \gamma^{\top} \omega>\gamma^{\top} \theta .$$ 

Thus, we can rewrite the optimization problem as 
\begin{equation*}
    \begin{aligned} 
    &\inf \frac{1}{2}\omega^\top A(\alpha) \omega 
    \\&\text{subject to } \exists \gamma \in \Gamma^\star_\theta(x), \gamma^{\top} \omega \geq \gamma^{\top} \theta.
    \end{aligned}
\end{equation*}

The Lagrangian for this optimization problem is
$$L(\omega, \rho) = \frac{1}{2}\omega^{\top} A(\alpha) \omega+\rho\left(-\gamma^{\top} \omega+\gamma^\top\theta\right),$$
with Lagrange multipliers $\rho \in \mathbb{R}$. Imposing the optimality conditions leads to the system
\begin{equation}
\begin{cases}
    \frac{\partial L}{\partial \omega} = A(\alpha)\omega-\rho \gamma=0 \Leftrightarrow A(\alpha) \omega= \rho\gamma \\ 
    \rho\frac{\partial L}{\partial \rho}=\rho(-\gamma^{\top} \omega+\gamma^{\top} \theta)=0 
    \\ \gamma^\top\omega \geq \gamma^\top \theta
    \\ \rho \geq 0
\end{cases}.
\label{eq:KKT_approx_delta_pac}
\end{equation}

Let $\rho\neq 0 \Rightarrow (-\gamma^{\top} \omega+\gamma^{\top} \theta)=0 $. For $A(\alpha) \succ 0$, solving for $\omega$ from the first equation of Eq. \eqref{eq:KKT_approx_delta_pac} and substituting in the second equation of Eq. \eqref{eq:KKT_approx_delta_pac}, we get
$$\rho = \frac{\gamma^\top\theta }{\|\gamma\|^2_{A(\alpha)^{-1}}}. $$
Note that $\rho > 0$, thus we have a feasible solution to the optimization problem.
We have $$\frac{1}{2}\omega^\top A(\alpha)\omega = \frac{(\gamma^\top \theta)^\top\gamma^\top A(\alpha)^{-1}A(\alpha)A(\alpha)^{-1}\gamma(\gamma^\top \theta )}{2\|\gamma\|_{A(\alpha)^{-1}}^4}= \frac{(\gamma^\top \theta)^\top\gamma^\top A(\alpha)^{-1}\gamma(\gamma^\top \theta )}{\|\gamma\|_{A(\alpha)^{-1}}^4} = \frac{(\gamma^\top \theta )^2 }{2\|\gamma\|^2_{A(\alpha)^{-1}}}.$$

In case $\lambda_{1}(A(\alpha)) = 0$ we have $\frac{\omega^\top A(\alpha)\omega}{2} = 0$. 
By substitution into the lower bound we get
\begin{align*}
    \inf_{\mu \in B(\theta, x, a)} \frac{1}{2}  \|\theta - \mu\|^2_{A(\alpha)} =
     \begin{cases}
    \frac{ (\theta^\top\gamma_{x,a})^2}{2\gamma_{x,a}^\top A(\alpha)^{-1} \gamma_{x,a}} & \text{ if } A(\alpha) \succ 0 \\
    0 &\text{ otherwise}
    \end{cases},
\end{align*}
where $\gamma_{x,a} = (\phi_{x,a^\star_\theta(x)} - \phi_{x,a})$.
Thus we may conclude that $\mathbb{E}_\theta[\tau] \gtrsim T^\star_{\theta}\log\left(\frac{1}{\delta}\right)$ with
\begin{equation*}
    T^\star_\theta = \begin{cases} \inf\limits_{\alpha\in\Lambda}\max\limits_{x \in \mathcal{X}, a \in \mathcal{A}\backslash\lbrace a_\theta^\star(x) \rbrace} \frac{ (\theta^\top\gamma_{x,a})^2}{2\gamma_{x,a}^\top A(\alpha)^{-1} \gamma_{x,a}} & \text{ if } A(\alpha) \succ 0 \\
    0 & \text{ otherwise}
    \end{cases}.
\end{equation*}
\end{proof}
\end{comment}
\section{Proofs}
\subsection{Proof of Theorem \ref{theorem:lb_eps_delta_discrete}}
\label{app:proof_th_eps_delta_lb}
\begin{proof}
%The proof follows the proof of Theorem \ref{theorem:lb_delta}. The main differences are at step $2$ (change of measure argument) and at step $5$ (solution of the optimization problem). %Indeed the main change is in the PAC policy definition that in turn modifies the set of confusing parameters and the optimization problem.
We divide the proof in $5$ steps:

\textit{1) The log-likelihood ratio:} Let $\nu^\theta$ and $\nu^{\mu}$ be two LCB bandit problems such that for all $(x,a) \in \mathcal{X}\times\mathcal{A}$ the distributions $\nu^\theta_{x,a}$ and $\nu^{\mu}_{x,a}$ are mutually absolutely continuous. We define the log-likelihood ratio of the observation under algorithm $(a_t,\tau,\hat{a}_\tau)$, for all $T \geq 1$ as
\begin{equation}
\label{label:log_like}
\begin{aligned}
    L_T^{\theta,\mu}(x_1,a_1,r_1,\dots,x_T,a_T,r_T) & =  \log\left(\frac{f^\theta(x_1,a_1,r_1,\dots,x_T,a_T,r_T)}{f^{\mu}(x_1,a_1,r_1,\dots,x_T,a_T,r_T)}\right)\\
    & = \sum_{t=1}^T \log\left(\frac{f^\theta(r_t\vert x_t, a_t)}{f^{\mu}(r_t \vert x_t,a_t)}\right) \\ 
    & =\sum_{t=1}^{T} \sum\limits_{(x,a) \in\mathcal{X}\times \mathcal{A}}\mathbbm{1}\left\{ x_{t}=x,a_{t}=a\right\} \log \left(\frac{f_{x,a}^\theta\left(r_{t}\right)}{f_{x,a}^{\mu}\left(r_{t}\right)}\right). \\
    \end{aligned}
\end{equation}

\textit{2) The change of measure argument:} Recall the definition of set of $\varepsilon$-optimal arms $\mathcal{A}_\varepsilon(\theta, x) = \{ b\in\mathcal{A}: \theta^\top (\phi_{x,a^\star_\theta(x)} - \phi_{x,b}) \le \varepsilon \}$. Define the set of confusing parameters as
$$ B_{\varepsilon}(\theta) \triangleq \left \lbrace \mu \in \mathbb{R}^d: \; \exists x \in \mathcal{X}, \forall b \in \mathcal{A}_\varepsilon(\theta,x), \; \mu^{\top}(\phi_{x,a_{\mu}^\star(x)}- \phi_{x,b})>\varepsilon \right\rbrace. $$
Define the event:

$$ \mathcal{E}_{\theta} = \{\forall x \in \mathcal{X}, \theta^{\top}(\phi_{x,a_{\theta}^\star(x)} - \phi_{x,\hat{a}_{\tau}(x)})< \varepsilon \} = \{ \forall x \in \mathcal{X}, \hat{a}_{\tau}(x) \in \mathcal{A}_\varepsilon(\theta,x) \}, $$ 
and note that, since the algorithm is $(\varepsilon,\delta)$-PAC, it holds that
$$
\mathbb{P}_{\theta}(\mathcal{E}_{\theta}) \ge 1-\delta,
$$
and $\forall \mu \in B_{\varepsilon}(\theta)$ 
$$
\mathbb{P}_{\mu}(\mathcal{E}_{\theta}) \leq \delta.
$$
The last inequality follows from the fact that $\forall \mu\in B_\varepsilon(\theta)$ we have $\mathcal{A}_\varepsilon(\theta, x) \cap \mathcal{A}_\varepsilon(\mu, x) = \emptyset$, and hence $\mathcal{A}_\varepsilon(\theta,x) \subseteq \mathcal{A}^c_\varepsilon(\mu,x)$. This in turn implies 
$$
\mathbb{P}_{\mu}(\mathcal{E}_{\theta}) = \mathbb{P}_{\mu}(\forall x \in \mathcal{X}, \hat{a}_{\tau}(x) \in \mathcal{A}_\varepsilon(\theta,x)) \leq \mathbb{P}_{\mu}(\forall x \in \mathcal{X}, \hat{a}_{\tau}(x) \in \mathcal{A}^{c}_{\varepsilon}(\mu,x)) \leq \delta.
$$
Therefore we get by Lemma 19 in \cite{Kauffman16} that
$$
\forall \mu \in B_{\varepsilon}(\theta) \qquad \mathbb{E}\left[ L_\tau^{\theta,\mu} \right] \ge \mathrm{kl}\left(1-\delta, \delta \right) \gtrsim \log(1/\delta).
$$

\textit{3) The expected log-likelihood ratio:} Taking the expectation of \eqref{label:log_like}, we get 
\begin{align*}
    \mathbb{E}_\theta\left[L_\tau^{\theta,\mu} \right] 
    & = \mathbb{E}_\theta \left[ \sum_{t=1}^\infty \mathbbm{1}\left\{ \tau > t-1 \right\} \sum\limits_{(x,a) \in\mathcal{X}\times \mathcal{A}} \mathbbm{1}\left\{X_{t}=x, A_{t}=a\right\} \log \left(\frac{f_{x,a}^\theta\left(R_{t}\right)}{f_{x,a}^{\mu}\left(R_{t}\right)}\right) \right]  
    \\ & =  \mathbb{E}_\theta \left[\sum_{t=1}^\infty \mathbb{E}_\theta \left[  \sum\limits_{(x,a) \in\mathcal{X}\times \mathcal{A}}\mathbbm{1}\left\{ \tau > t-1 \right\} \mathbbm{1}\left\{X_{t}=x, A_{t}=a\right\} \log \left(\frac{f_{x,a}^\theta\left(R_{t}\right)}{f_{x,a}^{\mu}\left(R_{t}\right)}\right)  \bigg\vert \mathcal{F}_{t-1}\right] \right] 
    \\ & = \mathbb{E}_\theta \left[\sum_{t=1}^\infty \sum\limits_{(x,a) \in\mathcal{X}\times \mathcal{A}}\mathbbm{1}\left\{ \tau > t-1 \right\} \mathbbm{1}\left\{X_{t}=x, A_{t}=a\right\} \mathbb{E}_\theta \left[ \log \left(\frac{f_{x,a}^\theta\left(R_{t}\right)}{f_{x,a}^{\mu}\left(R_{t}\right)}\right)  \bigg\vert \mathcal{F}_{t-1}\right] \right] 
    \\ & = \sum\limits_{(x,a) \in\mathcal{X}\times \mathcal{A}} \mathbb{E}_\theta \left[\sum_{t=1}^\infty \mathbbm{1}\left\{ \tau > t-1 \right\} \mathbbm{1}\left\{X_{t}=x, A_{t}=a\right\} \KL(\nu^\theta_{x,a},\nu^{\mu}_{x,a}) \right] \\
    & = \sum\limits_{(x,a) \in\mathcal{X}\times \mathcal{A}} \mathbb{E}_\theta \left[N_{x,a}(\tau)\right] \KL(\nu^\theta_{x,a},\nu^{\mu}_{x,a}),
\end{align*}
where we used $\lbrace x_t = x, a_t = a\rbrace, \lbrace \tau > t-1\rbrace \in \mathcal{F}_{t-1}$, noted that $\mathbb{E}_{\theta}\left[\log \left(\frac{f_{x,a}^\theta\left(Y_{x,a,t}\right)}{f_{   x,a}^{\mu}\left(Y_{x,a,t}\right)}\right)\right] = \KL(\nu^\theta_{x,a},\nu^{\mu}_{x,a})$, and introduced $N_{x,a}(\tau) = \sum_{t = 1}^\tau \mathbbm{1}\left\{x_{t}=x, a_{t}=a\right\}$. Some integrability assumptions are needed for the exchange of integrals but these are mild and we will assume that they hold. Under Gaussian noise we obtain 
\begin{equation}
    \mathbb{E}_\theta\left[ L_\tau^{\theta,\mu} \right] = \frac{1}{2} (\theta - \mu)^\top \left(\sum\limits_{(x,a) \in\mathcal{X}\times \mathcal{A}} \mathbb{E}_\theta\left[N_{x,a}(\tau)\right] \phi_{x,a} \phi_{x,a}^\top\right) (\theta - \mu)
\end{equation}


\textit{4) Optimizing the lower bound.} From the above we have 
\begin{align}
    \inf_{\mu \in B_\varepsilon(\theta)} \frac{1}{2} (\theta - \mu)^\top \left(\sum\limits_{(x,a) \in\mathcal{X}\times \mathcal{A}} \mathbb{E}_\theta\left[N_{x,a}(\tau)\right] \phi_{x,a} \phi_{x,a}^\top\right) (\theta - \mu) \ge \mathrm{kl}(1- \delta, \delta).
\label{eq:optimization_lb}
\end{align}
We may further note that 
\begin{equation}
\begin{aligned}
     \inf_{\mu \in B_\varepsilon(\theta)} \frac{1}{2} (\theta - \mu)^\top &  \left(\sum\limits_{(x,a) \in\mathcal{X}\times \mathcal{A}} \mathbb{E}_\theta\left[N_{x,a}(\tau)\right] \phi_{x,a} \phi_{x,a}^\top\right) (\theta - \mu)\\ 
     & = \mathbb{E}[\tau] \inf_{\mu \in B_\varepsilon(\theta)} \frac{1}{2} (\theta - \mu)^\top \left(\sum\limits_{(x,a) \in\mathcal{X}\times \mathcal{A}} \frac{\mathbb{E}_\theta\left[N_{x,a}(\tau)\right]}{\mathbb{E}_\theta\left[N_x(\tau)\right]}\frac{\mathbb{E}_\theta\left[N_{x}(\tau)\right]}{\mathbb{E}_\theta\left[\tau\right]} \phi_{x,a} \phi_{x,a}^\top\right) (\theta - \mu) \\
     & = \mathbb{E}_\theta[\tau] \inf_{\mu \in B_\varepsilon(\theta)} \frac{1}{2} (\theta - \mu)^\top \left(\sum\limits_{(x,a) \in\mathcal{X}\times \mathcal{A}} \alpha_{x,a}p_{\mathcal{X}}(x)\phi_{x,a} \phi_{x,a}^\top \right) (\theta - \mu) \\
     & \le \mathbb{E}[\tau] \sup_{\alpha \in \Lambda}\inf_{\mu \in B_\varepsilon(\theta)} \frac{1}{2} (\theta - \mu)^\top \left(\sum\limits_{(x,a) \in\mathcal{X}\times \mathcal{A}} \alpha_{x,a} p_{\mathcal{X}}(x) \phi_{x,a} \phi_{x,a}^\top\right) (\theta - \mu) \\
     & = \mathbb{E}[\tau] \sup_{\alpha \in \Lambda}\inf_{\mu \in B_\varepsilon(\theta)} \frac{1}{2} \|\theta - \mu\|^2_{A(\alpha)},
\end{aligned}
     \label{eq:optim_lb_discrete}
\end{equation}
where we introduced the context count $N_x(\tau) = \sum_{t =1}^\tau \mathbbm{1}\{x_t = x\}$, the conditional context-arm proportions $\alpha_{x,a} = \frac{\mathbb{E}_{\theta}\left[N_{x,a}(\tau)\right]}{\mathbb{E}_{\theta}\left[N_x(\tau)\right]}$, the matrix $A(\alpha) = \left(\sum\limits_{(x,a) \in\mathcal{X}\times \mathcal{A}} \alpha_{x,a} p_{\mathcal{X}(x)}\phi_{x,a} \phi_{x,a}^\top\right)$, $\Lambda =\lbrace \alpha \in [0,1]^{\vert \mathcal{X} \vert\times\vert \mathcal{A} \vert}: \forall x\in\mathcal{X} \; \sum_{a\in \mathcal{A}} \alpha_{x,a} = 1 \rbrace$ and noted that $ p_{\mathcal{X}}(x) = \frac{\mathbb{E}_\theta\left[N_x(\tau)\right]}{\mathbb{E}_\theta\left[\tau\right]}$. Here, $\alpha \in \Lambda$ may be interpreted as the asymptotic arm proportions conditioned on context $x$, i.e., the fraction of times that arm $a$ is selected given that context $x$ is observed. Define $\psi_{\varepsilon}^\star(\theta) = \sup_{\alpha \in \Lambda}\inf_{\mu \in B_\varepsilon(\theta)} \frac{1}{2} \|\theta - \mu\|^2_{A(\alpha)}$. We may write the lower bound as 
\begin{equation*}
    \mathbb{E}[\tau] \psi_{\varepsilon}^\star(\theta) \ge  \mathrm{kl}(1- \delta, \delta) %\gtrsim T^\star_{\theta,\varepsilon}\log\left(\frac{1}{\delta}\right).
\end{equation*}

\textit{4) The optimization problem:}
Now we aim at finding a closed-form solution to $\psi_{\varepsilon}(\theta,\alpha)$. What follows extends the approach in \cite[Sec. 3.1]{Soare15} for LB to LCB. Let $\Gamma^\star_\theta(x) = \{\phi_{x,a^\star_\theta(x)} - \phi_{x,a}, \forall a \in\mathcal{A}\}$ and $\omega = \theta-\mu$. 
The event that two arms differ under $\theta$ and $\mu$ implies that there exists at least one $\gamma \in \Gamma^\star_\theta(x)$ such that
$$ \gamma^{\top} \mu<0 \Leftrightarrow \gamma^{\top} \theta-\gamma^{\top} \mu>\gamma^{\top} \theta  \Leftrightarrow \gamma^{\top} \omega>\gamma^{\top} \theta .$$
Thus, we can rewrite the optimization problem as 
\begin{equation*}
    \begin{aligned} 
    &\inf_{\omega} \frac{1}{2}\omega^\top A(\alpha) \omega 
    \\&\text{subject to } \exists \gamma \in \Gamma^\star_\theta(x), \gamma^{\top} \omega \geq \gamma^{\top} \theta.
    \end{aligned}
\end{equation*}
Now, introduce the following function 
$$
\psi_\varepsilon(\theta, \alpha) =  \inf_{\mu \in B_{\varepsilon}(\theta)}  \frac{1}{2} \|\theta - \mu\|^2_{A(\alpha)},
$$
and note that set of confusing parameters may decomposed as
\begin{align*}
B_{\varepsilon}(\theta) & = \left\lbrace \mu \in \mathbb{R}^d: \; \exists x \in \mathcal{X}, \forall b \in \mathcal{A}_\varepsilon(\theta,x), \; \mu^{\top}(\phi_{x,a_{\mu}^\star(x)}- \phi_{x,b})>\varepsilon \right\rbrace
\\& = \bigcup_{x\in \mathcal{X}} \left\lbrace \mu \in \mathbb{R}^d: \; \forall b \in \mathcal{A}_\varepsilon(\theta,x), \; \mu^{\top}(\phi_{x,a_{\mu}^\star(x)}- \phi_{x,b})>\varepsilon \right\rbrace
\\& = \bigcup_{x\in \mathcal{X}} \bigcup_{a\in  \mathcal{A}^c_\varepsilon(\theta,x)} \left\lbrace \mu \in \mathbb{R}^d: \; \forall b \in \mathcal{A}_\varepsilon(\theta,x), \; \mu^{\top}(\phi_{x,a}- \phi_{x,b})>\varepsilon \right\rbrace \\& = \bigcup_{x\in \mathcal{X}} \bigcup_{a\in \mathcal{A}^c_\varepsilon(\theta,x)} B_{\varepsilon}(\theta,x,a),
\end{align*}
where $B_\varepsilon(\theta,x,a) = \left\lbrace \mu \in \mathbb{R}^d: \; \forall b \in \mathcal{A}_\varepsilon(\theta,x), \; \mu^{\top}\gamma^x_{a,b}\leq-\varepsilon \right\rbrace$ and $\gamma^x_{a,b} = \phi_{x,b}- \phi_{x,a}$. Hence, we can write
\begin{equation*}
    \psi_\varepsilon(\theta, \alpha) = \min_{x\in\mathcal{X}}\min_{a\in \mathcal{A}^c_\varepsilon(\theta,x)} \inf_{\mu \in B_{\varepsilon}(\theta, x, a)} \|\theta - \mu\|^2_{A(\alpha)}.
\end{equation*}
Define $\omega = \theta-\mu$, and rewrite the constraint as 
$$ \mu^{\top}\gamma^x_{a,b} \leq -\varepsilon  \iff \omega^{\top}\gamma^x_{a,b} > (\theta^{\top}\gamma^x_{a,b}  + \varepsilon) .$$ 
Formulate the optimization problem
\begin{equation}
\label{eq:linear_prog}
    \begin{aligned} 
    & \inf \frac{1}{2} \omega^\top A(\alpha) \omega \\  &\text{s.t. } \forall b \in \mathcal{A}_\varepsilon(\theta,x),\; \omega^{\top}
    \gamma^x_{a,b} \geq \theta^{\top} \gamma^x_{a,b} + \varepsilon.
    \end{aligned}
\end{equation}
Note that the problem in \eqref{eq:linear_prog} is a Quadratic Program with $|\mathcal{A}_\varepsilon(\theta,x)|$ linear constraints. Although the problem can be solved numerically in an efficient way (e.g. by active set methods, interior point methods, etc.), the solution cannot be easily expressed in closed form. To find a closed-form solution we define for $a\in \mathcal{A}_\varepsilon^c(\theta,x)$ the set  $\mathcal{A}_\varepsilon(\theta,x,a) = \{b\in \mathcal{A}_\varepsilon(\theta,x): \theta^\top (\phi_{x,b}-\phi_{x,a}) > \varepsilon\}$. In order to get a closed form solution we instead focus on solving a relaxed problem. Take a different decomposition of the set of confusing parameters as
\begin{align*}
B_{\varepsilon}(\theta) & = \bigcup_{x\in \mathcal{X}} \bigcup_{a\in \mathcal{A}^c_\varepsilon(\theta,x)} \left\lbrace \mu \in \mathbb{R}^d: \; \forall b \in \mathcal{A}_\varepsilon(\theta,x), \; \mu^{\top}(\phi_{x,a}- \phi_{x,b})>\varepsilon \right\rbrace \\ & \subseteq  \bigcup_{x\in \mathcal{X}} \bigcup_{a\in \mathcal{A}^c_\varepsilon(\theta,x)} \left\lbrace \mu \in \mathbb{R}^d: \; \exists b \in \mathcal{A}_\varepsilon(\theta,x,a), \; \mu^{\top}(\phi_{x,a}- \phi_{x,b})>\varepsilon \right\rbrace \\ & =  \bigcup_{x\in \mathcal{X}} \bigcup_{a\in \mathcal{A}^c_\varepsilon(\theta,x)} \bigcup_{b\in \mathcal{A}_\varepsilon(\theta,x,a)} \left\lbrace \mu \in \mathbb{R}^d: \mu^{\top}(\phi_{x,a}- \phi_{x,b})>\varepsilon \right\rbrace.
\end{align*}
Hence we have for $\bar{B}_\varepsilon(\theta,x,a) = \left\lbrace \mu \in \mathbb{R}^d: \; \exists b \in \mathcal{A}_\varepsilon(\theta,x), \; \mu^{\top}\gamma^x_{a,b}\leq-\varepsilon \right\rbrace$, 
$$  \bar{\psi}^\star_\varepsilon(\theta) = \sup_{\alpha\in\Lambda}\min_{x\in\mathcal{X}}\min_{a\in \mathcal{A}^c_\varepsilon(\theta,x)} \inf_{\mu \in \bar{B}_{\varepsilon}(\theta, x, a)} \|\theta - \mu\|^2_{A(\alpha)} \leq \psi^\star_\varepsilon(\theta),$$
%so that the lower bound can be written as 
%$$
%\mathbb{E}_\theta[\tau] \bar{\psi}^\star_\varepsilon(\theta)\geq \mathrm{kl}(1- \delta, \delta).
%$$
%The optimization problem becomes for $a\in\mathcal{A}^c_\varepsilon(\theta,x)$

\begin{equation*}
    \begin{aligned} 
    & \inf \frac{1}{2} \omega^\top A(\alpha) \omega \\  &\text{s.t. } \exists b \in \mathcal{A}_\varepsilon(\theta,x),\; \omega^{\top}
    \gamma^x_{a,b} \geq \theta^{\top} \gamma^x_{a,b} + \varepsilon.
    \end{aligned}
\end{equation*}
Let $\gamma = \gamma_{a,b}^x$, and define the Lagrangian of this optimization problem is
$$L(\omega, \rho) = \frac{1}{2}\omega^{\top} A(\alpha) \omega+\rho\left(-\gamma^{\top} \omega+\gamma^\top\theta + \varepsilon\right),$$
with Lagrange multipliers $\rho \in \mathbb{R}$. Imposing the optimality conditions leads to the system
\begin{equation}
\begin{cases}
    \frac{\partial L}{\partial \omega} = A(\alpha)\omega-\rho \gamma=0 \Leftrightarrow A(\alpha) \omega= \rho\gamma \\ 
    \rho\frac{\partial L}{\partial \rho}=\rho(-\gamma^{\top} \omega+\gamma^{\top} \theta + \varepsilon)=0 
    \\ \gamma^\top\omega \geq \gamma^\top \theta
    \\ \rho \geq 0
\end{cases}.
\label{eq:KKT_approx_delta_pac}
\end{equation}
Let $\rho\neq 0 \Rightarrow (-\gamma^{\top} \omega+\gamma^{\top} \theta + \varepsilon)=0 $. For $A(\alpha) \succ 0$, solving for $\omega$ in the first  of the Eq. in \eqref{eq:KKT_approx_delta_pac} and substituting in the second of the Eq. in \eqref{eq:KKT_approx_delta_pac}, we get
$$\rho = \frac{\gamma^\top\theta + \varepsilon}{\|\gamma\|^2_{A(\alpha)^{-1}}}. $$
Note that $\rho > 0$, thus we have a feasible solution to the optimization problem.
We have $$\frac{1}{2}\omega^\top A(\alpha)\omega = \frac{(\gamma^\top \theta + \varepsilon)^\top\gamma^\top A(\alpha)^{-1}A(\alpha)A(\alpha)^{-1}\gamma(\gamma^\top \theta + \varepsilon)}{2\|\gamma\|_{A(\alpha)^{-1}}^4}= \frac{(\gamma^\top \theta + \varepsilon)^\top\gamma^\top A(\alpha)^{-1}\gamma(\gamma^\top \theta + \varepsilon )}{\|\gamma\|_{A(\alpha)^{-1}}^4} = \frac{(\gamma^\top \theta +\varepsilon)^2 }{2\|\gamma\|^2_{A(\alpha)^{-1}}}.$$
Hence we get
\begin{align*}
    \bar{\psi}_\varepsilon(\theta,\alpha) = \inf_{\mu \in \hat{B}_\varepsilon(\theta, x, a)} \frac{1}{2} \|\theta - \mu\|^2_{A(\alpha)} =
     \begin{cases}
    \frac{ (\theta^\top\gamma^x_{a,b}+\varepsilon)^2}{2{\gamma_{a,b}^x}\top A(\alpha)^{-1} \gamma^x_{a,b}} & \text{ if } A(\alpha) \succ 0 \\
    0 &\text{ otherwise}
    \end{cases},
\end{align*}
Thus we may conclude that $\mathbb{E}_\theta[\tau] \gtrsim T^\star_{\theta,\varepsilon}\log\left(\frac{1}{\delta}\right)$ with

$$
    (T^\star_{\theta,\varepsilon})^{-1} = \begin{cases} \sup\limits_{\alpha\in\Lambda}\min\limits_{x\in \mathcal{X}} \min\limits_{a\in \mathcal{A}_\varepsilon^{c}(\theta,x)}\min\limits_{b\in \mathcal{A}_\varepsilon(\theta,x,a)} \frac{ (\theta^\top(\phi_{x,b}- \phi_{x,a})+\varepsilon)^2}{2(\phi_{x,b}- \phi_{x,a})^\top A(\alpha)^{-1} (\phi_{x,b}- \phi_{x,a})} & \text{ if } A(\alpha) \succ 0 \\
    0 & \text{ otherwise}
    \end{cases}.
$$
\end{proof}

\subsection{Proof of Theorem \ref{theorem:off_policy_lb}}
\begin{proof}
The proof follow closely the proof of Theorem \ref{theorem:lb_eps_delta_discrete}. 
The main differences are the following:
\begin{enumerate}
    \item At step $1$ (the log-likelihood ratio), we consider the log-likelihood ratio $ L_T^{\theta,\mu}$ between $\theta, \mu \in U$.
    \item At step $2$ (the change of measure argument),
    the set of confusing parameters is 
\begin{align*}
B_{\varepsilon}(\theta) & = \left\lbrace \mu \in U: \exists x \in \mathcal{X}, \forall b \in \mathcal{A}_\varepsilon({\theta},x), \; \mu^{\top}(\phi_{x,a_{\mu}^\star(x)}- \phi_{x,b})>\varepsilon \right\rbrace,
\end{align*}
and similarly, it holds
$$
\forall {\mu} \in B_\varepsilon({{\theta}}) \qquad \mathbb{E}\left[ L_\tau^{{\theta},{\mu}} \right] \ge \mathrm{kl}\left(1- \delta, \delta \right). 
$$
\item At step $5$ (solution to the optimization problem), when the invertibility of $A(\alpha)$ is required, we consider the pseudo-inverse $A(\alpha)^\dagger$. The condition $\text{dim}(U) > 0$ is required in order to avoid singularities. The solution to the optimization problem is similar to the one in the proof of Theorem \ref{theorem:lb_eps_delta_discrete}, with the exception that the condition for the invertibility in the solution to the optimization problem is ${\omega} =({\mu} - {\theta}) \in\Span(\Phi_\alpha)$.
\end{enumerate}
\end{proof}
\begin{comment}
\subsection{Proof of Lemma \ref{lem:T_star_scaling_delta_pac}}
The lemma follows naturally from the application of the Kiefer-Wolfowitz equivalence Theorem in \cite{Kiefer60}. 
We have 
\begin{align*}
T^\star_\theta & = \inf_{\alpha\in\Lambda}\max_{x\in\mathcal{X}}\max_{a\in\mathcal{A}\setminus 
\{a^\star_\theta(x)\}}\frac{\|\gamma_{x,a}\|^2_{A(\alpha)^{-1}}}{\Delta_{x,a}^2} \\&\leq \inf_{\alpha\in\Lambda}\max_{x\in\mathcal{X}}\max_{a\in\mathcal{A}\setminus\{a^\star_\theta(x)\}}\frac{\|\gamma_{x,a}\|^2_{A(\alpha)^{-1}}}{\Delta_{\min}^2} \\&\leq \inf_{\alpha\in\Lambda}\max_{x\in\mathcal{X}}\max_{a\in\mathcal{A}\setminus\{a^\star_\theta(x)\}}\frac{4\|\phi_{x,a}\|^2_{A(\alpha)^{-1}}}{\Delta_{\min}^2}  \leq \frac{4d}{\Delta_{\min}^2}.
\end{align*}
\end{comment}

\subsection{Proof of Lemma \ref{lem:T_star_scaling_eps_delta_pac}}
\begin{proof}
The lemma follows naturally from the application of the Kiefer-Wolfowitz equivalence Theorem in \cite{Kiefer60} and generalize Proposition $3$ from Soare et al. \cite{Soare15} in the LB case. For $\varepsilon>0$, we have
\begin{align*}
T^\star_{\theta,\varepsilon}& = \inf_{\alpha\in\Lambda} \max_{x\in\mathcal{X}}\max_{a\not \in \mathcal{A}_\varepsilon(\theta,x)}\max_{b\in \mathcal{A}_\varepsilon(\theta,x,a)}\frac{\|\gamma^x_{a,b}\|^2_{A(\alpha)^{-1}}}{(\theta^\top\gamma^x_{a,b}+\varepsilon)^2} \\&\leq \inf_{\alpha\in\Lambda}\max_{x\in\mathcal{X}}\max_{a\not \in \mathcal{A}_\varepsilon(\theta,x)}\max_{b\in \mathcal{A}_\varepsilon(\theta,x,a)}\frac{\|\gamma^x_{a,b}\|^2_{A(\alpha)^{-1}}}{4\varepsilon^2} \\&\leq \inf_{\alpha\in\Lambda}\max_{x\in\mathcal{X}}\max_{a\not \in \mathcal{A}_\varepsilon(\theta,x)}\frac{4\|\phi_{x,a}\|^2_{A(\alpha)^{-1}}}{4\varepsilon^2} \leq \frac{d}{\varepsilon^2}.
\end{align*}
For $\varepsilon = 0$, we have 
\begin{align*}
T^\star_{0,\theta} & = \inf_{\alpha\in\Lambda} \max_{x\in\mathcal{X}}\max_{a\neq a^\star_\theta(x)}\frac{\|\gamma^x_{a,a^\star_\theta(x)}\|^2_{A(\alpha)^{-1}}}{(\theta^\top\gamma^x_{a,a^\star_\theta(x)})^2} \\&\leq \inf_{\alpha\in\Lambda}\max_{x\in\mathcal{X}}\max_{a\neq a^\star_\theta(x)}\frac{\|\gamma^x_{a,a^\star_\theta(x)}\|^2_{A(\alpha)^{-1}}}{\Delta_{\min}^2} \\&\leq \inf_{\alpha\in\Lambda}\max_{x\in\mathcal{X}}\frac{4\|\phi_{x,a}\|^2_{A(\alpha)^{-1}}}{\Delta_{\min}^2} \leq \frac{4d}{\Delta_{\min}^2}.
\end{align*}
\end{proof}

\subsection{Proof of Lemma \ref{lem:properties_eps_delta}}
\begin{proof}

\textit{1) Continuity of $\psi_\varepsilon$:} 
Let $(\theta_t,\alpha_t)_{t\geq 1}$ be a sequence taking values in $\mathbb{R}^d\times \Lambda$, and converging to $(\theta,\alpha)$. Recall the definition of set of confusing parameters 
$$
 B_\varepsilon(\theta) = {\left\lbrace \mu\in\mathbb{R}^d: \exists x \in \mathcal{X}, \forall b \in \mathcal{A}_\varepsilon(\theta,x), \; \mu^{\top}(\phi_{x,a_{\mu}^\star(x)}- \phi_{x,b})>\varepsilon \right\rbrace}
$$
Since $(\theta_t,\alpha_t)$ converges to  $(\theta,\alpha)$, there exists $\upsilon < \varepsilon$, such that for some $t_1 \geq 1: \forall t\geq t_1$, $\|(\theta,\alpha) - (\theta_t,\alpha_t) \| <\upsilon$. Also, since $\mathcal{A}_\varepsilon(\theta,x)$ is defined as an open set $\forall x\in\mathcal{X}$, we have $B_\varepsilon(\theta) = B_\varepsilon(\theta_t)$. 
Now, define $g_\mu(\theta,\alpha) \triangleq \|\mu - \theta\|^2_{A(\alpha)}$, and note that $g_\mu(\theta,\alpha)$ is a polynomial in $(\theta,\alpha)$, and hence is continuous. As a consequence, there exist $
t_2\geq 1: \forall t \geq t_2$, 
$ |g_\mu(\theta,\alpha)- g_\mu(\theta_t,\alpha_t)| \leq \upsilon g_\mu(\theta,\alpha)$.  With our choice of $\upsilon$ and for $t\geq \max\{t_1,t_2\}$, we get
\begin{align*}
\left|\psi_\varepsilon(\theta,\alpha)-\psi\left(\mu_{t}, \alpha_{t}\right)\right| &=\left|\min_{\mu \in B_\varepsilon(\theta)} g_\mu(\theta, \alpha)-\min_{\mu \in B_\varepsilon(\theta)} g_\mu\left(\theta_t, \alpha_t\right)\right| 
\\ & \leq \upsilon\left|\min_{\mu \in B_\varepsilon(\theta)} g_\mu(\theta, \alpha)\right| 
\\ & \leq \upsilon|\psi_\varepsilon(\theta,\alpha)|.
\end{align*}

\textit{2) Invertibility of $A(\alpha_\theta^\star)$:}
By continuity of $\psi_\varepsilon$ in $\alpha$ and compactness of $\Lambda$, there exists $\alpha_\theta^\star \in \argsup_{\alpha \in\Lambda} \psi_\varepsilon(\theta,\alpha)$.
To verify that $A(\alpha_\theta^\star) \succ 0$, note that $\forall \mu \in B_\varepsilon(\theta)$. Since by assumption we have $\Span(\Phi) = \mathbb{R}^d$ and $\forall x \in\mathcal{X}$ $p_\mathcal{X}(x) >0$, we may construct an allocation $\tilde{\alpha} \in \Lambda$ such that $A(\tilde{\alpha}) \succ 0$.

\textit{3) Convexity, Compactness and Upper Hemicontinuity of $C^\star_\varepsilon(\theta)$ \& 4) Continuity of $\psi_\varepsilon^\star$ in $\theta$:} The result follows from an application of Berge's Theorem \cite{Berge63}. Since $\psi_\varepsilon$ is continuous in $(\theta,\alpha)$, $\Lambda$ is compact, convex, and non-empty, and $\psi_\varepsilon$ is concave in $\alpha$ for any $\theta'\in\mathbb{R}^d$ in an open neighborhood of $\theta'$. Hence the hypothesis of Berge's Theorem are satisfied and the result follows.
\end{proof}

\subsection{Proof of Lemma
\ref{lem:Nx_concentration_tight}}
\begin{proof}
The proof of this concentration results follows directly by the application of Theorem 3.5 in \cite{iosif_concentration}. Define $N_t-tp_\mathcal{X}=\sum_{s = 1}^t J_s,$
where $N_t$ is the random vector in $\mathbb{N}^{|\mathcal{X}|}$ with coordinates $N_t(x)$ for $x\in\mathcal{X}$, $p_\mathcal{X}$ is the vector with coordinates $p_\mathcal{X}(x)$ that lies in $\Lambda_\mathcal{X} = \{p_{\mathcal{X}}(x) \in[0,1]^{|\mathcal{X}|}: \sum_{x\in\mathcal{X}} p_\mathcal{X}(x) = 1\}$, and 
the $J_i$'s are i.i.d. zero-mean random vectors in $\mathbb R^{|\mathcal{X}|}$ with coordinates $J_s(x)=\mathbbm{1}\{x_s = x\} - p_\mathcal{X}(x)$ for $x\in \mathcal{X}$. We have 
$$\|J_s\|_2^2=\sum_{x\in\mathcal{X}}(\mathbbm{1}\{x_s=x\}-p_\mathcal{X}(x))^2
\le \sum_{x\in\mathcal{X
}}(\mathbbm{1}\{x_s=x\}+p_\mathcal{X}(x)^2) = 1+\sum_{x\in\mathcal{X}}p_\mathcal{X}(x)^2\le2.$$
Hence the assumption of Theorem 3.5 in  \cite{iosif_concentration} are satisfied with $r=t\varepsilon$, $D=1$, and $b_*^2=2t$, and we get
\begin{align*}
\mathbb{P}\left(\max_{x\in\mathcal{X}}\left|\frac{1}{t}\, N_t(x)-p_\mathcal{X}(x)\right|\ge\varepsilon\right) & = \mathbb{P}\left(\max_{x\in\mathcal{X}}\left|N_t(x)-tp_\mathcal{X}(x)\right|\ge t\varepsilon\right) \\& = \mathbb{P}\left(\|N_t-t p_\mathcal{X}\|_\infty \geq t\varepsilon\right) 
\\& \leq \mathbb{P}\left(\|N_t-t p_\mathcal{X}\|_2 \geq t\varepsilon\right) \\& \leq e^{-t\varepsilon^2/4}. 
\end{align*}
\end{proof}

\subsection{Proof of Lemma \ref{lem:stopping_rule_eps_delta_pac}}
\begin{proof}
Under the Gaussian noise assumption $f^{\theta}\left(r_{t}, a_{t}, x_{t} \ldots, r_{1}, a_{1}, x_{1}\right) \propto \exp \left(-\frac{1}{2} \sum_{s=1}^{t}\left(r_{s}-\theta^{\top} \phi_{x_s,a_s}\right)^{2}\right).$ By \cite[Lemma 7]{Jedra20}, we may write $Z^x_{a, b,\varepsilon}(t)$ in closed form as:
\begin{equation*}
Z^x_{a, b,\varepsilon}(t)=\operatorname{sign}\left(\hat{\theta}_{t}^{\top}(\phi_{x,a}-\phi_{x,b})+\varepsilon\right) \frac{\left(\hat{\theta}_{t}^{\top}(\phi_{x,a}-\phi_{x,b})+\varepsilon\right)^{2}}{2(\phi_{x,a}-\phi_{x,b})^{\top}\left(\sum_{s=1}^{t} \phi_{x_s,a_s}\phi_{x_s,a_s}^{\top}\right)^{-1}(\phi_{x,a}-\phi_{x,b})}, 
        \end{equation*}
where $\hat{\theta}_t$ is the LS estimator defined in \eqref{eq:LS_estimator}. Recall that, since $Z_\varepsilon^x(t) = \max_{a \in \mathcal{A}_\varepsilon(\hat{\theta}_t,x)} \min_{b \neq a} Z^x_{a, b, \varepsilon}(t)$ and $\hat{a}_t(x) \in \argmax_{a \in \mathcal{A}_\varepsilon(\hat{\theta}_t,x)} \min_{b \neq a} Z^x_{a, b, \varepsilon}(t) $, we have $\forall x \in\mathcal{X}$,
$$\min_{b \neq \hat{a}_t(x)}Z^x_{\hat{a}_t(x), b, \varepsilon}(t) \geq \max_{a \in \mathcal{A}_\varepsilon(\hat{\theta}_t,x)} \min_{b \neq a} Z^x_{a,b,\varepsilon}(t).$$
Define the event
\begin{align*}\mathcal{E}& = \left\{\exists t, \exists x: Z_\varepsilon^x(t)>\beta(\delta, t)\text{ and }  \theta^\top(\phi_{x,a^\star_\theta(x)} - \phi_{x,\hat{a}_t(x)})>\varepsilon  \text{ and } \sum_{s=1}^{t} \phi_{x_s,a_{s}}\phi_{x_s,a_{s}}^{\top} \succeq c I_{d} \right\} 
\\ & = \left\{\exists t,\exists x: \max_{a \in \mathcal{A}_\varepsilon(\hat{\theta}_t,x)} \min_{b \neq a} Z^x_{a, b, \varepsilon}(t) >\beta(\delta,t) \text{ and } \theta^\top(\phi_{x,a^\star_\theta(x)} - \phi_{x,\hat{a}_t(x)})>\varepsilon \text{ and } \sum_{s=1}^t\phi_{x_s,a_s}\phi_{x_s,a_s}^{\top} \succeq c I_{d}\right\}\\ & \subseteq  \left\{\exists t, \exists x: Z_{\hat{a}_t(x),  a^\star_\theta(x),\varepsilon}^x >\beta(\delta,t) \text{ and } \theta^\top(\phi_{x,a^\star_\theta(x)} -\phi_{x,\hat{a}_t(x)})>\varepsilon \text{ and } \sum_{s=1}^t\phi_{x_s,a_s}\phi_{x_s,a_s}^{\top} \succeq c I_{d}\right\}.
\end{align*}
On the event $\mathcal{E}$, it holds $\exists x\in\mathcal{X} : \hat{\theta}_t^\top(\phi_{x,\hat{a}_t(x)}-\phi_{x,a^\star_\theta(x)})\geq -\varepsilon$ and $\theta^\top(\phi_{x,\hat{a}_t(x)}-\phi_{x,a^\star_\theta(x)} )<
-\varepsilon$. Thus
\begin{align*}
    &\max\limits_{\left\{\mu: \mu^{\top}(\phi_{x,\hat{a}_t(x)}-\phi_{x,a^\star_\theta(x)}) \geq -\varepsilon\right\}} f^{\mu}\left(r_{t}, a_{t}, x_{t} \ldots, r_{1}, a_{1},x_{1}\right)= f^{\hat{\theta}}\left(r_{t}, a_{t}, x_{t} \ldots, r_{1}, a_{1},x_{1}\right),\\ 
    &\max\limits_{\left\{\mu: \mu^{\top}(\phi_{x,\hat{a}_t(x)}-\phi_{x,a^\star_\theta(x)}) \leq -\varepsilon \right\}} f^{\mu}\left(r_{t}, a_{t}, x_{t} \ldots, r_{1}, a_{1},x_{1}\right) \geq f^{\theta}\left(r_{t}, a_{t}, x_{t} \ldots, r_{1}, a_{1},x_{1}\right).
\end{align*}

\begin{align*}
 Z^x_{\hat{a}_t(x),a^\star_\theta(x),\varepsilon} &= \log \left(\frac{\max\limits_{\left\{\mu: \mu^{\top}(\phi_{x,\hat{a}_t(x)}-\phi_{x,a^\star_\theta(x)}) \geq -\varepsilon\right\}} f^{\mu}\left(r_{t}, a_{t}, x_{t} \ldots, r_{1}, a_{1},x_{1}\right)}{\max\limits_{\left\{\mu:\mu^{\top}(\phi_{x,\hat{a}_t(x)}-\phi_{x,a^\star_\theta(x)}) \leq -\varepsilon\right\}} f^{\mu}\left(r_{t}, a_{t}, x_{t} \ldots, r_{1}, a_{1}, x_{1}\right)}\right) \\& \leq \log \left(\frac{f^{\hat{\theta}_t}(r_{t}, a_{t}, x_{t} \ldots, r_{1}, a_{1})}{f^{\theta}(r_{t}, a_{t}, x_{t} \ldots, r_{1}, a_{1})}\right) \\&= \frac{1}{2} \| \theta - \hat{\theta}_t\|^2_{\sum_{s=1}^t \phi_{x_s,a_s}\phi_{x_s,a_s}^\top}. 
\end{align*}
Hence $ \mathcal{E} \subseteq \left\{\exists t\in\mathbb{N}^*,\exists x \in\mathcal{X}: \frac{1}{2} \| \theta - \hat{\theta}_t\|^2_{\sum_{s=1}^t \phi_{x_s,a_s}\phi_{x_s,a_s}^\top} >\beta(\delta,t) \text{ and } \sum_{s=1}^t\phi_{x_s,a_s}\phi_{x_s,a_s}^{\top} \succeq c I_{d}\right\}.$ The rest of the proof would go along the same line as \cite[Prop. 2]{Jedra20}. We note that for any $u>0$, $(1+u)(\sum_{s=1}^t\phi_{x_s,a_s}\phi_{x_s,a_s}^{\top} + cu I_d)^{-1} \succeq (\sum_{s=1}^t\phi_{x_s,a_s}\phi_{x_s,a_s}^{\top})^{-1}$. Hence
$$
\|\hat{\theta}_{t}-\theta\|_{\sum_{s=1}^t\phi_{x_s,a_s}\phi_{x_s,a_s}^{\top}}^{2}=\left\|\sum_{s=1}^{t} \phi_{x_s,a_{s}} \xi_{s}\right\|^{2}_{\left( \sum_{s=1}^t\phi_{x_s,a_s}\phi_{x_s,a_s}^{\top}\right)^{-1}} \leq(1+u)\left\|\sum_{s=1}^{t} \phi_{x_s,a_s} \xi_{s}\right\|_{\left(\sum_{s=1}^{t} \phi_{x_s,a_{s}} \phi_{x_s,a_{s}}^{\top}+u c I_{d}\right)^{-1}}^{2}.
$$
This implies 
$\mathcal{E}\subseteq\left\{\exists t \in \mathbb{N}^{*},\exists x \in\mathcal{X}:  \frac{1}{2}(1+u)\left\|\sum_{s=1}^{t} \phi_{x_s,a_s} \xi_{s}\right\|_{\left(\sum_{s=1}^{t} \phi_{x_s,a_{s}} \phi_{x_s,a_{s}}^{\top}+u c I_{d}\right)^{-1}}^{2} \geq \beta(\delta, t)\right\},$
and with the choice 
$$
\beta(\delta, t)=(1+u) \sigma^{2} \log \left(\frac{\operatorname{det}\left((u c)^{-1} \sum_{s=1}^{t} \phi_{x_s,a_{s}} \phi_{x_s,a_{s}}^{\top}+I_{d}\right)^{1 / 2}}{\delta}\right),
$$
it follows directly from \cite[Lemma 9]{Abbasi11} that $\mathbb{P}[\mathcal{E}] \leq \delta.$

\end{proof}


\subsection{Proof of Lemma \ref{lem:forced_exploration}}
\label{app:proof_forced_expl_delta}
The proof of this lemma is similar to that of the forced exploration for LB presented in \cite[Lemma 5]{Jedra20}, but there are crucial differences. As opposed to the deterministic result proved in \cite{Jedra20}, due to the random nature of the context arrivals and the fact that the feature vectors for context $x$ spans a different subspace of dimension $d_x \leq d$, the forced exploration may not be guaranteed at each time step. Hence, we prove a probabilistic (and stronger) result on the growth of the minimum eigenvalue by leveraging Lemma \ref{lem:Nx_concentration_tight}.

\begin{proof}
Let $t>0$, and for all $x\in\mathcal{X}$ define $\mathcal{I}_{x}(t) = \{i_k\in [1,t]:x_{i_k} = x\}$, the indices at which context $x$ is observed, with $k\in\{1,\dots,N_x(t)\}$. Note that, for all $x\in\mathcal{X}$, we have $d_x = \inf \{k>0: \sum_{j=1}^{k} \phi_{x,a_{i_j}} \phi_{x,a_{i_j}}^\top \succeq f_x(t)\}$. Fix an $x$, and assume there exists $k_0(x) > d_x$ such that 
$$\sum_{j=1}^{k_0(x)}\phi_{x,a_{i_j}}\phi_{x,a_{i_j}}^\top \succeq f_x(k_0(x)) \text{ and } \sum_{j=1}^{k_0(x)+1}\phi_{x,a_{i_j}}\phi_{x,a_{i_j}}^\top \prec f_x(k_0(x)+1).$$
Define $k_1(x) = \inf \left\{k>k_0(x): \sum_{j=1}^{k} \phi_{x,a_{i_j}} \phi_{x,a_{i_j}}^\top \succeq f_x(k)\right\}$, and note that for all $k$ such that $k_0(x) \leq k \leq k_1(x)$, we have
$$\sum_{j=1}^k\phi_{x,a_{i_j}}\phi_{x,a_{i_j}}^\top \succeq \sum_{j=1}^{k_0(x)}\phi_{x,a_{i_j}}\phi_{x,a_{i_j}}^\top \succeq f(k_0(x)).$$
Let $C_x = \frac{1}{\sqrt{d_x}}\sum_{a_x \in \mathcal{A}_x} \phi_{x,a_x} \phi_{x,a_x}^{\top}$. For $k_1(x)\geq k_0(x)+d_x+1$, we have
\begin{equation*}
\begin{aligned}
\sum_{j=1}^{k_{1}(x)} \phi_{x,a_{i_j}} \phi_{x,a_{i_j}}^{\top} & \succeq \sum_{j=1}^{k_{0}(x)+d_x+1} \phi_{x,a_{i_j}} \phi_{x,a_{i_j}}^{\top} \\
& \succeq \sum_{j=1}^{k_{0}(x)+1} \phi_{x,a_{i_j}} \phi_{x,a_{i_j}}^{\top}+\sum_{a_x \in \mathcal{A}_x} \phi_{x,a_x} \phi_{x,a_x}^{\top} \\
&=\sum_{j=1}^{k_{0}(x)+1} \phi_{x,a_{i_j}} \phi_{x,a_{i_j}}^{\top}+C_x\sqrt{d_x} \\
& \succeq \sum_{j=1}^{k_{0}(x)} \phi_{x,a_{i_j}} \phi_{x,a_{i_j}}^{\top}+C_x \sqrt{d_x} \\
& \succeq f_x\left(k_{0}(x)\right)+C_x \sqrt{d_x}.
\end{aligned}
\end{equation*}
However, we have
$$
k_{0}(x) \geq \frac{1}{4}\left(d_x+\frac{1}{d_x}+2\right) \Longrightarrow \sqrt{k_{0}(x)+d_x+1}+\sqrt{k_{0}(x)} \geq \sqrt{d_x}+\frac{1}{\sqrt{d_x}} \Longrightarrow f_x\left(k_{0}(x)\right)+C_x \sqrt{d_x} \succeq f_x\left(k_{0}(x)+d_x+1\right) .
$$
Therefore, if $k_{0}(x) \geq \frac{1}{4}\left(d_x+\frac{1}{d_x}+2\right),$ then it holds that $k_{1}(x) \leq k_{0}(x)+d_x+1$. In other words, we have shown that for all $N_x(t) \geq \frac{1}{4}\left(d_x+\frac{1}{d_x}+2\right)+d_x+1,$ we have
$$\sum_{k=1}^{N_x(t)} \phi_{x,a_{i_k}}\phi_{x,a_{i_k}}^{\top} \succeq C_x\sqrt{N_x(t)-d_x-1}
$$
Let $t_0 = \inf\left\{t\geq 0: \forall x\in\mathcal{X}, N_x(t) \geq \frac{1}{4}\left(d_x+\frac{1}{d_x}+2\right)+d_x+1\right\}$ and denote $p_{\min} = \min\limits_{x\in\mathcal{X}}p_\mathcal{X}(x)$. By Lemma \ref{lem:Nx_concentration_tight}, $\forall \varepsilon \in\left(0,p_{\min}\right)$ and $\forall t\geq t_0$, we get
$$
\mathbb{P}_\theta\left( \sum_{k=1}^{N_x(t)} \phi_{x,a_{i_k}}\phi_{x,a_{i_k}}^{\top} \succeq  C_x\sqrt{(p_\mathcal{X}(x)-\varepsilon)t - d_x - 1}\right) \geq 1-2 e^{-\frac{t\varepsilon^2}{4}}.
$$
Hence, w.p. at least $1-2 e^{-\frac{t\varepsilon^2}{4}}$, we get
\begin{align*}
\sum_{s = 1}^t\phi_{x_s,a_s}\phi_{x_s,a_s}^\top & = \sum_{x \in \mathcal{X}}\sum_{i_k \in\mathcal{I}_x }\phi_{x,a_{i_k}}\phi_{x,a_{i_k}}^\top 
\\ & \succeq \sum_{x \in \mathcal{X}} \left(C_x\sqrt{(p_\mathcal{X}(x)-\varepsilon)t-d_x-1} \right)
\\ & = \sum_{x\in\mathcal{X}}\sqrt{\frac{(p_\mathcal{X}(x)-\varepsilon)t-(d_x+1)}{d_x}}   \sum_{a_x \in \mathcal{A}_x} \phi_{x,a_x}\phi_{x,a_x}^{\top}
\\ & \succeq \sum_{x\in\mathcal{X}}\sqrt{\frac{(p_\mathcal{X}(x)-\varepsilon)t-(d_x+1)}{d_x}}  cI_d. 
\\ & \succeq \min_{x\in\mathcal{X}}\sqrt{\frac{(p_\mathcal{X}(x)-\varepsilon)t-(d_x+1)}{d_x}}  cI_d. 
\end{align*}
Now, let $x^\star = \arg\min_{x\in\mathcal{X}} \sqrt{\frac{(p_\mathcal{X}(x)-\varepsilon)t-(d_x+1)}{d_x}}$,  $0<\kappa< c\sqrt{\frac{p_\mathcal{X}(x^\star)-\varepsilon}{d_{x^\star}}}$, and $t_0' = \left\{\inf t: t \geq \left(\frac{\sqrt{\frac{d_{x^\star}+1}{d_x}}}{\sqrt{\frac{p_\mathcal{X}(x^\star)-\varepsilon}{d_{x^\star}}}-\kappa}\right)^2 \right\}$.
We have that for any 
$t\geq t_1 = \max\{t_0,t_0'(\kappa)\}$ we have  $\sqrt{\frac{(p_\mathcal{X}({x^\star})-\varepsilon)t-(d_{x^\star}+1)}{d_{x^\star}}} \geq \frac{\kappa}{c}\sqrt{t}$.
Hence, we have proved that $\exists t_1,\kappa: \forall t \geq t_1$ we have that     
$$
\mathbb{P}_\theta\left( \frac{1}{\sqrt{t}}\sum_{s = 1}^t\phi_{x_s,a_s}\phi_{x_s,a_s}^\top\succeq \kappa I_d\right) \geq 1-2 e^{-\frac{t\varepsilon^2}{4}}.
$$
\end{proof}

%\subsection{Proof of Corollary \ref{cor:Z}}
%Recall the expression of $\hat{O}_\varepsilon(\theta,x) = \{b\in\mathcal{A}: \max_{a\in\mathcal{A}}\hat{\theta}_t^\top (a-b) < \varepsilon\}$


\begin{comment}
\subsection{Proof of Lemma \ref{lem:stopping_rule_delta_pac}}
\begin{proof}
\label{app:proof_stopping_rule_delta_pac}
Under the Gaussian noise assumption $f^{\theta}\left(r_{t}, a_{t}, x_{t} \ldots, r_{1}, a_{1}, x_{1}\right) \propto \exp \left(-\frac{1}{2} \sum_{s=1}^{t}\left(r_{s}-\theta^{\top} \phi_{x_s,a_s}\right)^{2}\right).$ By Lemma \ref{lem:closed_form_Z}, we may write $Z^x_{a, b,\varepsilon}(t)$ in closed form as:
\begin{equation*}
Z^x_{a, b}(t)=\operatorname{sign}\left(\hat{\theta}_{t}^{\top}(\phi_{x,a}-\phi_{x,b})\right) \frac{\left(\hat{\theta}_{t}^{\top}(\phi_{x,a}-\phi_{x,b})\right)^{2}}{2(\phi_{x,a}-\phi_{x,b})^{\top}\left(\sum_{s=1}^{t} \phi_{x_s,a_s}\phi_{x_s,a_s}^{\top}\right)^{-1}(\phi_{x,a}-\phi_{x,b})},
\end{equation*}
where $\hat{\theta}_t$ is the LS estimator defined in \eqref{eq:LS_estimator}. Also, by Corollary 1 in \cite{Jedra20} it holds that $\forall x \in\mathcal{X}$ $$Z^x(t) = \max_{a\in\mathcal{A}}\min_{b\in\mathcal{A}\setminus\{a\}} = \min_{b\in\mathcal{A}\setminus\{\hat{a}_t(x)\}}Z_{\hat{a}(x),b}^x(t).$$

Define 
$\mathcal{E} \triangleq \left\{\exists t \in\mathbb{N}^*, \exists x\in\mathcal{X}: Z^x(t)>\beta(\delta, t) \text{ and }  a^\star_\theta(x) \neq \hat{a}_t(x)\text{ and } \sum_{s=1}^{t} \phi_{x_s,a_{s}}\phi_{x_s,a_{s}}^{\top} \succeq c I_{d}\right \},$ and note that %We need to show that $\mathbb{P}_{\theta}[\mathcal{E}] \leq \delta.$ 
\begin{align*}
\mathcal{E} & =\left\{ \exists t, \exists x:  Z^x(t) >\beta(\delta,t) \text{ and }  a^\star_\theta(x) \neq \hat{a}_t(x) \text{ and } \sum_{s=1}^t\phi_{x_s,a_s}\phi_{x_s,a_s}^{\top} \succeq c I_{d}\right\} \\ & = \left\{\exists t,\exists x: \min_{b\in\mathcal{A}\setminus\{\hat{a}_t(x)\}} Z_{\hat{a}_t(x),b}^x >\beta(\delta,t) \text{ and } a^\star_\theta(x) \neq \hat{a}_t(x) \text{ and } \sum_{s=1}^t\phi_{x_s,a_s}\phi_{x_s,a_s}^{\top} \succeq c I_{d}\right\}\\ & \subseteq  \left\{\exists t, \exists x: Z_{\hat{a}_t(x),  a^\star_\theta(x)}^x >\beta(\delta,t) \text{ and } \theta^\top(\phi_{x,a^\star_\theta(x)} -\phi_{x,\hat{a}_t(x)})>0 \text{ and } \sum_{s=1}^t\phi_{x_s,a_s}\phi_{x_s,a_s}^{\top} \succeq c I_{d}\right\}  
\end{align*}

%Define $\bar{\mathcal{X}}_t = \{x\in\mathcal{X}: \hat{a}_t(x) \neq a^\star_\theta(x)\}$, and note that on the event $\mathcal{E}$ the set $\bar{\mathcal{X}}_t$ is non-empty.

Note that on the event $\mathcal{E}$, it holds $\exists x\in\mathcal{X} : \hat{\theta}_t^\top(\phi_{x,\hat{a}_t(x)}-\phi_{x,a^\star_\theta(x)})\geq 0$ and $\theta^\top(\phi_{x,a^\star_\theta(x)} -\phi_{x,\hat{a}_t(x)})>0$. 
\begin{align*}
    &\max\limits_{\left\{\mu: \mu^{\top}(\phi_{x,\hat{a}_t(x)}-\phi_{x,a^\star_\theta(x)}) \geq 0\right\}} f^{\mu}\left(r_{t}, a_{t}, x_{t} \ldots, r_{1}, a_{1},x_{1}\right)= f^{\hat{\theta}}\left(r_{t}, a_{t}, x_{t} \ldots, r_{1}, a_{1},x_{1}\right),\\ 
    &\max\limits_{\left\{\mu: \mu^{\top}(\phi_{x,\hat{a}_t(x)}-\phi_{x,a^\star_\theta(x)}) \leq 0\right\}} f^{\mu}\left(r_{t}, a_{t}, x_{t} \ldots, r_{1}, a_{1},x_{1}\right) \geq f^{\theta}\left(r_{t}, a_{t}, x_{t} \ldots, r_{1}, a_{1},x_{1}\right).
\end{align*}
Hence, it follows that $\exists x \in\mathcal{X}$:
\begin{align*}
Z^x_{\hat{a}_t(x),a^\star_\theta(x)} &= \log \left(\frac{\max\limits_{\left\{\mu: \mu^{\top}(\phi_{x,\hat{a}_t(x)}-\phi_{x,a^\star_\theta(x)}) \geq 0\right\}} f^{\mu}\left(r_{t}, a_{t}, x_{t} \ldots, r_{1}, a_{1},x_{1}\right)}{\max\limits_{\left\{\mu:\mu^{\top}(\phi_{x,\hat{a}_t(x)}-\phi_{x,a^\star_\theta(x)}) \leq 0\right\}} f^{\mu}\left(r_{t}, a_{t}, x_{t} \ldots, r_{1}, a_{1}, x_{1}\right)}\right) \\& \leq \log \left(\frac{f^{\hat{\theta}_t}(r_{t}, a_{t}, x_{t} \ldots, r_{1}, a_{1})}{f^{\theta}(r_{t}, a_{t}, x_{t} \ldots, r_{1}, a_{1})    }\right) \\&= \frac{1}{2} \| \theta - \hat{\theta}_t\|^2_{\sum_{s=1}^t \phi_{x_s,a_s}\phi_{x_s,a_s}^\top}.
\end{align*}
Hence $ \mathcal{E} \subseteq \left\{\exists t\in\mathbb{N}^*,\exists x \in\mathcal{X}: \frac{1}{2} \| \theta - \hat{\theta}_t\|^2_{\sum_{s=1}^t \phi_{x_s,a_s}\phi_{x_s,a_s}^\top} >\beta(\delta,t) \text{ and } \sum_{s=1}^t\phi_{x_s,a_s}\phi_{x_s,a_s}^{\top} \succeq c I_{d}\right\}.$ The rest of the proof would go along the same line of \cite[Prop. 2]{Jedra20}. We note that for any $u>0$, $(1+u)(\sum_{s=1}^t\phi_{x_s,a_s}\phi_{x_s,a_s}^{\top} + cu I_d)^{-1} \succeq (\sum_{s=1}^t\phi_{x_s,a_s}\phi_{x_s,a_s}^{\top})^{-1}$. Hence
$$
\left\|\hat{\mu}_{t}-\mu\right\|^{2}=\left\|\sum_{s=1}^{t} \phi_{x_s,a_{s}} \xi_{s}\right\|^{2}_{\left( \sum_{s=1}^t\phi_{x_s,a_s}\phi_{x_s,a_s}^{\top}\right)^{-1}} \leq(1+u)\left\|\sum_{s=1}^{t} \phi_{x_s,a_s} \xi_{s}\right\|_{\left(\sum_{s=1}^{t} \phi_{x_s,a_{s}} \phi_{x_s,a_{s}}^{\top}+u c I_{d}\right)^{-1}}^{2}.
$$
This implies $\mathcal{E} \subseteq \left\{\exists t \in \mathbb{N}^{*},\exists x \in\mathcal{X}: \frac{1}{2}(1+u) \left\|\sum_{s=1}^{t} \phi_{x_s,a_s} \xi_{s}\right\|_{\left(\sum_{s=1}^{t} \phi_{x_s,a_{s}} \phi_{x_s,a_{s}}^{\top}+u c I_{d}\right)^{-1}}^{2} \geq \beta(\delta, t)\right\},$

and with the choice 
$$
\beta(\delta, t)=(1+u) \sigma^{2} \log \left(\frac{\operatorname{det}\left((u c)^{-1} \sum_{s=1}^{t} a_{s} a_{s}^{\top}+I_{d}\right)^{1 / 2}}{\delta}\right),
$$
it follows directly from \cite{Abbasi11} that  $\mathbb{P}[\exists x \in\mathcal{X}: a^\star_\theta(x) \neq \hat{a}_t(x), \tau < \infty] = \mathbb{P}[\mathcal{E}] \leq \delta.$

\end{proof}
\end{comment}
\subsection{Proof of Lemma
\ref{lem:tracking_lemma}}
\begin{proof}
Define for $x\in\mathcal{X}$, the projection operator $\text{proj}_x(\cdot)$ that takes $\alpha \in C$ as input, and outputs $\alpha_x$, the $K$-dimensional vector that contains the component of $\alpha$ relative to the context $x$. Let $C_x = \{\alpha_x: \alpha_x = \text{proj}_x(\alpha), \forall \alpha \in C\}$.
Note that, since $C \subset \Lambda$ is convex and non-empty, 
we have that each of the sets $C_x$, for $x\in\mathcal{X}$, is also convex. Also, note that 
$$
\exists t_0: \forall t\geq t_0, d_\infty(\alpha,C) \leq \varepsilon \Rightarrow \forall t\geq t_0, \forall x\in\mathcal{X}, d_\infty(\alpha_x, C_x) \leq \varepsilon.
$$
Now, define for all $x\in\mathcal{X}$, and $t \in \mathbb{N}^*$ such that $N_x(t) \geq 1$
$$
\bar{\alpha}_x(t) = \frac{1}{N_x(t)}\sum_{s = 1}^t \alpha_x(s)\mathbbm{1}\{x_s = x\}, \quad \hat{\alpha}_x(t)= \argmin_{\alpha' \in C_x} d_{\infty}(\bar{\alpha}_x(t), \alpha'), \quad v_x(t) = \argmin_{\alpha' \in C_x} d_{\infty}(\alpha_x(t), \alpha').$$  %Note that, by convexity of $C$, there exists $t_0'\geq t_0$ such that for all $t\geq t_0'$ we have 
%$$
%d_{\infty}\left(\left(N_{x,a}(t)/N_{x}(t)\right)_{(x,a) \in \mathcal{X}\times \mathcal{A}}, C\right) \leq d_{\infty}\left(\left(N_{x,a}(t)/N_{x}(t)\right)_{(x,a) \in \mathcal{X}\times \mathcal{A}}, \hat{\alpha}(t)\right).
%$$
Observe that for all $(x,a)\in\mathcal{X}\times \mathcal{A}$, we have 
\begin{align*}
& \left|\frac{1}{N_x(t)} \left(\sum_{s=1}^{t} \alpha_{x,a}(s)- \sum_{s=1}^{t} v_{x,a}(s)\right) \mathbbm{1}\{x_s = x\} \right| \\ &  \leq \frac{1}{N_x(t)} \sum_{s=1}^{t_{0}}\left|\alpha_{x,a}(s)-v_{x,a}(s)\right|\mathbbm{1}\{x_s = x\}+\frac{1}{N_x(t)} \sum_{s=t_{0}+1}^{t}\left|\alpha_{x,a}(s)-v_{x,a}(s)\right| \mathbbm{1}\{x_s = x\}\\
& \leq \frac{N_x(t_{0})}{N_x(t)}+\frac{N_x(t)-N_x(t_0)}{N_x(t)} \varepsilon.
\end{align*}
By Lemma \ref{lem:Nx_concentration_tight}, $\forall \kappa \in\left(0,p_{\min}\right)$ we get that w.p. at least $1-2e^{-\frac{t \kappa^2}{4}}$
$$ c_1(\kappa)t\leq N_x(t) \leq c_2(\kappa)t,$$
with $c_1(\kappa) =  (p_\mathcal{X}(x) -\kappa)$ and $c_2(\kappa) = (p_\mathcal{X}(x) +\kappa)$. Hence we get, w.p. at least $1-2e^{-\frac{t \kappa^2}{4}}$, that
$$
\left|\frac{1}{N_x(t)} \left(\sum_{s=1}^{t} \alpha_{x,a}(s)- \sum_{s=1}^{t} v_{x,a}(s)\right) \mathbbm{1}\{x_s = x\} \right| \leq \frac{t_{0}}{t c_1}+\frac{(t - t_0)}{tc_1}\varepsilon = \frac{t_0}{c_1t} + \frac{t-t_0}{c_1t}\varepsilon,
$$
with $c = \frac{1}{c_1}$. Hence for all $t \geq t_0' = \frac{t_0}{\varepsilon}$, we also have $d_{\infty}\left(\bar{\alpha}_x(t),\frac{1}{N_x(t)} \sum_{s = 1}^t v_x(s)\mathbbm{1}\{x_s = x\}\right)\leq 2c\varepsilon$, for all $x\in \mathcal{X}$. By convexity of $C_x$ we have $\frac{1}{N_x(t)}\sum_{s = 1}^tv_x(s)\mathbbm{1}\{x_s = x\} \in C_x$. Hence, we may conclude that
$$
\forall x\in\mathcal{X}, \forall t \geq t_{0}^{\prime} \quad d_{\infty}(\bar{\alpha}_x(t), \hat{\alpha}_x(t)) \leq d_{\infty}\left(\bar{\alpha}_x(t), \frac{1}{N_x(t)} \sum_{s=1}^{t} v_x(s)\mathbbm{1}\{x_s = x\}\right) \leq 2c\varepsilon.  
$$
Further define for all $t\geq 1$, $\varepsilon_{x,a,t} = N_{x,a}(t) - N_x(t)\hat{\alpha}_{x,a}(t)$, and the events
\begin{align*}
\mathcal{E}_{1}(t,x) &=\left\{a=\underset{a \in \supp(\bar{\alpha}_x(t))}{\argmin}\{N_{x,a}(t)- N_x(t) \bar{\alpha}_{x,a}(t)\}\right\}, \\
\mathcal{E}_{2}(t,x)&=\left\{A_x(t) \prec f_x(t) \quad \text { and } \quad a=a_x(i_t(x))\right\}.
\end{align*}
The rest of the proof will show that $\exists c'(\kappa)>0$, $\exists t_0'' \geq t_0'$ such that for all $t\geq t_0''$, for all $(x,a) \in\mathcal{X}\times \mathcal{A}$, and w.p. at least $1-2e^{-\frac{t \kappa^2}{4}}$, we have 
$$
\{a_{t+1}(x) = a\}\subseteq \mathcal{E}_{1}(t,x) \cup \mathcal{E}_{2}(t,x) \subseteq \{\varepsilon_{x,a,t} \leq c't\varepsilon\}.
$$
We differentiate two cases: 
\begin{enumerate}
    \item \textit{Case 1:} Let $x\in\mathcal{X}$. If $\{a_{t+1}(x) = a\}\subseteq \mathcal{E}_{1}(t,x)$, we have 
\begin{align*}
\varepsilon_{x,a,t} &= N_{x,a}(t)- N_x(t)\hat{\alpha}_{x,a}(t) \\
&= N_{x,a}(t) - N_x(t)\bar{\alpha}_{x,a}(t) + t\bar{\alpha}_{x,a}(t) - N_x(t)\hat{\alpha}_{x,a}(t) \\
& \leq N_{x,a}(t)- N_x(t)\bar{\alpha}_{x,a}(t)+ c\varepsilon t\\
& \leq \min_{a \in \operatorname{supp}(\bar{\alpha}_x(t))} {N_{x,a}(t)}- t\bar{\alpha}_{x,a}(t)+ 2c\varepsilon t\\
& \leq 2tc\varepsilon ,
\end{align*}
where the last inequality holds because 
$
\sum_{a \in \operatorname{supp}(\bar{\alpha}_x(t))} N_{x,a}(t)- N_x(t)\bar{\alpha}_{x,a}(t) \leq 0.
$
Hence $\mathcal{E}_1(t,x) \subseteq \{\varepsilon_{x,a,t}\leq 2ct\varepsilon\}$  $\forall x \in\mathcal{X}$. \newline
\item \textit{Case 2:} Let $x\in\mathcal{X}$. If $\{a_{t+1}(x) = a\}\subseteq \mathcal{E}_{2}(t,x)$, we have $a\in\mathcal{A}_x$. Define 

\begin{align*}
N_{x,a,1}(k)& = \sum_{s=1}^{k} \mathbbm{1}{\left\{x_{k} = x \text { and } a_{k}(x) = a \text { and } A_x(k-1) \prec f_x(k-1)\right\}}, \\
N_{x,a,2}(k)& = \sum_{s=1}^{k} \mathbbm{1}{\left\{ x_{k} = x \text { and }  a_{k}(x) = a \text { and } A_x(k-1) \succeq f_x(k-1)\right\}}.
\end{align*}

Note that $N_{x,a}(k)= N_{x,a,1}(k) + N_{x,a,2}(k)$, and by definition of the forced exploration sampling rule it follows that for all $x\in\mathcal{X}$ it holds $N_{x,a,1}(k)-1 \leq \min_{a_x \in \mathcal{A}_{x}} N_{x,a_x,1}(k) \leq N_{x,a, 1}(k)$. Since the event $\mathcal{E}_{2}(t,x)$ holds, we observe that
\begin{align*}
\left(N_{x,a,1}(t)-1\right)\lambda_{d_x}\left(\sum_{a_x \in \mathcal{A}_x} \phi_{x,a_x}\phi_{x,a_x}^\top \right) & \leq \min_{a_x \in \mathcal{A}_{x}} N_{x,a_x, 1}(t) \lambda_{d_x}\left(\sum_{a_x \in \mathcal{A}_x} \phi_{x,a_x}\phi_{x,a_x}^\top \right) \\& \leq \lambda_{d_x }\left(\sum_{s =1}^t \phi_{x_s,a_s}\phi_{x_s,a_s}^\top \mathbbm{1}\{x_s = x\} \right) \\& < f_x(t) = \sqrt{\frac{N_x(t)}{d_x}}\lambda_{d_x}\left(\sum_{a_x \in \mathcal{A}_x} \phi_{x,a_x}\phi_{x,a_x}^\top \right)
\end{align*}
Hence we obtain $ N_{x,a,1}(t) \leq \sqrt{N_x(t)/d_x} + 1. $
Let $k \leq t$ be the largest integer such that $N_{x,a,2}(k) = N_{x,a,2}(k-1) + 1$. Note that at
such $k$ the event $\mathcal{E}_1(k-1,x)$ must hold by definition of $N_{x,a,2}(k - 1)$, and we have 
$$
N_{x,a,2}(t)=N_{x,a,2}(k)=N_{x,a,2}(k-1)+1 \quad \text { and } \quad a_{k}(x)=\underset{a \in \operatorname{supp}(\bar{\alpha}_x(k-1))}{\argmin} N_{x,a}(k-1)-k \bar{\alpha}_{x,a}(k-1).
$$
We also have 
\begin{align*}
\varepsilon_{x,a,t} & = N_{x,a,t} - N_{x}(t)\hat{\alpha}_{x,a}(t)\\
&=N_{x,a, 1}(t)+N_{x,a,2}(t) - N_{x}(t) \hat{\alpha}_{x,a}(t) \\
& \leq \sqrt{N_x(t)/d_x} + 1 + N_{x,a,2}(t)-N_{x}(t) \hat{\alpha}_{x,a}(t)
\\& \leq \sqrt{c_2 t/d_x} + 1 + N_{x,a,2}(t)-N_{x}(t) \hat{\alpha}_{x,a}(t).
\end{align*}

If $k-1\leq t_0'$, then we have $N_{x,a,2}(k) \leq t_0'$, otherwise $\mathcal{E}_1(x,k-1)$ holds,and we have
\begin{align*}
N_{x,a,2}(t) &=1+N_{x,a,2}(k-1)-(k-1) \hat{\alpha}_{x,a}(k-1)+(k-1) \hat{\alpha}_{x,a}(k-1) \\
& \leq 1+2(k-1)c\varepsilon+(k-1) \hat{\alpha}_{x,a}(k-1).
\end{align*}

Hence we get
$$
\varepsilon_{x,a,t} \leq \sqrt{c_2 t/d_x} + 1 + \max\{t_0', 1+2(k-1)c\varepsilon + (k-1) \hat{\alpha}_{x,a}(k-1)-N_x(t) \hat{\alpha}_{x,a}(t)\},
$$
and since
\begin{align*}
(k-1) \hat{\alpha}_{x,a}(k-1)-N_x(t) \hat{\alpha}_{x,a}(t)= &(k-1) \hat{\alpha}_{x,a}(k-1)-(k-1) \bar{\alpha}_{x,a}(k-1) +(k-1) \bar{\alpha}_{x,a}(k-1)-N_x(t)\hat{\alpha}_{x,a}(t) \\
\leq &(k-1) \hat{\alpha}_{x,a}(k-1)-(k-1) \bar{\alpha}_{x,a}(k-1)+N_x(t) \bar{\alpha}_{x,a}(t)-N_x(t) \hat{\alpha}_{x,a}(t) \\
\leq & 2(k-1) c\varepsilon+2 N_x(t) \varepsilon\\
\leq & 2 ct\varepsilon+2 c_2 t \varepsilon \\
\leq & 2(c+c_2)t \varepsilon
\end{align*}
we can conclude that 
$$
\varepsilon_{x,a,t} \leq \sqrt{c_2 t/d_x} + 1 + \max\{t_0', 1+ 2t(c_2+2c)\varepsilon\} \leq \sqrt{t/d_x} + 1 + \max\{t_0', 1+ 2(1+2c)t\varepsilon\}.
$$
%Hence for $t\geq t_0'' =\max\left\{\frac{1}{c'\varepsilon},\frac{1+t_0'}{c'\varepsilon - \sqrt{\frac{c_2}{d}}},\frac{1}{\varepsilon(c'-2(c_2+2c))}- \frac{1}{\sqrt{d}}\right\}$ 
Hence for $t\geq t_0'' = \max\left\{\frac{9}{c'^2\varepsilon^2 d},\frac{3t_0'}{c'\varepsilon},\frac{6}{c'\varepsilon}\right\}$
it holds that $\varepsilon_{x,a,t} \leq c' t\varepsilon$ and thus
$\mathcal{E}_2(x,t) \subseteq \{\varepsilon_{x,a,t}\leq c' t\varepsilon\},$ for some $c'\geq 2(1+2c)$.
Thus we have proved that for our choice of $t_0'',c'$ and for all $t\geq t_0''$, for all $(x,a) \in\mathcal{X}\times \mathcal{A}$, we have 
$$
\{a_{t+1} = a\}\subseteq \mathcal{E}_{1}(t,x) \cup \mathcal{E}_{2}(t,x) \subseteq \{\varepsilon_{x,a,t} \leq c' t\varepsilon\},
$$
\end{enumerate}
Note that, since $c \geq 1$, we may pick $c' = 6$. This results in $ t_0'' = \max\left\{\frac{1}{4\varepsilon^2 d},\frac{t_0'}{2\varepsilon},\frac{1}{\varepsilon}\right\}$. Now, by Lemma 17 in \cite{Garivier16}, for all $(x,a)\in\mathcal{X}\times \mathcal{A}$, it holds that for all $t\geq t_0''$
$$
\varepsilon_{x,a,t} \leq \max\{\varepsilon_{x,a,t_0''},2t(c_2+2c)\varepsilon +1\} \leq\max\{t_0'',6 t\varepsilon +1\}.
$$
We note that for all $t\geq0$, we have $\bar{\alpha}_x(t-1) \subseteq \bar{\alpha}_x(t)$. Hence we have 
$$
\sum_{a \in \operatorname{supp}(\bar{\alpha}_x(t)) \cup \mathcal{A}_{x}} \varepsilon_{x,a, t}=\sum_{a \in \mathcal{A} \backslash \operatorname{supp}(\bar{\alpha}_x(t)) \cup \mathcal{A}_{x}} t \hat{\alpha}_{x,a}(t) \geq 0.
$$
Let $z_{t,x} = |\supp(\bar{\alpha}_x(t))\setminus \mathcal{A}_x|$, and $z_{t} = \max_{x\in \mathcal{X}} |\supp(\bar{\alpha}_x(t))\setminus \mathcal{A}_x|$ and note that
$$
\begin{array}{l}
\forall x\in\mathcal{X}, \forall a \in \operatorname{supp}(\bar{\alpha}_x(t)) \cup \mathcal{A}_{x}, \quad \max \left(t_{0}^{\prime \prime}, c' t \varepsilon+1\right) \geq \varepsilon_{x,a,t} \geq-\left(z_{t,x}+d-1\right) \max \left(t_{0}^{\prime \prime}, c' t \varepsilon+1\right), \\
\forall x\in\mathcal{X}, \forall a \in \mathcal{A} \backslash \operatorname{supp}(\bar{\alpha}_x(t)) \cup \mathcal{A}_{x}, \quad 0 \geq \varepsilon_{x,a, t} \geq - c_2 t \varepsilon,
\end{array}
$$
which implies for all $t\geq t_0''$    
$$
\max_{(x,a)\in\mathcal{X}\times \mathcal{A}}\left|\varepsilon_{x,a, t}\right| \leq\left(z_{t}+d- 1\right) \max \left\{t_{0}^{\prime \prime}, 6t \varepsilon+1\right\} \leq\left(z_{t}+d- 1\right) \max \left\{t_{0}^{\prime \prime}, 7\right\}  .
$$
This finally implies that for $t_1(\varepsilon,\kappa) = \frac{1}{c_1(\kappa)\varepsilon}\max\{t_0'',7\}$, we have for all $t \ge t_1$,
\begin{align*}
d_{\infty}\left(\left(N_{x,a}(t)/N_{x}(t)\right)_{(x,a) \in \mathcal{X}\times \mathcal{A}}, C\right) & \leq d_{\infty}\left(\left(N_{x,a}(t)/N_{x}(t)\right)_{(x,a) \in \mathcal{X}\times \mathcal{A}}, \hat{\alpha}(t)\right) \\& =\max_{(x,a) \in \mathcal{X}\times \mathcal{A}}\left|N_{x,a}(t) / N_x(t) -\hat{\alpha}_{x,a}(t)\right|\\& = \max _{(x,a) \in \mathcal{X}\times \mathcal{A}}\left|\frac{\varepsilon_{x,a, t}}{N_x(t)}\right| \leq\max _{(x,a) \in \mathcal{X}\times \mathcal{A}}\left|\frac{\varepsilon_{x,a, t}}{c_1(\kappa)t}\right| \leq\left(z_{t}+d-1\right) \varepsilon.
\end{align*}
More precisely, we have
\begin{equation}
\label{eq:t1}
t_1(\varepsilon,\kappa) =\max\left\{\frac{1}{4c_1(\kappa) d\varepsilon^3},\frac{t_0(\varepsilon)}{2c_1(\kappa)\varepsilon^3}\frac{1}{c_1(\kappa)\varepsilon^2}, \frac{7}{c_1(\kappa) \varepsilon}\right\}. %\max\left\{\frac{1}{c_1\varepsilon^2},\frac{1+t_0}{(c'\varepsilon - \sqrt{\frac{c_1}{d}})c_1\varepsilon},\frac{1}{\varepsilon^2 c_1(c'-2(c_1+2c))}- \frac{1}{\sqrt{d}c_1\varepsilon},\frac{c' +1}{c_1\varepsilon}\right\}.
\end{equation}

\end{proof}
\begin{comment}
    \subsection{Proof of Lemma
\ref{lem:tracking_lemma}}
\begin{proof}
Let $t>0$, and for all $x\in\mathcal{X}$ define $\mathcal{I}_{x}(t) = \{i_k\in [1,t]:x_{i_k} = x\}$, the indices at which context $x$ is observed, with $k\in\{1,\dots,N_x(t)\}$. Note that with probability at least $1-2^{-t\kappa^2/4}$, for all 
$$
|\mathcal{I}_x(t)| = N_x(t) \geq (p_\mathcal{X}(x)-\kappa)t
$$
Note that $C$ is non-empty, and for all $k>0$ define
$$
\bar{\alpha}_x(k) = \frac{1}{k}\sum_{j = 1}^k \alpha_x(i_j), \quad \hat{\alpha}(t)= \argmin_{\alpha \in C} d_{\infty}(\bar{\alpha}(t), \alpha), \quad v(t) = \argmin_{\alpha \in C} d_{\infty}(\alpha(t), \alpha).$$ 
Observe that $\exists k_0(x)$ such that $\forall k \geq k_0$, we have 
$$
    d_\infty(\alpha_x(k),C_x)\leq \varepsilon,
$$
where $C_x = \{\alpha_x \in[0,1]^K: \sum_{a = 1}^K \alpha_{x,a} = 1\}$ such that $C_x\cap C_y = \emptyset$, $\bigcup_{x\in\mathcal{X}} C_x = C$, and $\alpha_x = \text{proj}_{C_x}(\alpha)$. Now, observe that for all $a\in \mathcal{A}$, we have 
\begin{align*}
\left|\frac{1}{k} \sum_{j=1}^{k} \alpha_{x,a}(i_j)-\frac{1}{k} \sum_{j=1}^{k} v_{x,a}(i_j)\right| & \leq \frac{1}{k} \sum_{j=1}^{k_{0}}\left|\alpha_{x,a}(i_j)-v_{x,a}(i_j)\right|+\frac{1}{k} \sum_{j=k_{0}+1}^{k}\left|\alpha_{x,a}(i_j)-v_{x,a}(i_j)\right| \\
& \leq \frac{k_{0}}{k}+\frac{k-k_{0}}{k} \varepsilon.
\end{align*}
Hence for all $k_0$h
$N_x(t) \geq \frac{t(p_\mathcal{X}(x) -\kappa) }{\varepsilon}$, we  have $d_{\infty}\left(\bar{\alpha}_x(k),\frac{1}{k} \sum_{j =1}^k v_x(k)\right)\leq 2\varepsilon$. Since by convexity of $C_x$ we have $\frac{1}{k}\sum_{j = 1}^k v(i_j) \in C_x$, we may conclude that
$$
\forall k \geq k_{0}^{\prime} \quad d_{\infty}(\bar{\alpha}_x(k), \hat{\alpha}_x(k)) \leq d_{\infty}\left(\bar{\alpha}_x(k), \frac{1}{k} \sum_{j=1}^{k} v(i_j)\right) \leq 2 \varepsilon.  
$$
Further define for all $t\geq 1$, $\varepsilon_{x,a,t} = N_{x,a}(t) - N_x(t)\hat{\alpha}_{x,a}(t)$, and the events
\begin{align*}
\mathcal{E}_{1}(t,x) &=\left\{a=\underset{a \in \supp(\bar{\alpha}_x(t))}{\argmin}\{N_{x,a}(t)- N_x(t) \bar{\alpha}_{x,a}(t)\}\right\}, \\
\mathcal{E}_{2}(t,x)&=\left\{A_x(t) \prec f_x(t) \quad \text { and } \quad a=a_x(i_t(x))\right\}.
\end{align*}
The rest of the proof will be aimed at showing that exists $t_0'' \geq t_0'$ such that for all $t\geq t_0''$, for all $(x,a) \in\mathcal{X}\times \mathcal{A}$, we have 
$$
\{a_{t+1} = a\}\subseteq \mathcal{E}_{1}(t,x) \cup \mathcal{E}_{2}(t,x) \subseteq \{\varepsilon_{x,a,t} \leq 9N_x(t)\varepsilon\}.
$$
We differentiate two cases: 
\begin{enumerate}
    \item \textit{Case 1:} If $\{a_{t+1} = a\}\subseteq \mathcal{E}_{1}(t,x)$, we have 
\begin{align*}
\varepsilon_{x,a,t} &= N_{x,a(t)}- N_x(t)\hat{\alpha}_{x,a}(t) \\
&= {N_{x,a}(t)} - N_x(t)\bar{\alpha}_{x,a}(t) + N_x(t)\bar{\alpha}_{x,a}(t) - N_x(t)\hat{\alpha}_{x,a}(t) \\
& \leq N_{x,a}(t)- N_x(t)\bar{\alpha}_{x,a}(t)+ \varepsilon N_x(t) \\
& \leq \min_{a \in \operatorname{supp}(\bar{\alpha}_x(t))} {N_{x,a}(t)}- N_x(t)\bar{\alpha}_{x,a}(t)+ \varepsilon N_x(t) \\
& \leq 2 N_x(t) \varepsilon,
\end{align*}
where the last inequality holds because 
$
\sum_{a \in \operatorname{supp}(\bar{\alpha}_x(t))} N_{x,a}(t)- N_x(t)\bar{\alpha}_{x,a}(t) \leq 0.
$
Hence $\forall x \in\mathcal{X}, \mathcal{E}_1(t,x) \subseteq \{\varepsilon_{x,a,t}\leq 2t\varepsilon\}$. \newline
\item \textit{Case 2:} If $\{a_{t+1} = a\}\subseteq \mathcal{E}_{2}(t,x)$, we have $a\in\mathcal{A}_x$. Define 

\begin{align*}
N_{x,a,1}(k)& = \sum_{s=1}^{k} \mathbbm{1}{\left\{x_{k} = x \text { and } a_{k} = a \text { and } A_x(k-1) \prec f_x(k-1)\right\}}, \\
N_{x,a,2}(k)& = \sum_{s=1}^{k} \mathbbm{1}{\left\{ x_{k} = x \text { and }  a_{k} = a \text { and } A_x(k-1) \succeq f_x(k-1)\right\}}.
\end{align*}

Note that $N_{x,a}(k)= N_{x,a,1}(k) + N_{x,a,1}(k)$, and by definition of the forced exploration sampling rule it follows that for all $x\in\mathcal{X}$ it holds $N_{x,a,1}(k)-1 \leq \min_{a_x \in \mathcal{A}_{x}} N_{x,a_x,1}(k) \leq N_{a, 1}(k)$. Since the event $\mathcal{E}_{2}(t,x)$ holds, we observe that
\begin{align*}
\left(N_{x,a,1}(t)-1\right)\lambda_{d_x}\left(\sum_{a_x \in \mathcal{A}_x} \phi_{x,a_x}\phi_{x,a_x}^\top \right) & \leq \min_{a_x \in \mathcal{A}_{x}} N_{x,a, 1}(t) \lambda_{d_x}\left(\sum_{a_x \in \mathcal{A}_x} \phi_{x,a_x}\phi_{x,a_x}^\top \right) \\& \leq \lambda_{d_x }\left(\sum_{a_x \in \mathcal{A}_x} \phi_{x,a_x}\phi_{x,a_x}^\top \right) \\& \leq \sqrt{\frac{N_x(t)}{d_x}}\lambda_{d_x}\left(\sum_{a_x \in \mathcal{A}_x} \phi_{x,a_x}\phi_{x,a_x}^\top \right)
\end{align*}
Hence we obtain $ N_{x,a,1}(t) \leq \sqrt{N_x(t)/d_x} + 1. $
Let $k \leq t$ be the largest integer such that $N_{x,a,2}(k) = N_{x,a,2}(k-1) + 1$. Note that at
such $k$ the event $\mathcal{E}_1(k-1,x)$ must hold by definition of $N_{x,a,2}(k - 1)$, and we have 
$$
N_{x,a,2}(t)=N_{x,a,2}(k)=N_{x,a,2}(k-1)+1 \quad \text { and } \quad a_{k}=\underset{a \in \operatorname{supp}(\bar{\alpha}_x(k-1))}{\argmin} N_{x,a}(k-1)-k \bar{\alpha}_{x,a}(k-1).
$$
We also have 
\begin{align*}
\varepsilon_{x,a,t} & = N_{x,a,t} - N_{x}(t)\hat{\alpha}_{x,a}(t)\\
&=N_{x,a, 1}(t)+N_{x,a,2}(t) - N_{x}(t) \hat{\alpha}_{x,a}(t) \\
& \leq \sqrt{N_x(t)/d_x} + 1 + N_{x,a,2}(t)-N_{x}(t) \hat{\alpha}_{x,a}(t).
\end{align*}

If $k-1\leq t_0'$, then we have $N_{x,a,2}(k) \leq t_0'$, otherwise $\mathcal{E}_1(k-1)$ holds, we have
\begin{align*}
N_{x,a,2}(t) &=1+N_{x,a,2}(k-1)-(k-1) \hat{\alpha}_{x,a}(k-1)+(k-1) \hat{\alpha}_{x,a}(k-1) \\
& \leq 1+2(k-1) \varepsilon+(k-1) \hat{\alpha}_{x,a}(k-1).
\end{align*}

Hence
$$
\varepsilon_{x,a,t} \leq \sqrt{N_x(t)/d_x} + 1 + \max\{t_0', 1+2(k-1)\varepsilon\},
$$
and since
\begin{align*}
(k-1) \hat{\alpha}_{x,a}(k-1)-N_x(t) \hat{\alpha}_{x,a}(t)= &(k-1) \hat{\alpha}_{x,a}(k-1)-(k-1) \bar{\alpha}_{x,a}(k-1) +(k-1) \bar{\alpha}_{x,a}(k-1)-N_x(t)\hat{\alpha}_{x,a}(t) \\
\leq &(k-1) \hat{\alpha}_{x,a}(k-1)-(k-1) \bar{\alpha}_{x,a}(k-1)+N_x(t) \bar{\alpha}_{x,a}(t)-N_x(t) \hat{\alpha}_{x,a}(t) \\
\leq & 2(k-1) \varepsilon+2 N_x(t) \varepsilon \\
\leq & 4 N_x(t) \varepsilon
\end{align*}
we can conclude that 
$$
\varepsilon_{x,a,t} \leq \sqrt{N_x(t)/d_x} + 1 + \max\{t_0', 1+6N_x(t)\varepsilon\}. 
$$
Hence for $t\geq t_0'' =\max\left\{\frac{1}{\varepsilon},\frac{1}{\varepsilon^2 d_x},\frac{t_0'}{\varepsilon}\right\}$ it holds that $\varepsilon_{x,a,t} \leq 2t(c_2+2c)\varepsilon$ and thus
$
\mathcal{E}_2(x,t) \subseteq \{\varepsilon_{x,a,t}\leq 9N_x(t)\varepsilon\}.
$
Thus we have proved that for our choice of $t_0''$ and for all $t\geq t_0''$, for all $(x,a) \in\mathcal{X}\times \mathcal{A}$, we have 
$$
\{a_{t+1} = a\}\subseteq \mathcal{E}_{1}(t,x) \cup \mathcal{E}_{2}(t,x) \subseteq \{\varepsilon_{x,a,t} \leq 9N_x(t)\varepsilon\}.
$$
\end{enumerate}
By Lemma 17 in \cite{Garivier16} it holds that for all $x\in\mathcal{X}$
$$
\varepsilon_{x,a,t} \leq \max\{\varepsilon_{x,a,t_0''},c't\varepsilon +1\} \leq\max\{  t_0'',9c't\varepsilon +1\}.
$$
We note that for all $t\geq0$,$x\in\mathcal{X}$ we have $\bar{\alpha}_x(t-1) \subseteq \bar{\alpha}_x
(t)$. Hence we have 
$$
\sum_{a \in \operatorname{supp}(\bar{\alpha}_x(t)) \cup \mathcal{A}_{x}} \varepsilon_{x,a, t}=\sum_{a \in \mathcal{A} \backslash \operatorname{supp}(\bar{\alpha}_x(t)) \cup \mathcal{A}_{x}} t \hat{\alpha}_{x,a}(t) \geq 0.
$$
Let $z_{t,x} = |\supp(\bar{\alpha}_x(t))\setminus \mathcal{A}_x|$, $z_{t,x} = \max_{x} |\supp(\bar{\alpha}_x(t))\setminus \mathcal{A}_x|$, and note that
$$
\begin{array}{l}
\forall x\in\mathcal{X}, \forall a \in \operatorname{supp}(\bar{\alpha}_x(t)) \cup \mathcal{A}_{x}, \quad \max \left(t_{0}^{\prime \prime}, 9 N_x(t) \varepsilon+1\right) \geq \varepsilon_{x,a,t} \geq-\left(z_{t,x}+d-1\right) \max \left(t_{0}^{\prime \prime}, 9 N_x(t) \varepsilon+1\right), \\
\forall x\in\mathcal{X}, \forall a \in \mathcal{A} \backslash \operatorname{supp}(\bar{\alpha}_x(t)) \cup \mathcal{A}_{x}, \quad 0 \geq \varepsilon_{x,a, t} \geq-N_x(t) \varepsilon,
\end{array}
$$
which implies for all $t\geq t_0''$ and $x\in\mathcal{X}$ that    
$$
\max_{a \in \mathcal{A}}\left|\varepsilon_{x,a, t}\right| \leq\left(z_{t,x}+d-1\right) \max \left(t_{0}^{\prime \prime}, 9 N_x(t) \varepsilon+1\right).
$$
This finally implies that for $t_1 = \frac{1}{\varepsilon}$, we have for all $t \ge t_1$,
\begin{align*}
d_{\infty}\left(\left(N_{x,a}(t)/N_{x}(t)\right)_{(x,a) \in \mathcal{X}\times \mathcal{A}}, C\right) & \leq d_{\infty}\left(\left(N_{x,a}(t)/N_{x}(t)\right)_{(x,a) \in \mathcal{X}\times \mathcal{A}}, \hat{\alpha}(t)\right) \\& =\max_{(x,a) \in \mathcal{X}\times \mathcal{A}}\left|N_{x,a}(t) / N_x(t) -\hat{\alpha}_{x,a}(t)\right|\\& =\max _{(x,a) \in \mathcal{X}\times \mathcal{A}}\left|\frac{\varepsilon_{x,a, t}}{N_x(t)}\right| \leq\left(z_{t,x}+d-1\right) \varepsilon.
\end{align*}

By Lemma \ref{lem:Nx_concentration_tight}, $\forall \kappa \in\left(0,p_{\min}\right)$ we get that with probability at least $1-2e^{-\frac{t \kappa^2}{4}}$

$$ (p_\mathcal{X}(x) -\kappa)t\leq N_x(t) \leq (p_\mathcal{X}(x)+\kappa)t.$$

\end{proof}
\end{comment}

\subsection{Proof of Lemma \ref{lem:convergence_proportions}}
\begin{proof}
Fix $\varepsilon>0$. By Lemma \ref{lem:properties_eps_delta} there exists $g(q) >0$ such that for all $\theta'$ that satisfies $\|\theta' - \theta\| \leq g(q)$, we have $\sup_{\alpha \in C_\varepsilon(\theta')} d_\infty(\alpha, C^\star_\varepsilon(\theta)) \leq \varepsilon/2$. By Lemma \ref{lem:LS_concentration}, we have that $\hat{\theta}_t$ converges to $\theta$ a.s. Hence there exists $t_0 \geq 1$ such that for all $t\geq t_0$ we have 
$$
\|\hat{\theta}_t - \theta\| \leq g(q).
$$
The condition \eqref{eq:condition_convergence} implies that there exists $t_1\geq 1$, and there exists a sequence of integers $(h(t))_{t\geq 1}$ such that for all $t\geq t_1$ we have $h(t) \geq \ell(t) \geq t$, and $d_\infty(\alpha(t), C^\star_\varepsilon(\hat{\theta}_{h(t)})) < \varepsilon/2$. Hence for all $t\geq \max\{t_0,t_1\}$, we get

$$
d_{\infty}\left(\alpha(t), C_\varepsilon^{\star}(\theta)\right) \leq d_{\infty}\left(\alpha(t), C_\varepsilon^{\star}\left(\hat{\theta}_{h(t)}\right)\right)+\max _{\alpha \in C_\varepsilon^{\star}\left(\hat{\theta}_{h(t)}\right)} d_{\infty}\left(\alpha, C_\varepsilon^{\star}(\theta)\right)<\varepsilon.
$$
Hence we have that $\lim_{t\to \infty}d_{\infty}\left(\alpha(t), C_\varepsilon^{\star}(\theta)\right) = 0$ a.s., and by Lemma \ref{lem:tracking_lemma}, we can conclude that 
$$\lim_{t\to \infty}d_\infty\left(\left(\frac{N_{x,a}(t)}{N_x(t)}\right)_{(x,a)\in\mathcal{X}\times\mathcal{A}},C^\star_\varepsilon(\theta) \right) = 0, \text { a.s.}$$
\end{proof}

\subsection{Proof of Theorem \ref{th:optimality}}
\begin{proof}

\textit{1) Almost sure guarantee: } Define the event:
$$\mathcal{E}=\left\{d_{\infty}\left(\left(N_{x,a}(t)/N_x(t)\right)_{(x,a)\in\mathcal{X} \times \mathcal{A}}, C_\varepsilon^{\star}(\alpha)\right) \underset{t \rightarrow \infty}{\longrightarrow} 0 \text { and } \hat{\theta}_{t} \underset{t \rightarrow \infty}{\longrightarrow} \theta\right\},
$$
and, by Lemma \ref{lem:LS_concentration} and Lemma \ref{lem:convergence_proportions}, the event $\mathcal{E}$ holds with w.p. $1$. Note that an equivalent way to define $(T^\star_{\theta,\varepsilon})^{-1}$ is through a convex program: $\bar{\psi}_\varepsilon(\theta) = \sup_{\alpha\in\Lambda}\bar{\psi}_\varepsilon(\theta,\alpha)$, where 
$$
\bar{\psi}_\varepsilon(\theta,\alpha) = \min_{x\in\mathcal{X}}\min_{a\in \mathcal{A}^c_\varepsilon(\theta,x)} \inf_{\mu \in \hat{B}_{\varepsilon}(\theta, x, a)} \|\theta - \mu\|^2_{A(\alpha)}, %\inf_{{\left\lbrace \mu\in\mathbb{R}^d: \exists x \in \mathcal{X}, \forall a \in \mathcal{A}_\varepsilon(\theta,x), \; \mu^{\top}(\phi_{x,a_{\mu}^\star(x)}- \phi_{x,a})>\varepsilon \right\rbrace}}
$$
and $\hat{B}_\varepsilon(\theta,x,a) = \left\lbrace \mu \in \mathbb{R}^d: \; \exists b \in \mathcal{A}_\varepsilon(\theta,x), \; \mu^{\top}\gamma^x_{a,b}\leq-\varepsilon \right\rbrace$. Let $q>0$. By continuity of $\bar{\psi}_\varepsilon$ (Lemma \ref{lem:properties_eps_delta}), there exist an open neighborhood, $\mathcal{N}(q)$ of $\{\theta\}\times C_\varepsilon^\star(\theta)$, such that for all $(\theta',\alpha')\in \mathcal{N}(q)$, we have 
$$
    \bar{\psi}_\varepsilon(\theta',\alpha') \geq (1-q)\bar{\psi}_\varepsilon(\theta,\alpha^\star),
$$
for some $\alpha^\star \in C_\varepsilon^\star(\theta)$. Since $\mathcal{E}$ holds, there exists $t_0\geq1$ such that for all $t\geq t_0$ we have that $\left(\hat{\theta}_t,\left(N_{x,a}(t)/N_x(t)\right)_{(x,a)\in\mathcal{X} \times \mathcal{A}}\right) \in\mathcal{N}(q)$. Hence, for $t\geq t_0$ we have 
$$
    \bar{\psi}_\varepsilon\left(\hat{\theta}_t,\left(N_{x,a}(t)/N_x(t)\right)_{(x,a)\in\mathcal{X} \times \mathcal{A}}\right) \geq (1-q)\bar{\psi}_\varepsilon\left(\theta,\alpha^\star\right).
$$
%Since $\hat{\theta}_t \to \theta$, there exists $t_1 \geq 0$
Hence, $\forall x\in\mathcal{X}$ and $t\geq t_0$, we get:
\begin{align*}
    Z^x_\varepsilon(t) & = \max_{a\in\mathcal{A}_\varepsilon(\hat{\theta}_t,x)} \min_{b \neq a} \frac{(\hat{\theta}_{t}^{\top}\left(\phi_{x,a}-\phi_{x,b})+\varepsilon\right)^{2}}{2\left(\phi_{x,a}-\phi_{x,b}\right)^{\top}\left(\sum_{s=1}^{t} \phi_{x_s,a_s} \phi_{x_s,a_s}^{\top}\right)^{-1}\left(\phi_{x,a}-\phi_{x,b}\right)} \\& \geq 
    \min_{a\in\mathcal{A}_\varepsilon(\hat{\theta}_t,x)} \min_{b \in \mathcal{A}^c_\varepsilon(\hat{\theta}_t,x.a)} \frac{(\hat{\theta}_{t}^{\top}\left(\phi_{x,a}-\phi_{x,b})+\varepsilon\right)^{2}}{2\left(\phi_{x,a}-\phi_{x,b}\right)^{\top}\left(\sum_{s=1}^{t} \phi_{x_s,a_s} \phi_{x_s,a_s}^{\top}\right)^{-1}\left(\phi_{x,a}-\phi_{x,b}\right)}
    \\& \geq \min_{a\in\mathcal{A}_\varepsilon(\hat{\theta}_t,x)} \min_{b \in \mathcal{A}^c_\varepsilon(\hat{\theta}_t,x,a)} \frac{(\hat{\theta}_{t}^{\top}\left(\phi_{x,a}-\phi_{x,b})+\varepsilon\right)^{2}}{2\left(\phi_{x,a}-\phi_{x,b}\right)^{\top}\left(\sum_{s=1}^{t} \phi_{x_s,a_s} \phi_{x_s,a_s}^{\top}\right)^{-1}\left(\phi_{x,a}-\phi_{x,b}\right)}.% \\& =t \bar{\psi}_\varepsilon\left(\hat{\theta}_{t},\left(N_{x,a}(t)/N_x(t)\right)_{(x,a)\in\mathcal{X} \times \mathcal{A}}\right).
\end{align*}
Hence we get $$\min_{x\in\mathcal{X}} Z^x_\varepsilon(t) \geq \min_{x\in\mathcal{X}}\min_{a\in\mathcal{A}_\varepsilon(\hat{\theta}_t,x)} \min_{b \in \mathcal{A}^c_\varepsilon(\hat{\theta}_t,x,a)} \frac{(\hat{\theta}_{t}^{\top}\left(\phi_{x,a}-\phi_{x,b})+\varepsilon\right)^{2}}{2\left(\phi_{x,a}-\phi_{x,b}\right)^{\top}\left(\sum_{s=1}^{t} \phi_{x_s,a_s} \phi_{x_s,a_s}^{\top}\right)^{-1}\left(\phi_{x,a}-\phi_{x,b}\right)} = \bar{\psi}_\varepsilon(\theta,\alpha^\star). $$

By Lemma \ref{lem:forced_exploration}, for all $\varepsilon \in (0,p_{\min})$, there exists $\kappa$, $t_1(\kappa,\varepsilon) \geq 1$ such that for all $t \geq t_1$, we have $ \sum_{s = 1}^t \phi_{x_s,a_s}\phi_{x_s,a_s}^\top \succeq \sqrt{t}\kappa I_d$ with probability at least $1-2e^{-\varepsilon^2t/4}$ for some $\kappa>0$. By an immediate application of the first Borel-Cantelli Lemma, we obtain that the event $\left\{ \sum_{s = 1}^t\phi_{x_s,a_s}\phi_{x_s,a_s}^\top \not \succeq \sqrt{t}\kappa I_d \text{ i.o.}\right\}$ holds with probability $0$. Therefore, with probability $1$, there exists $t_2 \ge 0$ such that for all $t \ge t_2$, $ \sum_{s = 1}^t \phi_{x_s,a_s}\phi_{x_s,a_s}^\top \succeq \sqrt{t}\kappa I_d \succeq c I_d$. Let $t \ge \max\lbrace t_0, t_2\rbrace$, we have 

\begin{align*}
 \tau & =\inf \Big\{t \in \mathbb{N}^{*}: \forall x\in\mathcal{X}, Z_\varepsilon^x(t)>\beta(\delta, t) \text{ and } \sum_{s=1}^{t} \phi_{x_s,a_{s}}\phi_{x_s,a_{s}}^{\top} \succeq c I_{d}\Big\} \\&  \leq \max \{t_0,t_2\} \lor \inf \Big\{t \in \mathbb{N}^{*}: t(1-q) \bar{\psi}_\varepsilon\left(\theta,\alpha^\star \right)>\beta(\delta, t) \text{ and } \sum_{s=1}^{t} \phi_{x_s,a_{s}}\phi_{x_s,a_{s}}^{\top} \succeq c I_{d}\Big\}\\&  \leq \max \{t_0,t_2\} \lor \inf \Big\{t\in\mathbb{N}^*: t \bar{\psi}_\varepsilon\left(\theta,\alpha^\star \right)>\frac{1+u}{1-q} \log \left(\frac{\operatorname{det}\left((uc)^{-1} \sum_{s=1}^{t} \phi_{x_s,a_{s}}\phi_{x_s,a_{s}}^{\top}+I_{d}\right)^{\frac{1}{2}}}{\delta}\right) \text{ and } \sum_{s=1}^{t} \phi_{x_s,a_{s}}\phi_{x_s,a_{s}}^{\top} \succeq c I_{d}\Big\} \\ & \lesssim \max\left\{t_0,t_2, \frac{1}{1-q}T^\star_{\theta,\varepsilon}\log\left(\frac{1}{\delta}\right)\right\},
\end{align*}
where we used \cite[Lemma 18]{Garivier16} for $\delta$ sufficiently small in the last inequality. By letting $q\to 0$, we get 
$$
\mathbb{P}_\theta\Bigg(\limsup_{\delta \to 0} \frac{\tau}{\log \left(\frac{1}{\delta}\right)} \lesssim T_{\varepsilon,
\theta}^{\star}\Bigg) = 1.
$$
\textit{2) Guarantee in expectation.}

\textit{Step 1:} By continuity of $\bar{\psi}_\varepsilon$ (Lemma \ref{lem:properties_eps_delta}), there exist $g_1(q)>0$ such that for all $\theta' \in\mathbb{R}^d$ and $\alpha' \in \Lambda$
\begin{equation}
\label{eq:fact1}
    \left\{\begin{array}{ll}
    \left\|\theta^{\prime}-\theta\right\| & \leq g_1(q) \\
    d_{\infty}\left(\alpha^{\prime}, C_\varepsilon^{\star}(\theta)\right) & \leq g_1(q)
    \end{array} \Longrightarrow\left|\bar{\psi}_{\varepsilon}\left(\theta, \alpha^{\star}\right)-\bar{\psi}_\varepsilon\left(\theta^{\prime}, \alpha^{\prime}\right)\right| \leq q \bar{\psi}_\varepsilon\left(\theta, \alpha^{\star}\right) = q(T^\star_{\theta,\varepsilon})^{-1}\right .,
\end{equation}
for any $\alpha^\star \in\argmin_{\alpha \in C_\varepsilon^\star(\theta)}d_\infty(\alpha',\alpha)$. By the continuity properties of  $C^\star_\varepsilon(\theta)$, there exists a $g_2(q)>0$ such that for all $\theta'\in\mathbb{R}^d$ we have
$$
\|\theta - \theta'\| \leq g_2(q) \Rightarrow
\max_{\alpha'' \in C^\star_\varepsilon(\theta')}d_\infty(\alpha'',C^\star_\varepsilon(\theta)) \leq \frac{g_2(q)}{(K-1)}.
$$
Let $g(q) = \min\{g_1(q),g_2(q)\}$. Now we construct $T_0$ and an event $\mathcal{E}_T$ with $T\geq T_0$ under which for all $t\geq T$ we have 
$$
\|\hat{\theta}_t - \theta\|\leq g(q) \Rightarrow d_{\infty}\left(\left(N_{x,a}(t)/N_x(t)\right)_{(x,a)\in\mathcal{X} \times \mathcal{A}}, C_\varepsilon^{\star}(\alpha)\right) \leq  g_1(q).
$$
Define for $T\geq 1$ the events
\begin{align*}
\mathcal{E}_{1,T} & = \bigcap_{t = \ell(T)}^\infty   \{\|\theta- \hat{\theta}_t\|\leq g(q)\} 
\\ \mathcal{E}_{2, T} &=\bigcap_{t=T}^{\infty}\left\{\inf _{s \geq \ell(t)} d_{\infty}\left(\alpha(t), C_\varepsilon^{\star}\left(\hat{\theta}_{s}\right)\right) \leq \frac{g_{1}(q)}{4(K-1)}\right\} \\
& \subseteq \bigcap_{t=T}^{\infty}\left\{\exists s \geq \ell(t): d_{\infty}\left(\alpha(t), C_\varepsilon^{\star}\left(\hat{\theta}_{s}\right)\right) \leq \frac{g_{1}(q)}{2(K-1)}\right\}
\\  \mathcal{E}_{3,T} & = \bigcap_{t=T}^{\infty}\left\{ d_{\infty}\left(\left(N_{x,a}(t)/N_x(t)\right)_{(x,a)\in\mathcal{X} \times \mathcal{A}}, C_\varepsilon^{\star}(\theta)\right) \leq\left(z_{t}+d-1\right) \frac{g_{1}(q)}{K-1} \right\} \\ & \subseteq \bigcap_{t=T}^{\infty}\left\{ d_{\infty}\left(\left(N_{x,a}(t)/N_x(t)\right)_{(x,a)\in\mathcal{X} \times \mathcal{A}}, C_\varepsilon^{\star}(\theta)\right) \leq g_{1}(q) \right\} 
\\ \mathcal{E}_{4,T} & = \bigcap_{t=T}^{\infty}\left\{\sum_{s = 1}^t \phi_{x_s,a_s}\phi_{x_s,a_s}^\top \succeq c\sqrt{t} I_d \right\}
\end{align*}
Under the  $ \mathcal{E}_{1,T} \cap \mathcal{E}_{2,T}$, we have for all $t \geq T$, there exists $s\geq \ell(t)$ such that 
\begin{align*}
d_{\infty}\left(\alpha(t), C_\varepsilon^{\star}(\theta)\right) & \leq d_{\infty}\left(\alpha(t), C_\varepsilon^{\star}\left(\hat{\theta}_{s}\right)\right)+\max_{\alpha^{\prime} \in C_\varepsilon^{\star}\left(\hat{\theta}_{s}\right)} d_{\infty}\left(\alpha^{\prime}, C_\varepsilon^{\star}\left(\theta\right)\right) \\ &<\frac{g_{1}(q)}{2(K-1)}+\frac{g_{1}(q)}{2(K-1)}=\frac{g_{1}(q)}{K-1}.
\end{align*}
By lemma $3$, there exists a $t_1$ such that for $T\geq t_1$, the event 
$$
\left\{d_{\infty}\left(\left(N_{x,a}(t)/N_x(t)\right)_{(x,a)\in\mathcal{X} \times \mathcal{A}}, C_\varepsilon^{\star}(\theta)\right) \leq g_{1}(q)\right\},
$$
holds with probability at least $1-2 e^{-\frac{T\varepsilon^2}{4}}$. In particular we have
$q_1 = g_1(q)/(K-1)$ and $ t_1(q_1,\kappa) =\max\left\{\frac{1}{4c_1(\kappa) dq_1^3},\frac{T}{2c_1(\kappa)q_1^3},\frac{1}{c_1(\kappa)q_1^2}, \frac{7}{c_1(\kappa) q_1}\right\}.$ Hence for $T\geq \max\left\{  2q_1,14q_1^2,1/2d \right\}$ we have $t_1(q_1,\kappa) = \frac{T}{2 c_1 q_1^3}$. Hence, defining for $T\geq \lceil 1/(2c_1q_1^3)\rceil$, the event 
$$
\mathcal{E}_{1,\lceil 2c_1q_1^3T \rceil} \cap \mathcal{E}_{2,\lceil 2c_1q_1^3T \rceil} \cap \mathcal{E}_{3,\lceil 2c_1q_1^3T \rceil}
$$
we have shown that exists a $T_0$ such that for $T \geq T_0$% = \max\left\{a,v,\right\}$
, it holds that 
\begin{equation}
\label{eq:fact2}
    \forall t \geq T, \quad\left\|\theta-\hat{\theta}_{t}\right\| \leq g(q) \Longrightarrow d_{\infty}\left(\left(N_{x,a}(t)/N_x(t)\right)_{(x,a)\in\mathcal{X} \times \mathcal{A}}, C_\varepsilon^{\star}(\theta)\right)  \leq g_{1}(q) .
\end{equation}

Finally, combining the implication \eqref{eq:fact2} with the fact that \eqref{eq:fact1} holds under $\mathcal{E}_T$, we conclude that for $T \geq T_0$ we have 
\begin{equation}
\label{eq:inequality1_th3}
\bar{\psi}_\varepsilon\left(\hat{\theta}_t,\left(N_{x,a}(t)/N_x(t)\right)_{(x,a)\in\mathcal{X} \times \mathcal{A}}\right)\geq (1-q) \bar{\psi}_\varepsilon^\star(\theta).
\end{equation}


\textit{Step 2:} Now, by Lemma \ref{lem:forced_exploration}, we have that, for all $T\geq T_1(c)$, the event $\left\{\sum_{s = 1}^t \phi_{x_s,a_s}\phi_{x_s,a_s}^\top \succeq c\sqrt{t} I_d \right\}$ holds with probability at least $1-2 e^{-\frac{Tc^2}{4}}$, where $c$ is a constant independent of $\delta$. Now we note that for all $t\geq T_1$ we have  $Z_\varepsilon^x(t) \leq t \bar{\psi}_\varepsilon\left(\hat{\theta}_{t},\left(N_{x,a}(t)/N_x(t)\right)_{(x,a)\in\mathcal{X} \times \mathcal{A}}\right).$ Under the event $\mathcal{E}_T$ we have that \eqref{eq:inequality1_th3}, holds and we get
$$
Z_\varepsilon^x(t) \geq t(1-q)(T^\star_{\theta,\varepsilon})^{-1}.
$$
Hence, under $\mathcal{E}_T$, and for $T\geq \max\{T_0,T_1\}$, we get 
\begin{align*}
 \tau & =\inf \Big\{t \in \mathbb{N}^{*}: \forall x\in\mathcal{X}, Z_\varepsilon^x(t)>\beta(\delta, t) \text{ and } \sum_{s=1}^{t} \phi_{x_s,a_{s}}\phi_{x_s,a_{s}}^{\top} \succeq c I_{d}\Big\} \\& \leq \Big\{t: \forall x\in\mathcal{X}, Z_\varepsilon^x(t)>\beta(\delta, t) \Big\} \\& \leq T \lor \inf \Big\{t: \forall x\in\mathcal{X}, t(1-q)T^\star_{\theta,\varepsilon}>\beta(\delta, t) \Big\} \\& \leq T \lor \inf \Big\{t: \forall x\in\mathcal{X}, t(1-q) T^\star_{\theta,\varepsilon}>c_1\log(c_2t^\gamma/\delta)\Big\},
\end{align*}
where $k_1, k_2, \gamma$ appears in the definition of $\beta(\delta,t)$. Applying  \cite[Lemma 18]{Garivier16} leads to 
$$
\inf\Big\{t: \forall x\in\mathcal{X}, t(1-q)T^\star_{\theta,\varepsilon}>k_1\log(k_2t^\gamma/\delta)\Big\} \leq T_2(\delta),
$$
where $T_{2}^{\star}(\delta)=\frac{k_{1}}{1-q} T_{\theta,\varepsilon}^{\star} \log (1 / \delta)+o(\log (1 / \delta))$.
Hence, for $T\geq \max\{T_0,T_1,T_2^\star(\delta)\}$ we get $\mathcal{E}_T \subseteq \{\tau \leq T\}.$ Let $T_3^\star(\delta) = \max\{T_0,T_1,T_2^\star(\delta)\}$. Then for $T\geq T_3^\star(\delta)$ 
$$
\tau_{\delta} \leq \tau_{\delta} \wedge T_{3}^{\star}(\delta)+\tau_{\delta} \vee T_{3}^{\star}(\delta) \leq T_{3}^{\star}(\delta)+\tau_{\delta} \vee T_{3}^{\star}(\delta),
$$
and taking the expectation of the above inequality 
$$
\mathbb{E}[\tau_\delta] \leq T_{3}^{\star}(\delta)+\mathbb{E}[\tau_{\delta} \vee T_{3}^{\star}(\delta)]
$$
Now, note that
\begin{align*}
\mathbb{E}\left[\tau \vee T_{3}^{\star}(\delta)\right] &=\sum_{T=0}^{\infty} \mathbb{P}\left(\tau \vee T_{3}^{\star}(\delta)>T\right) \\
&=\sum_{T=T_{3}^{\star}(\delta)+1}^{\infty} \mathbb{P}\left(\tau \vee T_{3}^{\star}(\delta)>T\right) \\
&=\sum_{T=T_{3}^{\star}(\delta)+1}^{\infty} \mathbb{P}(\tau>T) \\
& \leq \sum_{T=T_{3}^{\star}(\delta)+1}^{\infty} \mathbb{P}\left(\mathcal{E}_{T}^{c}\right) \\
& \leq \sum_{T=T_{0} \vee T_{1}}^{\infty} \mathbb{P}\left(\mathcal{E}_{T}^{c}\right).
\end{align*}
Hence, we can conclude that 
$$\mathbb{E}[\tau] \leq \frac{k_{1}}{1-q} T_{\theta,\varepsilon}^{\star} \log (1 / \delta)+o(\log (1 / \delta))+T_{0} \vee T_{1}+\sum_{T=T_{0} \vee T_{1}}^{\infty} \mathbb{P}\left(\mathcal{E}_{T}^{c}\right).$$
\textit{Step 3:} The next step is to show that $\sum_{T=T_{0} \vee T_{1}}^{\infty} \mathbb{P}\left(\mathcal{E}_{T}^{c}\right) < \infty$ and it can be upper-bounded by a universal constant independent of $\delta$. We observe that there exists a $h(g_1(q))/4(K-1)>0$, $y>0$ such that for $T_0 \vee T_{1}$, 
\begin{align*}
\mathbb{P}\left(\mathcal{E}_{1,\left\lceil 2 c_1  q_{1}^{3} T \right\rceil}^{c}\right) & \leq \sum_{t=\left\lceil 2 c_1  q_{1}^{3} T \right\rceil}^{\infty} \mathbb{P}\left(\inf _{s \geq \ell(t)} d_{\infty}\left(\alpha(t), C^{\star}\left(\hat{\theta}_{s}\right)\right)>\frac{g_{1}(q)}{4(K-1)}\right) \\
& \leq h\left(\frac{g_{1}(q)}{4(K-1)}\right) \sum_{t=\left\lceil 2 c_1  q_{1}^{3} T \right\rceil}^{\infty} \frac{1}{t^{2+y}} \\
& \leq h\left(\frac{g_{1}(q)}{4(K-1)}\right) \int_{\left\lceil 2 c_1  q_{1}^{3} T \right\rceil-1}^{\infty} \frac{1}{t^{2+y}} d t \\
& \leq h\left(\frac{g_{1}(q)}{4(K-1)}\right) \frac{1}{(1+y)\left(\left\lceil 2 c_1  q_{1}^{3} T \right\rceil-1\right)^{1+y}}.
\end{align*}
Hence 
$$
\mathbb{P}\left(\mathcal{E}_{T}^{c}\right) \leq \mathbb{P}\left(\mathcal{E}_{1,\left\lceil 2 c_1  q_{1}^{3} T \right\rceil}^{c}\right) + \mathbb{P}\left(\mathcal{E}_{1,\left\lceil 2 c_1  q_{1}^{3} T \right\rceil}^{c}\right) \leq 2  h\left(\frac{g_{1}(q)}{4(K-1)}\right) \frac{1}{(1+y)\left(\left\lceil 2 c_1  q_{1}^{3} T \right\rceil-1\right)^{1+y}} \Rightarrow \sum_{T=T_{0} \vee T_{1}}^{\infty} \mathbb{P}\left(\mathcal{E}_{1,\left\lceil 2 c_1  q_{1}^{3} T \right\rceil}^{c}\right)<\infty.
$$
Second, we observe, using a union bound, and Lemma \ref{lem:LS_concentration}, that there exists strictly positive constants $c_3, c_4$ independent of $q$ and $T$, and such that
\begin{align*}
\mathbb{P}\left(\mathcal{E}_{2,\left\lceil 2 c_1  q_{1}^{3} T \right\rceil}^{c}\right) & \leq \sum_{t=\ell\left(\left\lceil 2 c_1  q_{1}^{3} T \right\rceil\right)}^{\infty} \mathbb{P}\left(\left\|\theta-\hat{\theta}_{t}\right\|>g(q)\right)\\
& \leq c_{3} \sum_{t=\ell\left(\left\lceil 2 c_1  q_{1}^{3} T \right\rceil\right)}^{\infty} t^{d/4} \exp \left(-c_{4} g(q)^{2} \sqrt{t}\right).
\end{align*}
For $t$ large enough, we have that the function $t \mapsto t^{d/4} \exp \left(-c_{4} g(q)^{2} \sqrt{t}\right)$ is decreasing. Also, since $(\ell(t))_{t\geq1}$ is non-decrasing, and $\lim_{t\to\infty}\ell(t) = \infty$, we may find $T_2\geq T_0 \lor T_1$ such that for all $t\geq T_2$ we have that $t \mapsto t^{d/4} \exp \left(-c_{4} g(q)^{2} \sqrt{t}\right)$ is decreasing on $[\ell(\varepsilon_1 T)-1,\infty)$. Thus for $T\geq T_2$, we get
$$
\mathbb{P}\left(\mathcal{E}_{2,\left\lceil 2 c_1  q_{1}^{3} T \right\rceil}^{c}\right) \leq c_{3} \int_{\ell\left(\left\lceil 2 c_1  q_{1}^{3} T \right\rceil\right)-1}^{\infty} t^{d / 4} \exp \left(-c_{4} g(q)^{2} \sqrt{t}\right) d t.
$$
Furthermore, for some $T_3 \geq T_2$ large enough, we may bound the integral for all $T \geq T_3$ as follows
$$
\int_{\ell\left(\left\lceil 2 c_1  q_{1}^{3} T \right\rceil\right)-1}^{\infty} t^{d / 4} \exp \left(-c_{4} g(q)^{2} \sqrt{t}\right) d t \lesssim \frac{\ell\left(\left(\left\lceil 2 c_1  q_{1}^{3} T \right\rceil\right)-1\right)^{d / 2+1}}{g(q)^{4} \exp \left(c_{4} g(q)^{2} \sqrt{\ell\left(\left\lceil 2 c_1  q_{1}^{3} T \right\rceil\right)-1}\right)}.
$$
Now the condition 
$$
\mathbb{P}\left(\mathcal{E}_{2,\left\lceil 2 c_1  q_{1}^{3} T \right\rceil}^{c}\right) \lesssim \frac{\ell\left(\left(\left\lceil 2 c_1  q_{1}^{3} T \right\rceil\right)-1\right)^{d / 2+1}}{g(q)^{4} \exp \left(c_{4} g(q)^{2} \sqrt{\ell\left(\left\lceil 2 c_1  q_{1}^{3} T \right\rceil\right)-1}\right)} \lesssim \frac{T^{d / 2+1}}{\exp \left(c_{5}(\varepsilon) T^{\gamma / 2}\right)}
$$
This show that 
\begin{align*}
\sum_{T=T_{0} \vee T_{1}}^{\infty} \mathbb{P}\left(\mathcal{E}_{2,\left\lceil 2 c_1  q_{1}^{3} T \right\rceil}^{c}\right) &=\sum_{T=T_{0} \vee T_{1}}^{T_{4}} \mathbb{P}\left(\mathcal{E}_{2,\left\lceil 2 c_1  q_{1}^{3} T \right\rceil}^{c}\right)+\sum_{T=T_{4}+1}^{\infty} \mathbb{P}\left(\mathcal{E}_{2,\left\lceil 2 c_1  q_{1}^{3} T \right\rceil}^{c}\right) \\
& \lesssim \sum_{T=T_{0} \vee T_{1}}^{T_{4}} \mathbb{P}\left(\mathcal{E}_{2,\left\lceil 2 c_1  q_{1}^{3} T \right\rceil}^{c}\right)+\sum_{T=T_{4}+1}^{\infty} \frac{T^{d / 2+1}}{\exp \left(c_{5}(\varepsilon) T \gamma / 2\right)} \\
&<\infty
\end{align*}
where the last inequality follows from the fact that we can upper bound the infinite sum by a Gamma function, which is convergent as long as 
$\gamma > 0$.
Hence we can conclude that 
$$
\sum_{T=T_{0} \vee T_{1}}^{\infty}\mathbb{P}\left(\mathcal{E}_{T}^{c}\right) \leq \sum_{T=T_{0} \vee T_{1}}^{\infty} \mathbb{P}\left(\mathcal{E}_{1,\left\lceil 2 c_1  q_{1}^{3} T \right\rceil}^{c}\right)+\mathbb{P}\left(\mathcal{E}_{1,\left\lceil 2 c_1  q_{1}^{3} T \right\rceil}^{c}\right) \leq \infty.
$$

We have shown that 
$$
\mathbb{E}[\tau] \leq \frac{k_{1}}{1-\varepsilon} T_{\theta,\varepsilon}^{\star} \log (1 / \delta)+o(\log (1 / \delta))+T_{0} \vee T_{1}+\sum_{T=T_{0} \vee T_{1}}^{\infty} \mathbb{P}\left(\mathcal{E}_{T}^{c}\right),
$$
where $\sum_{T=T_{0} \vee T_{1}}^{\infty}\mathbb{P}\left(\mathcal{E}_{T}^{c}\right)$ is independent of $\delta$.
Hence, 
$$
\limsup _{\delta \rightarrow 0} \frac{\mathbb{E}\left[\tau_{\delta}\right]}{\log (1 / \delta)} \leq \frac{k_{1}}{1-q} T_{\theta,\varepsilon}^{\star}.
$$
By Letting $q\to 0$, we get the result.
\end{proof}


==> Sections/deleted_text.tex <==
\begin{comment}
\begin{lemma}[Properties of the optimization problem]
Assume $a^\star_\theta(x)$ is unique $\forall x\in\mathcal{X}$, and
define $\psi(\theta,\alpha) = \sup_{\alpha \in \Lambda}\min_{x \in \mathcal{X}, a \in \mathcal{A}\backslash\lbrace a_\theta^\star(x) \rbrace} \frac{ (\theta^\top \gamma_{x, a})^2}{2\gamma_{x,a}^\top A(\alpha)^{-1} \gamma_{x,a}}$. Then $\psi$ is continuous in $\theta$ and $\alpha$, and $\alpha \mapsto \psi(\theta,\alpha)$ is concave and attains its maximum at a point $\alpha^\star\in\Lambda$ such that $A(\alpha^\star) \succ 0$.
\end{lemma}

Previous works \cite{Fiez19,Jedra20} use Frank-Wolfe type of algorithms to solve the problem of the optimal allocations in \eqref{eq:lb_delta}. We note that the problem of deriving the optimal allocation is a convex optimization problem since $h(\alpha) = \max\limits_{x \in \mathcal{X}}\max\limits_{a \in \mathcal{A}\setminus\{a^\star_\theta(x)\}} \frac{2\gamma_{x,a}^\top A(\alpha)^{-1} \gamma_{x,a}}{(\theta^\top
\gamma_{x,a})^2}$ is a maximum of convex functions, and hence is convex.
Thus, the optimal allocation problem corresponds to solve $\inf \limits_{\alpha \in \Lambda} h(\alpha)$, or equivalently: 
\begin{equation*}
    \begin{aligned} 
    \inf_{z,\alpha} \;& z
    \\\text{ s.t. } & z \geq \frac{2\gamma_{y,b}^\top A(\alpha)^{-1} \gamma_{y,b}}{(\theta^\top
    \gamma_{y,b})^2}, \;\; \forall y\in\mathcal{X}, \forall b \in\mathcal{A}\setminus\{a^\star_\theta(y)\} \\ &
    \mathbf{1}^{\top}\alpha = 1,
    \\& 0\preceq \alpha \preceq  1.
    \end{aligned}
\end{equation*}
\end{comment}

%for some $\alpha \in \Lambda$ and for all $t\geq 1$. Hence, an algorithm in the passive learning setting only accounts for devising $(\tau, \hat{a}_\tau)$. Note that since we do not control the sampling rule, it may not be possible to learn the best policy exactly. In this case, we focus on identifying the best learnable policy on a subset of $\mathbb{R}^d$. Let $U \subseteq \mathbb{R}^d$ and denote by $U^\perp = \left\{v \in \mathbb{R}^d : v \cdot u = 0,\; \forall u \in U\right\}$, the orthogonal complement of $U$. By the orthogonal decomposition Theorem we have that $\mathbb{R}^d = U \oplus U^\perp$, and each $\theta\in \mathbb{R}^d$ can be uniquely written as a sum $\theta = \tilde{\theta} + \theta_\perp$, where $\tilde{\theta} \in U$ and $\theta_\perp \in U^\perp$. We define the orthogonal projection operator $\text{proj}_U(\cdot):\mathbb{R}^d \to U$ such that for all $\theta \in \mathbb{R}^d$, $\text{proj}_U(\theta) = \tilde{\theta}$. We may define the \textit{projected reward} $\tilde{R}_t = \tilde{\theta}^{\top}\phi_{X_t,A_t} + \xi_t$ and the \textit{projected best arm} for context $x$ as $a^\star_{\tilde{\theta}}(x) = \argmax_{a\in\mathcal{A}} \tilde{\theta}^{\top}\phi_{x,a}$. Intuitively, $U$ may be thought as a subspace of $\mathbb{R}^d$ on which it is possible to learn a PAC algorithm. 

%In the passive learning case, we focus on identifying the best learnable policy on a subset of $\mathbb{R}^d$. Let $U \subseteq \mathbb{R}^d$ and denote by $U^\perp = \left\{v \in \mathbb{R}^d : v \cdot u = 0,\; \forall u \in U\right\}$, the orthogonal complement of $U$. By the orthogonal decomposition Theorem we have that $\mathbb{R}^d = U \oplus U^\perp$, and each $\theta\in \mathbb{R}^d$ can be uniquely written as a sum $\theta = \tilde{\theta} + \theta_\perp$, where $\tilde{\theta} \in U$ and $\theta_\perp \in U^\perp$. We define the orthogonal projection operator $\text{proj}_U(\cdot):\mathbb{R}^d \to U$ such that for all $\theta \in \mathbb{R}^d$, $\text{proj}_U(\theta) = \tilde{\theta}$. We may define the \textit{projected reward} $\tilde{R}_t = \tilde{\theta}^{\top}\phi_{X_t,A_t} + \xi_t$ and the \textit{projected best arm} for context $x$ as $a^\star_{\tilde{\theta}}(x) = \argmax_{a\in\mathcal{A}} \tilde{\theta}^{\top}\phi_{x,a}$. Intuitively, $U$ may be thought as a subspace of $\mathbb{R}^d$ on which it is possible to learn a PAC algorithm. 

%Theorem \ref{theorem:off_policy_lb} ensures that if $U \subseteq \mathcal{R}(A(\alpha))$ then $U$ is PAC-learnable. In particular, it implies that the maximal PAC-learnable set is achieved for $U = \mathcal{R}(A(\alpha))$, i.e., $\forall B\subseteq \mathbb{R}^d$ if $U = B$ is PAC-learnable and $\mathcal{R}(A(\alpha)) \subseteq B$, then $B = \mathcal{R}(A(\alpha))$. Similarly to Remark \ref{rem:delta_pac}, we can derive a lower bound for $(U,0,\delta)-$PAC policies. %Thus we conclude that the best choice is $U = \mathcal{R}(A(\alpha))$. 
\begin{lemma}[Convergence of $\alpha(t)$ to $C_\varepsilon^\star(\alpha)$]
\label{lem:convergence_C_star}
    Let $(l(t))_{t\geq 1}$ a non-decreasing sequence of integers such that $l(1) = 1$, $l(t-1) \leq t-1$ for $t > 1$, $\lim_{t\to \infty} l(t) = \infty$, and $\lim_{t\to\infty}\min_{s\geq l(t)} d_\infty(\alpha(t),C_\varepsilon^\star(\hat{\theta}_s)) = 0$ a.s. 
    Then under sampling rule \eqref{eq:sampling_rule_force}, \eqref{eq:sampling_rule_track} we have
    $$
    \lim_{t\to\infty} d_\infty(\alpha(t),C_\varepsilon^\star(\theta)) = 0 \quad \text{a.s.}
    $$
\end{lemma}

The following Lemma show that the optimization problem in \eqref{eq:eps_delta_equivalent_lb} satisfies a set of convenient properties.
\begin{lemma}[Properties of the optimization problem]
\label{lem:properties_eps_delta}Let $\psi_{\varepsilon}(\theta,\alpha) =  \inf_{\mu \in B_\varepsilon(\theta)}\frac{1}{2}\|\mu-\theta\|^2_{A(\alpha)}$, and $C_\varepsilon^\star(\theta) = \argsup_{\alpha \in \Lambda} \psi_\varepsilon(\theta,\alpha)$.  For any $\varepsilon\geq 0$, we have
\begin{enumerate}
    \item $\psi_\varepsilon$ is continuous in $\theta$ and $\alpha$,
    \item $\exists \; \alpha^\star \in C^\star_\varepsilon(\theta)$ such that $A(\alpha^\star) \succ 0$,
    \item $\psi_{\varepsilon}^\star$ is continuous in $\theta$,
    \item $C_\varepsilon^\star(\theta)$ is convex, compact and upper hemicontinuous. 
\end{enumerate}
\end{lemma}

\begin{comment}
\begin{lemma}[Closed-form solution of $Z^x_{a,b,\varepsilon}$ \cite{Jedra20}]
\label{lem:closed_form_Z}
Let $t\geq 1$ and $\sum_{s = 1}^t \phi_{x_s,a_s}\phi_{x_s,a_s}^\top \succ 0$. Then for for all $x \in\mathcal{X}$, $(a,b) \in\mathcal{A}^2: a\neq b$, we have
\begin{equation*}
    Z^x_{a, b, \varepsilon}(t)=\operatorname{sgn}\left(\hat{\theta}_{t}^{\top}\gamma^x_{a,b}+\varepsilon\right) \frac{\left(\hat{\theta}_{t}^{\top}\gamma^x_{a,b}+\varepsilon\right)^{2}}{2\|\gamma^x_{a,b}\|_{(\sum_{s=1}^{t} \phi_{x_s,a_s} \phi_{x_s,a_s}^{\top})^{-1}}}.
\end{equation*}
\end{lemma}
\end{comment}

\begin{comment}
Define $Z_\varepsilon^x(t) = \min_{\{b \in \mathcal{A}:|\hat{\theta}_t^\top(\phi_{x,\hat{a}_t(x)} - \phi_{x,b})| \geq \varepsilon\}} Z^x_{\hat{a}_t(x), b,\varepsilon}(t)$. The stopping time is 
\begin{align}
\begin{split}
    \tau =\inf \Bigg\{t \in \mathbb{N}^{*}: \forall x\in\mathcal{X}, Z_{\varepsilon}^x(t)>\beta(\delta, t) \text{ and } A_t \succeq \max \Bigg\{c, \frac{\rho(\delta, t)}{\|\hat{\theta}_{t}\|^{2}}\Bigg\}\Bigg\},
\end{split}
\label{eq:stopping_rule_eps_delta_pac}
\end{align}
where $\beta(\delta,t)$, and $\rho(\delta,t)$ are exploration thresholds defined in \eqref{eq:expl_rate_eps_delta_pac} and $c>0$. %With respect to the $\delta$-PAC case, we impose the additional condition $\min_{b\in O^c_\varepsilon(\theta,x)} \tilde{\theta}_t(\phi_{x,\hat{a}_t} - \phi_{x,b})$. 
The following Lemma provides a sufficient condition on the stopping rule of any $(\varepsilon,\delta)$-PAC algorithm. 
\begin{lemma}[Stopping rule $(\varepsilon,\delta)$-PAC]
\label{lem:stopping_rule_eps_delta_pac}
Let $\left(\delta_{t}\right)_{t \geq 1},\left(\varepsilon_{t}\right)_{t \geq 1}$ be two sequences with values in $(0,1)$ and $(0, \varepsilon)$, respectively, and such that $\sum_{t=1}^{\infty} \delta_{t}\leq \delta$, and $\lim _{t \rightarrow \infty} \varepsilon_{t}=\varepsilon .$ Let $\zeta_{t}=\log \left(2 \operatorname{det}\left(c^{-1} \sum_{s=1}^{t}\phi_{x_s,a_{s}} \phi_{x_s,a_{s}} ^{\top}+I_{d}\right)^{\frac{1}{2}}\right)-\log \left(\delta_{t}\right)$, and define:
\begin{equation}
\beta(\delta, t)=2 \zeta_{t} \quad \text { and } \quad \rho(\delta, t)=\frac{4  \varepsilon_{t}^{2} \zeta_{t}}{\left(\varepsilon-\varepsilon_{t}\right)^{2}}
\label{eq:expl_rate_eps_delta_pac}
\end{equation}
Under any sampling rule, and stopping rule \eqref{eq:stopping_rule_eps_delta_pac} with exploration threshold \eqref{eq:expl_rate_eps_delta_pac}, we have:
     $$\mathbb{P}_{\theta}\left(\exists x\in \mathcal{X}: \theta^\top (\phi_{x,a^\star_\theta(x)} - \phi_{x,\hat{a}_\tau(x)}) >\varepsilon, \tau <\infty\right)\leq\delta.$$
\end{lemma}
\end{comment}

\begin{comment}
\subsubsection{Discretized continuous contexts}
We consider a synthetic example of LCB-BPI problem with continuous context. We consider a uniform distribution $p_\mathcal{X} = \mathcal{U}(\mathcal{X})$ over $\mathcal{X} = [-1,1]$, with two actions $\mathcal{A} = \{a_1,a_2\}$. The feature vectors are specified as
$\phi_{x,a_1} = [1,x]$, $\phi_{x,a_2} = [1,-x]$,
$\theta = [1,1/2]$. Figure \ref{fig:continuous} shows the expected rewards and the gap $\Delta(x,\varepsilon) = |\theta^\top(\phi_{x,a_1} - \phi_{x,a_2})|$. In the $(\varepsilon,\delta)$-PAC setting, the goal is to learn the best policy on  $X_\varepsilon =  \mathbbm{1}\{|\theta^\top(\phi_{x,a_1}-\phi_{x,a_2})| > \varepsilon\}$, as shown in Figure \ref{fig:continuous}. 
\begin{figure}
    \centering
    \includegraphics[width = 7.5cm]{Figures/continuous.png}
    \caption{LCB instance in the continuous-context setting.}
    \label{fig:continuous}
\end{figure}
For each experiment, we report the theoretical lower bound on the sample complexity and the empirical sample complexity. The empirical quantities are reported in terms of mean and standard deviation, taken over $N_{\text{sim}} = 200$ Monte-Carlo runs with $\mathcal{X}$ discretized in $C = 10^{3}$ bins. For the passive learning setting we report results for the \textit{deterministic sampling rule}, selecting action $a_t(x) = a_1$, for all $x\in\mathcal{X}$, and the \textit{random sampling rule} selecting action $a_i$ with probability $\alpha_{x,a_1} = 1/2$, $\forall x \in \mathcal{X}$. For the active learning setting we report the results with the adaptive sampling rule.

\begin{table}[ht!]
\fontsize{9.3}{9.3}\selectfont
\centering
\caption{BPI results for the continuous-context example.}
\begin{tabular}{clrr}\toprule
Sampling rule & Parameter & Lower bound & Sample complexity  \\ \hline \hline
\multirow{3}{*}{Deterministic} 
& $\varepsilon= 0.10$  & $417.54$ & $504.34 \pm 165.87$ \\ & $\varepsilon = 0.05$ & $610.52$ & $583.33 \pm 111.06$\\ & $\varepsilon = 0.01$ & $610.52$ & $583.33 \pm 111.06$ \\ \hline 
\multirow{3}{*}{Random} 
& $\varepsilon= 0.10$  & $65.63$ & $234.05 \pm 48.04$\\ & $\varepsilon = 0.05$ & $193.30$ & $316.89\pm85.42$ \\ & $\varepsilon = 0.01$ & $610.52$ & $583.33 \pm 111.06$\\\hline  
\multirow{3}{*}{Adaptive} 
& $\varepsilon= 0.10$ & $65.63$ & $234.05 \pm 48.04$ \\ 
& $\varepsilon = 0.05$ & $193.30$ & $316.89\pm85.42$\\ & $\varepsilon = 0.01$ & $610.52$ & $583.33 \pm 111.06$\\ \bottomrule
\end{tabular} 
\label{tab:results_continuous}
\end{table}
\subsubsection{$(U,\delta)$-PAC synthetic example} 
\end{comment}

\begin{comment}
\begin{table}[ht!]
\fontsize{9.3}{9.3}\selectfont
\centering
\caption{Experimental results for the $3$-KPIs experiments.}
\begin{tabular}{clll}\hline 
Sampling Rule & Parameter & Lower bound & Sample complexity  \\ \hline 
\multirow{3}{*}{Rule-Based} 
& $\varepsilon= 0.10$  & $64.91$ & $456.55\pm 149.61$  \\ & $\varepsilon = 0.05$ & $259.11$ & $1887.22\pm 
472.71\pm142.93$  \\ & $\varepsilon = 0.025$ & $1531.47$ & $2384.03 \pm 313.01$  \\
\hline 
\multirow{3}{*}{Random} 
& $\varepsilon= 0.10$  & $69.40$ & $240.58\pm92.75$  \\ & $\varepsilon= 0.05$  & $231.69$ & $494.55 \pm 89.89$ \\ & $\varepsilon = 0.025$ & $1487.28$ & $1557.50\pm332.48$  \\ \hline
\end{tabular} 
\label{tab:results}
\end{table}
    \begin{table}[ht!]
\fontsize{9.3}{9.3}\selectfont
\centering
\caption{Experimental results for the $2$-KPIs experiments}
\begin{tabular}{llllll}\hline
Parameter & Lower bound & Sample complexity & BPI error & DM error & IPS error \\ \hline 
$\varepsilon = 0.20$ & $515.70$ & $744\pm228.43$ & $0.04 \pm 0.20$ & $0.10\pm 0.05$ & $0.17\pm 0.32$ \\
$\varepsilon = 0.15$ & $855.26$ & $1291.79\pm 289.09$ & $0.05 \pm 0.23$ & $0.12 \pm 0.05$ &  $0.16\pm 0.28$  \\
$\varepsilon= 0.10$ & $1276.13$ & $2766.48 \pm 416.02$  & $0.09 \pm 0.03$ &  $0.19\pm 0.25$ \\ \hline 
\end{tabular} 
\label{tab:results}
\end{table}
\end{comment}

%\textit{The lower bounds and the sample complexity for the active learning setting are lower than the ones for the passive setting}. This is to be expected since (i) the algorithm in the active setting adapts its proportions to $\hat{\alpha}_t$, and hence is supposed to achieve a sample complexity matching $T^\star_{\varepsilon,\theta}\log(1/\delta)$, and (ii) in our experiments $U = \mathbb{R}^d$ for both the random and the rule-based sampling rules. In fact, with our formulation, and when the context space is large, it is easy to ensure that $U = \mathbb{R}^d$. In particular, it is sufficient to have $\exists a \in \mathcal{A}$ and $\exists x_1,x_2,x_3 \in\mathcal{X}$ such that $p_\mathcal{X}(x_i)\alpha_{x_i,a} >0$, for $i = 1,2,3$. In our case, both the random and rule-based sampling rules satisfy this condition.

%\textit{The lower bounds and sample complexity for the random policy is lower than the one for the rule-based policy}. This may be imputed to the increased exploration ability of the random sampling rule compared to the rule-based one, resulting in faster identification of the best policy. We may also observe that, for the purpose of identifying the best antenna tilt update policy, the sample complexity achieved by the random policy is close to the one. 

%\textit{The sample complexity for all sampling rules match the lower bounds on the sample complexity up to a constant}. This show that the proposed algorithms matches the lower bounds and achieve good performance for the task of best policy identification. 

% By Lemma \ref{lem:forced_exploration}, there exists $t_1 \geq 0$ such that for all $t\geq t_1$, we have $ \sum_{s = 1}^t \phi_{x_s,a_s}\phi_{x_s,a_s}^\top \succeq c I_d$ with probability at least $1-2e^{-c^2t/4}$. This implies that for all $t \geq \max \{t_0,t_1\}$ we have 

%\begin{remark}[Alternative sampling rule]
%An alternative sampling strategy would be
%$$
%    a_{t+1}(x) =\left\{\begin{array}{ll}
%    d_{t}(x) & \text { if } \quad \sum_{s = 1}^t\phi_{x_s,a_s}\phi_{x_s,a_s}^\top \mathbbm{1}_{\{x_s = x\}}\succeq f_x(t) \\
%    \argmax\limits_{\tilde{a}_x \in\tilde{\mathcal{A}}_x}\lambda_{d_x}\left( \sum_{s = 1}^t \phi_{x_s,a_s}\phi_{x_s,a_s} + \phi_{x,\tilde{a}_x}\phi_{x,\tilde{a}_x}^\top \right) & \text { otherwise }
 %   \end{array} \right.
%$$
%This way, the forced exploration step would ensure that the feature vector leading to the maximum growth of the minimum eigenvalue is selected and would not require to keep track of indices for each context.  
%\end{remark}

%The result in Lemma \ref{lem:forced_exploration} implies that $\lim\inf_{t \to \infty }\lambda_{1}\left( \frac{1}{\sqrt{t}} \sum_{s = 1}^t (\phi_{x_s,a_s}\phi^\top_{x_s,a_s})\right) > 0$ a.s., and hence the sufficient condition on the convergence of the LS estimator is satisfied under the sampling rule \eqref{eq:sampling_rule_force}. 

%\begin{figure}
%    \centering
%     \includegraphics[width=\columnwidth]{figures/antenasv2.eps}
%     \caption{Abstract representation of the mobile network environment.}
%     \label{fig:env}
%\end{figure}

%\inf_{{\left\lbrace \mu\in\mathbb{R}^d: \exists x \in \mathcal{X}, \forall a \in \mathcal{A}_\varepsilon(\theta,x), \; \mu^{\top}(\phi_{x,a_{\mu}^\star(x)}- \phi_{x,a})>\varepsilon \right\rbrace}}

$$
    r^\theta_{s,t} = \theta^\top \phi_{x_{s,t},a_{s,t}}. 
$$
$$
    \phi_{s,t} = x_{s,t} \otimes a_{s,t}
$$
$$
    \theta = \left(\sum_{s = 1}^S \sum_{k = 1}^t \phi_{x_{s,k},a_{s,k}}\phi_{x_{s,k},a_{s,k}}\right)^\dagger \sum_{s = 1}^S \sum_{k = 1}^t\phi_{x_{s,k},a_{s,k}}p_{s,k}.
$$
$$
    p_{s,t} = w_\text{BC}(R_\text{BC}(s,t) -R_\text{BC}(s,t+1)) + w_\text{OS}(N_\text{OS}(s,t) -N_\text{OS}(s,t+1))
$$


% In fact, the LCB problem may be seen as a LB with time varying action space. %of the optimization problem involved, their algorithm is not easy to generalize to the contextual case when the number of context is large. 

  % T_{{\theta},\varepsilon}(\alpha) = \max\limits_{x\in \mathcal{X}} \max  \limits_{a\notin \mathcal{A}_\varepsilon({\theta},x)}\max\limits_{b\in \mathcal{A}_\varepsilon({\theta},x,a)} \frac{2 \|\gamma_{a,b}^x\|^2_{ (A(\alpha))^{\dagger}}}{ ({\theta}^\top\gamma_{a,b}^x+\varepsilon)^2}.
  
  %Z^x_{a, b, \varepsilon}(t)=\log \left(\frac{\max_{\left\{\mu: \mu^{\top}(\phi_{x,a}-\phi_{x,b}) \geq -\varepsilon\right\}} \prod_{s=1}^t f_{x_s,a_s}^{\mu}(r_s)}{\max _{\left\{\mu:\mu^{\top}(\phi_{x,a}-\phi_{x,b}) \leq -\varepsilon \right\}} \prod_{s=1}^t f_{x_s,a_s}^{\mu}(r_s) }\right). 
  
  
\subsection{Passive setting algorithm}
Define 
{\begin{equation*}
Z^x_{U,a, b, \varepsilon}(t)=\log \left(\frac{\max_{\left\{\mu \in U : \mu^{\top}\gamma_{a,b}^x \leq \varepsilon\right\}} \prod_{s=1}^t f_{x_s,a_s}^{\mu}(r_s)}{\max_{\left\{\mu \in U :\mu^{\top}\gamma_{a,b}^x \geq \varepsilon \right\}} \prod_{s=1}^t f_{x_s,a_s}^{\mu}(r_s)}\right).
\end{equation*}}
We can express $Z^x_{U,a, b, \varepsilon}(t)$, for $t$ such that $\lambda_1\left(P A_t P^\top\right) >0$, as 
$$Z^x_{U,a,b,\varepsilon} = \operatorname{sgn}\left(\hat{\theta}_{U,t}^{\top}(P\gamma^x_{b,a})+\varepsilon\right) \frac{\left(\hat{\theta}_{U,t}^{\top}(P\gamma^x_{b,a})+\varepsilon\right)^{2}}{2\|P \gamma^x_{b,a}\|_{(P^T A_tP)^{-1}}},$$
where $\hat{\theta}_{U,t} = \left(P A_t P^\top\right)^{-1} \left(P \sum_{s = 1}^T \phi_{x_s,a_s}r_s \right)$. The decision rule for the passive learning setting is defined as 
\begin{equation}
\label{eq:recommendation_rule}
    \hat{a}_\tau(x) = \argmax_{a \in \mathcal{A}_\varepsilon(\hat{\theta}_{U,\tau},x)} \min_{b \neq a} Z^x_{U,a, b, \varepsilon}(\tau), \quad \forall x\in\mathcal{X}.
\end{equation}
Define $Z_{U,\varepsilon}^x(t) = \max_{a \in \mathcal{A}_\varepsilon(\hat{\theta}_{U,\tau},x)} \min_{b \neq a} Z^x_{U, a, b, \varepsilon}(t)$. The stopping time is 
\begin{align}
\begin{split}
    \tau =\inf \Big\{t: \forall x\in\mathcal{X}, Z_{U,\varepsilon}^x(t)>\beta_U(\delta, t) \text{ and } P A_t P^\top \succeq c I_{r}\Big\},
\label{eq:stopping_rule_eps_delta_pac}
\end{split}
\end{align}

\begin{lemma}
\label{lem:stopping_rule_eps_delta_pac_passive}
Let $u>0$, and define the exploration threshold
\begin{equation}
    \label{eq:expl_rate_eps_delta_pac}
        \beta_U(\delta, t) = (1+u) \log \left(\frac{\operatorname{det}\left((uc)^{-1}  P A_t P^\top+I_{r}\right)^{\frac{1}{2}}}{\delta}\right).
\end{equation}
\noindent Under the stopping rule defined by
\eqref{eq:stopping_rule_eps_delta_pac}--\eqref{eq:expl_rate_eps_delta_pac} and under any sampling rule satisfying the hypotheses of Corollary \ref{cor:LS_concentration_passive}, we have
     $$\mathbb{P}_{\theta}\left(\exists x\in \mathcal{X}: \theta^\top (\phi_{x,a^\star_\theta(x)} - \phi_{x,\hat{a}_\tau(x)}) >\varepsilon, \tau <\infty\right)\leq\delta.$$
\end{lemma}


\begin{corollary}
    \label{cor:LS_concentration_passive}
    Let $\theta \in U$, and assume the sampling rule satisfies $\lim\inf_{t \to \infty }\lambda_{1}\left(\frac{1}{t^\alpha}(P A_t P^\top)\right) > 0$ a.s. for some, $\alpha\in(0,1)$. Then $\lim_{t \to \infty} \hat{\theta}_t = \theta $. In particular, for all $\beta \in (0,\alpha/2)$, 
   $ \|\hat{\theta}_t - \theta\| = o\left(t^{-\beta}\right)$ a.s.
\end{corollary}

\begin{comment}
\subsection{Algorithm}
The optimal allocation problem is a convex program since $h(\alpha) = \max\limits_{x \in \mathcal{X}, a \in \mathcal{A}\setminus\{a^\star_\theta(x)\}} \frac{2\gamma_{x,a}^\top A(\alpha)^{-1} \gamma_{x,a}}{(\theta^\top
\gamma_{x,a})^2}$ is the maximum of convex functions. Thus, the optimal allocation problem corresponds to solving $\inf \limits_{\alpha \in \Lambda} h(\alpha)$. Previous works use Frank-Wolfe type of algorithms to solve the optimal allocation problem exactly for all $t \in \mathbb{N}^+$ \cite{Fiez19} or for a subset $t \in \mathcal{T} \subseteq \mathbb{N}^+$ \cite{Jedra20}. The major drawback of this strategy is that solving a new convex optimization problem is computationally expensive, especially when $|\mathcal{X} \times \mathcal{A}|$ pair is large. We take a different approach based on the computation of an approximate solution to \eqref{eq:lb_delta} at each time step: we take $n$ gradient steps for all $t\in\mathbb{N^+}$. This will allow to decrease the sample complexity while retaining the asymptotic optimality of the algorithm. Denote by $(x_\star,a_\star) = \argmax\limits_{x \in \mathcal{X}, a \in \mathcal{A}\setminus\{a^\star_\theta(x)\}} \frac{2\gamma_{x,a}^\top A(\alpha)^{-1} \gamma_{x,a}}{(\theta^\top
\gamma_{x,a})^2}$, then we can express the gradients coordinates as 
$$\left(\nabla h(\alpha)\right)_{x,a} = \left( \frac{\gamma_\star^\top A(\alpha)^{-1} \phi_{x,a}}{\theta^\top \gamma_\star}\right)^2.$$

\begin{algorithm}[H]
\SetAlgoLined
\textbf{Input:} $\delta$, $\Tilde{\mathcal{A}}_x = \left\{\Tilde{a}_x(1),\dots,\Tilde{a}_x(d_x)\right\}$ for all $x\in\mathcal{X}$
\\ \textbf{Initialization:} $t=0, (i(x))_{x\in\mathcal{X}} = 0, (N_x(0))_{x\in\mathcal{X}} = 0, (N_{x,a}(0))_{(x,a)\in\mathcal{X}\times \mathcal{A}} = 0$, $(\alpha_{x,a}(0))_{(x,a)\in\mathcal{X}\times \mathcal{A}} = \frac{1}{K}$
\\ \While{Stopping rule not satisfied}{
\\  $x_t \sim p_\mathcal{X}$
\\ \eIf{$\sum_{s = 1}^t\phi_{x_s,a_s}\phi_{x_s,a_s}^\top \mathbbm{1}_{\{x_s = x\}}\succeq f_x(t)$}{
   $a_t(x_t) \leftarrow  \argmin_{a\in \text{supp}\left(\sum_{s =1}^t \alpha_{x,a}(s)\right)} \left( \frac{N_{x,a}(t)}{N_x(t)} - \sum_{s = 1}^t \alpha_{x,a}(s) \right)$ 
   }{$a_t(x_t)\leftarrow \tilde{a}_{x_t}(i_{t}(x_t)), i_{t+1}(x) = (i_t(x) \mod d_x)$}
  $t \leftarrow t+1$, update $N_x(t)$, $N_{x,a}(t)$ $\hat{\theta}_t$, $Z_\varepsilon(t)$,  
  \\ $s^\star(t) \leftarrow \arg\min_{s\in \Lambda} s^T \left( \frac{\hat{\gamma}_\star^\top A(\alpha_t)^{-1} \phi_{x,a}}{\hat{\theta}^\top \hat{\gamma}_\star}\right)^2$
  \\$\alpha(t) \leftarrow \alpha(t-1) + \frac{2}{t+2}(\alpha(t-1)- s^\star(t))$
 }
 \textbf{return} $\hat{a}_\tau(x) = \argmax_{a \in\mathcal{A}} \hat{\theta}_\tau \phi_{x,a}$, for all $x\in\mathcal{X}$
\caption{Online Gradient Track and Stop}
\end{algorithm} 

%Unlike the Lazy-TS algorithm here we execute a single gradient update step at each time step. This drastically reduces the computational complexity. 
Formulate the Lagrangian of the problem:
$$
L(z,\alpha,\rho) = z + \sum_{(y,b)\in\mathcal{X}\times\mathcal{A}\setminus\{a^\star_\theta(y)\}}\lambda_{y,b}\left(\frac{2\gamma_{y,b}^\top A(\alpha)^{-1} \gamma_{y,b}}{(\theta^\top
    \gamma_{y,b})^2}-z \right) +  \rho(\mathbf{1}^{\top}\alpha - 1).
$$
The first-order optimality condition impose:
\begin{equation*}
\begin{cases}
(i) \;\frac{dL}{dz} = 1 - \sum_{(y,b)}\lambda_{y,b} = 0
\\ 
(ii) \;\frac{dL}{d\alpha_{x,a}} = -\sum_{(y,b)}\frac{2{\gamma_{y,b}}^\top A(\alpha)^{-1}\phi_{x,a}\phi_{x,a}^\top A(\alpha)^{-1}{\gamma_{y,b}}}{(\theta^\top\gamma_{y,b})^2}\lambda_{y,b} + \rho = 0, \;\forall (x,a)\in\mathcal{X}\times\mathcal{A}
\\ (iii) \; \frac{dL}{d\rho} = \mathbf{1}^{\top}\alpha - 1 = 0
\\ (vi) \; \frac{dL}{d\lambda_{y,b}} = \frac{2\gamma_{x,a}^\top A(\alpha)^{-1} \gamma_{x,a}}{(\theta^\top\gamma_{x,a})^2}-z =0
\\ (v) \; \rho(\mathbf{1}^{\top}\alpha - 1) = 0
\\ (vi) \;\rho \geq 0,\lambda_{y,b} \geq 0.
\end{cases}
\end{equation*}
The size of the constraint set scales in linearly with $\mathcal{X}$ and $\mathcal{A}$.
%From $(ii)$ we get 
%$$
%\sum_{(y,b)}\frac{2\lambda_{y,b}}{(\theta^\top\gamma_{y,b})^2}\gamma_{y,b}^\top(A(\alpha)^{-1}(\phi_{x,a}\phi_{x,a}^{\top}-\phi_{x,c}\phi_{x,c}^{\top})A(\alpha)^{-1})\gamma_{y,b} = 0, \; \forall (a,c)\in\mathcal{A}^2
%$$
%We can conclude that the optimal allocation satisfy the following set of equations:
%\begin{equation*}
%\begin{cases}
%\frac{\|\gamma^\star\|^2}{|\mathcal{X}||\mathcal{A}|}\sum_{x,a}\frac{1}{\|\phi_{x,a}\|^2\alpha_{x,a}^2}={\gamma_\star}^\top A(\alpha)^{-1}\phi_{x,a}\phi_{x,a}^\top A(\alpha)^{-1}{\gamma_\star}, \;\forall (x,a)\in\mathcal{X}\times\mathcal{A}
%\\ \sum_{x,a}\alpha_{x,a} = 1.
%\end{cases}
%\end{equation*}
\end{comment}
%For $\varepsilon\geq0$, $x\in\mathcal{X}$, and $\theta\in\mathbb{R}^d$, define the set of $\varepsilon$-optimal arms as $\mathcal{A}_\varepsilon(\theta,x) = \{a\in\mathcal{A}: \theta^\top(\phi_{x,a^\star_\theta(x)}-\phi_{x,a})<\varepsilon\}$, and for $a\in \mathcal{A}_\varepsilon^c(\theta,x)$ the set $\mathcal{A}_\varepsilon(\theta,x,a) = \{b\in \mathcal{A}_\varepsilon(\theta,x): \theta^\top (\phi_{x,b}-\phi_{x,a}) \geq \varepsilon\}$.  Denote by $\mathbb{P}_\theta(\cdot)$ the probability measure of observations under the LCB problem defined by $\theta$ and by $\mathbb{E}_\theta[\cdot]$ its expectation. Define the simplex $\Lambda = \left\{\alpha \in [0,1]^{\vert \mathcal{X}\vert \times \vert \mathcal{A}\vert}: \forall x\in\mathcal{X} \; \sum_{a\in \mathcal{A}} \alpha_{x,a} = 1 \right\}.


%The \textit{coverage} indicator measures to what extent the area of interest is covered with a minimum signal power and is computed using measurements of the Reference Signal Received Power (RSRP). The \textit{capacity} indicator measures the amount of UE that the cell can handle simultaneously (e.g., in terms of number of calls) with a reference bit rate. The antenna tilt is a key parameters that determines a trade-off between coverage and capacity. On the one hand, low tilt values result in a larger covered area and smaller capacity due to an increased number of served UE; excessively low tilt values  may increase cell overshooting, causing the scope of antenna coverage to exceed the one intended and increasing the interference in neighbouring cells. On the other hand, high tilt values result in a smaller covered area with a lower number of UE served with increased capacity, but it risks to create \textit{coverage holes} in the cells. The joint optimization of coverage and capacity ensures that the targeted area remains covered while maximizing the capacity.

%In Contextual Bandits (CBs), an agent observes an input context, selects an action, and in turn receives a random reward sample. Given its versatility, several CB algorithms have been effectively employed in a broad range of real-world applications such as recommendation systems and network parameters optimization \cite{Langford08,Saxena19}. The Contextual Linear Multi-Armed Bandits (CL-MAB) problem \cite{Li11} is a particular instance of CBs in which the expected reward is modeled linearly in the feature vector encoding a context-action pair.

%The Best Policy Identification (BPI) problem with fixed confidence consists of devising a Probably Approximately Correct (PAC) algorithm using the least possible number of samples. The BPI problem can be studied in (i) \textit{active learning}, in which the agent adaptively selects its sampling rule based on the accumulated experience,  or (ii) \textit{passive learning}, in which the sampling rule is fixed and imposed. 

%In this paper we provide lower bound on the sample complexity of different types of PAC algorithms in both the active and passive learning settings. We then devise optimal algorithms matching such lower bounds. We apply our method to the RET optimization problem in 4G cellular networks. The experimental results show that our method is able to produce an optimal tilt update policy with intuitive interpretations of the results. To the best of our knowledge, this is the first paper considering BPI in the CL-MAB setting applied to RET optimization, and the first to consider the passive learning setting in CL-MAB-BPI.

%value maximization. The authors of \cite{Vannella20} apply off-policy estimators to the RET optimization problem. However such estimators are often unreliable, especially when data are biased or contain high amount of noise and do not provide a stopping rule. 

%Another related line of work is the one of off-policy evaluation and learning. Previous works in the off-policy setting, mostly focused on the general CB problem without reward structure \cite{Strehl10, Dudik14}. These work focused on learning a policy maximizing the value of a policy using data from an offline policy and off-policy value estimators. 

%These results reflects the trade-off between network coverage and capacity discussed in Section \ref{sec:introduction}. 

% there exists a sequence $(\ell(t))_{t\geq 1}$ of integers with $\ell(1) = 1$ and $\ell(t-1) \leq t-1$ for $t>1$, such that 
%\begin{equation}
%\label{eq:condition_convergence}
%\lim _{t \rightarrow \infty} \min _{s \geq \ell(t)} d_{\infty}\left(\alpha(t), C_\varepsilon^{\star}\left(\hat{\theta}_{s}\right)\right)=0 . \quad \text {a.s.}
%\end{equation}
